An Empirical Study of Deep Learning Sentiment Detection Tools for Software Engineering in Cross-Platform Settings

Sentiment detection in software engineering (SE) has shown promise to support diverse development activities. However, given the diversity of SE platforms, SE-specific sentiment detection tools may suffer in performance in cross-platform settings. Recently deep learning (DL)-based SE-specific sentiment detection tools are found to offer superior performance than shallow machine learning (ML) based/rule-based tools. However, it is not known how the DL tools perform in cross-platform settings. In this paper, we study whether SE-specific DL sentiment detectors are more effective than shallow ML-based/rule-based sentiment detectors in cross-platform settings. In three datasets, we study three DL tools (SEntiMoji, BERT4SEntiSE, RNN4SentiSE) and compare those against three baselines: two shallow learning tools (Senti4SD, SentiCR) and one rule-based tool (SentistrengthSE). We find that (1) The deep learning SD tools for SE, BERT4SentiSE outperform other supervised tools in cross-platform settings in most cases, but then the tool is outperformed by the rule-based tool SentistrengthSE in most cases. (2) BERT4SentiSE outperforms SentistrengthSE by large margin in within-platform settings across the three datasets and is only narrowly outperformed by SentiStrengthSE in four out of the six cross-platform settings. This finding offers hope for the feasibility to further improve a pre-trained transformer model like BERT4SentiSE in cross-platform settings. (3) The two best-performing deep learning tools (BERT4SentiSE and SentiMoji) show varying level performance drop across the three datasets. We find that this inconsistency is mainly due to the "subjectivity in annotation" and performance improvement for the studied supervised tools in cross-platform settings may require the fixing of the datasets.

==> RQ0_tables.tex <==
% %If the table is too wide, replace \begin{table}[!htp]...\end{table} with
% %\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
% % \begin{table}[!htp]\centering
% % \caption{Percentage of misclassification in cross platform settings compared to within-platform settings.}
% % \resizebox{\columnwidth}{!}{%
% % \begin{tabular}{llrr|rr|rrr}\toprule
% % {\textbf{DL SD}} &{\textbf{\% Correct}} 

% % % &\multicolumn{2}{c}{\textbf{Test Dataset}} &\multicolumn{2}{c}{\textbf{Test Dataset}} &\multicolumn{2}{c}{\textbf{Test Dataset}} \\\cmidrule{3-8}
% % &   &\multicolumn{2}{c}{Test in GitHub} &\multicolumn{2}{c}{Test in SO} &\multicolumn{2}{c}{Test in Jira} \\\cmidrule{3-8}
% % {\textbf{Tool}} & {\textbf{Misclassified}} &\textbf{Train SO} &\textbf{Train Jira} &\textbf{Train GitHub} &\textbf{Train Jira} &\textbf{Train GitHub} &\textbf{Train SO} \\\midrule
% % \multirow{3}{*}{\textbf{BERT4SentiSE}} &\%Overall &19 &30 &8 &18 &11 &10 \\
% % & \%Severe &3 &1 &0 &0 &1 &1 \\
% % &\%Mild &16 &28 &7 &18 &11 &10 \\
% % \midrule
% % \multirow{3}{*}{\textbf{SentiMoji}} &\%Overall &19 &30 &10 &29 &11 &10 \\
% % &\%Severe &1 &1 &1 &0 &0 &0 \\
% % &\%Mild &18 &29 &9 &29 &11 &10 \\
% % \bottomrule
% % \end{tabular}%
% % }
% % \end{table}

% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[t]
%   \centering
%   \caption{Percentage of misclassification in cross platform settings compared to within-platform}
%   \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{ll|rr|rr|rr}\toprule
%     {\textbf{SD}} & \textbf{\% Correct} & \multicolumn{2}{c}{\textbf{Test in GitHub}} & \multicolumn{2}{c}{\textbf{Test in SO}} & \multicolumn{2}{c}{\textbf{Test in Jira}} \\
%     \cmidrule{3-8}
%     {\textbf{Tool}} & \textbf{Misclassified} & {\textbf{Train SO}} & {\textbf{Train Jira}} & {\textbf{Train GitHub}} & {\textbf{Train Jira}} & {\textbf{Train GitHub}} & {\textbf{Train SO}} \\
%     \midrule
%     \multirow{3}[0]{*}{\textbf{BERT4SentiSE}} & \textbf{Overall} & 19    & 30    & 8     & 18    & 11    & 10 \\
%           & \textbf{Severe} & 3     & 1     & 0     & 0     & 1     & 1 \\
%           & \textbf{Mild} & 16    & 28    & 7     & 18    & 11    & 10 \\
%           \midrule
%     \multirow{3}[0]{*}{\textbf{SentiMoji}} & \textbf{Overall} & 19    & 30    & 10    & 29    & 11    & 10 \\
%           & \textbf{Severe} & 1     & 1     & 1     & 0     & 0     & 0 \\
%           & \textbf{Mild} & 18    & 29    & 9     & 29    & 11    & 10 \\
%           \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:rq-error-analysis}%
% \end{table}%






% % \begin{table}[t]%\centering
% % \caption{Percentage of new misclassification in cross platform settings.} 
% % %[Alamin: I'll update and fix the table format later tonight. But if the table is missing information then please comment]}
% % %\scriptsize
% % \resizebox{\columnwidth}{!}{%
% % \begin{tabular}{lrr|rr|rr}\toprule
% % \multirow{3}{*}{\textbf{Tool}} &\multicolumn{6}{c}{\textbf{\% of Correct Classification that Were Misclassified from Wtinin to Cross-Platform Settings}} \\\cmidrule{2-7}
% % &\multicolumn{2}{c}{\bf{Test in GitHub}} &\multicolumn{2}{c}{\textbf{Test in SO}} &\multicolumn{2}{c}{\textbf{Test in Jira}} \\\cmidrule{2-7}
% % &\textbf{Train in SO} &\textbf{Train in Jira} &\textbf{Train in GitHub} &\textbf{Train in Jira} &\textbf{Train in GitHub} &\textbf{Train in SO} \\\midrule
% % \textbf{SentiMoji} &76 &85 &46 &69 &52 &50 \\
% % \textbf{BERT4SentiSE} &70 &79 &47 &76 &50 &46 \\
% % \bottomrule
% % \end{tabular}%
% % }
% % \label{tab:cross_platform_new_errors}%
% % \end{table}

==> RQ1_tables.tex <==





% % \begin{sidewaystable}
% % \vspace{15cm}
% \begin{table*}%[t]
% \footnotesize
% % \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Performance of SE-specific sentiment analysis in cross-platform settings (SentiSE = SentistrengthSE)}
%   %\vspace{-3mm}
%   % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{ll|rrr|rrr|rrr|rrr|rrr}
%     \toprule{}

%     \multirow{2}{*}{\textbf{Setting}}  & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiSE}}\\
%     \cmidrule{3-17}
%     {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
    
%     %\multicolumn{18}{c}{\textbf{Test dataset: GitHub}} \\
%     %\midrule
 
%      \multirow{5}{1.4cm}{Test:  GitHub Train: GitHub  (Within)}
%      & Negative &  .89 & .85 & .87  & .89 & .91 & .90  & .90 & .89 & .90  & .87 & .69 & .77  & .81 & .71 & .76   \\ 
%      & Neutral &   .87 & .92 & .89  & .92 & .90 & .91   & .89 & .92 & .91  & .77 & .91 & .84  & .74 & .86 & .79   \\ 
%      & Positive &  .94 & .92 & .93  & .93 & .94 & .94   & .94 & .91 & .93  & .89 & .84 & .86  & .85 & .76 & .80   \\ 
%      & Micro-avg &  .90 & .90 & .90  & \textbf{.92} & \textbf{.92} & \textbf{.92}   & .91 & .91 & .91  & .83 & .83 & .83  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .90 & .89 & .90  & \textbf{.91} & \textbf{.92} & \textbf{.92}   & \textbf{.91} & .91 & .91  & .84 & .81 & .82  & .80 & .78 & .78   \\ 

%     \cmidrule{2-17}     

%      % Test dataset: Github
% \multirow{5}{1.4cm}{Test:  GitHub Train: SO  (Cross)}
%  & Negative &  .85 & .62 & .72  & .83 & .73 & .78      & .79 & .56 & .66  & .83 & .37 & .51  & .81 & .71 & .76   \\ 
%  & Neutral &   .67 & .91 & .77  & .71 & .91 & .80      & .71 & .82 & .76  & .60 & .94 & .73  & .74 & .86 & .79   \\ 
%  & Positive &  .88 & .65 & .75  & .88 & .63 & .73   & .76 & .81 & .78  & .86 & .62 & .72  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .75 & .75 & .75  & .78 & .78 & .78   & .74 & .74 & .74  & .68 & .68 & .68  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  .80 & .73 & .75  & \textbf{.81} & .76 & .77   & .75 & .73 & .73  & .76 & .64 & .66  & .80 & \textbf{.78} & \textbf{.78}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.15 & -.15 & -.15 & -.14 & -.14 & -.14 & -.02 & -.02 & -.02 & -.17 & -.17 & -.17 & -.14 & -.14 & -.14  \\ 
% % & & Macro-avg &  -.10 & -.17 & -.15 & -.11 & -.16 & -.15 & .01 & -.05 & -.04 & -.16 & -.18 & -.18 & -.08 & -.17 & -.17  \\ 
% \cmidrule{2-17}
    
    
    
%     % Test dataset: Github
%     \multirow{5}{1.4cm}{Test: GitHub Train: Jira  (Cross)} 
%      & Negative &  .91 & .39 & .55  & .90 & .43 & .58      & .85 & .52 & .64  & .88 & .27 & .41  & .81 & .71 & .76   \\ 
%  & Neutral &       .56 & .98 & .72  & .59 & .97 & .73    & .60 & .96 & .74  & .52 & .98 & .68  & .74 & .86 & .79   \\ 
%  & Positive &      .94 & .45 & .60  & .91 & .51 & .65   & .90 & .46 & .61  & .89 & .38 & .53  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .66 & .66 & .66  & .68 & .68 & .68    & .69 & .69 & .69  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  \textbf{.80} & .61 & .62  & \textbf{.80} & .64 & .65    & .78 & .65 & .67  & .76 & .54 & .54  & \textbf{.80} & \textbf{.78} & \textbf{.78}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.24 & -.24 & -.24 & -.23 & -.23 & -.23 & -.08 & -.08 & -.08 & -.22 & -.22 & -.22 & -.23 & -.23 & -.23  \\ 
% % & & Macro-avg &  -.10 & -.29 & -.28 & -.12 & -.28 & -.26 & .02 & -.14 & -.14 & -.13 & -.26 & -.24 & -.08 & -.27 & -.28  \\ 

% \midrule





% %    \multicolumn{18}{c}{\textbf{Test dataset: Stack Overflow}} \\
% %    \midrule
%     \multirow{5}{1.4cm}{Test: SO Train: SO  (Within)} 
%  & Negative &  .84 & .83 & .83  & .86 & .85 & .85    & .80 & .83 & .82  & .80 & .72 & .76  & .76 & .76 & .76   \\ 
%  & Neutral &  .83 & .84 & .84  & .86 & .85 & .85    & .84 & .79 & .81  & .79 & .82 & .81  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .93 & .93  & .93 & .94 & .93    & .90 & .93 & .91  & .88 & .91 & .89  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}    & .85 & .85 & .85  & .82 & .82 & .82  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}    & .85 & .85 & .85  & .82 & .82 & .82  & .80 & .79 & .79   \\ 
 

%     \cmidrule{2-17}
    
%     % Test dataset: Stack Overflow
%     \multirow{5}{1.4cm}{Test: SO Train: GitHub  (Cross)} 
%  & Negative &  .82 & .76 & .79  & .80 & .86 & .83       & .69 & .76 & .72  & .64 & .49 & .55  & .76 & .76 & .76   \\ 
%  & Neutral &   .75 & .85 & .80  & .84 & .80 & .82    & .73 & .76 & .75  & .65 & .85 & .74  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .85 & .89  & .93 & .91 & .92    & .92 & .82 & .87  & .88 & .74 & .80  & .91 & .82 & .86   \\ 
%  & Micro-avg & .83 & .83 & .83  & \textbf{.85} & \textbf{.85} & \textbf{.85}    & .78 & .78 & .78  & .71 & .71 & .71  & .79 & .79 & .79   \\ 
%  & Macro-avg & .83 & .82 & .82  & \textbf{.85} & \textbf{.86} & \textbf{.85}    & .78 & .78 & .78  & .72 & .69 & .70  & .80 & .79 & .79   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.12 & -.12 & -.12 & -.07 & -.07 & -.07 & -.11 & -.11 & -.11  \\ 
% % & & Macro-avg &  -.03 & -.05 & -.04 & -.03 & -.02 & -.03 & -.11 & -.12 & -.12 & -.06 & -.07 & -.07 & -.10 & -.12 & -.12  \\ 

%     \cmidrule{2-17}


%     % Test dataset: Stack Overflow
%     \multirow{5}{1.4cm}{Test: SO Train: Jira  (Cross)}
%  & Negative &  .93 & .31 & .47  & .88 & .55 & .68      & .75 & .30 & .43  & .67 & .22 & .33  & .76 & .76 & .76   \\ 
%  & Neutral &   .54 & .98 & .70  & .63 & .94 & .76    & .54 & .93 & .69  & .50 & .95 & .66  & .73 & .79 & .75   \\ 
%  & Positive &  .98 & .62 & .76  & .97 & .74 & .84    & .96 & .64 & .76  & .96 & .52 & .67  & .91 & .82 & .86   \\ 
%  & Micro-avg & .67 & .67 & .67  & .76 & .76 & .76    & .66 & .66 & .66  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg & .82 & .64 & .64  & \textbf{.83} & .74 & .76   & .75 & .62 & .63  & .71 & .56 & .55  & .80 & \textbf{.79} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.20 & -.20 & -.20 & -.12 & -.12 & -.12 & -.21 & -.21 & -.21 & -.19 & -.19 & -.19 & -.22 & -.22 & -.22  \\ 
% % & & Macro-avg &  -.05 & -.23 & -.23 & -.05 & -.14 & -.12 & -.12 & -.23 & -.24 & -.10 & -.23 & -.22 & -.11 & -.25 & -.27  \\ 

%     \midrule





%     % Test dataset: Jira
% %    \multicolumn{18}{c}{\textbf{Test dataset: Jira}} \\
% %    \midrule
%     \multirow{5}{1.4cm}{Test: Jira Train: Jira  (Within)} 
%  & Negative &  .84 & .68 & .75  & .82 & .76 & .79      & .71 & .55 & .62  & .79 & .66 & .72  & .68 & .73 & .71   \\ 
%  & Neutral &   .89 & .91 & .90  & .90 & .90 & .90     & .84 & .88 & .86  & .89 & .89 & .89  & .92 & .82 & .87   \\ 
%  & Positive &  .79 & .80 & .79  & .78 & .80 & .79    & .73 & .71 & .72  & .75 & .85 & .80  & .68 & .92 & .78   \\ 
%  & Micro-avg &  \textbf{.86} & \textbf{.86} & \textbf{.86}  & \textbf{.86} & \textbf{.86} & \textbf{.86}    & .81 & .81 & .81  & .85 & .85 & .85  & .83 & .83 & .83   \\ 
%  & Macro-avg &  \textbf{.84} & .80 & .81  & .83 & \textbf{.82} & \textbf{.83}   & .76 & .72 & .73  & .81 & .80 & .80  & .76 & \textbf{.82} & .79   \\ 

%     \cmidrule{2-17}
    
    
%     % Test dataset: Jira
%     \multirow{5}{1.4cm}{Test: Jira Train: GitHub (Cross)} 
%  & Negative &  .63 & .75 & .69  & .66 & .74 & .70     & .61 & .64 & .62  & .69 & .60 & .64  & .68 & .73 & .71   \\ 
%  & Neutral &   .93 & .79 & .85  & .93 & .80 & .86    & .89 & .78 & .83  & .90 & .85 & .87  & .92 & .82 & .87   \\ 
%  & Positive &  .66 & .91 & .77  & .65 & .91 & .76    & .62 & .86 & .72  & .69 & .89 & .78  & .68 & .92 & .78   \\ 
%  & Micro-avg & .81 & .81 & .81  & .81 & .81 & .81    & .78 & .78 & .78  & .82 & .82 & .82  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg & .74 & \textbf{.82} & .77  & .75 & \textbf{.82} & .77    & .71 & .76 & .73  & \textbf{.76}& .78 & .76  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.05 & -.05 & -.05 & -.05 & -.05 & -.05 & -.14 & -.14 & -.14 & -.03 & -.03 & -.03 & -.03 & -.03 & -.03  \\ 
% % & & Macro-avg &  -.09 & .02 & -.04 & -.09 & -.00 & -.05 & -.12 & .05 & -.07 & -.05 & .05 & -.01 & -.05 & -.02 & -.04  \\ 

%     \cmidrule{2-17}
    
    
%     % Test dataset: Jira
%     \multirow{5}{1.4cm}{Test: Jira Train: SO (Cross)}
%  & Negative &  .67 & .68 & .67  & .72 & .68 & .70       & .50 & .29 & .37  & .36 & .06 & .10  & .68 & .73 & .71   \\ 
%  & Neutral &   .92 & .81 & .86  & .92 & .82 & .87    & .82 & .81 & .81  & .75 & .94 & .83  & .92 & .82 & .87   \\ 
%  & Positive &  .67 & .93 & .78  & .65 & .93 & .76    & .59 & .80 & .68  & .71 & .49 & .58  & .68 & .92 & .78   \\ 
%  & Micro-avg & .82 & .82 & .82  & .82 & .82 & .82    & .74 & .74 & .74  & .73 & .73 & .73  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg & .75 & .81 & .77  & \textbf{.76} & .81 & .78    & .64 & .63 & .62  & .61 & .49 & .50  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.07 & -.07 & -.07 & -.12 & -.12 & -.12  \\ 
% % & & Macro-avg &  -.08 & .01 & -.04 & -.07 & -.01 & -.05 & -.05 & .06 & .00 & -.12 & -.08 & -.11 & -.20 & -.30 & -.30  \\ 


%     \bottomrule
%     \end{tabular}%
% %}
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance}%
% \end{table*}%
% % \end{sidewaystable}





% % \begin{sidewaystable}
% % \vspace{15cm}
% \begin{table*}%[t]
% \footnotesize
% % \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Performance drop in SE-specific supervised sentiment analysis tools in cross-platform settings (SO = Stack Overflow)}
%   %\vspace{-3mm}
%   % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{cl|rrr|rrr|rrr|rrr}
%     \toprule{}

%     \multirow{2}{*}{\textbf{Train}} & \multirow{2}{*}{\textbf{Performance}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} &  \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} \\
%     \cmidrule{3-14}
%     \textbf{Dataset} & \centering \textbf{Drop} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
    
%     \multicolumn{14}{c}{\textbf{Test dataset: GitHub}} \\
%     \midrule
 
%     \multirow{2}{*}{\textbf{SO}} & $\triangledown$ Micro-avg &  -16\% & -16\% & -16\% & -15\% & -15\% & -15\%  & -18\% & -18\% & -18\% & -17\% & -17\% & -17\%    \\ 
%     &  $\triangledown$ Macro-avg &  -11\% & -19\% & -17\% & -12\% & -18\% & -16\% &  -17\% & -20\% & -19\% & -10\% & -21\% & -20\%  \\ 
%     \cmidrule{2-14}
    
%     \multirow{2}{*}{\textbf{Jira}} &  $\triangledown$ Micro-avg &  -27\% & -27\% & -27\% & -26\% & -26\% & -26\%  & -24\% & -24\% & -24\% & -27\% & -27\% & -27\%   \\ 
%     &  $\triangledown$ Macro-avg &  -11\% & -32\% & -31\% & -13\% & -31\% & -29\% &  -14\% & -29\% & -27\% & -9\% & -34\% & -34\%  \\ 
%     % \cmidrule{2-17}
%     \midrule
    
    
%     \multicolumn{14}{c}{\textbf{Test dataset: Stack Overflow}} \\
%     \midrule
%     \multirow{2}{*}{\textbf{GitHub}} & $\triangledown$  Micro-avg &  -5\% & -5\% & -5\% & -3\% & -3\% & -3\% &  -8\% & -8\% & -8\% & -13\% & -13\% & -13\%   \\ 
%     & $\triangledown$  Macro-avg &  -4\% & -5\% & -5\% & -3\% & -3\% & -3\%  & -7\% & -8\% & -8\% & -12\% & -15\% & -15\%  \\ 
%     \cmidrule{2-14}
%     \multirow{2}{*}{\textbf{Jira}} &  $\triangledown$ Micro-avg &  -23\% & -23\% & -23\% & -13\% & -13\% & -13\%  & -22\% & -22\% & -22\% & -27\% & -27\% & -27\%   \\ 
%     &  $\triangledown$ Macro-avg &  -6\% & -27\% & -26\% & -6\% & -16\% & -14\%  & -11\% & -27\% & -26\% & -14\% & -31\% & -33\%  \\ 
%     % \cmidrule{2-17}
%     \midrule
    
%     \multicolumn{14}{c}{\textbf{Test dataset: Jira}} \\
%     \midrule
%     \multirow{2}{*}{\textbf{GitHub}} &  $\triangledown$ Micro-avg &  -6\% & -6\% & -6\% & -6\% & -6\% & -6\% &  -4\% & -4\% & -4\% & -3\% & -3\% & -3\%    \\ 
%     &  $\triangledown$ Macro-avg &  -11\% & 3\% & -5\% & -10\% & 0\% & -7\% &  -7\% & 7\% & -1\% & -6\% & -2\% & -5\%  \\ 
%     \cmidrule{2-14}
%     \multirow{2}{*}{\textbf{SO}} & $\triangledown$  Micro-avg &  -5\% & -5\% & -5\% & -5\% & -5\% & -5\%  & -9\% & -9\% & -9\% & -14\% & -14\% & -14\%   \\ 
%     &  $\triangledown$ Macro-avg &  -10\% & 1\% & -5\% & -8\% & -1\% & -6\%  & -16\% & -12\% & -15\% & -25\% & -38\% & -37\%  \\ 
%     % \cmidrule{2-17}
%     \midrule



%     \bottomrule
%     \end{tabular}%
% %}
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance_drop}%
% \end{table*}%
% % \end{sidewaystable}





% \begin{figure*}[t]
% \centering
% \captionsetup[subfigure]{labelformat=empty}
% \pgfplotstableread{

% 1	.88  .97 .75 .77     .88  .97  .82 .85      .87  .96  .77 .77
% 2	.87  .96 .62 .65     .85  .93  .64 .76      .85  .93  .77 .78
% }\datatable
%       \subfloat[Test on GitHub]
%       {
%       \resizebox{1.5in}{!}{%
%       \begin{tikzpicture}
%         	\begin{axis}[
%         	%ylabel=label,
%         	xtick=data,
%         	xticklabels={Trained on SO, Trained on Jira},
%         	enlarge y limits=false,
%         	enlarge x limits=0.55,
%         % 	axis y line = none,
%         % 	axis y line=left,
%         %   axis line style={-},
%             axis y line=none,
%             % hide y axis,
%             axis x line*=bottom,
%             axis y line*=left,
%         % 	axis x line=left,
%         % 	axis x line=bottom,
%         % 	axis line style={draw=none},
%         %	nodes near coords,
%         	ymin=0,ymax=1,
%         	ybar,
%         	bar width=0.7cm,
%         	width=3.6in,
%         	height = 2.3in,
%         % 	ytick={0,20,...,80},
%             % yticklabels={0\%,20\%,40\%,60\%,80\%},
%         	%ylabel={Accepted Answer (\%)},
%         	ymajorgrids=false,
%         %	xminorgrids=true,
%          	yticklabel style={font=\LARGE},
%         	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
%         	major x tick style = {opacity=0},
%         	minor x tick num = 1,    
%         	minor tick length=1ex,
%         	legend columns=2, 
%             legend style={
%                 /tikz/column 2/.style={
%                     column sep=5pt,
%                 },
%                 },
%         	legend style={at={(0.5,1.40)},
%         	legend style={font=\LARGE},
%             anchor=north,legend columns=-1
%             },
%             % nodes near coords,
%             nodes near coords style={font=\huge},
%             nodes near coords style={rotate=90,  anchor=west}, %
%         	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
%         	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
%         	]
%         	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=1] \datatable;
%         	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=2] \datatable;
%         	\addplot[draw=black!80, fill=black!70] table[x index=0,y index=3] \datatable;
%         	\addplot[draw=black!80, fill=black!100] table[x index=0,y index=4] \datatable;
        
%             \legend{JS Divergence,
%             		 Cosine Similarity,
%             		 }
%         	\end{axis}
%     	\end{tikzpicture}
%      	}
%     %  	\hspace{-1mm}
%     	\label{presentation-inconsistency}
%     } 
%     \subfloat[Test on Stack Overflow (SO)]
%      {
%       \resizebox{1.5in}{!}{%
%       \begin{tikzpicture}
%         	\begin{axis}[
%         	%ylabel=label,
%         	xtick=data,
%         	xticklabels={Train on GitHub, Train on Jira},
%         	enlarge y limits=false,
%         	enlarge x limits=0.55,
%         % 	axis y line = none,
%         % 	axis y line=left,
%         %   axis line style={-},
%             axis y line=none,
%             % hide y axis,
%             axis x line*=bottom,
%             axis y line*=left,
%         % 	axis x line=left,
%         % 	axis x line=bottom,
%         % 	axis line style={draw=none},
%         %	nodes near coords,
%         	ymin=0,ymax=1,
%         	ybar,
%         	bar width=0.7cm,
%         	width=3.6in,
%         	height = 2.3in,
%         % 	ytick={0,20,...,80},
%             % yticklabels={0\%,20\%,40\%,60\%,80\%},
%         	%ylabel={Accepted Answer (\%)},
%         	ymajorgrids=false,
%         %	xminorgrids=true,
%          	yticklabel style={font=\LARGE},
%          	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
%         	major x tick style = {opacity=0},
%         	minor x tick num = 1,    
%         	minor tick length=1ex,
%         	legend columns=2, 
%             legend style={
%                 /tikz/column 2/.style={
%                     column sep=5pt,
%                 },
%                 },
%         	legend style={at={(0.5,1.40)},
%         	legend style={font=\LARGE},
%             anchor=north,legend columns=-1
%             },
%             nodes near coords style={font=\huge},
%             nodes near coords style={rotate=90,  anchor=west}, %
%         	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
%         	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
%         	]
%         	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=5] \datatable; 
%         	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=6] \datatable; %, postaction={pattern=horizontal lines}
%         	\addplot[draw=black!80, fill=black!60] table[x index=0,y index=7] \datatable;   %, postaction={pattern=vertical lines}
%             \addplot[draw=black!80, fill=black!100] table[x index=0,y index=8] \datatable;  %, postaction={pattern=vertical lines}
%             \legend{,,
%             		 SEntiMoji F1,
%             		 BERT4SentiSE F1
%             		 }
%             % \legend{JS Divergence,
%             % 		 Cosine Similarity,
%             % 		 SEntiMoji F1,
%             % 		 BERT4SentiSE F1
%             % 		 }
%         	\end{axis}
%     	\end{tikzpicture}
%     	}
%     % 	\hspace{-1mm}
%     	\label{signature-inconsistency}
%     }
%     \subfloat[Test on Jira]
%      {
%       \resizebox{1.5in}{!}{%
%       \begin{tikzpicture}
%         	\begin{axis}[
%         	%ylabel=label,
%         	xtick=data,
%         	xticklabels={Train on GitHub, Train on SO
%         	},
%         	enlarge y limits=false,
%         	enlarge x limits=0.55,
%             axis y line=none,
%             % hide y axis,
%             axis x line*=bottom,
%             axis y line*=left,,
%         	ymin=0,ymax=1.08,
%         	ybar,
%         	bar width=0.7cm,
%         	width=3.4in,
%         	height = 2.3in,
%         % 	ytick={0,20,...,80},
%         %     yticklabels={0\%,20\%,40\%,60\%,80\%},
%         	%ylabel={Accepted Answer (\%)},
%         	ymajorgrids=false,
%         %	xminorgrids=true,
%          	yticklabel style={font=\LARGE},
%          	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
%         	major x tick style = {opacity=0},
%         	minor x tick num = 1,    
%         	minor tick length=1ex,
%         	legend style={
%          	at={(0.6,0.98)},
%             anchor=north,legend columns=-1
%             },
%             nodes near coords style={font=\huge},
%             nodes near coords style={rotate=90,  anchor=west}, %
%         	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
%         	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
%         	]
%         	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=9] \datatable;
%         	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=10] \datatable; %, postaction={pattern=horizontal lines}
%         	\addplot[draw=black!80, fill=black!60] table[x index=0,y index=11] \datatable; %, postaction={pattern=vertical lines}
%             \addplot[draw=black!80, fill=black!100] table[x index=0,y index=12] \datatable; %, postaction={pattern=vertical lines}

%         	\end{axis}
%     	\end{tikzpicture}
%     	}
%     % 	%\hspace{-1mm}
%     	\label{fig:status-inconsistency}
%     }
    


    
    
% %\vspace{-3mm}
% \caption{Similarity scores between datasets vs Macro F1-scores per tool (BERT4SentiSE \& SentiMoji) in cross platform settings}


% \vspace{-3mm}
% \label{fig:diversity_performance}
% \end{figure*}







% \begin{sidewaystable}
% \vspace{15cm}
% % \begin{table}
% \renewcommand{\thetable}{\arabic{table}a}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Performance of SE-specific sentiment analysis in cross-platform setting (\bf{Test dataset: GitHub)}}
%     \begin{tabular}{ll|rrr|rrr|rrr|rrr|rrr|ccc}
%     \toprule
%     \multirow{2}{*}{\textbf{Train Dataset}}  & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiSE}}\\
%     \cmidrule{3-20}
%     {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
% \multirow{5}{*}{\parbox{2cm} {\centering GitHub \\ (Within Platform)}} 
% & Negative &  .91 & .39 & .55  & .90 & .43 & .58  & .75 & .39 & .52  & .85 & .52 & .64  & .88 & .27 & .41  & .81 & .71 & .76   \\ 
%  & Neutral &  .56 & .98 & .72  & .59 & .97 & .73  & .54 & .95 & .69  & .60 & .96 & .74  & .52 & .98 & .68  & .74 & .86 & .79   \\ 
%  & Positive &  .94 & .45 & .60  & .91 & .51 & .65  & .80 & .30 & .44  & .90 & .46 & .61  & .89 & .38 & .53  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .66 & .66 & .66  & .68 & .68 & .68  & .60 & .60 & .60  & .69 & .69 & .69  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  \textbf{.80} & .61 & .62  & \textbf{.80} & .64 & .65  & .70 & .55 & .55  & .78 & .65 & .67  & .76 & .54 & .54  & \textbf{.80} & \textbf{.78} & \textbf{.78}   \\
% % \cmidrule{2-20} 
% \midrule

% \multirow{5}{*}{\parbox{2cm} {\centering Stack Overflow \\ (Cross Platform)}} 
%  & Negative &  .85 & .62 & .72  & .83 & .73 & .78  & .69 & .49 & .58  & .79 & .56 & .66  & .83 & .37 & .51  & .81 & .71 & .76   \\ 
%  & Neutral &  .67 & .91 & .77  & .71 & .91 & .80  & .61 & .84 & .71  & .71 & .82 & .76  & .60 & .94 & .73  & .74 & .86 & .79   \\ 
%  & Positive &  .88 & .65 & .75  & .88 & .63 & .73  & .78 & .57 & .66  & .76 & .81 & .78  & .86 & .62 & .72  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .75 & .75 & .75  & .78 & .78 & .78  & .66 & .66 & .66  & .74 & .74 & .74  & .68 & .68 & .68  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  .80 & .73 & .75  & \textbf{.81} & .76 & .77  & .69 & .63 & .65  & .75 & .73 & .73  & .76 & .64 & .66  & .80 & \textbf{.78} & \textbf{.78}   \\ 
%  \cmidrule{2-20}
% \multirow{2}{2cm}{Difference with within-platform} & Micro-avg &  -.15 & -.15 & -.15 & -.14 & -.14 & -.14 & -.02 & -.02 & -.02 & -.17 & -.17 & -.17 & -.14 & -.14 & -.14 & & \multirow{2}{*}{NA}   \\ 
% & Macro-avg &  -.10 & -.17 & -.15 & -.11 & -.16 & -.15 & .01 & -.05 & -.04 & -.16 & -.18 & -.18 & -.08 & -.17 & -.17  \\ 

% \midrule


% \multirow{5}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%      & Negative &  .91 & .39 & .55  & .90 & .43 & .58  & .75 & .39 & .52  & .85 & .52 & .64  & .88 & .27 & .41  & .81 & .71 & .76   \\ 
%  & Neutral &  .56 & .98 & .72  & .59 & .97 & .73  & .54 & .95 & .69  & .60 & .96 & .74  & .52 & .98 & .68  & .74 & .86 & .79   \\ 
%  & Positive &  .94 & .45 & .60  & .91 & .51 & .65  & .80 & .30 & .44  & .90 & .46 & .61  & .89 & .38 & .53  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .66 & .66 & .66  & .68 & .68 & .68  & .60 & .60 & .60  & .69 & .69 & .69  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  \textbf{.80} & .61 & .62  & \textbf{.80} & .64 & .65  & .70 & .55 & .55  & .78 & .65 & .67  & .76 & .54 & .54  & \textbf{.80} & \textbf{.78} & \textbf{.78}   \\ 
% \cmidrule{2-20} 
% \multirow{2}{2cm}{Difference with within-platform} & Micro-avg &  -.24 & -.24 & -.24 & -.23 & -.23 & -.23 & -.08 & -.08 & -.08 & -.22 & -.22 & -.22 & -.23 & -.23 & -.23 & &  \multirow{2}{*}{NA}   \\ 
% & Macro-avg &  -.10 & -.29 & -.28 & -.12 & -.28 & -.26 & .02 & -.14 & -.14 & -.13 & -.26 & -.24 & -.08 & -.27 & -.28  \\ 


%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance_github}%
% % \end{table}%
% \end{sidewaystable}


% % =================================================================================================================== b

% \begin{sidewaystable}
% \vspace{15cm}
% % \begin{table}
% \addtocounter{table}{-1}
% \renewcommand{\thetable}{\arabic{table}b}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Performance of SE-specific sentiment analysis in cross-platform setting (\bf{Test dataset: Stack Overflow)}}
%     \begin{tabular}{ll|rrr|rrr|rrr|rrr|rrr|rrr}
%     \toprule
%     \multirow{2}{*}{\textbf{Train Dataset}}  & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiSE}}\\
%     \cmidrule{3-20}
%     {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
% \multirow{5}{*}{\parbox{2cm} {\centering Stack Overflow \\ (Within Platform)}} 
%  & Negative &  .84 & .83 & .83  & .86 & .85 & .85  & .74 & .73 & .74  & .80 & .83 & .82  & .80 & .72 & .76  & .76 & .76 & .76   \\ 
%  & Neutral &  .83 & .84 & .84  & .86 & .85 & .85  & .75 & .77 & .76  & .84 & .79 & .81  & .79 & .82 & .81  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .93 & .93  & .93 & .94 & .93  & .85 & .85 & .85  & .90 & .93 & .91  & .88 & .91 & .89  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}  & .78 & .78 & .78  & .85 & .85 & .85  & .82 & .82 & .82  & .79 & .79 & .79 \\ 
%  & Macro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}  & .78 & .78 & .78  & .85 & .85 & .85  & .82 & .82 & .82  & .80 & .79 & .79   \\ 

% % \cmidrule{2-20} 
% \midrule

% \multirow{5}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & Negative &  .82 & .76 & .79  & .80 & .86 & .83  & .66 & .60 & .63  & .69 & .76 & .72  & .64 & .49 & .55  & .76 & .76 & .76   \\ 
%  & Neutral &  .75 & .85 & .80  & .84 & .80 & .82  & .61 & .64 & .63  & .73 & .76 & .75  & .65 & .85 & .74  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .85 & .89  & .93 & .91 & .92  & .73 & .74 & .74  & .92 & .82 & .87  & .88 & .74 & .80  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .83 & .83 & .83  & \textbf{.85} & \textbf{.85} & \textbf{.85}  & .67 & .67 & .67  & .78 & .78 & .78  & .71 & .71 & .71  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .83 & .82 & .82  & \textbf{.85} & \textbf{.86} & \textbf{.85}  & .67 & .66 & .66  & .78 & .78 & .78  & .72 & .69 & .70  & .80 & .79 & .79   \\ 
%  \cmidrule{2-20}
% \multirow{2}{2cm}{Difference with within-platform} & Micro-avg &  -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.12 & -.12 & -.12 & -.07 & -.07 & -.07 & -.11 & -.11 & -.11  & & \multirow{2}{*}{NA}   \\ 
%  & Macro-avg &  -.03 & -.05 & -.04 & -.03 & -.02 & -.03 & -.11 & -.12 & -.12 & -.06 & -.07 & -.07 & -.10 & -.12 & -.12  \\ 

% \midrule


% \multirow{5}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%  & Negative &  .93 & .31 & .47  & .88 & .55 & .68  & .66 & .31 & .42  & .75 & .30 & .43  & .67 & .22 & .33  & .76 & .76 & .76   \\ 
%  & Neutral &  .54 & .98 & .70  & .63 & .94 & .76  & .50 & .91 & .65  & .54 & .93 & .69  & .50 & .95 & .66  & .73 & .79 & .75   \\ 
%  & Positive &  .98 & .62 & .76  & .97 & .74 & .84  & .83 & .42 & .56  & .96 & .64 & .76  & .96 & .52 & .67  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .67 & .67 & .67  & .76 & .76 & .76  & .58 & .58 & .58  & .66 & .66 & .66  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  .82 & .64 & .64  & \textbf{.83} & .74 & .76  & .66 & .55 & .54  & .75 & .62 & .63  & .71 & .56 & .55  & .80 & \textbf{.79} & \textbf{.79}   \\ 

% \cmidrule{2-20} 
% \multirow{2}{2cm}{Difference with within-platform} & Micro-avg &  -.20 & -.20 & -.20 & -.12 & -.12 & -.12 & -.21 & -.21 & -.21 & -.19 & -.19 & -.19 & -.22 & -.22 & -.22 & & \multirow{2}{*}{NA}   \\ 
% & Macro-avg &  -.05 & -.23 & -.23 & -.05 & -.14 & -.12 & -.12 & -.23 & -.24 & -.10 & -.23 & -.22 & -.11 & -.25 & -.27  \\  


%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance_so}%
% % \end{table}%
% \end{sidewaystable}


% % =================================================================================================================== c

% \begin{sidewaystable}
% \vspace{15cm}
% % \begin{table}
% \addtocounter{table}{-1}
% \renewcommand{\thetable}{\arabic{table}c}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Performance of SE-specific sentiment analysis in cross-platform setting (\bf{Test dataset: Jira)}}
%     \begin{tabular}{ll|rrr|rrr|rrr|rrr|rrr|rrr}
%     \toprule
%     \multirow{2}{*}{\textbf{Train Dataset}}  & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiSE}}\\
%     \cmidrule{3-20}
%     {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
% \multirow{5}{*}{\parbox{2cm} {\centering Jira \\ (Within Platform)}} 
%  & Negative &  .84 & .68 & .75  & .82 & .76 & .79  & .69 & .46 & .55  & .71 & .55 & .62  & .79 & .66 & .72  & .68 & .73 & .71   \\ 
%  & Neutral &  .89 & .91 & .90  & .90 & .90 & .90  & .83 & .89 & .86  & .84 & .88 & .86  & .89 & .89 & .89  & .92 & .82 & .87   \\ 
%  & Positive &  .79 & .80 & .79  & .78 & .80 & .79  & .73 & .72 & .72  & .73 & .71 & .72  & .75 & .85 & .80  & .68 & .92 & .78   \\ 
%  & Micro-avg &  \textbf{.86} & \textbf{.86} & \textbf{.86}  & \textbf{.86} & \textbf{.86} & \textbf{.86}  & .80 & .80 & .80  & .81 & .81 & .81  & .85 & .85 & .85  & .83 & .83 & .83   \\ 
%  & Macro-avg &  \textbf{.84} & .80 & .81  & .83 & \textbf{.82} & \textbf{.83}  & .75 & .69 & .71  & .76 & .72 & .73  & .81 & .80 & .80  & .76 & \textbf{.82} & .79   \\ 

% % \cmidrule{2-20} 
% \midrule

% \multirow{5}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & Negative &  .63 & .75 & .69  & .66 & .74 & .70  & .51 & .71 & .60  & .61 & .64 & .62  & .69 & .60 & .64  & .68 & .73 & .71   \\ 
%  & Neutral &  .93 & .79 & .85  & .93 & .80 & .86  & .92 & .58 & .71  & .89 & .78 & .83  & .90 & .85 & .87  & .92 & .82 & .87   \\ 
%  & Positive &  .66 & .91 & .77  & .65 & .91 & .76  & .45 & .92 & .61  & .62 & .86 & .72  & .69 & .89 & .78  & .68 & .92 & .78   \\ 
%  & Micro-avg &  .81 & .81 & .81  & .81 & .81 & .81  & .66 & .66 & .66  & .78 & .78 & .78  & .82 & .82 & .82  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg &  .74 & \textbf{.82} & .77  & .75 & \textbf{.82} & .77  & .63 & .74 & .64  & .71 & .76 & .73  & \textbf{.76} & .78 & .76  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\
%  \cmidrule{2-20}
% \multirow{2}{2cm}{Difference with within-platform} & Micro-avg &  -.05 & -.05 & -.05 & -.05 & -.05 & -.05 & -.14 & -.14 & -.14 & -.03 & -.03 & -.03 & -.03 & -.03 & -.03 & & \multirow{2}{*}{NA}   \\ 
% &  Macro-avg &  -.09 & .02 & -.04 & -.09 & -.00 & -.05 & -.12 & .05 & -.07 & -.05 & .05 & -.01 & -.05 & -.02 & -.04  \\ 

% \midrule


% \multirow{5}{*}{\parbox{2cm} {\centering Stack Overflow \\ (Cross Platform)}} 
%  & Negative &  .67 & .68 & .67  & .72 & .68 & .70  & .58 & .61 & .59  & .50 & .29 & .37  & .36 & .06 & .10  & .68 & .73 & .71   \\ 
%  & Neutral &  .92 & .81 & .86  & .92 & .82 & .87  & .88 & .77 & .82  & .82 & .81 & .81  & .75 & .94 & .83  & .92 & .82 & .87   \\ 
%  & Positive &  .67 & .93 & .78  & .65 & .93 & .76  & .62 & .89 & .73  & .59 & .80 & .68  & .71 & .49 & .58  & .68 & .92 & .78   \\ 
%  & Micro-avg &  .82 & .82 & .82  & .82 & .82 & .82  & .77 & .77 & .77  & .74 & .74 & .74  & .73 & .73 & .73  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg &  .75 & .81 & .77  & \textbf{.76} & .81 & .78  & .69 & .75 & .71  & .64 & .63 & .62  & .61 & .49 & .50  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\  

% \cmidrule{2-20} 
% \multirow{2}{2cm}{Difference with within-platform} & Micro-avg &  -.04 & -.04 & -.04 & -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.07 & -.07 & -.07 & -.12 & -.12 & -.12 & & \multirow{2}{*}{NA}   \\ 
% &  Macro-avg &  -.08 & .01 & -.04 & -.07 & -.01 & -.05 & -.05 & .06 & .00 & -.12 & -.08 & -.11 & -.20 & -.30 & -.30  \\


%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance_jira}%
% % \end{table}%
% \end{sidewaystable}













% \begin{sidewaystable}
% \vspace{15cm}

% \end{sidewaystable}





% \begin{sidewaystable}
% \vspace{15cm}
\begin{table*}%[t]
\footnotesize
% \small
  \centering
  %\vspace{-.1in}
  \caption{Performance drop in SE-specific supervised sentiment analysis tools in cross-platform settings (SO = Stack Overflow)}
  %\vspace{-3mm}
  % \resizebox{\textwidth}{!}{%
    \begin{tabular}{cl|rrr|rrr|rrr|rrr|rrr}
    \toprule{}

    \multirow{2}{*}{\textbf{Train}} & \multirow{2}{*}{\textbf{Performance}} & 
    \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} \\
    \cmidrule{3-17}
    \textbf{Dataset} & \centering \textbf{Drop} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
    \midrule
    
    \multicolumn{17}{c}{\textbf{Test dataset: GitHub}} \\
    \midrule
 
    \multirow{2}{*}{\textbf{SO}} & $\triangledown$ Micro-avg &  -16\% & -16\% & -16\% & -15\% & -15\% & -15\% & -3\% & -3\% & -3\% & -18\% & -18\% & -18\% & -17\% & -17\% & -17\%    \\ 
    &  $\triangledown$ Macro-avg &  -11\% & -19\% & -17\% & -12\% & -18\% & -16\% & 2\% & -8\% & -5\% & -17\% & -20\% & -19\% & -10\% & -21\% & -20\%  \\ 
    \cmidrule{2-17}
    
    \multirow{2}{*}{\textbf{Jira}} &  $\triangledown$ Micro-avg &  -27\% & -27\% & -27\% & -26\% & -26\% & -26\% & -12\% & -12\% & -12\% & -24\% & -24\% & -24\% & -27\% & -27\% & -27\%   \\ 
    &  $\triangledown$ Macro-avg &  -11\% & -32\% & -31\% & -13\% & -31\% & -29\% & 2\% & -21\% & -20\% & -14\% & -29\% & -27\% & -9\% & -34\% & -34\%  \\ 
    % \cmidrule{2-17}
    \midrule
    
    
    \multicolumn{17}{c}{\textbf{Test dataset: Stack Overflow}} \\
    \midrule
    \multirow{2}{*}{\textbf{GitHub}} & $\triangledown$  Micro-avg &  -5\% & -5\% & -5\% & -3\% & -3\% & -3\% & -15\% & -15\% & -15\% & -8\% & -8\% & -8\% & -13\% & -13\% & -13\%   \\ 
    & $\triangledown$  Macro-avg &  -4\% & -5\% & -5\% & -3\% & -3\% & -3\% & -15\% & -15\% & -15\% & -7\% & -8\% & -8\% & -12\% & -15\% & -15\%  \\ 
    \cmidrule{2-17}
    \multirow{2}{*}{\textbf{Jira}} &  $\triangledown$ Micro-avg &  -23\% & -23\% & -23\% & -13\% & -13\% & -13\% & -26\% & -26\% & -26\% & -22\% & -22\% & -22\% & -27\% & -27\% & -27\%   \\ 
    &  $\triangledown$ Macro-avg &  -6\% & -27\% & -26\% & -6\% & -16\% & -14\% & -15\% & -30\% & -31\% & -11\% & -27\% & -26\% & -14\% & -31\% & -33\%  \\ 
    % \cmidrule{2-17}
    \midrule
    
    \multicolumn{17}{c}{\textbf{Test dataset: Jira}} \\
    \midrule
    \multirow{2}{*}{\textbf{GitHub}} &  $\triangledown$ Micro-avg &  -6\% & -6\% & -6\% & -6\% & -6\% & -6\% & -17\% & -17\% & -17\% & -4\% & -4\% & -4\% & -3\% & -3\% & -3\%    \\ 
    &  $\triangledown$ Macro-avg &  -11\% & 3\% & -5\% & -10\% & 0\% & -7\% & -16\% & 7\% & -10\% & -7\% & 7\% & -1\% & -6\% & -2\% & -5\%  \\ 
    \cmidrule{2-17}
    \multirow{2}{*}{\textbf{SO}} & $\triangledown$  Micro-avg &  -5\% & -5\% & -5\% & -5\% & -5\% & -5\% & -4\% & -4\% & -4\% & -9\% & -9\% & -9\% & -14\% & -14\% & -14\%   \\ 
    &  $\triangledown$ Macro-avg &  -10\% & 1\% & -5\% & -8\% & -1\% & -6\% & -7\% & 9\% & 1\% & -16\% & -12\% & -15\% & -25\% & -38\% & -37\%  \\ 
    % \cmidrule{2-17}
    \midrule



    \bottomrule
    \end{tabular}%
%}
  % \vspace{-.25in}
  \label{tab:cross_platform_performance_drop}%
\end{table*}%
% \end{sidewaystable}


==> RQ2.tex <==

\subsection{RQ$_3$ Can similarity analysis between the studied datasets explain the drop in performance 
of the deep learning SD tools in the datasets in cross-platform settings?}\label{sec:rq-cross-platform-similarity}
\subsubsection{Motivation} Across the supervised SD tools for SE in our three studied datasets, we observe 
a drop in performance in cross-platform settings. While the two deep learning SD tools (BERT4SentiSE and SentiMoji) offer better performance than the 
other supervised SD tools in the majority of cross-platform settings, their performance still varies across the datasets. 
For example, as we noted in RQ$_1$, the tools suffered the most performance drop when the tools were trained in Jira and then tested in the other two datasets. Intuitively, the more similar the textual contents are between the pair of datasets, the less drop we can expect in performance for a tool in those two datasets in cross-platform settings. Therefore, it 
is important to know whether there is a correlation between content similarity of the studied datasets and the performance 
of the studied tools in cross-platform settings. 

% While we observe a drop in performance in
% cross-platform settings, the drop is not uniform across the datasets.
% Intuitively, the more similar the two datasets are in terms of textual contents,
% the less drop in performance we may expect for a tool in cross-platform
% settings. This assumption, however, can be challenged when the two datasets
% differ in size (among other differences). Therefore, it would be interesting to
% know whether and how the similarity between the datasets in our study could be
% correlated with their performance in the tools for cross-platform settings. Such
% insights can be useful to decide when cross-platform adoption of a tool is more
% useful for a suite of SE-specific datasets.


% From our RQ1, we find that DL-based tools perform quite well in within platform and slightly better in cross-platform settings. 
%
% From RQ1, we observer a drop in performance for all machine learning based classifiers. Additionally we notice the drop is more steep when trained on Jira dataset. So, in this research question we aim to explore the correlation of divergence, i.e., difference between each pair of these three benchmark datasets and the drop in performance in cross platform settings. 
% Table \ref{tab:cross_platform_performance} shows that the performance of the DL-based classifiers are not significantly better than shallow ML-based classifiers. But SEntiMoji and BERT4SentiSE are pre-trained DL-based classifier that are already trained on large NLP datasets. These models already have an intuitive understanding about language and use transfer learning to train and learn on new tasks. So, generally we expect that the performance of these pre-trained DL-based tools will be better in cross platform settings (i.e., datasets from different distributions) than shallow ML-based classifiers. 
% However,  So, it motivated us to investigate further into analysing the similarity and diversity of these datasets and their correlation with performance of DL-based classifiers on them in cross platform settings.
% Ideally we want to find the how similar these datasets
% are in terms of software domain specific context. As these three datasets come
% from three different type of software engineering platforms, we expect there are
% certain technical jargons that are common in them and some are more prevalent in
% one dataset than others. 

\subsubsection{Approach} For this analysis, we focus on the two best performing deep learning SD tools for SE from RQ$_1$, i.e., BERT4SentiSE and SentiMoji. 
For each tool and for each cross-platform setting involving two datasets (i.e., one dataset for training and another for testing). we analyze whether there is any correlation between the performance 
of the tool in cross-platform settings and the textual similarity between the two datasets. 
We compute the similarity
between two datasets using two standard metrics, Cosine similarity, and Jensen-Shannon Divergence. We discuss below how we use the two metrics to compute the similarity between two given datasets.

\begin{inparaenum}[(1)]
\item\bf{Cosine similarity~\cite{Manning-IRIntroBook-Cambridge2009}} helps to
find text similarity between two documents irrespective of the size of the
documents.
For each dataset, we take the top 10,000 unigrams after removing stopwords (we
used stopwords from the Python `nltk' library). We then combine those to create a
unified vocabulary list ($V$) for all the datasets. We use $V$ to create a
vectorized representation of each dataset based on the frequency of the words of
each sentence in the dataset. For any two datasets (e.g., A, B), we fed their
resulting vectors into \eq\ref{eq:consine} to compute the similarity between the two
datasets. We cosine\_similarity method from Sklearn library
\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.metrics.pairwise.cosine_similarity.html}}.
%The higher the Cosine distance, the more similar the datasets are.

\begin{equation}\label{eq:consine}
Cosine_{Similarity}(A,B) = \frac{A.B}{|A||B|}   
\end{equation}

\item \bf{Jensen-Shannon Divergence~\cite{fuglede2004jensen} ($D_{JS}$)} is a
symmetric and smoothed version of Kullback-Leibler Divergence $D_{KL}$,
$D_{KL}(A||B) = \sum_{i}^{N} a_i log \frac{a_i}{b_i}$. $D_{KL}$ is a probability
distribution of A and B. While $D_{KL}$ is undefined when any element $a_i \in
A$, has zero probability. Whereas, $D_{JS}$ is a probability distribution of
every word in vocabulary $V$. The metric is originally proposed to calculate the
similarity between two datasets A and B as follows:
\begin{equation}\label{eq:jsd}
D_{JS}(A,B) = \frac{1}{2} [D_{KL}(A||B)+D_{KL}(B||A)]    
\end{equation} With \eq\ref{eq:jsd}, a value of $D_{JS}$ = 0, it signifies the
datasets are most similar a value of 1.0 denotes they are completely different.
Given that Cosine similarity adopts an opposite notion for similarity (i.e., 1
as completely similar), we change \eq\ref{eq:jsd} as follows:
\begin{equation}\label{eq:jsd}
D_{JS}(A,B) = 1- \frac{1}{2} [D_{KL}(A||B)+D_{KL}(B||A)]    
\end{equation} Thus in our case, when $D_{JS}$ = 1.0, it signifies the datasets
are most similar and when $D_{JS}$ = 0.0 it signifies that the datasets are
completely diverse from each other. We compute the metric for each pair of
datasets (A, B) as follows. Similar to cosine similarity approach we create a
vectorized representation of each dataset. For any two datasets (e.g., A, B), we
fed their resulting vectors into \eq\ref{eq:jsd} to compute $D_{JS}$ similarity
between the two datasets.
\end{inparaenum} 

% We also report the internal $D_{JS}$ for each datasets. We randomly shuffle each datasets for 50 times and then we divide each dataset in two equal halves. Then we calculate the $D_{JS}$ for this two halves. Then we report the mean and standard deviation for the 50 $D_{JS}$ distance values for each dataset.

We compute the correlation between the similarity in the two datasets and the performance of a tool in cross-platform settings using 
Mann-Whitney (MW) U Test~\cite{mcknight2010mann}. MW test is non-parametric, which is suitable for our data where data is not normally distributed. We report the significance of correlation using p-value and the effect size using Cliff's $\delta$ value. 
We interpret the $\delta$ following Romano et al.~\cite{Romano-EffectSize-2006}:
\begin{equation}
  \tr{Effect Size} =\left\{
  \begin{array}{@{}ll@{}}
    {negligible~(N)}, & \tr{if}\ |\delta| \leq 0.147 \\
    {small~(S)}, & \tr{if}\ 0.147 < |\delta| \leq 0.33 \\
    {medium~(M)}, & \tr{if}\ 0.33 < |\delta| \leq 0.474 \\
    {large~(L)}, & \tr{if}\ 0.474 < |\delta| \leq 1 
  \end{array}\right.
\end{equation} The effect size categories (negligible, small, medium, 
or large) quantify the differences between the distributions.


%\input{RQ2_tables}



\subsubsection{Results}  \bf{There is a statistically significant correlation
between content similarity of the datasets and their Macro F1 score in
cross-platform settings.} In
\tbl\ref{tab:corrSimAcc}, we report the p-value of the correlation analysis between the dataset similarity and tool performance values using MW U test. We also show the effect size.
\begin{table}[t]
  \centering
  \caption{Correlation between dataset similarity values and Macro-F1 scores in cross-platform settings}
    \begin{tabular}{lrr|rr}\toprule
          & \multicolumn{2}{c}{\bf{BERT4SentiSE}} & \multicolumn{2}{c}{\bf{SentiMoji}} \\
          \cmidrule{2-5}
          & {p-value} & Effect Size     & {p-value} & Effect Size \\
          \midrule
    Jansen Shannon    & 0.04*  & Large (0.6) & 0.003** & Large (1.0) \\
    Cosine & 0.002** & Large (1.0) & 0.003** & Large (1.0) \\
    \bottomrule
    \multicolumn{5}{l}{Signif. codes:  ***$p < 0.001$, **$p < 0.01$, *$p < 0.05$}
    \end{tabular}%
  \label{tab:corrSimAcc}%
\end{table}%
In \fig\ref{fig:diversity_performance}, we show the
similarity scores between the datasets and compare the Macro F1-scores between the datasets for the two best performing
deep learning SD tools from RQ$_1$ (i.e., BERT4SentiSE and SentiMoji). For
example, in the first block (i.e., Test on GitHub), we have two sets of bars:
similarity scores between GitHub and SO datasets and Macro F1-scores of
BERT4SentiSE and SentiMoji for the cross-platform setting (i.e., trained on SO
and tested on GitHub). The Jansen similarity scores between the datasets are at least
0.87 and at least 0.93 for cosine similarity. Therefore, while datasets are produced from different platforms, they
have a considerable number of similar words. Thus the more similar two datasets are, the less performance drop 
we can expect in cross-platform settings. 
\begin{figure*}[h]
\centering
\captionsetup[subfigure]{labelformat=empty}
\pgfplotstableread{

1	.88  .97 .75 .77     .88  .97  .82 .85      .87  .96  .77 .77
2	.87  .96 .62 .65     .85  .93  .64 .76      .85  .93  .77 .78
}\datatable
      \subfloat[Test on GitHub]
      {
      \resizebox{1.5in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Trained on SO, Trained on Jira},
        	enlarge y limits=false,
        	enlarge x limits=0.55,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.7cm,
        	width=3.6in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},
        	major x tick style = {opacity=0},
        	minor x tick num = 1,
        	minor tick length=1ex,
        	legend columns=2,
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend style={draw=none},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\huge},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	]
        	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=1] \datatable;
        	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=2] \datatable;
        	\addplot[draw=black!80, fill=black!70] table[x index=0,y index=3] \datatable;
        	\addplot[draw=black!80, fill=black!100] table[x index=0,y index=4] \datatable;

            \legend{JS Divergence,
            		 Cosine Similarity,
            		 }
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    }
    \subfloat[Test on Stack Overflow (SO)]
     {
      \resizebox{1.5in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub, Train on Jira},
        	enlarge y limits=false,
        	enlarge x limits=0.55,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.7cm,
        	width=3.6in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
         	xticklabel style={font=\LARGE, /pgf/number format/fixed},
        	major x tick style = {opacity=0},
        	minor x tick num = 1,
        	minor tick length=1ex,
        	legend columns=2,
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend style={draw=none},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            nodes near coords style={font=\huge},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	]
        	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=5] \datatable;
        	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=6] \datatable; %, postaction={pattern=horizontal lines}
        	\addplot[draw=black!80, fill=black!60] table[x index=0,y index=7] \datatable;   %, postaction={pattern=vertical lines}
            \addplot[draw=black!80, fill=black!100] table[x index=0,y index=8] \datatable;  %, postaction={pattern=vertical lines}
            \legend{,,
            		 SEntiMoji F1,
            		 BERT4SentiSE F1
            		 }
            % \legend{JS Divergence,
            % 		 Cosine Similarity,
            % 		 SEntiMoji F1,
            % 		 BERT4SentiSE F1
            % 		 }
        	\end{axis}
    	\end{tikzpicture}
    	}
    % 	\hspace{-1mm}
    	\label{signature-inconsistency}
    }
    \subfloat[Test on Jira]
     {
      \resizebox{1.5in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub, Train on SO
        	},
        	enlarge y limits=false,
        	enlarge x limits=0.55,
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,,
        	ymin=0,ymax=1.08,
        	ybar,
        	bar width=0.7cm,
        	width=3.4in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
        %     yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
         	xticklabel style={font=\LARGE, /pgf/number format/fixed},
        	major x tick style = {opacity=0},
        	minor x tick num = 1,
        	minor tick length=1ex,
        	legend style={
         	at={(0.6,0.98)},
            anchor=north,legend columns=-1
            },
            nodes near coords style={font=\huge},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	]
        	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=9] \datatable;
        	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=10] \datatable; %, postaction={pattern=horizontal lines}
        	\addplot[draw=black!80, fill=black!60] table[x index=0,y index=11] \datatable; %, postaction={pattern=vertical lines}
            \addplot[draw=black!80, fill=black!100] table[x index=0,y index=12] \datatable; %, postaction={pattern=vertical lines}

        	\end{axis}
    	\end{tikzpicture}
    	}
    % 	%\hspace{-1mm}
    	\label{fig:status-inconsistency}
    }





%\vspace{-3mm}
\caption{Similarity scores between datasets vs Macro F1-scores per tool (BERT4SentiSE \& SentiMoji) in cross platform settings}
\vspace{-3mm}
\label{fig:diversity_performance}
\end{figure*}


% Table generated by Excel2LaTeX from sheet 'similary_vs_perfdrop'
\begin{table}[h]
\newcolumntype{C}{>{\centering\arraybackslash}p{9em}}
  \centering
  \caption{Distribution of dataset content similarity vs drop in performance (Macro F1-score) in Cross-Platform Settings compared to Within Platform Settings for BERT4SentiSE and SentiMoji}
    \begin{tabular}{lccc|CC}\toprule
    {\textbf{Test}} & {\textbf{Train}} & \multicolumn{2}{c}{\textbf{Similarity Score}} & \multicolumn{2}{c}{\textbf{\% Performance drop in cross-platform  Test Dataset}} \\
    \cmidrule{3-6}
    {\textbf{Dataset}} & \textbf{Dataset} & {\textbf{JS divergence}} & {\textbf{Cosine distance}} & \textbf{SentiMoji} & \textbf{Bert4SentiSE} \\
    \midrule
    \multicolumn{1}{l}{\multirow{2}[0]{*}{GitHub}} & SO    & 0.88  & 0.97  & 17    & 16 \\
          & Jira  & 0.87  & 0.96  & 31    & 29 \\
          \midrule
    \multicolumn{1}{l}{\multirow{2}[0]{*}{SO}} & GitHub & 0.88  & 0.97  & 5     & 3 \\
          & Jira  & 0.85  & 0.93  & 26    & 14 \\
          \midrule
    \multicolumn{1}{l}{\multirow{2}[0]{*}{Jira}} & GitHub & 0.87  & 0.96  & 5     & 7 \\
          & SO    & 0.85  & 0.93  & 5     & 6 \\
          \bottomrule
    \end{tabular}%
  \label{tab:sim_vs_drop}%
\end{table}%

\bf{The significance analysis cannot explain the varying degrees of performance between Jira and non-Jira datasets in cross-platform settings.} Our findings in RQ$_1$ 
show the largest performance drop in the two deep learning SD tools when trained in the Jira dataset and tested in the other two datasets. 
The significance analysis in \tbl\ref{tab:corrSimAcc} suggests that this performance drop could be attributed to the similarity (or lack of thereof) between Jira and the other two datasets. However, \fig\ref{fig:diversity_performance} shows that the Jira dataset has almost similar content similarity scores with the SO and GitHub 
as do SO and GitHub with each other. Moreover, the tools suffer a much bigger drop in performance only when they 
are trained in Jira. For example, BERT4SentiSE shows a Macro F1-score of 0.65 when trained in Jira and tested in GitHub, but it shows 
an F1-score of 0.77 when trained in GitHub and then tested in Jira. In \tbl\ref{tab:sim_vs_drop}, we 
show the percentage drop in Macro F1-score compared to within platform setting for each cross-platform settings. For example, the first two rows in 
\tbl\ref{tab:sim_vs_drop} show that when trained in the SO dataset and then tested in the GitHub dataset, the drop in performance in BERT4SentiSE is 16\% compared to the performance 
of BERT4SentiSE when trained and tested in GitHub. However, when BERT4SentiSE is trained in the Jira dataset and then tested in the GitHub dataset, the drop in performance 
is 29\%. The cosine similarity between GitHub and SO is 0.97 and between GitHub and Jira is 0.96. 
When the tool was trained in GitHub and tested in SO, the drop was 3\%, but the drop was 14\% when the tool was trained in Jira and tested in SO. 
The cosine similarity between SO and GitHub is 0.97, and between SO and Jira is 0.93. Therefore, the drop in performance while using the Jira 
dataset could be due to reasons other than content similarity. 

Instead, the the distribution of the polarity classes in the Jira dataset could offer an alternative explanation (see 
\tbl\ref{tab:benchmark_dataset}). While both GitHub and SO are more balanced towards the three polarity classes (around 27-35\% of sentences per polarity class), the Jira dataset is imbalanced with only 19\% positive and 14\% negative classes. {This means that a tool trained using the Jira dataset 
does not have enough information of the two polarity classes compared to when it is trained 
in the other two datasets.} The imbalance in the Jira dataset may also have
introduced bias in the polarity labeling (e.g., by showing more preference
towards neutral classes), contributing to the high percentage of mild disagreements in 
\tbl\ref{tab:agreement_with_manual_labelling}. This happened despite each tool is designed to 
handle the class imbalance problem in model training.


%Similarly SentiMoji also shows similar performance for the three classes in cross-platform settings. 



\begin{table}[t]
  \centering
  \caption{Distribution of False Neutral and False Non-neutral prediction in cross-platform settings. (False Neutral = Prediction is neutral for non-neutral, False Non-neutral = Prediction is non-neutral for neutral sentences)}
  \resizebox{\columnwidth}{!}{%
    \begin{tabular}{ll|cc|cc|cc}\toprule
    {\textbf{SD}} & \textbf{\% Correct} & \multicolumn{2}{c}{\textbf{Train in GitHub}} & \multicolumn{2}{c}{\textbf{Train in SO}} & \multicolumn{2}{c}{\textbf{Train in Jira}} \\
    \cmidrule{3-8}
    {\textbf{Tool}} & \textbf{Misclassified} & {\textbf{Test SO}} & {\textbf{Test Jira}} & {\textbf{Test GitHub}} & {\textbf{Test Jira}} & {\textbf{Test GitHub}} & {\textbf{Test SO}} \\
    \midrule
\multirow{2}{*}{\textbf{SentiMoji}} &False Neutral &61 &22 &75 &28 &\textbf{94} &\textbf{97} \\
&False Non-neutral &34 &74 &15 &69 &\textbf{2} &\textbf{3} \\
\midrule
\multirow{2}{*}{\textbf{BERT4SentiSE}} &False Neutral &41 &23 &69 &26 &\textbf{91} &\textbf{88} \\
&False Non-neutral &52 &72 &17 &69 &\textbf{3} &\textbf{10} \\

          \bottomrule
    \end{tabular}%
    }
  \label{tab:rq-mild-error-analysis}%
\end{table}%


\textbf{When trained on the imbalanced Jira dataset (67\% neutral), the most dominant error case (around 90\%) is that all the supervised tools predict neutral polarity for non-neutral sentences.}
From Table~\ref{tab:cross_platform_performance}, we can see that when trained in Jira dataset and tested on non-Jira datasets, both SentiMoji and BERT4SentiSE show high precision and low recall for both the non-neutral classes. At the same time, these tools exhibit high recall and low precision for the neutral class. For example, when trained on the Jira dataset and tested on GitHub dataset, BERT4SentiSE shows a precision of 0.90 and recall of 0.43 for the negative class. The tool shows a precision of 0.91 and a recall of 0.51 for the positive class. At the same time, they report a high recall of .97 and low precision of 0.59 for the neutral class. 
This observation is consistent with SentiMoji in cross-platform settings.
Table~\ref{tab:rq-mild-error-analysis} presents details about the drop in performance when the supervised SD tools are trained on cross-platform settings. 
Around 95\% to 99\% misclassifications fall under mild errors (i.e., the sum of `False Neutral' and `False Non-neutral'). Around 88\% to 97\% of the errors are due to `False Neutral' prediction, i.e., the manual label is non-neutral, but the tool predicts as neutral. For example, when BERT4SentiSE is trained on the Jira dataset and tested on GitHub, it has around 29\% performance drop in terms of macro F1-score and 94\% of its total errors are mild error, and 6\% are severe errors. Our analysis shows that in that settings, 91\% of the errors fall under the `False Neutral' category, and only 3\% of errors fall under the `False Non-neutral' category. Novelli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020} also reported a similar performance drop in cross-platform settings for the supervised tools, and the deep-learning-based SD tools outperformed all non-DL based SD tools in within-platform settings even for the imbalanced Jira dataset. As mentioned in \sec\ref{sec:studied-tools}, for this study, we used the best model configuration, hyperparameters, and settings for the studied supervised tools reported by the original authors in respective studies. 






%\bf{Some characteristics of the dataset other than content similarity between them are responsible for the drop in performance in cross platform settings}. To better understand the causes of variation in the drop of performance of the tools across the three datasets, we next check the number of misclassifications in within vs. cross-platform settings. In \fig\ref{fig:diversity_performance_misssclf}, we show three blocks of bars, one block per test dataset. For example, the first block uses GitHub as the test dataset, i.e., it is trained on the other two datasets and then tested on GitHub. The first bar for `Test of GitHub' shows the ratio of misclassified cases in GitHub for within platform setting. Here, the ratio is the total number of misclassified sentences out of all sentences in the GitHub dataset. The second bar shows the ratio of misclassified cases while trained on SO and tested on GitHub, and the third bar shows the ratio of misclassified cases while trained on Jira and tested on GitHub. For both cross-platform cases where Jira is used to train  (i.e., Test on GitHub and Test on SO), we see 19-29\% of misclassified cases. In contrast, we see at most 14\% misclassified cases while Jira is used as the test dataset and GitHub or SO is used as the training dataset. \bf{This denotes that while the three datasets show content similarity, the variation in the drop in performance across the datasets might be due to characteristics specific to the individual datasets that are not necessarily specific to content similarity.}

% Our two similarity metrics shows that the similarity of these datasets are quite high. Figure \ref{fig:diversity_performance} shows that the Jensen-Shannon Divergence and Cosine similarity of the datasets and the micro F1 score of SEntiMoji and BERT4SentiSE. Our experiments show that GitHub has higher similarity with SO than Jira and so when tested on GitHub both SentiMoji and BERT4SentiSE has higher micro F1 score. Similar pattern can also be found when the test on Stack Overflow or Jira dataset.

% From our experiments of internal $D_{JS}$ divergence, we find Jira dataset has the highest diversity and Stack Overflow dataset has the lowest internal divergence. The mean of internal $D_{JS}$ divergence of GitHub, Stack Overflow and Jira datasets are 0.92, 0.93, and 0.87 respectively. In all cases the standard deviation is less than 0.001.

% Mean is 0.915153 and Standard Deviation of Sample set is 0.0007074900782077775
% Mean is 0.930979 and Standard Deviation of Sample set is 0.0005455997749518836
% Mean is 0.870792 and Standard Deviation of Sample set is 0.0009510214319267058


\begin{tcolorbox}[flushleft upper,boxrule=1pt,arc=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=white,after=\ignorespacesafterend\par\noindent]
 \bf{RQ$_3$ Can similarity analysis between the studied datasets explain the drop in performance of the deep learning SD tools in the datasets in cross-platform settings?} There
is a statistically significant positive correlation between similarity of
contents between any two datasets and the performance of a pre-trained DL-based
tools between the two datasets in cross-platform settings (i.e., more similarity
results in more performance). However, the significance analysis is not sufficient to explain the drop in performance in the tools for cross-platform 
settings involving the Jira dataset, which is highly imbalanced and has a much fewer number of non-neutral classes in the data compared to the other two datasets.
%  The drop in performance and ratio of misclassified cases in cross-platform setting is the most for Jira dataset in the cross-platform settings, i.e., tools are more error-prone while they used Jira as the training dataset.
\end{tcolorbox}
















% \begin{table*}[h]
%   \centering
%   %\vspace{-.1in}
%   \caption{Distribution of Error Categories for the deep-learning tools}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{lll}
%     \toprule{}
%     % \textbf{Topics} & \textbf{Authentication} & \textbf{Deployment} & \textbf{Documentation} & \textbf{Feature} & \textbf{Testing/Debugging}\\
%     \textbf{Category} & \textbf{Description} & \textbf{\#Units} \\
%     \midrule

%     Subjectivity in Annotation & Sentences that are labelled inconsistently with-in platform or Cross-platform & 114 (29\%) \\
%     General Error & Tools failing to process linguistic cues & 82 (21\%) \\
%     Implicit Sentiment & Sentences that express emotion without explicit linguistic cues & 57 (14\%) \\
%     Context/Pragmatics & Tools failing to understand the underlying context to detect overall polarity & 55 (14\%) \\
%     Domain Specific & Sentences with polarity in SE-specific context & 49 (12\%) \\
%     Politeness & A neutral sentence is labelled with polar sentiment due to politeness & 27 (7\%) \\
%     Figurative language & Sentences containing humour or irony & 16 (4\%) \\
    

%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:misclassification}%
% \end{table*}%










==> RQ4_tables.tex <==

% \begin{table}[]
%   \footnotesize
% %   \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Agreement metrics between  tools with manual labelling}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{clrrrr}
%     \toprule{}
%     %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
%     %\cmidrule{3-6}
%     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Classifier }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
%     \cmidrule{5-6}
%     {Dataset} &  & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule
% \multicolumn{6}{c}{\textbf{Test dataset: GitHub}} \\
% \midrule
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Within-platform)}} 
%  & SEntiMoji & 0.84 & 90\% & 1\% & 9\%  \\
%  & BERT4SentiSE & 0.87 & 92\% & 1\% & 7\%  \\
%  & RNN4SentiSE & 0.52 & 68\% & 7\% & 25\%  \\
%  & Senti4SD & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiCR & 0.73 & 83\% & 2\% & 15\%  \\
% % \midrule
% \cmidrule{2-6}
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow \\ (Cross-platform)}}  
%  & SEntiMoji & 0.61 & 75\% & 2\% & 23\%  \\
%  & BERT4SentiSE & 0.65 & 78\% & 3\% & 19\%  \\
%  & RNN4SentiSE & 0.47 & 66\% & 4\% & 30\%  \\
%  & Senti4SD & 0.60 & 74\% & 4\% & 22\%  \\
%  & SentiCR & 0.49 & 68\% & 2\% & 29\%  \\
% % \midrule
% \cmidrule{2-6}
% 
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Cross-platform)}} 
%  & SEntiMoji & 0.44 & 66\% & 1\% & 33\%  \\
%  & BERT4SentiSE & 0.48 & 68\% & 2\% & 30\%  \\
%  & RNN4SentiSE & 0.35 & 60\% & 4\% & 36\%  \\
%  & Senti4SD & 0.50 & 69\% & 2\% & 28\%  \\
%  & SentiCR & 0.34 & 60\% & 1\% & 39\%  \\
% \midrule
% 
% 
% 
% \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% \midrule
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow (Within-platform)}}
%  & SEntiMoji & 0.80 & 87\% & 1\% & 12\%  \\
%  & BERT4SentiSE& 0.82 & 88\% & 1\% & 11\%  \\
%  & RNN4SentiSE & 0.67 & 78\% & 3\% & 19\%  \\
%  & Senti4SD & 0.77 & 85\% & 1\% & 14\%  \\
%  & SentiCR & 0.73 & 82\% & 3\% & 15\%  \\
% % \midrule
% \cmidrule{2-6}
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Cross-platform)}} 
%  & SEntiMoji & 0.73 & 83\% & 1\% & 16\%  \\
%  & BERT4SentiSE & 0.78 & 85\% & 1\% & 14\%  \\
%  & RNN4SentiSE & 0.49 & 67\% & 4\% & 29\%  \\
%  & Senti4SD & 0.67 & 78\% & 2\% & 20\%  \\
%  & SentiCR & 0.56 & 71\% & 5\% & 23\%  \\
% % \midrule
% \cmidrule{2-6}
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Cross-platform)}} 
%  & SEntiMoji & 0.48 & 67\% & 0\% & 33\%  \\
%  & BERT4SentiSE & 0.63 & 76\% & 1\% & 23\%  \\
%  & RNN4SentiSE & 0.34 & 58\% & 4\% & 38\%  \\
%  & Senti4SD & 0.47 & 66\% & 1\% & 33\%  \\
%  & SentiCR & 0.37 & 60\% & 2\% & 38\%  \\
% \midrule
% 
% 
% 
% 
% 
% 
% 
% \multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
% \midrule
% \multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Within-platform)}}
%  & SEntiMoji & 0.71 & 86\% & 0\% & 14\%  \\
%  & BERT4SentiSE& 0.72 & 86\% & 0\% & 13\%  \\
%  & RNN4SentiSE & 0.57 & 80\% & 1\% & 20\%  \\
%  & Senti4SD & 0.59 & 81\% & 0\% & 19\%  \\
%  & SentiCR & 0.69 & 85\% & 0\% & 15\%  \\
% % \midrule
% \cmidrule{2-6}
% 
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Cross-platform)}} 
%  & SEntiMoji & 0.65 & 81\% & 1\% & 18\%  \\
%  & BERT4SentiSE & 0.65 & 81\% & 1\% & 18\%  \\
%  & RNN4SentiSE & 0.45 & 66\% & 2\% & 32\%  \\
%  & Senti4SD & 0.58 & 78\% & 1\% & 21\%  \\
%  & SentiCR & 0.65 & 82\% & 1\% & 17\%  \\
% % \midrule
% \cmidrule{2-6}
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow \\ (Cross-platform)}} 
%  & SEntiMoji & 0.65 & 82\% & 1\% & 18\%  \\
%  & BERT4SentiSE & 0.66 & 82\% & 1\% & 17\%  \\
%  & RNN4SentiSE & 0.57 & 77\% & 1\% & 22\%  \\
%  & Senti4SD & 0.46 & 74\% & 1\% & 25\%  \\
%  & SentiCR & 0.34 & 73\% & 1\% & 26\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_with_manual_labelling}%
% \end{table}%


















% ===================================================================================================>
% \resizebox{\textwidth}{!}{%
\begin{sidewaystable}
\vspace{15cm}
% \hvFloat[rotAngle=90,nonFloat=true,capWidth=w]
% \begin{table}
\parbox{.3\linewidth}{
\renewcommand{\thetable}{\arabic{table}a}
  \footnotesize
%   \small
  \centering
  \caption{Agreement between SD tools (Test dataset: GitHub)}
    \begin{tabular}{clrr|rr}
    \toprule
    \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagree}}\\
    \cmidrule{3-6}
    & & {\bf{$\kappa$}} & {\textbf{P}} & \textbf{S} & \textbf{M} \\
    \midrule
\multirow{15}{*}{G (W)} 
% ==========================  within setting GitHub =========
 & Mji vs Brt & 0.86 & 91\% & 1\% & 8\%  \\
 & Mji vs Rnn & 0.52 & 68\% & 7\% & 25\%  \\
 & Mji vs S4D & 0.83 & 89\% & 1\% & 10\%  \\
 & Mji vs SCr & 0.76 & 85\% & 2\% & 13\%  \\
 & Mji vs SSt & 0.68 & 79\% & 2\% & 18\%  \\
 & Brt vs Rnn & 0.53 & 69\% & 7\% & 24\%  \\
 & Brt vs S4D & 0.85 & 90\% & 2\% & 8\%  \\
 & Brt vs SCr & 0.74 & 83\% & 2\% & 14\%  \\
 & Brt vs SSt & 0.68 & 80\% & 2\% & 18\%  \\
 & Rnn vs S4D & 0.52 & 69\% & 7\% & 25\%  \\
 & Rnn vs SCr & 0.43 & 63\% & 7\% & 31\%  \\
 & Rnn vs SSt & 0.44 & 63\% & 6\% & 31\%  \\
 & S4D vs SCr & 0.74 & 83\% & 2\% & 14\%  \\
 & S4D vs SSt & 0.67 & 79\% & 3\% & 18\%  \\
 & SCr vs SSt & 0.63 & 77\% & 3\% & 21\%  \\
\midrule


\multirow{15}{*}{S(C)} 
% ...........test dataset: GitHub train_dataset: DatasetSenti4SDSO  .........
 & Mji vs Brt & 0.72 & 83\% & 1\% & 15\%  \\
 & Mji vs Rnn & 0.58 & 76\% & 2\% & 22\%  \\
 & Mji vs S4D & 0.51 & 70\% & 3\% & 27\%  \\
 & Mji vs SCr & 0.40 & 68\% & 2\% & 30\%  \\
 & Mji vs SSt & 0.57 & 74\% & 2\% & 25\%  \\
 & Brt vs Rnn & 0.59 & 76\% & 2\% & 22\%  \\
 & Brt vs S4D & 0.52 & 70\% & 4\% & 26\%  \\
 & Brt vs SCr & 0.39 & 66\% & 3\% & 31\%  \\
 & Brt vs SSt & 0.61 & 76\% & 2\% & 22\%  \\
 & Rnn vs S4D & 0.43 & 65\% & 4\% & 31\%  \\
 & Rnn vs SCr & 0.30 & 62\% & 3\% & 35\%  \\
 & Rnn vs SSt & 0.48 & 68\% & 3\% & 29\%  \\
 & S4D vs SCr & 0.45 & 68\% & 2\% & 30\%  \\
 & S4D vs SSt & 0.55 & 72\% & 3\% & 25\%  \\
 & SCr vs SSt & 0.45 & 68\% & 2\% & 31\%  \\
\midrule


\multirow{15}{*}{J(C)} 
% ...........test dataset: GitHub train_dataset: OrtuJIRA  .........
 & Mji vs Brt & 0.78 & 90\% & 0\% & 10\%  \\
 & Mji vs Rnn & 0.54 & 81\% & 1\% & 19\%  \\
 & Mji vs S4D & 0.60 & 82\% & 1\% & 18\%  \\
 & Mji vs SCr & 0.65 & 87\% & 0\% & 13\%  \\
 & Mji vs SSt & 0.46 & 69\% & 0\% & 30\%  \\
 & Brt vs Rnn & 0.56 & 81\% & 1\% & 18\%  \\
 & Brt vs S4D & 0.60 & 81\% & 1\% & 18\%  \\
 & Brt vs SCr & 0.67 & 87\% & 0\% & 13\%  \\
 & Brt vs SSt & 0.51 & 71\% & 1\% & 28\%  \\
 & Rnn vs S4D & 0.44 & 74\% & 2\% & 24\%  \\
 & Rnn vs SCr & 0.45 & 79\% & 1\% & 20\%  \\
 & Rnn vs SSt & 0.36 & 63\% & 2\% & 34\%  \\
 & S4D vs SCr & 0.52 & 79\% & 1\% & 20\%  \\
 & S4D vs SSt & 0.48 & 70\% & 2\% & 29\%  \\
 & SCr vs SSt & 0.39 & 66\% & 0\% & 34\%  \\

    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:agreement_test_github}%
% \end{table}%
% \end{sidewaystable}
}
% \begin{sidewaystable}
% \vspace{15cm}
% \begin{table}
\hfill
\parbox{.3\linewidth}{
\addtocounter{table}{-1}
\renewcommand{\thetable}{\arabic{table}b}
  \footnotesize
%   \small
  \centering
  \caption{Agreement between SD tools (Test dataset: SO)}
    \begin{tabular}{clrr|rr}
    \toprule
    \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagree}}\\
    \cmidrule{3-6}
    & & {\bf{$\kappa$}} & {\textbf{P}} & \textbf{S} & \textbf{M} \\
    \midrule

\multirow{15}{*}{ S (W)} 
% ==========================  within setting DatasetSenti4SDSO =========
 & Mji vs Brt & 0.86 & 91\% & 1\% & 8\%  \\
 & Mji vs Rnn & 0.70 & 80\% & 3\% & 17\%  \\
 & Mji vs S4D & 0.81 & 88\% & 1\% & 12\%  \\
 & Mji vs SCr & 0.78 & 85\% & 2\% & 12\%  \\
 & Mji vs SSt & 0.72 & 81\% & 1\% & 17\%  \\
 & Brt vs Rnn & 0.71 & 81\% & 2\% & 17\%  \\
 & Brt vs S4D & 0.83 & 88\% & 1\% & 11\%  \\
 & Brt vs SCr & 0.78 & 85\% & 3\% & 12\%  \\
 & Brt vs SSt & 0.72 & 81\% & 1\% & 18\%  \\
 & Rnn vs S4D & 0.70 & 80\% & 3\% & 17\%  \\
 & Rnn vs SCr & 0.65 & 77\% & 4\% & 19\%  \\
 & Rnn vs SSt & 0.63 & 75\% & 3\% & 21\%  \\
 & S4D vs SCr & 0.78 & 85\% & 3\% & 12\%  \\
 & S4D vs SSt & 0.73 & 82\% & 1\% & 17\%  \\
 & SCr vs SSt & 0.70 & 81\% & 2\% & 17\%  \\

\midrule

\multirow{15}{*}{ G (C)} 
 % ...........test dataset: DatasetSenti4SDSO train_dataset: GitHub  .........
 & Mji vs Brt & 0.79 & 86\% & 1\% & 13\%  \\
 & Mji vs Rnn & 0.53 & 70\% & 4\% & 27\%  \\
 & Mji vs S4D & 0.70 & 80\% & 3\% & 17\%  \\
 & Mji vs SCr & 0.62 & 75\% & 5\% & 20\%  \\
 & Mji vs SSt & 0.67 & 79\% & 1\% & 20\%  \\
 & Brt vs Rnn & 0.53 & 69\% & 5\% & 26\%  \\
 & Brt vs S4D & 0.73 & 82\% & 2\% & 16\%  \\
 & Brt vs SCr & 0.60 & 74\% & 5\% & 21\%  \\
 & Brt vs SSt & 0.69 & 79\% & 1\% & 20\%  \\
 & Rnn vs S4D & 0.54 & 69\% & 4\% & 26\%  \\
 & Rnn vs SCr & 0.40 & 61\% & 6\% & 33\%  \\
 & Rnn vs SSt & 0.48 & 66\% & 4\% & 30\%  \\
 & S4D vs SCr & 0.58 & 73\% & 4\% & 23\%  \\
 & S4D vs SSt & 0.65 & 77\% & 1\% & 22\%  \\
 & SCr vs SSt & 0.56 & 71\% & 4\% & 25\%  \\
\midrule


\multirow{15}{*}{ J (C)} 
% ...........test dataset: DatasetSenti4SDSO train_dataset: OrtuJIRA  .........
 & Mji vs Brt & 0.66 & 82\% & 0\% & 18\%  \\
 & Mji vs Rnn & 0.47 & 75\% & 1\% & 23\%  \\
 & Mji vs S4D & 0.60 & 81\% & 1\% & 19\%  \\
 & Mji vs SCr & 0.56 & 80\% & 1\% & 19\%  \\
 & Mji vs SSt & 0.49 & 68\% & 0\% & 31\%  \\
 & Brt vs Rnn & 0.43 & 70\% & 2\% & 28\%  \\
 & Brt vs S4D & 0.57 & 77\% & 1\% & 22\%  \\
 & Brt vs SCr & 0.52 & 75\% & 1\% & 25\%  \\
 & Brt vs SSt & 0.60 & 75\% & 0\% & 25\%  \\
 & Rnn vs S4D & 0.42 & 72\% & 2\% & 27\%  \\
 & Rnn vs SCr & 0.33 & 70\% & 1\% & 29\%  \\
 & Rnn vs SSt & 0.36 & 60\% & 3\% & 36\%  \\
 & S4D vs SCr & 0.51 & 77\% & 1\% & 22\%  \\
 & S4D vs SSt & 0.46 & 66\% & 1\% & 33\%  \\
 & SCr vs SSt & 0.40 & 63\% & 1\% & 36\%  \\

% \midrule

    \bottomrule
    \end{tabular}%
  \label{tab:agreement_test_so}%
% \end{table}%
% \end{sidewaystable}
}
\hfill
\parbox{.3\linewidth}{
% \begin{sidewaystable}
% \begin{table}[]
  \addtocounter{table}{-1}
  \renewcommand{\thetable}{\arabic{table}c}
  \footnotesize
%   \small
  \centering
  \caption{Agreement between SD tools (Test dataset: Jira)}
    \begin{tabular}{clrr|rr}
    \toprule
    \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagree}}\\
    \cmidrule{3-6}
    & & {\bf{$\kappa$}} & {\textbf{P}} & \textbf{S} & \textbf{M} \\
    \midrule

\multirow{15}{*}{ J (W)} 
% ==========================  within setting OrtuJIRA =========
 & Mji vs Brt & 0.85 & 93\% & 0\% & 7\%  \\
 & Mji vs Rnn & 0.68 & 86\% & 0\% & 14\%  \\
 & Mji vs S4D & 0.72 & 87\% & 0\% & 13\%  \\
 & Mji vs SCr & 0.81 & 91\% & 0\% & 9\%  \\
 & Mji vs SSt & 0.75 & 87\% & 0\% & 13\%  \\
 & Brt vs Rnn & 0.68 & 85\% & 1\% & 14\%  \\
 & Brt vs S4D & 0.72 & 87\% & 0\% & 13\%  \\
 & Brt vs SCr & 0.79 & 90\% & 0\% & 10\%  \\
 & Brt vs SSt & 0.75 & 87\% & 0\% & 13\%  \\
 & Rnn vs S4D & 0.61 & 83\% & 0\% & 17\%  \\
 & Rnn vs SCr & 0.70 & 86\% & 1\% & 14\%  \\
 & Rnn vs SSt & 0.63 & 81\% & 1\% & 18\%  \\
 & S4D vs SCr & 0.70 & 86\% & 0\% & 13\%  \\
 & S4D vs SSt & 0.67 & 83\% & 1\% & 16\%  \\
 & SCr vs SSt & 0.77 & 88\% & 1\% & 11\%  \\
\midrule

\multirow{15}{*}{ G (C)} 
% ...........test dataset: OrtuJIRA train_dataset: GitHub  .........
 & Mji vs Brt & 0.81 & 89\% & 1\% & 10\%  \\
 & Mji vs Rnn & 0.56 & 72\% & 3\% & 25\%  \\
 & Mji vs S4D & 0.72 & 84\% & 1\% & 14\%  \\
 & Mji vs SCr & 0.75 & 86\% & 1\% & 13\%  \\
 & Mji vs SSt & 0.75 & 86\% & 1\% & 13\%  \\
 & Brt vs Rnn & 0.57 & 73\% & 3\% & 24\%  \\
 & Brt vs S4D & 0.73 & 85\% & 1\% & 14\%  \\
 & Brt vs SCr & 0.75 & 87\% & 1\% & 13\%  \\
 & Brt vs SSt & 0.75 & 86\% & 1\% & 13\%  \\
 & Rnn vs S4D & 0.52 & 70\% & 3\% & 27\%  \\
 & Rnn vs SCr & 0.50 & 69\% & 2\% & 28\%  \\
 & Rnn vs SSt & 0.54 & 71\% & 2\% & 27\%  \\
 & S4D vs SCr & 0.68 & 83\% & 1\% & 16\%  \\
 & S4D vs SSt & 0.70 & 83\% & 1\% & 16\%  \\
 & SCr vs SSt & 0.76 & 87\% & 1\% & 12\%  \\
\midrule


\multirow{15}{*}{ S (C)} 
% ...........test dataset: OrtuJIRA train_dataset: DatasetSenti4SDSO  .........
 & Mji vs Brt & 0.80 & 89\% & 1\% & 10\%  \\
 & Mji vs Rnn & 0.70 & 84\% & 1\% & 15\%  \\
 & Mji vs S4D & 0.61 & 79\% & 1\% & 19\%  \\
 & Mji vs SCr & 0.35 & 70\% & 1\% & 29\%  \\
 & Mji vs SSt & 0.77 & 87\% & 1\% & 12\%  \\
 & Brt vs Rnn & 0.72 & 84\% & 1\% & 14\%  \\
 & Brt vs S4D & 0.60 & 79\% & 2\% & 19\%  \\
 & Brt vs SCr & 0.36 & 71\% & 1\% & 28\%  \\
 & Brt vs SSt & 0.77 & 87\% & 1\% & 12\%  \\
 & Rnn vs S4D & 0.56 & 77\% & 2\% & 22\%  \\
 & Rnn vs SCr & 0.30 & 67\% & 1\% & 32\%  \\
 & Rnn vs SSt & 0.70 & 83\% & 1\% & 16\%  \\
 & S4D vs SCr & 0.41 & 76\% & 1\% & 23\%  \\
 & S4D vs SSt & 0.59 & 78\% & 2\% & 20\%  \\
 & SCr vs SSt & 0.34 & 70\% & 1\% & 29\%  \\
% \midrule
    % \midrule  
    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:agreement_test_jira}%
 }
% \end{table}%
\end{sidewaystable}





% \begin{table}
% \renewcommand{\thetable}{\arabic{table}a}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Agreement between  tools (Test dataset: GitHub)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule
% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Within Platform)}} 
%  & SentiMoji vs BERT4SE & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiMoji vs RNN4SE & 0.52 & 68\% & 7\% & 25\%  \\
%  & SentiMoji vs Senti4SD & 0.83 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs SentiCR & 0.76 & 85\% & 2\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.53 & 69\% & 7\% & 24\%  \\
%  & BERT4SE vs Senti4SD & 0.85 & 90\% & 2\% & 8\%  \\
%  & BERT4SE vs SentiCR & 0.74 & 83\% & 2\% & 14\%  \\
%  & RNN4SE vs Senti4SD & 0.52 & 69\% & 7\% & 25\%  \\
%  & RNN4SE vs SentiCR & 0.43 & 63\% & 7\% & 31\%  \\
%  & Senti4SD vs SentiCR & 0.74 & 83\% & 2\% & 14\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.72 & 83\% & 1\% & 15\%  \\
%  & SentiMoji vs RNN4SE & 0.58 & 76\% & 2\% & 22\%  \\
%  & SentiMoji vs Senti4SD & 0.51 & 70\% & 3\% & 27\%  \\
%  & SentiMoji vs SentiCR & 0.40 & 68\% & 2\% & 30\%  \\
%  & BERT4SE vs RNN4SE & 0.59 & 76\% & 2\% & 22\%  \\
%  & BERT4SE vs Senti4SD & 0.52 & 70\% & 4\% & 26\%  \\
%  & BERT4SE vs SentiCR & 0.39 & 66\% & 3\% & 31\%  \\
%  & RNN4SE vs Senti4SD & 0.43 & 65\% & 4\% & 31\%  \\
%  & RNN4SE vs SentiCR & 0.30 & 62\% & 3\% & 35\%  \\
%  & Senti4SD vs SentiCR & 0.45 & 68\% & 2\% & 30\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.78 & 90\% & 0\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.54 & 81\% & 1\% & 19\%  \\
%  & SentiMoji vs Senti4SD & 0.60 & 82\% & 1\% & 18\%  \\
%  & SentiMoji vs SentiCR & 0.65 & 87\% & 0\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.56 & 81\% & 1\% & 18\%  \\
%  & BERT4SE vs Senti4SD & 0.60 & 81\% & 1\% & 18\%  \\
%  & BERT4SE vs SentiCR & 0.67 & 87\% & 0\% & 13\%  \\
%  & RNN4SE vs Senti4SD & 0.44 & 74\% & 2\% & 24\%  \\
%  & RNN4SE vs SentiCR & 0.45 & 79\% & 1\% & 20\%  \\
%  & Senti4SD vs SentiCR & 0.52 & 79\% & 1\% & 20\%  \\

%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_github}%
% \end{table}%


% ==================================================================================================>

% \begin{table}
% \addtocounter{table}{-1}
% \renewcommand{\thetable}{\arabic{table}b}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Agreement between  tools (Test dataset: SO)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Within Platform)}} 
%  & SentiMoji vs BERT4SE & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiMoji vs RNN4SE & 0.70 & 80\% & 3\% & 17\%  \\
%  & SentiMoji vs Senti4SD & 0.81 & 88\% & 1\% & 12\%  \\
%  & SentiMoji vs SentiCR & 0.78 & 85\% & 2\% & 12\%  \\
%  & BERT4SE vs RNN4SE & 0.71 & 81\% & 2\% & 17\%  \\
%  & BERT4SE vs Senti4SD & 0.83 & 88\% & 1\% & 11\%  \\
%  & BERT4SE vs SentiCR & 0.78 & 85\% & 3\% & 12\%  \\
%  & RNN4SE vs Senti4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & RNN4SE vs SentiCR & 0.65 & 77\% & 4\% & 19\%  \\
%  & Senti4SD vs SentiCR & 0.78 & 85\% & 3\% & 12\%  \\
% \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.79 & 86\% & 1\% & 13\%  \\
%  & SentiMoji vs RNN4SE & 0.53 & 70\% & 4\% & 27\%  \\
%  & SentiMoji vs Senti4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & SentiMoji vs SentiCR & 0.62 & 75\% & 5\% & 20\%  \\
%  & BERT4SE vs RNN4SE & 0.53 & 69\% & 5\% & 26\%  \\
%  & BERT4SE vs Senti4SD & 0.73 & 82\% & 2\% & 16\%  \\
%  & BERT4SE vs SentiCR & 0.60 & 74\% & 5\% & 21\%  \\
%  & RNN4SE vs Senti4SD & 0.54 & 69\% & 4\% & 26\%  \\
%  & RNN4SE vs SentiCR & 0.40 & 61\% & 6\% & 33\%  \\
%  & Senti4SD vs SentiCR & 0.58 & 73\% & 4\% & 23\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.66 & 82\% & 0\% & 18\%  \\
%  & SentiMoji vs RNN4SE & 0.47 & 75\% & 1\% & 23\%  \\
%  & SentiMoji vs Senti4SD & 0.60 & 81\% & 1\% & 19\%  \\
%  & SentiMoji vs SentiCR & 0.56 & 80\% & 1\% & 19\%  \\
%  & BERT4SE vs RNN4SE & 0.43 & 70\% & 2\% & 28\%  \\
%  & BERT4SE vs Senti4SD & 0.57 & 77\% & 1\% & 22\%  \\
%  & BERT4SE vs SentiCR & 0.52 & 75\% & 1\% & 25\%  \\
%  & RNN4SE vs Senti4SD & 0.42 & 72\% & 2\% & 27\%  \\
%  & RNN4SE vs SentiCR & 0.33 & 70\% & 1\% & 29\%  \\
%  & Senti4SD vs SentiCR & 0.51 & 77\% & 1\% & 22\%  \\
% % \midrule

%     \bottomrule
%     \end{tabular}%
%   \label{tab:agreement_test_so}%
% \end{table}%

% % ===================================================================================================>

% \begin{table}[]
%   \addtocounter{table}{-1}
%   \renewcommand{\thetable}{\arabic{table}c}

% %   \footnotesize
%   \small
%   \centering
%   \caption{Agreement between  tools (Test dataset: Jira)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Within Platform}} 
%  & SentiMoji vs BERT4SE & 0.85 & 93\% & 0\% & 7\%  \\
%  & SentiMoji vs RNN4SE & 0.68 & 86\% & 0\% & 14\%  \\
%  & SentiMoji vs Senti4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & SentiMoji vs SentiCR & 0.81 & 91\% & 0\% & 9\%  \\
%  & BERT4SE vs RNN4SE & 0.68 & 85\% & 1\% & 14\%  \\
%  & BERT4SE vs Senti4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & BERT4SE vs SentiCR & 0.79 & 90\% & 0\% & 10\%  \\
%  & RNN4SE vs Senti4SD & 0.61 & 83\% & 0\% & 17\%  \\
%  & RNN4SE vs SentiCR & 0.70 & 86\% & 1\% & 14\%  \\
%  & Senti4SD vs SentiCR & 0.70 & 86\% & 0\% & 13\%  \\
% \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.81 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.56 & 72\% & 3\% & 25\%  \\
%  & SentiMoji vs Senti4SD & 0.72 & 84\% & 1\% & 14\%  \\
%  & SentiMoji vs SentiCR & 0.75 & 86\% & 1\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.57 & 73\% & 3\% & 24\%  \\
%  & BERT4SE vs Senti4SD & 0.73 & 85\% & 1\% & 14\%  \\
%  & BERT4SE vs SentiCR & 0.75 & 87\% & 1\% & 13\%  \\
%  & RNN4SE vs Senti4SD & 0.52 & 70\% & 3\% & 27\%  \\
%  & RNN4SE vs SentiCR & 0.50 & 69\% & 2\% & 28\%  \\
%  & Senti4SD vs SentiCR & 0.68 & 83\% & 1\% & 16\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.80 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.70 & 84\% & 1\% & 15\%  \\
%  & SentiMoji vs Senti4SD & 0.61 & 79\% & 1\% & 19\%  \\
%  & SentiMoji vs SentiCR & 0.35 & 70\% & 1\% & 29\%  \\
%  & BERT4SE vs RNN4SE & 0.72 & 84\% & 1\% & 14\%  \\
%  & BERT4SE vs Senti4SD & 0.60 & 79\% & 2\% & 19\%  \\
%  & BERT4SE vs SentiCR & 0.36 & 71\% & 1\% & 28\%  \\
%  & RNN4SE vs Senti4SD & 0.56 & 77\% & 2\% & 22\%  \\
%  & RNN4SE vs SentiCR & 0.30 & 67\% & 1\% & 32\%  \\
%  & Senti4SD vs SentiCR & 0.41 & 76\% & 1\% & 23\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_jira}%
% \end{table}%








\begin{table}
  \footnotesize
%   \small

  \centering
  \caption{Performance comparison of majority voting based ensemble tools with the SD tools (All- All of the SD tools except baseline DL-RNN4SEntiSE, BTPC-Best SD tool from PMT DL-based (BERT4SentiSE), Shallow ML-based (Senti4SD), Rule-based (SentiStrengthSE) }
    \begin{tabular}{ccllll}
    \toprule
    \multirow{2}{*}{\bf{Test Dataset}} & \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\textbf{Ensemble}} & \multicolumn{3}{c}{\textbf{Macro Performance}}\\
    \cmidrule{4-6}
    & & & {\bf{$P$}} & {\bf{$R$}} & {\bf{$F1$}} \\
    \midrule
    
\multirow{16}{*}{GitHub}  &  \multirow{8}{*}{Stack Overflow} & Baseline: Best (SentiStrengthSE) & .80 & .78 & .78\\
% \cmidrule{4-6}
& & Majority-All &  .78 & .80 & .78  \\
& & Majority-All (Except RNN4SentiSE) &  .80 & .81 & .80  \\
& & Majority-PMT DL &  .81 & .78 & .79  \\
& & Majority-Shallow ML &  .76 & .75 & .75  \\
& & Majority-PMT DL + Rule &  .82 & .83 & .82  \\
& & Majority-Shallow ML + Rule &  .78 & .80 & .79  \\
& & Majority-BTPC &  .80 & .81 & .80  \\
\cmidrule{3-6}

& \multirow{8}{*}{Jira} & Baseline: Best (SentiStrengthSE) & .80 & .78 & .78\\
% \cmidrule{4-6}
& & Majority-All &  .80 & .80 & .80  \\
& & Majority-All (Except RNN4SentiSE) &  .81 & .81 & .81  \\
& & Majority-PMT DL &  .80 & .66 & .68  \\
& & Majority-Shallow ML &  .79 & .67 & .69  \\
& & Majority-PMT DL + Rule &  .82 & .80 & .81  \\
& & Majority-Shallow ML + Rule &  .81 & .80 & .80  \\
& & Majority-BTPC &  .81 & .81 & .81  \\

\midrule
\multirow{16}{*}{Stack Overflow}  &  \multirow{8}{*}{GitHub} & Baseline: Best (BERT4SentiSE) & .85 & .86 & .85\\
% \cmidrule{4-6}
& & Majority-All &  .78 & .78 & .75  \\
& & Majority-All (Except RNN4SentiSE) &  .82 & .83 & .81  \\
& & Majority-PMT DL &  .85 & .86 & .85  \\
& & Majority-Shallow ML &  .77 & .77 & .77  \\
& & Majority-PMT DL + Rule &  .84 & .85 & .84  \\
& & Majority-Shallow ML + Rule &  .81 & .81 & .80  \\
& & Majority-BTPC &  .83 & .83 & .82  \\
\cmidrule{3-6}

& \multirow{8}{*}{Jira} & Baseline: Best (BERT4SentiSE) & .80 & .79 & .79\\
% \cmidrule{4-6}
& & Majority-All &  .80 & .81 & .81  \\
& & Majority-All (Except RNN4SentiSE) &  .82 & .83 & .83  \\
& & Majority-PMT DL &  .84 & .77 & .78  \\
& & Majority-Shallow ML &  .75 & .67 & .68  \\
& & Majority-PMT DL + Rule &  .82 & .83 & .82  \\
& & Majority-Shallow ML + Rule &  .80 & .81 & .80  \\
& & Majority-BTPC &  .82 & .83 & .83  \\

\midrule
\multirow{16}{*}{Jira}  &  \multirow{8}{*}{GitHub} & Baseline: Best (SentiStrengthSE) & .76 & .82 & .79\\
% \cmidrule{4-6}
& & Majority-All &  .61 & .76 & .61  \\
& & Majority-All (Except RNN4SentiSE) &  .68 & .81 & .70  \\
& & Majority-PMT DL &  .72 & .82 & .75  \\
& & Majority-Shallow ML &  .71 & .80 & .73  \\
& & Majority-PMT DL + Rule &  .70 & .83 & .74  \\
& & Majority-Shallow ML + Rule &  .70 & .81 & .73  \\
& & Majority-BTPC &  .69 & .82 & .72  \\
\cmidrule{3-6}

& \multirow{8}{*}{Stack Overflow} & Baseline: Best (SentiStrengthSE) & .76 & .82 & .79\\
% \cmidrule{4-6}
& & Majority-All &  .67 & .80 & .69  \\
& & Majority-All (Except RNN4SentiSE) &  .69 & .81 & .72  \\
& & Majority-PMT DL &  .74 & .82 & .76  \\
& & Majority-Shallow ML &  .62 & .63 & .61  \\
& & Majority-PMT DL + Rule &  .72 & .83 & .75  \\
& & Majority-Shallow ML + Rule &  .70 & .80 & .73  \\
& & Majority-BTPC &  .71 & .82 & .74  \\
% \multirow{10}{*}{S(C)} 

% \midrule


% \multirow{10}{*}{J(C)}
    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:ensemble_result}%
\end{table}%

\begin{figure*}[t]
\centering
\captionsetup[subfigure]{labelformat=empty}
\pgfplotstableread{
1	.78 .78 .80 .79 .75 .82 .79 .80      .80 .78 .80 .81 .76 .82 .78 .80    .85 .75 .81 .85 .77 .84 .80 .82     .85 .78 .82 .85 .77 .84 .81 .83    .79 .61 .70 .75 .73 .74 .73 .72    .76 .61 .68 .72 .71 .70 .70 .69
2	.78 .80 .81 .68 .69 .81 .80 .81      .80 .80 .81 .80 .79 .82 .81 .81    .79 .81 .83 .78 .68 .82 .80 .83     .80 .80 .82 .84 .75 .82 .80 .82    .79 .69 .72 .76 .61 .75 .73 .74    .76 .67 .69 .74 .62 .72 .70 .71
}\datatable
\pgfplotscreateplotcyclelist{xcolor}{%
red!60, orange, yellow, blue!50, brown, violet, purple, black!60
}

\edef\mylst{"a", "b", "c", "d", "e", "f", "g", "h"}

      \subfloat[Test on GitHub (F1 score)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
      
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Trained on SO\\(Baseline: SentiStrengthSE), Trained on Jira\\(Baseline: SentiStrengthSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.5,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend style={draw=none},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        % 	nodes near coords=\pgfmathsetmacro{\mystring}{{\mylst}[\coordindex]}\mystring,
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=1] \datatable;
        % 	\node [above] at (axis cs:  100,  92.021) {a};
        	\addplot table[x index=0,y index=2] \datatable;
        % 	\node [above] at (axis cs:  100,  92.021) {b};
        	\addplot table[x index=0,y index=3] \datatable;
        	\addplot table[x index=0,y index=4] \datatable;
            \addplot table[x index=0,y index=5] \datatable;
        	\addplot table[x index=0,y index=6] \datatable;
        	\addplot table[x index=0,y index=7] \datatable;
        	\addplot table[x index=0,y index=8] \datatable;

            % \foreach \Point [count=\i] in {
            %     1, 2, 3, 4, 5, 6, 7, 8
            % }{
            % %  \node[dot,label=\i] at \Point {};
            %  \addplot table[x index=0,y index=\Point] \datatable node[above] {a};
            % %  \node[above] at ($(axis cs:table[x index=0,y index=\Point] \datatable$) {200};
            %  \node[label=\i] at (table[x index=0,y index=\Point] \datatable) {};
            % %  \node [above,color=black] at (endofplotsquare) {a};
            % }

            \legend{Baseline,
            		 Majority-All, , ,
                     Majority-Shallow ML,
                     Majority-PMT DL + Rule, , ,
            		 }
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } 
    \subfloat[Test on GitHub (Precision)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Trained on SO\\(Baseline: SentiStrengthSE), Trained on Jira\\(Baseline: SentiStrengthSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.50,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=9] \datatable;
        	\addplot table[x index=0,y index=10] \datatable;
        	\addplot table[x index=0,y index=11] \datatable;
        	\addplot table[x index=0,y index=12] \datatable;
            \addplot table[x index=0,y index=13] \datatable;
        	\addplot table[x index=0,y index=14] \datatable;
        	\addplot table[x index=0,y index=15] \datatable;
        	\addplot table[x index=0,y index=16] \datatable;

            \legend{, , Majority-All (Except RNN4SentiSE),
            		 Majority-PMT DL, , ,
                     Majority-Shallow ML + Rule,
                     Majority-BTP
            		}
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } \\
    
    \subfloat[Test on Stack Overflow (SO) (F1 score)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub\\(Baseline: BERT4SentiSE), Train on Jira\\(Baseline: BERT4SentiSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.5,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=17] \datatable;
        	\addplot table[x index=0,y index=18] \datatable;
        	\addplot table[x index=0,y index=19] \datatable;
        	\addplot table[x index=0,y index=20] \datatable;
            \addplot table[x index=0,y index=21] \datatable;
        	\addplot table[x index=0,y index=22] \datatable;
        	\addplot table[x index=0,y index=23] \datatable;
        	\addplot table[x index=0,y index=24] \datatable;

            % \legend{Baseline, ,
            % 		 Majority-All,
            % 		 Majority-All (Except RNN4SentiSE),
            % 		 Majority-PMT DL,
            % 		 }
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } 
    \subfloat[Test on Stack Overflow (SO) (Precision)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub\\(Baseline: BERT4SentiSE), Train on Jira\\(Baseline: BERT4SentiSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.50,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=25] \datatable;
        	\addplot table[x index=0,y index=26] \datatable;
        	\addplot table[x index=0,y index=27] \datatable;
        	\addplot table[x index=0,y index=28] \datatable;
            \addplot table[x index=0,y index=29] \datatable;
        	\addplot table[x index=0,y index=30] \datatable;
        	\addplot table[x index=0,y index=31] \datatable;
        	\addplot table[x index=0,y index=32] \datatable;

            % \legend{, , , ,
            %          Majority-Shallow ML,
            %          Majority-PMT DL + Rule,
            %          Majority-Shallow ML + Rule,
            %          Majority-BTP
            % 		}
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } \\
    
    \subfloat[Test on Jira (F1 score)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub\\(Baseline: SentiStrengthSE), Train on SO\\(Baseline: SentiStrengthSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.5,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=33] \datatable;
        	\addplot table[x index=0,y index=34] \datatable;
        	\addplot table[x index=0,y index=35] \datatable;
        	\addplot table[x index=0,y index=36] \datatable;
            \addplot table[x index=0,y index=37] \datatable;
        	\addplot table[x index=0,y index=38] \datatable;
        	\addplot table[x index=0,y index=39] \datatable;
        	\addplot table[x index=0,y index=40] \datatable;

            % \legend{Baseline, ,
            % 		 Majority-All,
            % 		 Majority-All (Except RNN4SentiSE),
            % 		 Majority-PMT DL,
            % 		 }
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } 
    \subfloat[Test on Jira (Precision)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub\\(Baseline: SentiStrengthSE), Train on SO\\(Baseline: SentiStrengthSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.50,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=41] \datatable;
        	\addplot table[x index=0,y index=42] \datatable;
        	\addplot table[x index=0,y index=43] \datatable;
        	\addplot table[x index=0,y index=44] \datatable;
            \addplot table[x index=0,y index=45] \datatable;
        	\addplot table[x index=0,y index=46] \datatable;
        	\addplot table[x index=0,y index=47] \datatable;
        	\addplot table[x index=0,y index=48] \datatable;

            % \legend{, , , ,
            %          Majority-Shallow ML,
            %          Majority-PMT DL + Rule,
            %          Majority-Shallow ML + Rule,
            %          Majority-BTP
            % 		}
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } \\
    
\vspace{-5mm}
\caption{Performance comparison of majority voting based ensemble tools with the SD tools (All- All of the SD tools except baseline DL-RNN4SEntiSE, BTPC-Best SD tool from PMT DL-based (BERT4SentiSE), Shallow ML-based (Senti4SD), Rule-based (SentiStrengthSE)}


\vspace{-5mm}
\label{fig:ensemble_result}
\end{figure*}




==> Raf/Rq4_table_backup.tex <==

\begin{table}[]
  \footnotesize
%   \small
  \centering
  %\vspace{-.1in}
  \caption{Agreement metrics between  tools with manual labelling}
  % \vspace{-3mm}
    % \resizebox{\columnwidth}{!}{%
    \begin{tabular}{clrrrr}
    \toprule{}
    %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
    %\cmidrule{3-6}
    \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Classifier }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
    \cmidrule{5-6}
    {Dataset} &  & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
    \midrule
\multicolumn{6}{c}{\textbf{Test dataset: GitHub}} \\
\midrule

\multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Within-platform)}} 
 & SEntiMoji & 0.84 & 90\% & 1\% & 9\%  \\
 & BERT4SentiSE & 0.87 & 92\% & 1\% & 7\%  \\
 & RNN4SentiSE & 0.52 & 68\% & 7\% & 25\%  \\
 & Senti4SD & 0.86 & 91\% & 1\% & 8\%  \\
 & SentiCR & 0.73 & 83\% & 2\% & 15\%  \\
% \midrule
\cmidrule{2-6}

\multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow \\ (Cross-platform)}}  
 & SEntiMoji & 0.61 & 75\% & 2\% & 23\%  \\
 & BERT4SentiSE & 0.65 & 78\% & 3\% & 19\%  \\
 & RNN4SentiSE & 0.47 & 66\% & 4\% & 30\%  \\
 & Senti4SD & 0.60 & 74\% & 4\% & 22\%  \\
 & SentiCR & 0.49 & 68\% & 2\% & 29\%  \\
% \midrule
\cmidrule{2-6}


\multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Cross-platform)}} 
 & SEntiMoji & 0.44 & 66\% & 1\% & 33\%  \\
 & BERT4SentiSE & 0.48 & 68\% & 2\% & 30\%  \\
 & RNN4SentiSE & 0.35 & 60\% & 4\% & 36\%  \\
 & Senti4SD & 0.50 & 69\% & 2\% & 28\%  \\
 & SentiCR & 0.34 & 60\% & 1\% & 39\%  \\
\midrule



\multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
\midrule

\multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow (Within-platform)}}
 & SEntiMoji & 0.80 & 87\% & 1\% & 12\%  \\
 & BERT4SentiSE& 0.82 & 88\% & 1\% & 11\%  \\
 & RNN4SentiSE & 0.67 & 78\% & 3\% & 19\%  \\
 & Senti4SD & 0.77 & 85\% & 1\% & 14\%  \\
 & SentiCR & 0.73 & 82\% & 3\% & 15\%  \\
% \midrule
\cmidrule{2-6}

\multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Cross-platform)}} 
 & SEntiMoji & 0.73 & 83\% & 1\% & 16\%  \\
 & BERT4SentiSE & 0.78 & 85\% & 1\% & 14\%  \\
 & RNN4SentiSE & 0.49 & 67\% & 4\% & 29\%  \\
 & Senti4SD & 0.67 & 78\% & 2\% & 20\%  \\
 & SentiCR & 0.56 & 71\% & 5\% & 23\%  \\
% \midrule
\cmidrule{2-6}

\multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Cross-platform)}} 
 & SEntiMoji & 0.48 & 67\% & 0\% & 33\%  \\
 & BERT4SentiSE & 0.63 & 76\% & 1\% & 23\%  \\
 & RNN4SentiSE & 0.34 & 58\% & 4\% & 38\%  \\
 & Senti4SD & 0.47 & 66\% & 1\% & 33\%  \\
 & SentiCR & 0.37 & 60\% & 2\% & 38\%  \\
\midrule







\multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
\midrule
\multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Within-platform)}}
 & SEntiMoji & 0.71 & 86\% & 0\% & 14\%  \\
 & BERT4SentiSE& 0.72 & 86\% & 0\% & 13\%  \\
 & RNN4SentiSE & 0.57 & 80\% & 1\% & 20\%  \\
 & Senti4SD & 0.59 & 81\% & 0\% & 19\%  \\
 & SentiCR & 0.69 & 85\% & 0\% & 15\%  \\
% \midrule
\cmidrule{2-6}


\multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Cross-platform)}} 
 & SEntiMoji & 0.65 & 81\% & 1\% & 18\%  \\
 & BERT4SentiSE & 0.65 & 81\% & 1\% & 18\%  \\
 & RNN4SentiSE & 0.45 & 66\% & 2\% & 32\%  \\
 & Senti4SD & 0.58 & 78\% & 1\% & 21\%  \\
 & SentiCR & 0.65 & 82\% & 1\% & 17\%  \\
% \midrule
\cmidrule{2-6}

\multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow \\ (Cross-platform)}} 
 & SEntiMoji & 0.65 & 82\% & 1\% & 18\%  \\
 & BERT4SentiSE & 0.66 & 82\% & 1\% & 17\%  \\
 & RNN4SentiSE & 0.57 & 77\% & 1\% & 22\%  \\
 & Senti4SD & 0.46 & 74\% & 1\% & 25\%  \\
 & SentiCR & 0.34 & 73\% & 1\% & 26\%  \\
% \midrule
    % \midrule  
    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:agreement_with_manual_labelling}%
\end{table}%


















% ===================================================================================================>
% \resizebox{\textwidth}{!}{%
\begin{sidewaystable}
\vspace{15cm}
% \hvFloat[rotAngle=90,nonFloat=true,capWidth=w]
% \begin{table}
\parbox{.3\linewidth}{
\renewcommand{\thetable}{\arabic{table}a}
%   \footnotesize
  \small
  \centering
  \caption{Agreement between  tools (Test dataset: GitHub)}
    \begin{tabular}{clrr|rr}
    \toprule
    \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagree}}\\
    \cmidrule{3-6}
    & & {\bf{$\kappa$}} & {\textbf{P}} & \textbf{S} & \textbf{M} \\
    \midrule
\multirow{10}{*}{G (W)} 
 & SM $\leftrightarrow$ BS & 0.86 & 91\% & 1\% & 8\%  \\
 & SM $\leftrightarrow$ RS & 0.52 & 68\% & 7\% & 25\%  \\
 & SM $\leftrightarrow$ SD & 0.83 & 89\% & 1\% & 10\%  \\
 & SM $\leftrightarrow$ SC & 0.76 & 85\% & 2\% & 13\%  \\
 & BS $\leftrightarrow$ RS & 0.53 & 69\% & 7\% & 24\%  \\
 & BS vs SD & 0.85 & 90\% & 2\% & 8\%  \\
 & BS vs SC & 0.74 & 83\% & 2\% & 14\%  \\
 & RS vs SD & 0.52 & 69\% & 7\% & 25\%  \\
 & RS vs SC & 0.43 & 63\% & 7\% & 31\%  \\
 & SD vs SC & 0.74 & 83\% & 2\% & 14\%  \\
\midrule


\multirow{10}{*}{S(C)} 
 & SM vs BS & 0.72 & 83\% & 1\% & 15\%  \\
 & SM vs RS & 0.58 & 76\% & 2\% & 22\%  \\
 & SM vs SD & 0.51 & 70\% & 3\% & 27\%  \\
 & SM vs SC & 0.40 & 68\% & 2\% & 30\%  \\
 & BS vs RS & 0.59 & 76\% & 2\% & 22\%  \\
 & BS vs SD & 0.52 & 70\% & 4\% & 26\%  \\
 & BS vs SC & 0.39 & 66\% & 3\% & 31\%  \\
 & RS vs SD & 0.43 & 65\% & 4\% & 31\%  \\
 & RS vs SC & 0.30 & 62\% & 3\% & 35\%  \\
 & SD vs SC & 0.45 & 68\% & 2\% & 30\%  \\
\midrule


\multirow{10}{*}{J(C)} 
 & SM vs BS & 0.78 & 90\% & 0\% & 10\%  \\
 & SM vs RS & 0.54 & 81\% & 1\% & 19\%  \\
 & SM vs SD & 0.60 & 82\% & 1\% & 18\%  \\
 & SM vs SC & 0.65 & 87\% & 0\% & 13\%  \\
 & BS vs RS & 0.56 & 81\% & 1\% & 18\%  \\
 & BS vs SD & 0.60 & 81\% & 1\% & 18\%  \\
 & BS vs SC & 0.67 & 87\% & 0\% & 13\%  \\
 & RS vs SD & 0.44 & 74\% & 2\% & 24\%  \\
 & RS vs SC & 0.45 & 79\% & 1\% & 20\%  \\
 & SD vs SC & 0.52 & 79\% & 1\% & 20\%  \\

    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:agreement_test_github}%
% \end{table}%
% \end{sidewaystable}
}
% \begin{sidewaystable}
% \vspace{15cm}
% \begin{table}
\hfill
\parbox{.3\linewidth}{
\addtocounter{table}{-1}
\renewcommand{\thetable}{\arabic{table}b}
%   \footnotesize
  \small
  \centering
  \caption{Agreement between  tools (Test dataset: SO)}
    \begin{tabular}{clrr|rr}
    \toprule
    \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagree}}\\
    \cmidrule{3-6}
    & & {\bf{$\kappa$}} & {\textbf{P}} & \textbf{S} & \textbf{M} \\
    \midrule

\multirow{10}{*}{ S (W)} 
 & SM vs BS & 0.86 & 91\% & 1\% & 8\%  \\
 & SM vs RS & 0.70 & 80\% & 3\% & 17\%  \\
 & SM vs SD & 0.81 & 88\% & 1\% & 12\%  \\
 & SM vs SC & 0.78 & 85\% & 2\% & 12\%  \\
 & BS vs RS & 0.71 & 81\% & 2\% & 17\%  \\
 & BS vs SD & 0.83 & 88\% & 1\% & 11\%  \\
 & BS vs SC & 0.78 & 85\% & 3\% & 12\%  \\
 & RS vs SD & 0.70 & 80\% & 3\% & 17\%  \\
 & RS vs SC & 0.65 & 77\% & 4\% & 19\%  \\
 & SD vs SC & 0.78 & 85\% & 3\% & 12\%  \\
\midrule

\multirow{10}{*}{ G (C)} 
 & SM vs BS & 0.79 & 86\% & 1\% & 13\%  \\
 & SM vs RS & 0.53 & 70\% & 4\% & 27\%  \\
 & SM vs SD & 0.70 & 80\% & 3\% & 17\%  \\
 & SM vs SC & 0.62 & 75\% & 5\% & 20\%  \\
 & BS vs RS & 0.53 & 69\% & 5\% & 26\%  \\
 & BS vs SD & 0.73 & 82\% & 2\% & 16\%  \\
 & BS vs SC & 0.60 & 74\% & 5\% & 21\%  \\
 & RS vs SD & 0.54 & 69\% & 4\% & 26\%  \\
 & RS vs SC & 0.40 & 61\% & 6\% & 33\%  \\
 & SD vs SC & 0.58 & 73\% & 4\% & 23\%  \\
\midrule


\multirow{10}{*}{ J (C)} 
 & SM vs BS & 0.66 & 82\% & 0\% & 18\%  \\
 & SM vs RS & 0.47 & 75\% & 1\% & 23\%  \\
 & SM vs SD & 0.60 & 81\% & 1\% & 19\%  \\
 & SM vs SC & 0.56 & 80\% & 1\% & 19\%  \\
 & BS vs RS & 0.43 & 70\% & 2\% & 28\%  \\
 & BS vs SD & 0.57 & 77\% & 1\% & 22\%  \\
 & BS vs SC & 0.52 & 75\% & 1\% & 25\%  \\
 & RS vs SD & 0.42 & 72\% & 2\% & 27\%  \\
 & RS vs SC & 0.33 & 70\% & 1\% & 29\%  \\
 & SD vs SC & 0.51 & 77\% & 1\% & 22\%  \\
% \midrule

    \bottomrule
    \end{tabular}%
  \label{tab:agreement_test_so}%
% \end{table}%
% \end{sidewaystable}
}
\hfill
\parbox{.3\linewidth}{
% \begin{sidewaystable}
% \begin{table}[]
  \addtocounter{table}{-1}
  \renewcommand{\thetable}{\arabic{table}c}
%   \footnotesize
  \small
  \centering
  \caption{Agreement between  tools (Test dataset: Jira)}
    \begin{tabular}{clrr|rr}
    \toprule
    \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagree}}\\
    \cmidrule{3-6}
    & & {\bf{$\kappa$}} & {\textbf{P}} & \textbf{S} & \textbf{M} \\
    \midrule

\multirow{10}{*}{ J (W)} 
 & SM vs BS & 0.85 & 93\% & 0\% & 7\%  \\
 & SM vs RS & 0.68 & 86\% & 0\% & 14\%  \\
 & SM vs SD & 0.72 & 87\% & 0\% & 13\%  \\
 & SM vs SC & 0.81 & 91\% & 0\% & 9\%  \\
 & BS vs RS & 0.68 & 85\% & 1\% & 14\%  \\
 & BS vs SD & 0.72 & 87\% & 0\% & 13\%  \\
 & BS vs SC & 0.79 & 90\% & 0\% & 10\%  \\
 & RS vs SD & 0.61 & 83\% & 0\% & 17\%  \\
 & RS vs SC & 0.70 & 86\% & 1\% & 14\%  \\
 & SD vs SC & 0.70 & 86\% & 0\% & 13\%  \\
\midrule

\multirow{10}{*}{ G (C)} 
 & SM vs BS & 0.81 & 89\% & 1\% & 10\%  \\
 & SM vs RS & 0.56 & 72\% & 3\% & 25\%  \\
 & SM vs SD & 0.72 & 84\% & 1\% & 14\%  \\
 & SM vs SC & 0.75 & 86\% & 1\% & 13\%  \\
 & BS vs RS & 0.57 & 73\% & 3\% & 24\%  \\
 & BS vs SD & 0.73 & 85\% & 1\% & 14\%  \\
 & BS vs SC & 0.75 & 87\% & 1\% & 13\%  \\
 & RS vs SD & 0.52 & 70\% & 3\% & 27\%  \\
 & RS vs SC & 0.50 & 69\% & 2\% & 28\%  \\
 & SD vs SC & 0.68 & 83\% & 1\% & 16\%  \\
\midrule


\multirow{10}{*}{ S (C)} 
 & SM vs BS & 0.80 & 89\% & 1\% & 10\%  \\
 & SM vs RS & 0.70 & 84\% & 1\% & 15\%  \\
 & SM vs SD & 0.61 & 79\% & 1\% & 19\%  \\
 & SM vs SC & 0.35 & 70\% & 1\% & 29\%  \\
 & BS vs RS & 0.72 & 84\% & 1\% & 14\%  \\
 & BS vs SD & 0.60 & 79\% & 2\% & 19\%  \\
 & BS vs SC & 0.36 & 71\% & 1\% & 28\%  \\
 & RS vs SD & 0.56 & 77\% & 2\% & 22\%  \\
 & RS vs SC & 0.30 & 67\% & 1\% & 32\%  \\
 & SD vs SC & 0.41 & 76\% & 1\% & 23\%  \\
% \midrule
    % \midrule  
    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:agreement_test_jira}%
 }
% \end{table}%
\end{sidewaystable}





% \begin{table}
% \renewcommand{\thetable}{\arabic{table}a}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Agreement between  tools (Test dataset: GitHub)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule
% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Within Platform)}} 
%  & SentiMoji vs BERT4SE & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiMoji vs RNN4SE & 0.52 & 68\% & 7\% & 25\%  \\
%  & SentiMoji vs Senti4SD & 0.83 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs SentiCR & 0.76 & 85\% & 2\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.53 & 69\% & 7\% & 24\%  \\
%  & BERT4SE vs Senti4SD & 0.85 & 90\% & 2\% & 8\%  \\
%  & BERT4SE vs SentiCR & 0.74 & 83\% & 2\% & 14\%  \\
%  & RNN4SE vs Senti4SD & 0.52 & 69\% & 7\% & 25\%  \\
%  & RNN4SE vs SentiCR & 0.43 & 63\% & 7\% & 31\%  \\
%  & Senti4SD vs SentiCR & 0.74 & 83\% & 2\% & 14\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.72 & 83\% & 1\% & 15\%  \\
%  & SentiMoji vs RNN4SE & 0.58 & 76\% & 2\% & 22\%  \\
%  & SentiMoji vs Senti4SD & 0.51 & 70\% & 3\% & 27\%  \\
%  & SentiMoji vs SentiCR & 0.40 & 68\% & 2\% & 30\%  \\
%  & BERT4SE vs RNN4SE & 0.59 & 76\% & 2\% & 22\%  \\
%  & BERT4SE vs Senti4SD & 0.52 & 70\% & 4\% & 26\%  \\
%  & BERT4SE vs SentiCR & 0.39 & 66\% & 3\% & 31\%  \\
%  & RNN4SE vs Senti4SD & 0.43 & 65\% & 4\% & 31\%  \\
%  & RNN4SE vs SentiCR & 0.30 & 62\% & 3\% & 35\%  \\
%  & Senti4SD vs SentiCR & 0.45 & 68\% & 2\% & 30\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.78 & 90\% & 0\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.54 & 81\% & 1\% & 19\%  \\
%  & SentiMoji vs Senti4SD & 0.60 & 82\% & 1\% & 18\%  \\
%  & SentiMoji vs SentiCR & 0.65 & 87\% & 0\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.56 & 81\% & 1\% & 18\%  \\
%  & BERT4SE vs Senti4SD & 0.60 & 81\% & 1\% & 18\%  \\
%  & BERT4SE vs SentiCR & 0.67 & 87\% & 0\% & 13\%  \\
%  & RNN4SE vs Senti4SD & 0.44 & 74\% & 2\% & 24\%  \\
%  & RNN4SE vs SentiCR & 0.45 & 79\% & 1\% & 20\%  \\
%  & Senti4SD vs SentiCR & 0.52 & 79\% & 1\% & 20\%  \\

%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_github}%
% \end{table}%


% ==================================================================================================>

% \begin{table}
% \addtocounter{table}{-1}
% \renewcommand{\thetable}{\arabic{table}b}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Agreement between  tools (Test dataset: SO)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Within Platform)}} 
%  & SentiMoji vs BERT4SE & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiMoji vs RNN4SE & 0.70 & 80\% & 3\% & 17\%  \\
%  & SentiMoji vs Senti4SD & 0.81 & 88\% & 1\% & 12\%  \\
%  & SentiMoji vs SentiCR & 0.78 & 85\% & 2\% & 12\%  \\
%  & BERT4SE vs RNN4SE & 0.71 & 81\% & 2\% & 17\%  \\
%  & BERT4SE vs Senti4SD & 0.83 & 88\% & 1\% & 11\%  \\
%  & BERT4SE vs SentiCR & 0.78 & 85\% & 3\% & 12\%  \\
%  & RNN4SE vs Senti4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & RNN4SE vs SentiCR & 0.65 & 77\% & 4\% & 19\%  \\
%  & Senti4SD vs SentiCR & 0.78 & 85\% & 3\% & 12\%  \\
% \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.79 & 86\% & 1\% & 13\%  \\
%  & SentiMoji vs RNN4SE & 0.53 & 70\% & 4\% & 27\%  \\
%  & SentiMoji vs Senti4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & SentiMoji vs SentiCR & 0.62 & 75\% & 5\% & 20\%  \\
%  & BERT4SE vs RNN4SE & 0.53 & 69\% & 5\% & 26\%  \\
%  & BERT4SE vs Senti4SD & 0.73 & 82\% & 2\% & 16\%  \\
%  & BERT4SE vs SentiCR & 0.60 & 74\% & 5\% & 21\%  \\
%  & RNN4SE vs Senti4SD & 0.54 & 69\% & 4\% & 26\%  \\
%  & RNN4SE vs SentiCR & 0.40 & 61\% & 6\% & 33\%  \\
%  & Senti4SD vs SentiCR & 0.58 & 73\% & 4\% & 23\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.66 & 82\% & 0\% & 18\%  \\
%  & SentiMoji vs RNN4SE & 0.47 & 75\% & 1\% & 23\%  \\
%  & SentiMoji vs Senti4SD & 0.60 & 81\% & 1\% & 19\%  \\
%  & SentiMoji vs SentiCR & 0.56 & 80\% & 1\% & 19\%  \\
%  & BERT4SE vs RNN4SE & 0.43 & 70\% & 2\% & 28\%  \\
%  & BERT4SE vs Senti4SD & 0.57 & 77\% & 1\% & 22\%  \\
%  & BERT4SE vs SentiCR & 0.52 & 75\% & 1\% & 25\%  \\
%  & RNN4SE vs Senti4SD & 0.42 & 72\% & 2\% & 27\%  \\
%  & RNN4SE vs SentiCR & 0.33 & 70\% & 1\% & 29\%  \\
%  & Senti4SD vs SentiCR & 0.51 & 77\% & 1\% & 22\%  \\
% % \midrule

%     \bottomrule
%     \end{tabular}%
%   \label{tab:agreement_test_so}%
% \end{table}%

% % ===================================================================================================>

% \begin{table}[]
%   \addtocounter{table}{-1}
%   \renewcommand{\thetable}{\arabic{table}c}

% %   \footnotesize
%   \small
%   \centering
%   \caption{Agreement between  tools (Test dataset: Jira)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Within Platform}} 
%  & SentiMoji vs BERT4SE & 0.85 & 93\% & 0\% & 7\%  \\
%  & SentiMoji vs RNN4SE & 0.68 & 86\% & 0\% & 14\%  \\
%  & SentiMoji vs Senti4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & SentiMoji vs SentiCR & 0.81 & 91\% & 0\% & 9\%  \\
%  & BERT4SE vs RNN4SE & 0.68 & 85\% & 1\% & 14\%  \\
%  & BERT4SE vs Senti4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & BERT4SE vs SentiCR & 0.79 & 90\% & 0\% & 10\%  \\
%  & RNN4SE vs Senti4SD & 0.61 & 83\% & 0\% & 17\%  \\
%  & RNN4SE vs SentiCR & 0.70 & 86\% & 1\% & 14\%  \\
%  & Senti4SD vs SentiCR & 0.70 & 86\% & 0\% & 13\%  \\
% \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.81 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.56 & 72\% & 3\% & 25\%  \\
%  & SentiMoji vs Senti4SD & 0.72 & 84\% & 1\% & 14\%  \\
%  & SentiMoji vs SentiCR & 0.75 & 86\% & 1\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.57 & 73\% & 3\% & 24\%  \\
%  & BERT4SE vs Senti4SD & 0.73 & 85\% & 1\% & 14\%  \\
%  & BERT4SE vs SentiCR & 0.75 & 87\% & 1\% & 13\%  \\
%  & RNN4SE vs Senti4SD & 0.52 & 70\% & 3\% & 27\%  \\
%  & RNN4SE vs SentiCR & 0.50 & 69\% & 2\% & 28\%  \\
%  & Senti4SD vs SentiCR & 0.68 & 83\% & 1\% & 16\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.80 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.70 & 84\% & 1\% & 15\%  \\
%  & SentiMoji vs Senti4SD & 0.61 & 79\% & 1\% & 19\%  \\
%  & SentiMoji vs SentiCR & 0.35 & 70\% & 1\% & 29\%  \\
%  & BERT4SE vs RNN4SE & 0.72 & 84\% & 1\% & 14\%  \\
%  & BERT4SE vs Senti4SD & 0.60 & 79\% & 2\% & 19\%  \\
%  & BERT4SE vs SentiCR & 0.36 & 71\% & 1\% & 28\%  \\
%  & RNN4SE vs Senti4SD & 0.56 & 77\% & 2\% & 22\%  \\
%  & RNN4SE vs SentiCR & 0.30 & 67\% & 1\% & 32\%  \\
%  & Senti4SD vs SentiCR & 0.41 & 76\% & 1\% & 23\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_jira}%
% \end{table}%








\begin{table}
  \footnotesize
%   \small

  \centering
  \caption{Performance comparison of majority voting based ensemble tools with the SD tools (All- All of the SD tools except baseline DL-RNN4SEntiSE, BTPC-Best SD tool from PMT DL-based (BERT4SentiSE), Shallow ML-based (Senti4SD), Rule-based (SentiStrengthSE) }
    \begin{tabular}{ccllll}
    \toprule
    \multirow{2}{*}{\bf{Test Dataset}} & \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\textbf{Ensemble}} & \multicolumn{3}{c}{\textbf{Macro Performance}}\\
    \cmidrule{4-6}
    & & & {\bf{$P$}} & {\bf{$R$}} & {\bf{$F1$}} \\
    \midrule
    
\multirow{16}{*}{GitHub}  &  \multirow{8}{*}{Stack Overflow} & Baseline: Best & .80 & .78 & .78\\
% \cmidrule{4-6}
& & Majority-All &  .78 & .80 & .78  \\
& & Majority-All (Except RNN4SentiSE) &  .80 & .81 & .80  \\
& & Majority-PMT DL &  .81 & .78 & .79  \\
& & Majority-Shallow ML &  .76 & .75 & .75  \\
& & Majority-PMT DL + Rule &  .82 & .83 & .82  \\
& & Majority-Shallow ML + Rule &  .78 & .80 & .79  \\
& & Majority-BTPC &  .80 & .81 & .80  \\
\cmidrule{3-6}

& \multirow{8}{*}{Jira} & Baseline: Best & .80 & .78 & .78\\
% \cmidrule{4-6}
& & Majority-All &  .80 & .80 & .80  \\
& & Majority-All (Except RNN4SentiSE) &  .81 & .81 & .81  \\
& & Majority-PMT DL &  .80 & .66 & .68  \\
& & Majority-Shallow ML &  .79 & .67 & .69  \\
& & Majority-PMT DL + Rule &  .82 & .80 & .81  \\
& & Majority-Shallow ML + Rule &  .81 & .80 & .80  \\
& & Majority-BTPC &  .81 & .81 & .81  \\

\midrule
\multirow{16}{*}{Stack Overflow}  &  \multirow{8}{*}{GitHub} & Baseline: Best & .85 & .86 & .85\\
% \cmidrule{4-6}
& & Majority-All &  .78 & .78 & .75  \\
& & Majority-All (Except RNN4SentiSE) &  .82 & .83 & .81  \\
& & Majority-PMT DL &  .85 & .86 & .85  \\
& & Majority-Shallow ML &  .77 & .77 & .77  \\
& & Majority-PMT DL + Rule &  .84 & .85 & .84  \\
& & Majority-Shallow ML + Rule &  .81 & .81 & .80  \\
& & Majority-BTPC &  .83 & .83 & .82  \\
\cmidrule{3-6}

& \multirow{8}{*}{Jira} & Baseline: Best & .80 & .79 & .79\\
% \cmidrule{4-6}
& & Majority-All &  .80 & .81 & .81  \\
& & Majority-All (Except RNN4SentiSE) &  .82 & .83 & .83  \\
& & Majority-PMT DL &  .84 & .77 & .78  \\
& & Majority-Shallow ML &  .75 & .67 & .68  \\
& & Majority-PMT DL + Rule &  .82 & .83 & .82  \\
& & Majority-Shallow ML + Rule &  .80 & .81 & .80  \\
& & Majority-BTPC &  .82 & .83 & .83  \\

\midrule
\multirow{16}{*}{Jira}  &  \multirow{8}{*}{GitHub} & Baseline: Best & .76 & .82 & .79\\
% \cmidrule{4-6}
& & Majority-All &  .61 & .76 & .61  \\
& & Majority-All (Except RNN4SentiSE) &  .68 & .81 & .70  \\
& & Majority-PMT DL &  .72 & .82 & .75  \\
& & Majority-Shallow ML &  .71 & .80 & .73  \\
& & Majority-PMT DL + Rule &  .70 & .83 & .74  \\
& & Majority-Shallow ML + Rule &  .70 & .81 & .73  \\
& & Majority-BTPC &  .69 & .82 & .72  \\
\cmidrule{3-6}

& \multirow{8}{*}{Stack Overflow} & Baseline: Best & .76 & .82 & .79\\
% \cmidrule{4-6}
& & Majority-All &  .67 & .80 & .69  \\
& & Majority-All (Except RNN4SentiSE) &  .69 & .81 & .72  \\
& & Majority-PMT DL &  .74 & .82 & .76  \\
& & Majority-Shallow ML &  .62 & .63 & .61  \\
& & Majority-PMT DL + Rule &  .72 & .83 & .75  \\
& & Majority-Shallow ML + Rule &  .70 & .80 & .73  \\
& & Majority-BTPC &  .71 & .82 & .74  \\
% \multirow{10}{*}{S(C)} 

% \midrule


% \multirow{10}{*}{J(C)}
    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:ensemble_result}%
\end{table}%





==> Raf/alltools.tex <==

% % \begin{sidewaystable}
% % \vspace{15cm}
% \begin{table*}%[t]
% \footnotesize
% % \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Performance of SE-specific sentiment analysis in cross-platform settings (SentiSE = SentistrengthSE)}
%   %\vspace{-3mm}
%   % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{ll|rrr|rrr|rrr|rrr|rrr|rrr}
%     \toprule{}

%     \multirow{2}{*}{\textbf{Setting}}  & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiSE}}\\
%     \cmidrule{3-20}
%     {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
    
%     %\multicolumn{18}{c}{\textbf{Test dataset: GitHub}} \\
%     %\midrule
 
%      \multirow{5}{1.4cm}{Test:  GitHub Train: GitHub  (Within)}
%      & Negative &  .89 & .85 & .87  & .89 & .91 & .90  & .68 & .69 & .68  & .90 & .89 & .90  & .87 & .69 & .77  & .81 & .71 & .76   \\ 
%      & Neutral &  .87 & .92 & .89  & .92 & .90 & .91  & .73 & .66 & .69  & .89 & .92 & .91  & .77 & .91 & .84  & .74 & .86 & .79   \\ 
%      & Positive &  .94 & .92 & .93  & .93 & .94 & .94  & .64 & .72 & .68  & .94 & .91 & .93  & .89 & .84 & .86  & .85 & .76 & .80   \\ 
%      & Micro-avg &  .90 & .90 & .90  & \textbf{.92} & \textbf{.92} & \textbf{.92}  & .68 & .68 & .68  & .91 & .91 & .91  & .83 & .83 & .83  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .90 & .89 & .90  & \textbf{.91} & \textbf{.92} & \textbf{.92}  & .68 & .69 & .68  & \textbf{.91} & .91 & .91  & .84 & .81 & .82  & .80 & .78 & .78   \\ 

%     \cmidrule{2-20}     

%      % Test dataset: Github
% \multirow{5}{1.4cm}{Test:  GitHub Train: SO  (Cross)}
%  & Negative &  .85 & .62 & .72  & .83 & .73 & .78  & .69 & .49 & .58  & .79 & .56 & .66  & .83 & .37 & .51  & .81 & .71 & .76   \\ 
%  & Neutral &  .67 & .91 & .77  & .71 & .91 & .80  & .61 & .84 & .71  & .71 & .82 & .76  & .60 & .94 & .73  & .74 & .86 & .79   \\ 
%  & Positive &  .88 & .65 & .75  & .88 & .63 & .73  & .78 & .57 & .66  & .76 & .81 & .78  & .86 & .62 & .72  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .75 & .75 & .75  & .78 & .78 & .78  & .66 & .66 & .66  & .74 & .74 & .74  & .68 & .68 & .68  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  .80 & .73 & .75  & \textbf{.81} & .76 & .77  & .69 & .63 & .65  & .75 & .73 & .73  & .76 & .64 & .66  & .80 & \textbf{.78} & \textbf{.78}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.15 & -.15 & -.15 & -.14 & -.14 & -.14 & -.02 & -.02 & -.02 & -.17 & -.17 & -.17 & -.14 & -.14 & -.14  \\ 
% % & & Macro-avg &  -.10 & -.17 & -.15 & -.11 & -.16 & -.15 & .01 & -.05 & -.04 & -.16 & -.18 & -.18 & -.08 & -.17 & -.17  \\ 
% \cmidrule{2-20}
    
    
    
%     % Test dataset: Github
%     \multirow{5}{1.4cm}{Test: GitHub Train: Jira  (Cross)} 
%      & Negative &  .91 & .39 & .55  & .90 & .43 & .58  & .75 & .39 & .52  & .85 & .52 & .64  & .88 & .27 & .41  & .81 & .71 & .76   \\ 
%  & Neutral &  .56 & .98 & .72  & .59 & .97 & .73  & .54 & .95 & .69  & .60 & .96 & .74  & .52 & .98 & .68  & .74 & .86 & .79   \\ 
%  & Positive &  .94 & .45 & .60  & .91 & .51 & .65  & .80 & .30 & .44  & .90 & .46 & .61  & .89 & .38 & .53  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .66 & .66 & .66  & .68 & .68 & .68  & .60 & .60 & .60  & .69 & .69 & .69  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  \textbf{.80} & .61 & .62  & \textbf{.80} & .64 & .65  & .70 & .55 & .55  & .78 & .65 & .67  & .76 & .54 & .54  & \textbf{.80} & \textbf{.78} & \textbf{.78}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.24 & -.24 & -.24 & -.23 & -.23 & -.23 & -.08 & -.08 & -.08 & -.22 & -.22 & -.22 & -.23 & -.23 & -.23  \\ 
% % & & Macro-avg &  -.10 & -.29 & -.28 & -.12 & -.28 & -.26 & .02 & -.14 & -.14 & -.13 & -.26 & -.24 & -.08 & -.27 & -.28  \\ 

% \midrule





% %    \multicolumn{18}{c}{\textbf{Test dataset: Stack Overflow}} \\
% %    \midrule
%     \multirow{5}{1.4cm}{Test: SO Train: SO  (Within)} 
%  & Negative &  .84 & .83 & .83  & .86 & .85 & .85  & .74 & .73 & .74  & .80 & .83 & .82  & .80 & .72 & .76  & .76 & .76 & .76   \\ 
%  & Neutral &  .83 & .84 & .84  & .86 & .85 & .85  & .75 & .77 & .76  & .84 & .79 & .81  & .79 & .82 & .81  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .93 & .93  & .93 & .94 & .93  & .85 & .85 & .85  & .90 & .93 & .91  & .88 & .91 & .89  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}  & .78 & .78 & .78  & .85 & .85 & .85  & .82 & .82 & .82  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}  & .78 & .78 & .78  & .85 & .85 & .85  & .82 & .82 & .82  & .80 & .79 & .79   \\ 
 

%     \cmidrule{2-20}
    
%     % Test dataset: Stack Overflow
%     \multirow{5}{1.4cm}{Test: SO Train: GitHub  (Cross)} 
%  & Negative &  .82 & .76 & .79  & .80 & .86 & .83  & .66 & .60 & .63  & .69 & .76 & .72  & .64 & .49 & .55  & .76 & .76 & .76   \\ 
%  & Neutral &  .75 & .85 & .80  & .84 & .80 & .82  & .61 & .64 & .63  & .73 & .76 & .75  & .65 & .85 & .74  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .85 & .89  & .93 & .91 & .92  & .73 & .74 & .74  & .92 & .82 & .87  & .88 & .74 & .80  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .83 & .83 & .83  & \textbf{.85} & \textbf{.85} & \textbf{.85}  & .67 & .67 & .67  & .78 & .78 & .78  & .71 & .71 & .71  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .83 & .82 & .82  & \textbf{.85} & \textbf{.86} & \textbf{.85}  & .67 & .66 & .66  & .78 & .78 & .78  & .72 & .69 & .70  & .80 & .79 & .79   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.12 & -.12 & -.12 & -.07 & -.07 & -.07 & -.11 & -.11 & -.11  \\ 
% % & & Macro-avg &  -.03 & -.05 & -.04 & -.03 & -.02 & -.03 & -.11 & -.12 & -.12 & -.06 & -.07 & -.07 & -.10 & -.12 & -.12  \\ 

%     \cmidrule{2-20}


%     % Test dataset: Stack Overflow
%     \multirow{5}{1.4cm}{Test: SO Train: Jira  (Cross)}
%  & Negative &  .93 & .31 & .47  & .88 & .55 & .68  & .66 & .31 & .42  & .75 & .30 & .43  & .67 & .22 & .33  & .76 & .76 & .76   \\ 
%  & Neutral &  .54 & .98 & .70  & .63 & .94 & .76  & .50 & .91 & .65  & .54 & .93 & .69  & .50 & .95 & .66  & .73 & .79 & .75   \\ 
%  & Positive &  .98 & .62 & .76  & .97 & .74 & .84  & .83 & .42 & .56  & .96 & .64 & .76  & .96 & .52 & .67  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .67 & .67 & .67  & .76 & .76 & .76  & .58 & .58 & .58  & .66 & .66 & .66  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  .82 & .64 & .64  & \textbf{.83} & .74 & .76  & .66 & .55 & .54  & .75 & .62 & .63  & .71 & .56 & .55  & .80 & \textbf{.79} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.20 & -.20 & -.20 & -.12 & -.12 & -.12 & -.21 & -.21 & -.21 & -.19 & -.19 & -.19 & -.22 & -.22 & -.22  \\ 
% % & & Macro-avg &  -.05 & -.23 & -.23 & -.05 & -.14 & -.12 & -.12 & -.23 & -.24 & -.10 & -.23 & -.22 & -.11 & -.25 & -.27  \\ 

%     \midrule





%     % Test dataset: Jira
% %    \multicolumn{18}{c}{\textbf{Test dataset: Jira}} \\
% %    \midrule
%     \multirow{5}{1.4cm}{Test: Jira Train: Jira  (Within)} 
%  & Negative &  .84 & .68 & .75  & .82 & .76 & .79  & .69 & .46 & .55  & .71 & .55 & .62  & .79 & .66 & .72  & .68 & .73 & .71   \\ 
%  & Neutral &  .89 & .91 & .90  & .90 & .90 & .90  & .83 & .89 & .86  & .84 & .88 & .86  & .89 & .89 & .89  & .92 & .82 & .87   \\ 
%  & Positive &  .79 & .80 & .79  & .78 & .80 & .79  & .73 & .72 & .72  & .73 & .71 & .72  & .75 & .85 & .80  & .68 & .92 & .78   \\ 
%  & Micro-avg &  \textbf{.86} & \textbf{.86} & \textbf{.86}  & \textbf{.86} & \textbf{.86} & \textbf{.86}  & .80 & .80 & .80  & .81 & .81 & .81  & .85 & .85 & .85  & .83 & .83 & .83   \\ 
%  & Macro-avg &  \textbf{.84} & .80 & .81  & .83 & \textbf{.82} & \textbf{.83}  & .75 & .69 & .71  & .76 & .72 & .73  & .81 & .80 & .80  & .76 & \textbf{.82} & .79   \\ 

%     \cmidrule{2-20}
    
    
%     % Test dataset: Jira
%     \multirow{5}{1.4cm}{Test: Jira Train: GitHub (Cross)} 
%  & Negative &  .63 & .75 & .69  & .66 & .74 & .70  & .51 & .71 & .60  & .61 & .64 & .62  & .69 & .60 & .64  & .68 & .73 & .71   \\ 
%  & Neutral &  .93 & .79 & .85  & .93 & .80 & .86  & .92 & .58 & .71  & .89 & .78 & .83  & .90 & .85 & .87  & .92 & .82 & .87   \\ 
%  & Positive &  .66 & .91 & .77  & .65 & .91 & .76  & .45 & .92 & .61  & .62 & .86 & .72  & .69 & .89 & .78  & .68 & .92 & .78   \\ 
%  & Micro-avg &  .81 & .81 & .81  & .81 & .81 & .81  & .66 & .66 & .66  & .78 & .78 & .78  & .82 & .82 & .82  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg &  .74 & \textbf{.82} & .77  & .75 & \textbf{.82} & .77  & .63 & .74 & .64  & .71 & .76 & .73  & \textbf{.76} & .78 & .76  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.05 & -.05 & -.05 & -.05 & -.05 & -.05 & -.14 & -.14 & -.14 & -.03 & -.03 & -.03 & -.03 & -.03 & -.03  \\ 
% % & & Macro-avg &  -.09 & .02 & -.04 & -.09 & -.00 & -.05 & -.12 & .05 & -.07 & -.05 & .05 & -.01 & -.05 & -.02 & -.04  \\ 

%     \cmidrule{2-20}
    
    
%     % Test dataset: Jira
%     \multirow{5}{1.4cm}{Test: Jira Train: SO (Cross)}
%  & Negative &  .67 & .68 & .67  & .72 & .68 & .70  & .58 & .61 & .59  & .50 & .29 & .37  & .36 & .06 & .10  & .68 & .73 & .71   \\ 
%  & Neutral &  .92 & .81 & .86  & .92 & .82 & .87  & .88 & .77 & .82  & .82 & .81 & .81  & .75 & .94 & .83  & .92 & .82 & .87   \\ 
%  & Positive &  .67 & .93 & .78  & .65 & .93 & .76  & .62 & .89 & .73  & .59 & .80 & .68  & .71 & .49 & .58  & .68 & .92 & .78   \\ 
%  & Micro-avg &  .82 & .82 & .82  & .82 & .82 & .82  & .77 & .77 & .77  & .74 & .74 & .74  & .73 & .73 & .73  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg &  .75 & .81 & .77  & \textbf{.76} & .81 & .78  & .69 & .75 & .71  & .64 & .63 & .62  & .61 & .49 & .50  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.07 & -.07 & -.07 & -.12 & -.12 & -.12  \\ 
% % & & Macro-avg &  -.08 & .01 & -.04 & -.07 & -.01 & -.05 & -.05 & .06 & .00 & -.12 & -.08 & -.11 & -.20 & -.30 & -.30  \\ 


%     \bottomrule
%     \end{tabular}%
% %}
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance}%
% \end{table*}%
% % \end{sidewaystable}





% % \begin{sidewaystable}
% % \vspace{15cm}
% \begin{table*}%[t]
% \footnotesize
% % \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Performance drop in SE-specific supervised sentiment analysis tools in cross-platform settings (SO = Stack Overflow)}
%   %\vspace{-3mm}
%   % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{cl|rrr|rrr|rrr|rrr|rrr}
%     \toprule{}

%     \multirow{2}{*}{\textbf{Train}} & \multirow{2}{*}{\textbf{Performance}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} \\
%     \cmidrule{3-17}
%     \textbf{Dataset} & \centering \textbf{Drop} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
    
%     \multicolumn{17}{c}{\textbf{Test dataset: GitHub}} \\
%     \midrule
 
%     \multirow{2}{*}{\textbf{SO}} & $\triangledown$ Micro-avg &  -16\% & -16\% & -16\% & -15\% & -15\% & -15\% & -3\% & -3\% & -3\% & -18\% & -18\% & -18\% & -17\% & -17\% & -17\%    \\ 
%     &  $\triangledown$ Macro-avg &  -11\% & -19\% & -17\% & -12\% & -18\% & -16\% & 2\% & -8\% & -5\% & -17\% & -20\% & -19\% & -10\% & -21\% & -20\%  \\ 
%     \cmidrule{2-17}
    
%     \multirow{2}{*}{\textbf{Jira}} &  $\triangledown$ Micro-avg &  -27\% & -27\% & -27\% & -26\% & -26\% & -26\% & -12\% & -12\% & -12\% & -24\% & -24\% & -24\% & -27\% & -27\% & -27\%   \\ 
%     &  $\triangledown$ Macro-avg &  -11\% & -32\% & -31\% & -13\% & -31\% & -29\% & 2\% & -21\% & -20\% & -14\% & -29\% & -27\% & -9\% & -34\% & -34\%  \\ 
%     % \cmidrule{2-17}
%     \midrule
    
    
%     \multicolumn{17}{c}{\textbf{Test dataset: Stack Overflow}} \\
%     \midrule
%     \multirow{2}{*}{\textbf{GitHub}} & $\triangledown$  Micro-avg &  -5\% & -5\% & -5\% & -3\% & -3\% & -3\% & -15\% & -15\% & -15\% & -8\% & -8\% & -8\% & -13\% & -13\% & -13\%   \\ 
%     & $\triangledown$  Macro-avg &  -4\% & -5\% & -5\% & -3\% & -3\% & -3\% & -15\% & -15\% & -15\% & -7\% & -8\% & -8\% & -12\% & -15\% & -15\%  \\ 
%     \cmidrule{2-17}
%     \multirow{2}{*}{\textbf{Jira}} &  $\triangledown$ Micro-avg &  -23\% & -23\% & -23\% & -13\% & -13\% & -13\% & -26\% & -26\% & -26\% & -22\% & -22\% & -22\% & -27\% & -27\% & -27\%   \\ 
%     &  $\triangledown$ Macro-avg &  -6\% & -27\% & -26\% & -6\% & -16\% & -14\% & -15\% & -30\% & -31\% & -11\% & -27\% & -26\% & -14\% & -31\% & -33\%  \\ 
%     % \cmidrule{2-17}
%     \midrule
    
%     \multicolumn{17}{c}{\textbf{Test dataset: Jira}} \\
%     \midrule
%     \multirow{2}{*}{\textbf{GitHub}} &  $\triangledown$ Micro-avg &  -6\% & -6\% & -6\% & -6\% & -6\% & -6\% & -17\% & -17\% & -17\% & -4\% & -4\% & -4\% & -3\% & -3\% & -3\%    \\ 
%     &  $\triangledown$ Macro-avg &  -11\% & 3\% & -5\% & -10\% & 0\% & -7\% & -16\% & 7\% & -10\% & -7\% & 7\% & -1\% & -6\% & -2\% & -5\%  \\ 
%     \cmidrule{2-17}
%     \multirow{2}{*}{\textbf{SO}} & $\triangledown$  Micro-avg &  -5\% & -5\% & -5\% & -5\% & -5\% & -5\% & -4\% & -4\% & -4\% & -9\% & -9\% & -9\% & -14\% & -14\% & -14\%   \\ 
%     &  $\triangledown$ Macro-avg &  -10\% & 1\% & -5\% & -8\% & -1\% & -6\% & -7\% & 9\% & 1\% & -16\% & -12\% & -15\% & -25\% & -38\% & -37\%  \\ 
%     % \cmidrule{2-17}
%     \midrule



%     \bottomrule
%     \end{tabular}%
% %}
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance_drop}%
% \end{table*}%
% % \end{sidewaystable}



==> SubmissionTOSEM/RQ0.tex <==

\subsection{RQ$_1$ Can deep learning sentiment detection tools for software engineering perform equally well both within and in cross-platform settings?}\label{sec:rq0}

\subsubsection{Motivation} Research in SE finds that cross-domain SD tools can be insufficiently accurate for SE datasets. Such 
findings motivated the development of SE-specific SD tools.  
The recent advances in deep learning techniques influenced the development of several deep learning SD tools for SE. The most recent deep learning SD tools for SE
are BERT4SentiSE, SentiMoji, and RNN4SentSE. BERT4SentiSE and SentiMoji are found to have outperformed other SE-specific SD tools. However, 
the experimentation was conducted in within-platform settings. This means that the tools were trained and tested using the same dataset. 
 Recent research in SE also finds that the SE-specific shallow learning SD tools (Senti4SD and SentiCR) 
can suffer from a drop in performance in cross-platform settings, i.e., when trained in one SE dataset and tested on another SE dataset. 
It is thus necessary to know whether the tools show similar performance in cross-platform settings because that would 
indicate the broader applicability of the tools.
% 
% The three deep learning tools, 
% especially BERT4SentiSE~\cite{Biswas-ReliableSentiSEBERT-ICSME2020} and SentiMoji~\cite{Chen-SentiEmoji-FSE2019} are found to be the best performers 
% in several SE-specific sentiment datasets. However, the experimentation was done 
% for within-platform setting.  

%\input{RQ0_tables}
\subsubsection{Approach} \label{sec:rq0-approach}
We investigate the performance of three most recent deep learning SD tools for SE: BERT4SentiSE, RNN4SentiSE, and SentiMoji. 
We compare the performance of each tool between within and cross-platform settings. 
For each tool, we checked six cross-platform settings: two for each dataset
(i.e., train on a dataset and test on another dataset). We compute the performance of each tool in the settings as follows.
\begin{itemize}[leftmargin=10pt]

 \item \ib{Within platform.} We use k-fold cross validation~\cite{stone1974cross} to train and test a tool in a given dataset. 
In this study, we employ 10-fold cross-validation settings where the dataset is
 divided into ten folds, and each fold is used as a test set at some point. First,
 we divide each dataset into 10-folds using the Scikit
 StratifiedKFold \footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.model_selection.StratifiedKFold.html}}
 technique, which ensures that each fold contains the same proportion of
 polarity classes as the original dataset.
 We train and test each supervised SD tool for each dataset in ten iterations.
 In the first iteration, we use fold 1 of the dataset as the test set and the remaining 9 folds as the training set. In the second iteration, we use fold 2 as the test set and the remaining 9 folds for training the supervised tool. This
 process continues ten times until all of the ten folds are used as a test set. Then we merge the predictions of the tool for each test fold and calculate the tool's overall performance on that dataset.


 \item \ib{Cross Platform.} We train each tool on one dataset (e.g., SO) and test it on the other two datasets (e.g., GitHub and Jira). 
 We report the performance of each tool per testing dataset. This means that for a given dataset under test, we check the correct and incorrect cases on all the 
 sentences/units of analysis in the dataset. Therefore, similar to the within-platform setting, we are checking an entire dataset for performance analysis in cross-platform 
 setting. In within-platform setting, we do ten iterations in a 10-fold cross-validation setup. For cross-platform 
 setting, we run the tool once in a train dataset (to create a trained model) and then run the trained model once on the other two test datasets.  
\end{itemize}







We report performance using three standard metrics of information
retrieval: precision ($P$), recall ($R$), and F1-score ($F1$)~\cite{sokolova2009systematic}. \textit{Precision} signifies the number of samples correctly predicted as positive out of total samples predicted as positive. \textit{Recall} signifies the number of samples correctly identified as positives out of total samples that are actually positive. \textit{$F1$ measure} is the harmonic average of precision ($P$) and recall ($R$). 
{%\scriptsize %, $TN = $ \# of true negatives, and $FP = $\# of false positives.}
% A &= \sum_{n=-\infty}^{+\infty} f(x) \\
\begin{align} \label{eq:metrics}
% \begin{eqnarray*}
P  = \frac{\sum_{i=1}^{l} TP_i}{\sum_{i=1}^{l} TP_i+FP_i},~
R = \frac{\sum_{i=1}^{l} TP_i}{\sum_{i=1}^{l} TP_i+FN_i},~
F1 = 2*\frac{P*R}{P+R}
% \end{eqnarray*}
% \end{equation}
\end{align}
} {$TP = $ \# of true positives, $FP =$ \# of false positives, $FN =$ \# of false negatives.}. 

In our multi-class sentiment problem, a $TP$, $FP$, and $FN$ are calculated for each class. For example, we have three possible sentiment classes (positive, neutral, and negative). 
For a particular class (e.g., neutral sentiment) $TP$ occurs when the tool predicts `neutral'. For the same class, $FN$ occurs when the tool predicts any other classes (e.g., positive or negative), and $TN$ occurs when the tool predicts `neutral' but the original label is not `neutral'.
We use the confusion matrix in \tbl\ref{tab:conmat-sentiment} and Equation~\cite{sokolova2009systematic} (\ref{eq:metrics}) following state of the art~\cite{Novielli-BenchmarkStudySentiSE-MSR2018,Calefato-Senti4SD-EMSE2017,Sebastiani-MachineLearningTextCategorization-ACMSurveys2002,Uddin-OpinionValue-TSE2019}. 
% We use precision\_recall\_fscore\_support method from Sklearn to calculate these metrics \footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.metrics.precision_recall_fscore_support.html}}
% A macro-average will compute the metric independently for each class and then take the average (hence treating all classes equally), whereas a micro-average will aggregate the contributions of all classes to compute the average metric.
We report overall performance using micro and macro averages and by each
polarity class. The macro-average computes the metrics for each class and then
averages thus it treats each classes equally. On the other hand, the
micro-average aggregates the contribution of all classes. Micro-average is
influenced by the performance of the majority class~\cite{Sebastiani-MachineLearningTextCategorization-ACMSurveys2002}
because most number of examples belong to this class. We use Macro F1-score to
report the best tool, following standard
practices~\cite{Novielli-BenchmarkStudySentiSE-MSR2018,Manning-IRIntroBook-Cambridge2009}.
\begin{table}[t]
  \centering
  \caption{Confusion matrix for multi-class (three) sentiment detection}
  %\vspace{-2mm}
%   \resizebox{\columnwidth}{!}{%
    \begin{tabular}{crr|r|r}\toprule
          &       & \multicolumn{3}{c}{\textbf{Predicted}} \\
          \cmidrule{3-5}
          &       & \textbf{Positive (P)} & \textbf{Negative (N)} & \textbf{Neutral (O)} \\
          \cmidrule{2-5}
    \multirow{3}[0]{*}{\textbf{Actual}} & \textbf{Positive (P)} & TP$_P$ & FP$_N$, FN$_P$ & FP$_O$, FN$_P$ \\
          & \textbf{Negative (N)} & FP$_P$, FN$_N$ & TP$_N$ & FP$_O$, FN$_N$ \\
          & \textbf{Neutral (O)} & FP$_P$, FN$_O$ & FP$_N$, FN$_O$ & TP$_O$ \\
          \bottomrule
    \end{tabular}%
    % }
    %\vspace{-7pt}
  \label{tab:conmat-sentiment}%
\end{table}%

\begin{table*}%[t]
\footnotesize
% \small
  \centering
  %\vspace{-.1in}
  \caption{Performance of SE-specific sentiment analysis tools in cross-platform settings (SentiSE = SentistrengthSE).}
  %\vspace{-3mm}
 \resizebox{\columnwidth}{!}{%
    \begin{tabular}{ll|rrr|rrr|rrr|rrr|rrr|rrr}
    \toprule{}

    % \multirow{2}{*}{\textbf{Setting}}  & \multirow{2}{*}{\textbf{Polarity}} & 
    % \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiSE}}\\
    % \cmidrule{3-20}
    % {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
\multirow{3}{*}{\textbf{Setting}} &\multirow{3}{*}{\textbf{Polarity}} &\multicolumn{9}{c|}{\textbf{Deep-learning based SD Tools}} &\multicolumn{6}{c|}{\textbf{Shallow ML-based}} &\multicolumn{3}{c}{\textbf{Rule-based}} \\
\cmidrule{3-20}
& &\multicolumn{3}{c}{\textbf{SEntiMoji}} &\multicolumn{3}{c}{\textbf{BERT4SEntiSE}} &\multicolumn{3}{c}{\textbf{RNN4SentiSE}} &\multicolumn{3}{c}{\textbf{Senti4SD}} &\multicolumn{3}{c}{\textbf{SentiCR}} &\multicolumn{3}{c}{\textbf{SentiSE}} \\
\cmidrule{3-20}
& &\textbf{P} &\textbf{R} &\textbf{F1} &\textbf{P} &\textbf{R} &\textbf{F1} &\textbf{P} &\textbf{R} &\textbf{F1} &\textbf{P} &\textbf{R} &\textbf{F1} &\textbf{P} &\textbf{R} &\textbf{F1} &\textbf{P} &\textbf{R} &\textbf{F1} \\   
    
    
    \midrule
\multicolumn{20}{c}{\bf{Test Dataset: GitHub}} \\
\cmidrule{2-20}    
    %\multicolumn{18}{c}{\textbf{Test dataset: GitHub}} \\
    %\midrule
 
     \multirow{5}{1.4cm}{Test:  GitHub Train: GitHub  (Within-platform)}
     & -NEG &  .89 & .85 & .87  & .89 & .91 & .90  & .68 & .69 & .68  & .90 & .89 & .90  & .87 & .69 & .77  & .81 & .71 & .76   \\ 
     & Neutral &  .87 & .92 & .89  & .92 & .90 & .91  & .73 & .66 & .69  & .89 & .92 & .91  & .77 & .91 & .84  & .74 & .86 & .79   \\ 
     & +POS &  .94 & .92 & .93  & .93 & .94 & .94  & .64 & .72 & .68  & .94 & .91 & .93  & .89 & .84 & .86  & .85 & .76 & .80   \\ 
     & Micro &  .90 & .90 & .90  & \textbf{.92} & \textbf{.92} & \textbf{.92}  & .68 & .68 & .68  & .91 & .91 & .91  & .83 & .83 & .83  & .79 & .79 & .79   \\ 
 & Macro &  .90 & .89 & .90  & \textbf{.91} & \textbf{.92} & \textbf{.92}  & .68 & .69 & .68  & \textbf{.91} & .91 & .91  & .84 & .81 & .82  & .80 & .78 & .78   \\ 

    \cmidrule{2-20}     

     % Test dataset: Github
\multirow{5}{1.4cm}{Test:  GitHub Train: SO  (Cross-platform)}
 & -NEG &  .85 & .62 & .72  & .83 & .73 & .78  & .69 & .49 & .58  & .79 & .56 & .66  & .83 & .37 & .51  & .81 & .71 & .76   \\ 
 & Neutral &  .67 & .91 & .77  & .71 & .91 & .80  & .61 & .84 & .71  & .71 & .82 & .76  & .60 & .94 & .73  & .74 & .86 & .79   \\ 
 & +POS &  .88 & .65 & .75  & .88 & .63 & .73  & .78 & .57 & .66  & .76 & .81 & .78  & .86 & .62 & .72  & .85 & .76 & .80   \\ 
 & Micro &  .75 & .75 & .75  & .78 & .78 & .78  & .66 & .66 & .66  & .74 & .74 & .74  & .68 & .68 & .68  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
 & Macro &  .80 & .73 & .75  & \textbf{.81} & .76 & .77  & .69 & .63 & .65  & .75 & .73 & .73  & .76 & .64 & .66  & .80 & \textbf{.78} & \textbf{.78}   \\ 

% \multirow{2}{*}{Diff.} & & Micro &  -.15 & -.15 & -.15 & -.14 & -.14 & -.14 & -.02 & -.02 & -.02 & -.17 & -.17 & -.17 & -.14 & -.14 & -.14  \\ 
% & & Macro &  -.10 & -.17 & -.15 & -.11 & -.16 & -.15 & .01 & -.05 & -.04 & -.16 & -.18 & -.18 & -.08 & -.17 & -.17  \\ 
\cmidrule{2-20}
    
    
    
    % Test dataset: Github
    \multirow{5}{1.4cm}{Test: GitHub Train: Jira  (Cross-platform)} 
     & -NEG &  .91 & .39 & .55  & .90 & .43 & .58  & .75 & .39 & .52  & .85 & .52 & .64  & .88 & .27 & .41  & .81 & .71 & .76   \\ 
 & Neutral &  .56 & .98 & .72  & .59 & .97 & .73  & .54 & .95 & .69  & .60 & .96 & .74  & .52 & .98 & .68  & .74 & .86 & .79   \\ 
 & +POS &  .94 & .45 & .60  & .91 & .51 & .65  & .80 & .30 & .44  & .90 & .46 & .61  & .89 & .38 & .53  & .85 & .76 & .80   \\ 
 & Micro &  .66 & .66 & .66  & .68 & .68 & .68  & .60 & .60 & .60  & .69 & .69 & .69  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
 & Macro &  \textbf{.80} & .61 & .62  & \textbf{.80} & .64 & .65  & .70 & .55 & .55  & .78 & .65 & .67  & .76 & .54 & .54  & \textbf{.80} & \textbf{.78} & \textbf{.78}   \\ 

% \multirow{2}{*}{Diff.} & & Micro &  -.24 & -.24 & -.24 & -.23 & -.23 & -.23 & -.08 & -.08 & -.08 & -.22 & -.22 & -.22 & -.23 & -.23 & -.23  \\ 
% & & Macro &  -.10 & -.29 & -.28 & -.12 & -.28 & -.26 & .02 & -.14 & -.14 & -.13 & -.26 & -.24 & -.08 & -.27 & -.28  \\ 

\midrule
\multicolumn{20}{c}{\bf{Test Dataset: Stack Overflow (SO)}} \\
\cmidrule{2-20}    





%    \multicolumn{18}{c}{\textbf{Test dataset: Stack Overflow}} \\
%    \midrule
    \multirow{5}{1.4cm}{Test: SO Train: SO  (Within-platform)} 
 & -NEG &  .84 & .83 & .83  & .86 & .85 & .85  & .74 & .73 & .74  & .80 & .83 & .82  & .80 & .72 & .76  & .76 & .76 & .76   \\ 
 & Neutral &  .83 & .84 & .84  & .86 & .85 & .85  & .75 & .77 & .76  & .84 & .79 & .81  & .79 & .82 & .81  & .73 & .79 & .75   \\ 
 & +POS &  .93 & .93 & .93  & .93 & .94 & .93  & .85 & .85 & .85  & .90 & .93 & .91  & .88 & .91 & .89  & .91 & .82 & .86   \\ 
 & Micro &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}  & .78 & .78 & .78  & .85 & .85 & .85  & .82 & .82 & .82  & .79 & .79 & .79   \\ 
 & Macro &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}  & .78 & .78 & .78  & .85 & .85 & .85  & .82 & .82 & .82  & .80 & .79 & .79   \\ 
 

    \cmidrule{2-20}
    
    % Test dataset: Stack Overflow
    \multirow{5}{1.4cm}{Test: SO Train: GitHub  (Cross-platform)} 
 & -NEG &  .82 & .76 & .79  & .80 & .86 & .83  & .66 & .60 & .63  & .69 & .76 & .72  & .64 & .49 & .55  & .76 & .76 & .76   \\ 
 & Neutral &  .75 & .85 & .80  & .84 & .80 & .82  & .61 & .64 & .63  & .73 & .76 & .75  & .65 & .85 & .74  & .73 & .79 & .75   \\ 
 & +POS &  .93 & .85 & .89  & .93 & .91 & .92  & .73 & .74 & .74  & .92 & .82 & .87  & .88 & .74 & .80  & .91 & .82 & .86   \\ 
 & Micro &  .83 & .83 & .83  & \textbf{.85} & \textbf{.85} & \textbf{.85}  & .67 & .67 & .67  & .78 & .78 & .78  & .71 & .71 & .71  & .79 & .79 & .79   \\ 
 & Macro &  .83 & .82 & .82  & \textbf{.85} & \textbf{.86} & \textbf{.85}  & .67 & .66 & .66  & .78 & .78 & .78  & .72 & .69 & .70  & .80 & .79 & .79   \\ 

% \multirow{2}{*}{Diff.} & & Micro &  -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.12 & -.12 & -.12 & -.07 & -.07 & -.07 & -.11 & -.11 & -.11  \\ 
% & & Macro &  -.03 & -.05 & -.04 & -.03 & -.02 & -.03 & -.11 & -.12 & -.12 & -.06 & -.07 & -.07 & -.10 & -.12 & -.12  \\ 

    \cmidrule{2-20}


    % Test dataset: Stack Overflow
    \multirow{5}{1.4cm}{Test: SO Train: Jira  (Cross-platform)}
 & -NEG &  .93 & .31 & .47  & .88 & .55 & .68  & .66 & .31 & .42  & .75 & .30 & .43  & .67 & .22 & .33  & .76 & .76 & .76   \\ 
 & Neutral &  .54 & .98 & .70  & .63 & .94 & .76  & .50 & .91 & .65  & .54 & .93 & .69  & .50 & .95 & .66  & .73 & .79 & .75   \\ 
 & +POS &  .98 & .62 & .76  & .97 & .74 & .84  & .83 & .42 & .56  & .96 & .64 & .76  & .96 & .52 & .67  & .91 & .82 & .86   \\ 
 & Micro &  .67 & .67 & .67  & .76 & .76 & .76  & .58 & .58 & .58  & .66 & .66 & .66  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
 & Macro &  .82 & .64 & .64  & \textbf{.83} & .74 & .76  & .66 & .55 & .54  & .75 & .62 & .63  & .71 & .56 & .55  & .80 & \textbf{.79} & \textbf{.79}   \\ 

% \multirow{2}{*}{Diff.} & & Micro &  -.20 & -.20 & -.20 & -.12 & -.12 & -.12 & -.21 & -.21 & -.21 & -.19 & -.19 & -.19 & -.22 & -.22 & -.22  \\ 
% & & Macro &  -.05 & -.23 & -.23 & -.05 & -.14 & -.12 & -.12 & -.23 & -.24 & -.10 & -.23 & -.22 & -.11 & -.25 & -.27  \\ 

    \midrule
\multicolumn{20}{c}{\bf{Test Dataset: Jira}} \\
\cmidrule{2-20}    





    % Test dataset: Jira
%    \multicolumn{18}{c}{\textbf{Test dataset: Jira}} \\
%    \midrule
    \multirow{5}{1.4cm}{Test: Jira Train: Jira  (Within-platform)} 
 & -NEG &  .84 & .68 & .75  & .82 & .76 & .79  & .69 & .46 & .55  & .71 & .55 & .62  & .79 & .66 & .72  & .68 & .73 & .71   \\ 
 & Neutral &  .89 & .91 & .90  & .90 & .90 & .90  & .83 & .89 & .86  & .84 & .88 & .86  & .89 & .89 & .89  & .92 & .82 & .87   \\ 
 & +POS &  .79 & .80 & .79  & .78 & .80 & .79  & .73 & .72 & .72  & .73 & .71 & .72  & .75 & .85 & .80  & .68 & .92 & .78   \\ 
 & Micro &  \textbf{.86} & \textbf{.86} & \textbf{.86}  & \textbf{.86} & \textbf{.86} & \textbf{.86}  & .80 & .80 & .80  & .81 & .81 & .81  & .85 & .85 & .85  & .83 & .83 & .83   \\ 
 & Macro &  \textbf{.84} & .80 & .81  & .83 & \textbf{.82} & \textbf{.83}  & .75 & .69 & .71  & .76 & .72 & .73  & .81 & .80 & .80  & .76 & \textbf{.82} & .79   \\ 

    \cmidrule{2-20}
    
    
    % Test dataset: Jira
    \multirow{5}{1.4cm}{Test: Jira Train: GitHub (Cross-platform)} 
 & -NEG &  .63 & .75 & .69  & .66 & .74 & .70  & .51 & .71 & .60  & .61 & .64 & .62  & .69 & .60 & .64  & .68 & .73 & .71   \\ 
 & Neutral &  .93 & .79 & .85  & .93 & .80 & .86  & .92 & .58 & .71  & .89 & .78 & .83  & .90 & .85 & .87  & .92 & .82 & .87   \\ 
 & +POS &  .66 & .91 & .77  & .65 & .91 & .76  & .45 & .92 & .61  & .62 & .86 & .72  & .69 & .89 & .78  & .68 & .92 & .78   \\ 
 & Micro &  .81 & .81 & .81  & .81 & .81 & .81  & .66 & .66 & .66  & .78 & .78 & .78  & .82 & .82 & .82  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
 & Macro &  .74 & \textbf{.82} & .77  & .75 & \textbf{.82} & .77  & .63 & .74 & .64  & .71 & .76 & .73  & \textbf{.76} & .78 & .76  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\ 

% \multirow{2}{*}{Diff.} & & Micro &  -.05 & -.05 & -.05 & -.05 & -.05 & -.05 & -.14 & -.14 & -.14 & -.03 & -.03 & -.03 & -.03 & -.03 & -.03  \\ 
% & & Macro &  -.09 & .02 & -.04 & -.09 & -.00 & -.05 & -.12 & .05 & -.07 & -.05 & .05 & -.01 & -.05 & -.02 & -.04  \\ 

    \cmidrule{2-20}
    
    
    % Test dataset: Jira
    \multirow{5}{1.4cm}{Test: Jira Train: SO (Cross-platform)}
 & -NEG &  .67 & .68 & .67  & .72 & .68 & .70  & .58 & .61 & .59  & .50 & .29 & .37  & .36 & .06 & .10  & .68 & .73 & .71   \\ 
 & Neutral &  .92 & .81 & .86  & .92 & .82 & .87  & .88 & .77 & .82  & .82 & .81 & .81  & .75 & .94 & .83  & .92 & .82 & .87   \\ 
 & +POS &  .67 & .93 & .78  & .65 & .93 & .76  & .62 & .89 & .73  & .59 & .80 & .68  & .71 & .49 & .58  & .68 & .92 & .78   \\ 
 & Micro &  .82 & .82 & .82  & .82 & .82 & .82  & .77 & .77 & .77  & .74 & .74 & .74  & .73 & .73 & .73  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
 & Macro &  .75 & .81 & .77  & \textbf{.76} & .81 & .78  & .69 & .75 & .71  & .64 & .63 & .62  & .61 & .49 & .50  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\ 

% \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.07 & -.07 & -.07 & -.12 & -.12 & -.12  \\ 
% & & Macro-avg &  -.08 & .01 & -.04 & -.07 & -.01 & -.05 & -.05 & .06 & .00 & -.12 & -.08 & -.11 & -.20 & -.30 & -.30  \\ 


    \bottomrule
    \end{tabular}%
}
  % \vspace{-.25in}
  \label{tab:cross_platform_performance}%
\end{table*}%
\begin{table*}%[t]
%\footnotesize
% \small
  \centering
  %\vspace{-.1in}
  \caption{Performance drop in SE-specific supervised sentiment analysis tools in cross-platform settings (SO = Stack Overflow)}
  %\vspace{-3mm}
  % \resizebox{\textwidth}{!}{%
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{cl|rrr|rrr|rrr|rrr|rrr}
    \toprule{}

    % \multirow{2}{*}{\textbf{Train}} & \multirow{2}{*}{\textbf{Metric}} & 
    % \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} \\
    % \cmidrule{3-17}
    % \textbf{Dataset} & \centering  & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
    
\multirow{3}{*}{\textbf{Train}} &\multirow{3}{*}{\textbf{Metric}} &\multicolumn{9}{c}{\textbf{Deep-learning based}} &\multicolumn{6}{c}{\textbf{Shallow ML-based}} \\
\cmidrule{3-17}
 & &\multicolumn{3}{c}{\textbf{SEntiMoji}} &\multicolumn{3}{c}{\textbf{BERT4SEntiSE}} &\multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} &\multicolumn{3}{c}{\textbf{SentiCR}} \\
\cmidrule{3-17}
\centering \textbf{Dataset} & &\textbf{P} &\textbf{R} &\textbf{F1} &\textbf{P} &\textbf{R} &\textbf{F1} &\textbf{P} &\textbf{R} &\textbf{F1} &\textbf{P} &\textbf{R} &\textbf{F1} &\textbf{P} &\textbf{R} &\textbf{F1} \\


    
    
    \midrule
    
    \multicolumn{17}{c}{\textbf{Test dataset: GitHub}} \\
    \midrule
 
    \multirow{2}{*}{\textbf{SO}} & $\triangledown$ Micro &  -16\% & -16\% & -16\% & -15\% & -15\% & -15\% & -3\% & -3\% & -3\% & -18\% & -18\% & -18\% & -17\% & -17\% & -17\%    \\ 
    &  $\triangledown$ Macro &  -11\% & -19\% & -17\% & -12\% & -18\% & -16\% & 2\% & -8\% & -5\% & -17\% & -20\% & -19\% & -10\% & -21\% & -20\%  \\ 
    \cmidrule{2-17}
    
    \multirow{2}{*}{\textbf{Jira}} &  $\triangledown$ Micro &  -27\% & -27\% & -27\% & -26\% & -26\% & -26\% & -12\% & -12\% & -12\% & -24\% & -24\% & -24\% & -27\% & -27\% & -27\%   \\ 
    &  $\triangledown$ Macro &  -11\% & -32\% & -31\% & -13\% & -31\% & -29\% & 2\% & -21\% & -20\% & -14\% & -29\% & -27\% & -9\% & -34\% & -34\%  \\ 
    % \cmidrule{2-17}
    \midrule
    
    
    \multicolumn{17}{c}{\textbf{Test dataset: Stack Overflow}} \\
    \midrule
    \multirow{2}{*}{\textbf{GitHub}} & $\triangledown$  Micro &  -5\% & -5\% & -5\% & -3\% & -3\% & -3\% & -15\% & -15\% & -15\% & -8\% & -8\% & -8\% & -13\% & -13\% & -13\%   \\ 
    & $\triangledown$  Macro &  -4\% & -5\% & -5\% & -3\% & -3\% & -3\% & -15\% & -15\% & -15\% & -7\% & -8\% & -8\% & -12\% & -15\% & -15\%  \\ 
    \cmidrule{2-17}
    \multirow{2}{*}{\textbf{Jira}} &  $\triangledown$ Micro &  -23\% & -23\% & -23\% & -13\% & -13\% & -13\% & -26\% & -26\% & -26\% & -22\% & -22\% & -22\% & -27\% & -27\% & -27\%   \\ 
    &  $\triangledown$ Macro &  -6\% & -27\% & -26\% & -6\% & -16\% & -14\% & -15\% & -30\% & -31\% & -11\% & -27\% & -26\% & -14\% & -31\% & -33\%  \\ 
    % \cmidrule{2-17}
    \midrule
    
    \multicolumn{17}{c}{\textbf{Test dataset: Jira}} \\
    \midrule
    \multirow{2}{*}{\textbf{GitHub}} &  $\triangledown$ Micro &  -6\% & -6\% & -6\% & -6\% & -6\% & -6\% & -17\% & -17\% & -17\% & -4\% & -4\% & -4\% & -3\% & -3\% & -3\%    \\ 
    &  $\triangledown$ Macro &  -11\% & 3\% & -5\% & -10\% & 0\% & -7\% & -16\% & 7\% & -10\% & -7\% & 7\% & -1\% & -6\% & -2\% & -5\%  \\ 
    \cmidrule{2-17}
    \multirow{2}{*}{\textbf{SO}} & $\triangledown$  Micro &  -5\% & -5\% & -5\% & -5\% & -5\% & -5\% & -4\% & -4\% & -4\% & -9\% & -9\% & -9\% & -14\% & -14\% & -14\%   \\ 
    &  $\triangledown$ Macro &  -10\% & 1\% & -5\% & -8\% & -1\% & -6\% & -7\% & 9\% & 1\% & -16\% & -12\% & -15\% & -25\% & -38\% & -37\%  \\ 
    % \cmidrule{2-17}
   % \midrule



    \bottomrule
    \end{tabular}%
}
  % \vspace{-.25in}
  \label{tab:cross_platform_performance_drop}%
\end{table*}%

%\input{RQ1_tables}

%\input{RQ0_tables}
\begin{table}[t]
  \centering
  \caption{Percentage of correctly classified sentences in within platform settings that were misclassified in cross-platform settings (each value is rounded to the nearest integer)}
  \resizebox{\columnwidth}{!}{%
    \begin{tabular}{ll|cc|cc|cc}\toprule
    {\textbf{SD}} & \textbf{\% Correct} & \multicolumn{2}{c}{\textbf{Test in GitHub}} & \multicolumn{2}{c}{\textbf{Test in SO}} & \multicolumn{2}{c}{\textbf{Test in Jira}} \\
    \cmidrule{3-8}
    {\textbf{Tool}} & \textbf{Misclassified} & {\textbf{Train SO}} & {\textbf{Train Jira}} & {\textbf{Train GitHub}} & {\textbf{Train Jira}} & {\textbf{Train GitHub}} & {\textbf{Train SO}} \\
    \midrule
    \multirow{3}[0]{*}{\textbf{BERT4SentiSE}} & \textbf{Overall} & 19    & 30    & 8     & 18    & 11    & 10 \\
          & \textbf{Severe} & 3     & 1     & 0     & 0     & 1     & 1 \\
          & \textbf{Mild} & 16    & 28    & 7     & 18    & 11    & 10 \\
          \midrule
    \multirow{3}[0]{*}{\textbf{SentiMoji}} & \textbf{Overall} & 19    & 30    & 10    & 29    & 11    & 10 \\
          & \textbf{Severe} & 1     & 1     & 1     & 0     & 0     & 0 \\
          & \textbf{Mild} & 18    & 29    & 9     & 29    & 11    & 10 \\
          \bottomrule
    \end{tabular}%
    }
  \label{tab:rq-error-analysis}%
\end{table}%


\subsubsection{Results} In Table \ref{tab:cross_platform_performance}, the third to fifth columns (SentiMoji, BERT4SentiSE, RNN4SentiSE) 
show the performance of the three deep learning SD tools for SE. The table is divided into three sections, each separated from the other section via a full-length horizontal line. For example, under the title `Test Dataset: GitHub', we show how each tool performs while using GitHub as the test dataset in within and cross-platform 
settings. This means that \begin{inparaenum}[(1)]
\item first we show how a tool performs within the GitHub dataset (i.e., using train-test splitting technique) and
\item second we show how each tool performed on GitHub dataset when they have been trained on the other two datasets, i.e., once trained on Stack Overflow (SO) and another trained on Jira dataset.
\end{inparaenum} Therefore, the first setup is within-platform, and the last two setups are cross-platform settings. 
For a given setting (i.e., within or cross-platform), we report our three performance metrics, Precision (P), Recall (R), and F1-measure (F1) for each of the three polarity classes (i.e., positive, 
negative, neutral). For each setting, we then report the overall performance of each tool using two metrics: Micro-avg and Macro-avg. We discuss significant observations below.   

\bf{Each deep learning SD tool for SE suffers a drop in performance in cross-platform settings compared to its within-platform performance.} There is a notable drop in performance of each of the deep learning SD tools from within to cross-platform settings. The drop, however, varies among the six cross-platform settings. The drop 
also varies among the three DL tools. In \tbl\ref{tab:cross_platform_performance_drop}, we show the percentage drop for each tool from within to cross-platform settings based on the two overall metrics: Macro and Micro avg. In terms of Macro-F1 score, RNN4SentiSE shows the largest drop of 31\% when trained in Jira and then tested in the SO dataset. That means that RNN4SentSE shows a Macro-F1 score of 0.78 tested on SO in within platform setting, but it shows a Macro F1-score of 0.54 for SO when trained in Jira. For the tool SentiMoji, the largest drop happens when the tool is trained in Jira and tested in GitHub (31\%). SentiMoji shows a Macro F1-score of 0.90 when trained and tested in GitHub (Within-platform), but it shows a Macro-F1 score of 0.62 when trained in Jira and then tested in GitHub. For the tool BERT4SentiSE, the largest drop in performance happens when the tool is trained in Jira and then tested in GitHub (29\%). BERT4SentiSE shows a Macro-F1 score of 0.92 when trained and tested in GitHub (Within-platform), but it shows a Macro F1-score of 0.65 when trained in Jira and tested in GitHub. Therefore, we find that three DL tools suffer the largest drop in performance when they are trained in the Jira dataset and then tested in the other two datasets. 


\bf{BERT4SentiSE is the best performer among the three deep learning SD tools for SE both in within and cross-platform settings.} BERT4SentiSE shows Macro F1-scores of 0.92, 0.88, and 0.83 for within-platform settings in the three datasets: GitHub, SO, and Jira, respectively. The second best deep learning SD performer for within-platform settings is SentiMoji, which shows Macro F1-scores of 0.90, 0.87, and 0.81 in the three datasets: GitHub, SO, and Jira, respectively. RNN4SentiSE shows Macro F1-scores of 0.68, 0.78, 0.71 for the three datasets respectively. Similar to the close gaps in performance we observed between BERT4SentiSE and SentiMoji for within platform settings, the gaps in performance between the two tools remain close across the six cross-platform settings. For example, when trained in SO and tested in GitHub, BERT4SentiSE shows a Macro F1-score of 0.77, which SentiMoji shows a Macro F1-score of 0.75. In contrast, RNN4SentiSE shows a Macro F1-score of 0.65 for the same setup. Both BERT4SentiSE and SentiMoji are developed based on the principles of pre-trained models, i.e., the two tools were trained on a large corpus of non-SE datasets (e.g., Twitter, Wikipedia) to learn about general word embedding and representations. The architecture of RNN4SentiSE does not allow such pre-trained embedding. Pre-trained transformer models like BERT show superior performance in other natural language processing tasks~\cite{sun2019fine}. Therefore, it is intuitive that BERT4SentiSE and SentiMoji show less drop in performance than the other deep learning SD tool RNN4SentiSE.

% For each setting, we observed a drop in
% performance in the deep learning SD tools in cross-platform settings. The drop is most in RNN4SentiSE~\cite{Biswas-SentiSEWordEmbedding-MSR2019} across the 
% three datasets. 
% \gias{Here I need two tables. Table 1. show the within and cross-platform performance of each DL tool (don't show those difference rows). Table 2. percentange 
% difference between within and cross platform for each dataset.}
% \gias{After this RQ, we will not show anything related to RNN4SentiSE in the subsequent RQs, given it did not perform well. we will still talk about RNN4SentiSE in RQ2, i.e., we will 
% keep your texts comparing this tool with shallow tools.} 

% Error example
\bf{The deep learning SD Tools suffer a drop in performance in cross-platform settings due mainly to their incorrect labeling of neutral sentences to non-neutral or vice-versa.} In \tbl\ref{tab:rq-error-analysis}, we show how the two best performing deep learning SD tools (BERT4SentiSE and SentiMoji) misclassify sentences in cross-platform settings that they correctly classified in within platform settings. 
For example, out of the sentences that are correctly classified by BERT4SentiSE in the GitHub dataset in within platform setting, 30\% of those were misclassified when trained in Jira and then tested in the same GitHub dataset. Only 1\% of those were severe misclassification, i.e., incorrectly predicted as positive/negative when the correct label was negative/positive. The rest (i.e., 29\%) of the misclassifications are mild, i.e., incorrectly predicted as neutral/non-neutral when the correct label was non-neutral/neutral. 
For example, BERT4SentiSE correctly predicts within platform settings ``that's because it's old API. :( (GitHub, oracle: negative)'' but mispredicts (neutral) in cross-platform settings when trained on Stack Overflow.
Similarly, SentiMoji correctly predicts within platform settings ``sorry for the delay (Jira, oracle: negative)'' but mispredicts (neutral) in cross-platform settings when trained on Stack Overflow.
The above observations denote that the deep learning SD tools suffer in cross-platform settings mainly due to mild errors and not due to severe errors in classifications. 

% BERT4SentiSE correctly predicts within platform settings ``finally getting somewhere( (GitHub, oracle: Positive)'' but mispredicts (neutral) in cross platform settings when trained on Stack Overflow.
% SentiMoji correctly predicts within platform settings ``bug is a duplicate of HIVE-3253. (Jira, oracle: neutral)'' but wrongly predicts (negative) in cross platform settings when trained on GitHub.
% SentiMoji makes correct prediction in within platform settings ``Fixed and I've tested it. (Jira, Oracle: neutral)''. We believe this is an example of subjective annotation. But SentiMoji overfits in within platform settings and makes wrong prediction (positive) when trained on SO dataset. But positive prediction is more suited for this example.

%Future improvements in the tools need to focus more on the causes of such mild errors. 





\begin{tcolorbox}[flushleft upper,boxrule=1pt,arc=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=white,after=\ignorespacesafterend\par\noindent]
 \bf{RQ$_1$ Can deep learning sentiment detection tools for software engineering perform equally well for within and in cross-platform settings?} Each of three deep learning SD tools for SE suffers a drop in performance across our three studied datasets, with the most drop occurred when the tools were trained in the Jira dataset and then tested in the other two datasets. BERT4SentiSE is the best performing tool out of the three SD tools, followed closely by SentiMoji. The misclassifications in the cross-platform setting compared the within platform settings happened mainly due to mild errors, i.e., the tools misclassified neutral to non-neutral and vice-versa.
\end{tcolorbox}

==> SubmissionTOSEM/RQ0_tables.tex <==
% %If the table is too wide, replace \begin{table}[!htp]...\end{table} with
% %\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
% % \begin{table}[!htp]\centering
% % \caption{Percentage of misclassification in cross platform settings compared to within-platform settings.}
% % \resizebox{\columnwidth}{!}{%
% % \begin{tabular}{llrr|rr|rrr}\toprule
% % {\textbf{DL SD}} &{\textbf{\% Correct}} 

% % % &\multicolumn{2}{c}{\textbf{Test Dataset}} &\multicolumn{2}{c}{\textbf{Test Dataset}} &\multicolumn{2}{c}{\textbf{Test Dataset}} \\\cmidrule{3-8}
% % &   &\multicolumn{2}{c}{Test in GitHub} &\multicolumn{2}{c}{Test in SO} &\multicolumn{2}{c}{Test in Jira} \\\cmidrule{3-8}
% % {\textbf{Tool}} & {\textbf{Misclassified}} &\textbf{Train SO} &\textbf{Train Jira} &\textbf{Train GitHub} &\textbf{Train Jira} &\textbf{Train GitHub} &\textbf{Train SO} \\\midrule
% % \multirow{3}{*}{\textbf{BERT4SentiSE}} &\%Overall &19 &30 &8 &18 &11 &10 \\
% % & \%Severe &3 &1 &0 &0 &1 &1 \\
% % &\%Mild &16 &28 &7 &18 &11 &10 \\
% % \midrule
% % \multirow{3}{*}{\textbf{SentiMoji}} &\%Overall &19 &30 &10 &29 &11 &10 \\
% % &\%Severe &1 &1 &1 &0 &0 &0 \\
% % &\%Mild &18 &29 &9 &29 &11 &10 \\
% % \bottomrule
% % \end{tabular}%
% % }
% % \end{table}

% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[t]
%   \centering
%   \caption{Percentage of misclassification in cross platform settings compared to within-platform}
%   \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{ll|rr|rr|rr}\toprule
%     {\textbf{SD}} & \textbf{\% Correct} & \multicolumn{2}{c}{\textbf{Test in GitHub}} & \multicolumn{2}{c}{\textbf{Test in SO}} & \multicolumn{2}{c}{\textbf{Test in Jira}} \\
%     \cmidrule{3-8}
%     {\textbf{Tool}} & \textbf{Misclassified} & {\textbf{Train SO}} & {\textbf{Train Jira}} & {\textbf{Train GitHub}} & {\textbf{Train Jira}} & {\textbf{Train GitHub}} & {\textbf{Train SO}} \\
%     \midrule
%     \multirow{3}[0]{*}{\textbf{BERT4SentiSE}} & \textbf{Overall} & 19    & 30    & 8     & 18    & 11    & 10 \\
%           & \textbf{Severe} & 3     & 1     & 0     & 0     & 1     & 1 \\
%           & \textbf{Mild} & 16    & 28    & 7     & 18    & 11    & 10 \\
%           \midrule
%     \multirow{3}[0]{*}{\textbf{SentiMoji}} & \textbf{Overall} & 19    & 30    & 10    & 29    & 11    & 10 \\
%           & \textbf{Severe} & 1     & 1     & 1     & 0     & 0     & 0 \\
%           & \textbf{Mild} & 18    & 29    & 9     & 29    & 11    & 10 \\
%           \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:rq-error-analysis}%
% \end{table}%






% % \begin{table}[t]%\centering
% % \caption{Percentage of new misclassification in cross platform settings.} 
% % %[Alamin: I'll update and fix the table format later tonight. But if the table is missing information then please comment]}
% % %\scriptsize
% % \resizebox{\columnwidth}{!}{%
% % \begin{tabular}{lrr|rr|rr}\toprule
% % \multirow{3}{*}{\textbf{Tool}} &\multicolumn{6}{c}{\textbf{\% of Correct Classification that Were Misclassified from Wtinin to Cross-Platform Settings}} \\\cmidrule{2-7}
% % &\multicolumn{2}{c}{\bf{Test in GitHub}} &\multicolumn{2}{c}{\textbf{Test in SO}} &\multicolumn{2}{c}{\textbf{Test in Jira}} \\\cmidrule{2-7}
% % &\textbf{Train in SO} &\textbf{Train in Jira} &\textbf{Train in GitHub} &\textbf{Train in Jira} &\textbf{Train in GitHub} &\textbf{Train in SO} \\\midrule
% % \textbf{SentiMoji} &76 &85 &46 &69 &52 &50 \\
% % \textbf{BERT4SentiSE} &70 &79 &47 &76 &50 &46 \\
% % \bottomrule
% % \end{tabular}%
% % }
% % \label{tab:cross_platform_new_errors}%
% % \end{table}

==> SubmissionTOSEM/RQ1.tex <==
\subsection{RQ$_2$ Do the deep learning SD tools perform better than non-deep learning SD tools in cross-platform settings?}\label{sec:rq-cross-platform-performance}
\subsubsection{Motivation}\label{sec:rq-cross-platform-performance-motivation}
Our findings from RQ1 show that all the three deep learning SD tools for SE in our study (BERT4SentiSE, SentiMoji, RNN4SentiSE) 
suffer from a drop in performance in cross-platform settings. This finding is consistent with those of Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020} who 
observed a drop in performance in the shallow machine learning based SD tools (Senti4SD, SentiCR) in cross-platform settings. 
Given that the deep learning SD tools were previously found to have outperformed non-deep learning SD tools in SE in within-platform settings, 
it is thus necessary to also know whether the deep learning SD tools, despite their drop in performance in cross-platform settings, 
can still outperform non-deep learning tools in cross-platform settings.
 
% The diversity of data sources (i.e., platforms) in SE can make it challenging
% for a SE-specific SD tool trained in one platform to be equally effective in
% another platform. Studies by Novielli et
% al.~\cite{Novielli-SEToolCrossPlatform-MSR2020} find that SE shallow learning SD
% tools experience a performance drop in cross-platform settings. Recently
% developed SE deep learning SD tools offer better performance than shallow
% learning SD tools. However, the deep learning SD tools are not tested in
% cross-platform settings. A better performing deep learning SD tool both in
% within and cross-platform settings can be a better candidate for SE datasets
% across diverse platforms.

\subsubsection{Approach}\label{sec:rq-cross-platform-performance-approach} 
To compare the performance of the three deep learning SD tools against non-deep learning SD tools, we 
pick the best performing three non-deep learning SD tools from Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020} in cross-platform 
settings: Senti4SD, SentiCR, and SentiStrengthSE. Out of the non-deep learning tools, Senti4SD and SentiCR are shallow machine learning-based, and SentiStrengthSE is rule-based. We compute the performance of the two shallow learning 
SD tools in our datasets following the same process that applied for the three deep learning tools in RQ$_1$. The approach 
is described in \sec\ref{sec:rq0-approach}, which is divided into within-platform and cross-platform settings. SentiStrengthSE is rule-based, and we do not need to train it on any dataset. Therefore, we simply run it once on each dataset and compute the performance metrics. 
We use the same performance metrics introduced in \sec\ref{sec:rq0} to report the performance.      
 

% Macro average is useful to emphasize the performance on polarities with few instances (e.g., positive/negative in the Jira dataset). In contrast, 
% the micro average is influenced mainly by the performance of the majority polarity (e.g., neutral)~\cite{sebastiani2002machine}, because it takes the average of each polarity.
% The macro and micro definition here is wrong, i.e., reverted.
 
\begin{table}[]
  \footnotesize
%   \small
  \centering
  %\vspace{-.1in}
  \caption{Agreement metrics between a tool and manual labeling.}
  % \vspace{-3mm}
    % \resizebox{\columnwidth}{!}{%
    \begin{tabular}{clrrrr}
    \toprule{}
    %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
    %\cmidrule{3-6}
    \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Classifier }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
    \cmidrule{5-6}
    {Dataset} &  & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
    \midrule
\multicolumn{6}{c}{\textbf{Test dataset: GitHub}} \\
\midrule

\multirow{6}{*}{\parbox{2.5cm} {\centering GitHub \\ (Within-platform)}} 
 & SEntiMoji & 0.84 & 90\% & 1\% & 9\%  \\
 & BERT4SentiSE & 0.87 & 92\% & 1\% & 7\%  \\
 & RNN4SentiSE & 0.52 & 68\% & 7\% & 25\%  \\
 & Senti4SD & 0.86 & 91\% & 1\% & 8\%  \\
 & SentiCR & 0.73 & 83\% & 2\% & 15\%  \\
 & SentiStrengthSE & 0.67 & 79\% & 2\% & 19\%  \\
% \midrule
\cmidrule{2-6}

\multirow{6}{*}{\parbox{2.5cm} {\centering Stack Overflow \\ (Cross-platform)}}  
 & SEntiMoji & 0.61 & 75\% & 2\% & 23\%  \\
 & BERT4SentiSE & 0.65 & 78\% & 3\% & 19\%  \\
 & RNN4SentiSE & 0.47 & 66\% & 4\% & 30\%  \\
 & Senti4SD & 0.60 & 74\% & 4\% & 22\%  \\
 & SentiCR & 0.49 & 68\% & 2\% & 29\%  \\
 & SentiStrengthSE & 0.67 & 79\% & 2\% & 19\%  \\
% \midrule
\cmidrule{2-6}


\multirow{6}{*}{\parbox{2.5cm} {\centering Jira \\ (Cross-platform)}} 
 & SEntiMoji & 0.44 & 66\% & 1\% & 33\%  \\
 & BERT4SentiSE & 0.48 & 68\% & 2\% & 30\%  \\
 & RNN4SentiSE & 0.35 & 60\% & 4\% & 36\%  \\
 & Senti4SD & 0.50 & 69\% & 2\% & 28\%  \\
 & SentiCR & 0.34 & 60\% & 1\% & 39\%  \\
 & SentiStrengthSE & 0.67 & 79\% & 2\% & 19\%  \\
\midrule



\multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
\midrule

\multirow{6}{*}{\parbox{2.5cm} {\centering Stack Overflow (Within-platform)}}
 & SEntiMoji & 0.80 & 87\% & 1\% & 12\%  \\
 & BERT4SentiSE& 0.82 & 88\% & 1\% & 11\%  \\
 & RNN4SentiSE & 0.67 & 78\% & 3\% & 19\%  \\
 & Senti4SD & 0.77 & 85\% & 1\% & 14\%  \\
 & SentiCR & 0.73 & 82\% & 3\% & 15\%  \\
 & SentiStrengthSE & 0.68 & 79\% & 1\% & 20\%  \\

% \midrule
\cmidrule{2-6}

\multirow{6}{*}{\parbox{2.5cm} {\centering GitHub \\ (Cross-platform)}} 
 & SEntiMoji & 0.73 & 83\% & 1\% & 16\%  \\
 & BERT4SentiSE & 0.78 & 85\% & 1\% & 14\%  \\
 & RNN4SentiSE & 0.49 & 67\% & 4\% & 29\%  \\
 & Senti4SD & 0.67 & 78\% & 2\% & 20\%  \\
 & SentiCR & 0.56 & 71\% & 5\% & 23\%  \\
 & SentiStrengthSE & 0.68 & 79\% & 1\% & 20\%  \\
% \midrule
\cmidrule{2-6}

\multirow{6}{*}{\parbox{2.5cm} {\centering Jira \\ (Cross-platform)}} 
 & SEntiMoji & 0.48 & 67\% & 0\% & 33\%  \\
 & BERT4SentiSE & 0.63 & 76\% & 1\% & 23\%  \\
 & RNN4SentiSE & 0.34 & 58\% & 4\% & 38\%  \\
 & Senti4SD & 0.47 & 66\% & 1\% & 33\%  \\
 & SentiCR & 0.37 & 60\% & 2\% & 38\%  \\
 & SentiStrengthSE & 0.68 & 79\% & 1\% & 20\%  \\
\midrule







\multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
\midrule
\multirow{6}{*}{\parbox{2.5cm} {\centering Jira \\ (Within-platform)}}
 & SEntiMoji & 0.71 & 86\% & 0\% & 14\%  \\
 & BERT4SentiSE& 0.72 & 86\% & 0\% & 13\%  \\
 & RNN4SentiSE & 0.57 & 80\% & 1\% & 20\%  \\
 & Senti4SD & 0.59 & 81\% & 0\% & 19\%  \\
 & SentiCR & 0.69 & 85\% & 0\% & 15\%  \\
 & SentiStrengthSE & 0.67 & 83\% & 0\% & 17\%  \\
% \midrule
\cmidrule{2-6}


\multirow{6}{*}{\parbox{2.5cm} {\centering GitHub \\ (Cross-platform)}} 
 & SEntiMoji & 0.65 & 81\% & 1\% & 18\%  \\
 & BERT4SentiSE & 0.65 & 81\% & 1\% & 18\%  \\
 & RNN4SentiSE & 0.45 & 66\% & 2\% & 32\%  \\
 & Senti4SD & 0.58 & 78\% & 1\% & 21\%  \\
 & SentiCR & 0.65 & 82\% & 1\% & 17\%  \\
 & SentiStrengthSE & 0.67 & 83\% & 0\% & 17\%  \\
% \midrule
\cmidrule{2-6}

\multirow{6}{*}{\parbox{2.5cm} {\centering Stack Overflow \\ (Cross-platform)}} 
 & SEntiMoji & 0.65 & 82\% & 1\% & 18\%  \\
 & BERT4SentiSE & 0.66 & 82\% & 1\% & 17\%  \\
 & RNN4SentiSE & 0.57 & 77\% & 1\% & 22\%  \\
 & Senti4SD & 0.46 & 74\% & 1\% & 25\%  \\
 & SentiCR & 0.34 & 73\% & 1\% & 26\%  \\
 & SentiStrengthSE & 0.67 & 83\% & 0\% & 17\%  \\
% \midrule
    % \midrule  
    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:agreement_with_manual_labelling}%
\end{table}%

\subsubsection{Results}\label{sec:rq-cross-platform-performance-results} 
In \tbl\ref{tab:cross_platform_performance}, we show the performance of the two shallow learning SD tools (Senti4SD, SentiCR) and the rule-based tool SentiStrengthSE in the 
last three columns. In \tbl\ref{tab:cross_platform_performance_drop}, the last two columns show the percentage drop in performance of the shallow ML-based tools 
in cross-platform settings compared to their within platform settings.  As SentiStrengthSE does not need to be retrained, it does not have any performance drop in cross-platform settings and thus skipped in \tbl\ref{tab:cross_platform_performance_drop}.

\bf{Across all the SD tools for SE in our study, SentiStrengthSE is the best performer in five out of the six cross-platform settings, while BERT4SentiSE is the best performer in one cross-platform setting.} While BERT4SentiSE \it{considerably} outperforms SentiStrengthSE within platform settings, 
SentiStrengthSE \it{marginally} outperforms BERT4SentiSE in five out of the six cross-platform settings. SentiStrengthSE has a Macro F1-score of 0.78 
compared to 0.77 of BERT4SentiSE, when BERT4SentiSE is trained in SO and then tested in GitHub (F1-score difference = 0.01). Overall, the difference in Macro F1 scores 
between  SentiStrengthSE and BERT4SentiSE across the five cross-platform settings where SentiStrengthSE outperforms BERT4SentiSE is between 0.01 - 0.02 except when BERT4SentiSE 
is trained in Jira and tested on GitHub (Macro F1 difference is 0.13). 
The one cross-platform setting where BERT4SentiSE outperforms 
SentiStrengthSE is when it is trained in GitHub and tested in SO, where the difference in Macro F1-score is 0.06. Therefore, the difference in performance 
between SentiStrengthSE and BERT4SentiSE in cross-platform settings is at most 0.06 except when BERT4SentiSE is trained in a dataset other than Jira. Therefore, the performance of 
a supervised tool like BERT4SentiSE and whether it can outperform 
a rule-based tool like SentiStrengthSE in cross-platform settings can depend on the type of training dataset. 
    


\bf{Between the shallow learning and deep learning SD tools for SE, BERT4SentiSE is the best performer in five out of six cross-platform settings, while Senti4SD 
is the best performer in one cross-platform setting.} The difference in Macro F1-score between BERT4SentiSE and Senti4SD 
is between 0.04 - 0.16 across the five cross-platform settings where BERT4SentiSE outperforms Senti4SD. Senti4SD outperforms BERT4SentiSE in one cross-platform setting (Macro F1 score of 0.67 vs. 0.65, i.e., difference = 0.02) 
when the tools were trained in Jira and tested in GitHub. BERT4SentiSE also outperforms Senti4SD in all three within platform settings. BERT4SentiSE 
also outperforms other tools across the three within platform settings. The findings confirm that similar to other domains for text classification, in SE also transformer pre-trained tools like BERT4SentiSE are superior to other supervised SD tools. BERT4SentiSE is also slightly inferior to rule-based tool SentiStrengthSE and thus could be a sensible choice both for within and cross-platform settings.    

\bf{RNN4SentiSE exhibits most severe and mild errors among the supervised SD tools for within and cross-platform settings.} In \tbl\ref{tab:agreement_with_manual_labelling}, 
we show how each of the five supervised SD tools in our study agrees with the manual labels during within and cross-platform settings. We also report the agreement of rule-based SentiStrengthSE and manual labels, but as it does not require re-training, its cross-platform agreement does not change. We compute the agreement using two metrics: Cohen $\kappa$~\cite{cohen1968weighted} and percent agreement. We compute the disagreement between a tool's prediction and manual label as severe (when a sentence with a manual label as positive is predicted as negative and vice-versa) and mild (when a sentence with a neutral label is predicted as non-neutral and vice-versa). Among the SD tools, the two-deep learning SD 
tools (BERT4SentiSE and SentiMoji) show the least amount of severe and mild disagreements with the manual labels. 
In \tbl\ref{tab:agreement_with_manual_labelling}, we show the agreements and disagreements for within and cross-platform settings. Overall, 
for any given test dataset, the amount of severe and mild disagreements increase for a tool from within to cross-platform settings. However, 
similar to RQ1, where we noted that BERT4SentiSE and SentiMoji suffer mainly from mild errors in cross-platform settings, all the supervised SD tools (except RNN4SentiSE) 
show similar pattern with manual label in \tbl\ref{tab:agreement_with_manual_labelling}. Thus the supervised SD tools can benefit 
more from fixing the mild errors during classification in cross-platform settings.    

\textbf{The two best performing deep learning SD tools (BERT4SentiSE and SentiMoji) have the lowest severe disagreement with manual
annotation among the supervised SD tools.} In Table \ref{tab:agreement_with_manual_labelling}, we report the
paired comparisons with the tools' predictions with manual labeling. In
cross-platform settings, when it is trained on Stack Overflow dataset and tested
on GitHub dataset, both BERT4SentiSE and SentiMoji has the highest severe
disagreement (3\% and 2\% respectively) as well as the highest mild disagreement (30\% and 33\%
respectively) with manual labeling. 
% After further digging, we find these
% disagreements are in line with our error analysis in RQ3.
We find that most of
the severe disagreements (61\%) are because of subjectivity in annotation  or
examples lacking proper context. For example, a sample in the GitHub dataset
(e.g., ``It's quite a bad practice to do so :)'')  both Bert4SentiSE and
SentiMoji was able to understand the underlying context of this sentence correctly, i.e., the `:)' emoji did not confuse the DL tools and both of them
predicted negative sentiment for this sample. However, for the particular
example, the oracle is `positive', i.e., the human annotator probably had some more
context which prompted the annotator to annotate this, or this is because of
subjectivity among annotators (subjectivity in annotation is discussed further under RQ$_4$).

% 
% 
% Table (\ref{tab:cross_platform_performance_github}, \ref{tab:cross_platform_performance_so}, \ref{tab:cross_platform_performance_jira}) reports the performance of the six SD tools in within and 
% cross-platform settings in GitHub, Stack Overflow and Jira dataset respectively. For each setting and dataset, we highlight the best results in bold. We also report the drop of performance in cross platform settings with respect to with-in platform settings.
% 
% \textbf{PTM DL-based tools performs well in within-platform settings and shows less drop in performance in cross platform settings.} The deep learning tool BERT4SentiSE is the best performer in within platform setting across the three datasets. This observation is consistent with Biswas et al.~\cite{Biswas-ReliableSentiSEBERT-ICSME2020}, who developed the tool.  The second-best performer across the datasets is another deep learning tool SentiMoji. Similar to previous studies~\cite{Novielli-SEToolCrossPlatform-MSR2020}, we notice a drop in performance in all the supervised SD tools in cross-platform settings compared to within platform settings. The drop in performance is lower in the two pre-trained Deep learning tools (SEntiMoji and BERT4SentiSE) than the other supervised SD tools. This means that these two tools are more reliable than the shallow learning SD tools in SE datasets across within and cross-platform settings. 
% 
% \textbf{In cross-platform settings lexicon-based SentiStrengthSE is the best SD tools and PTM DL-based BERT4SentiSE is in close second position.} Similar to Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}, lexicon-based rule-based SD tool SentiStrengthSE outperforms the shallow learning SD tools in cross-platform settings. However, BERT4SentiSE  manages to outperform SentiStrengthSE in one out of six cross-platform cases. Here, a case denotes a cross-platform setting with a dataset. For example,  when we train a tool using the GitHub dataset and then test it on SO and Jira datasets, we have two cases, one for SO and Jira. BERT4SentiSE is the best performer in cross-platform settings in one case: when it is trained on GitHub and tested on SO. For the other five cases, SentiStrengthSE is the best performer. In the five cases, BERT4SentiSE is the close second-based performer for four cases: \begin{inparaenum}
%  \item SO (Train) to GitHub (Test): 0.78 Macro F1 for SentiStrengthSE vs 0.77 Macro F1 for BERT4SentiSE.
%  \item Jira (Train) to SO (Test): 0.79 for SentiStrengthSE vs 0.76 for BERT4SentiSE.
%  \item GitHub (Train) Jira (Test): 0.79 for SentiStrengthSE vs 0.77 for BERT4SentiSE.
%  \item SO (Train) Jira (Test): 0.79 for SentiStrengthSE vs 0.78 for BERT4SentiSE.
% \end{inparaenum} In the other case, Senti4SD is the second-best performer: 
% Jira (Test) GitHub (Train): 0.78 Macro F1 for SentiStrengthSE vs 0.67 for Senti4SD vs 0.65 for BERT4SentiSE. 
% Therefore, while BERT4SentiSE is the second-best performer to SentiStrengthSE in the above cases, the differences in Macro F1-score are very low (0.01-0.03 in four cases and 0.13 in one case). However, BERT4SentiSE outperforms SentiStrengthSE in within platform settings by much larger margins across the three datasets: \begin{inparaenum}
%  \item GitHub: 0.92 Macro F1-score for BERT4SentiSE vs 0.78 for SentiStrengthSE, 
%  \item SO: 0.88 for BERT4SentiSE vs 0.79 for SentiStrengthSE, 
%  \item Jira: 0.83 for BERT4SentiSE vs 0.79 for SentiStrengthSE.
% \end{inparaenum} While the two deep learning tools (BERT4SentiSE and SentiMoji) are pre-trained on large datasets, RNN4SentiSE is not pre-trained. As such, the poor performance of RNN4SentiSE suggests that without pre-training, the deep learning tools do not perform well in both settings.
% We also notice the highest performance drop (37\%) is for SentiCR it trained on Jira and tested on Stack Overflow. The Jira dataset is more imbalanced than the other two datasets, with fewer non-neutral polarity cases. As such, tools like SentiCR do not have an embedding like SO-based Word2Vec in Senti4SD suffer more drop in performance in cross-platform settings.

% and SentiMoji's by 23\% (Micro F1 from 0.87 to 0.67). When trained on Jira and tested on GitHub SentiCR's performance drop by around 27\% (Micro F1 from 0.83 to 0.60) and SentiMoji's by 26\% (Micro F1 from 0.90 to 0.66). When trained on Jira and tested on GitHub, the Senti4SD performs best with Micro F1 = 0.69 and Macro F1 = 0.69. Jira dataset is very imbalanced, i.e., around 70\% of its samples belong to the neutral class. So, Macro-avg metrics makes more sense when it is tested on the Jira dataset. When it is trained on GitHub or Stack Overflow and tested on the Jira dataset, the BERT4SEntiSE provides the best Macro-F1 score of 0.77 and 0.78, respectively. As Jira dataset is quite unbalanced, its no surprise that there is big drop in performance when these machine learning classifiers are trained on Jira dataset. For negative polarity classed SentiCR's performance drop by more than 50\% then it is trained in Jira dataset. When trained on Jira dataset the SentiCR classifier has the lowest micro F1 score (0.6 for GitHub and Stack Overflow test dataset). SentiCR uses fixed uni and bi-grams and this result shows that the tool is failing to generalize and over-fitting.




% perform slightly better than shallow ML-based tools. BERT4SentiSE provides the best performance in all cross-platform experiments. Exception is when tested on GitHub and trained on Jira the Senti4SD provides the best result (Micro F1 = 0.69). RNN4SentiSE is a general RNN based classifier that is trained on the SE dataset from ground up. The poor performance of the RNN4SentiSE suggests that DL-based classifiers do not generalize well on small datasets without pre-training on large NLP datasets.



% The other deep learning tool RNN4SentiSE is, however, the worst performer among the tools in  

% RNN4SentiSE is used as a for DL-based baseline for the other two DL-based pre-trained classifiers. It also shows the performance of each polarity class and overall performance. We highlight the best result for each metric in bold. We also report the performance of these tools within platform settings to provide a comparison of performance degradation in cross-platform settings. 
% We use k-fold stratified cross-validation settings. We present the agreement of these tools with manual labelingin terms of weighted Cohen $K$ and the percentage of cases where the tools perfectly agree with each other as well as severe and mild disagreement in Table \ref{tab:agreement}.


 

% In cross-platform settings, when trained on Stack Overflow and tested on GitHub dataset, BERT4SentiSE provides the best result with Micro F1 = 0.78 and Macro F1 = 0.77. RNN4SEntiSE performs worst with Micro F1=0.66 and Macro F1=0.65. 






\begin{tcolorbox}[flushleft upper,boxrule=1pt,arc=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=white,after=\ignorespacesafterend\par\noindent]
\bf{RQ$_2$ Do the deep learning SD tools perform better than non-deep learning SD tools in cross-platform settings?}
Across all the SD tools for SE in our study, SentiStrengthSE is the best performer with narrow margin with BERT4SentiSE in five out of the six cross-platform settings and BERT4SentiSE is the 
best performer in the other cross-platform setting in our three studied datasets. Between the shallow learning and deep learning SD tools for SE, 
BERT4SentiSE is the best performer in five out of six cross-platform settings, while Senti4SD 
is the best performer in one cross-platform setting.
\end{tcolorbox}









%  In within-platform settings, we divided each datast into 10-folds using Scikit StratifiedKFold technique. 
%  We then run each 
%  As mention in Table \ref{tab:agreement_with_manual_labelling}, the datasets have a class imbalance, especially the Jira dataset. So we use the stratified sampling with Scikit-learn\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.model_selection.StratifiedKFold.html}} to ensure each fold contains the same proportion of polarity classes as the original dataset. We train and test each classifier 10 times for each dataset. For example, first we train a classifier on folds 1 through 9 and then test on the samples of fold 0. Once the training and testing for 10 folds are completed we merge the results and calculate the overall performance of the classifier on that dataset.

% In cross platform settings, we train each classifier on one benchmark dataset (e.g., Stack Overflow) and test it on the other two benchmark datasets (e.g., GitHub and Jira). In this way, in cross-platform settings each tools makes two predictions for every sample unit in each dataset.
% % Our final 10-folded cross-validated dataset and code is publicly available in our replication package.

% Furthermore, following similar studies\cite{Novielli-SEToolCrossPlatform-MSR2020, jongeling2017negative}, we present the agreement of these tools with manual labelingin terms of weighted Cohen $K$ and the percentage of cases where the tools perfectly agree with each other as well as have severe or mild disagreement. Severe disagreement occurs when a classifier's prediction and the manual labelingis of opposite polarity classes. Mild disagreement happens when the tool predicts positive and negative polarity and manual labelingis neutral and vice versa.

==> SubmissionTOSEM/RQ1_tables.tex <==





% % \begin{sidewaystable}
% % \vspace{15cm}
% \begin{table*}%[t]
% \footnotesize
% % \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Performance of SE-specific sentiment analysis in cross-platform settings (SentiSE = SentistrengthSE)}
%   %\vspace{-3mm}
%   % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{ll|rrr|rrr|rrr|rrr|rrr}
%     \toprule{}

%     \multirow{2}{*}{\textbf{Setting}}  & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiSE}}\\
%     \cmidrule{3-17}
%     {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
    
%     %\multicolumn{18}{c}{\textbf{Test dataset: GitHub}} \\
%     %\midrule
 
%      \multirow{5}{1.4cm}{Test:  GitHub Train: GitHub  (Within)}
%      & Negative &  .89 & .85 & .87  & .89 & .91 & .90  & .90 & .89 & .90  & .87 & .69 & .77  & .81 & .71 & .76   \\ 
%      & Neutral &   .87 & .92 & .89  & .92 & .90 & .91   & .89 & .92 & .91  & .77 & .91 & .84  & .74 & .86 & .79   \\ 
%      & Positive &  .94 & .92 & .93  & .93 & .94 & .94   & .94 & .91 & .93  & .89 & .84 & .86  & .85 & .76 & .80   \\ 
%      & Micro-avg &  .90 & .90 & .90  & \textbf{.92} & \textbf{.92} & \textbf{.92}   & .91 & .91 & .91  & .83 & .83 & .83  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .90 & .89 & .90  & \textbf{.91} & \textbf{.92} & \textbf{.92}   & \textbf{.91} & .91 & .91  & .84 & .81 & .82  & .80 & .78 & .78   \\ 

%     \cmidrule{2-17}     

%      % Test dataset: Github
% \multirow{5}{1.4cm}{Test:  GitHub Train: SO  (Cross)}
%  & Negative &  .85 & .62 & .72  & .83 & .73 & .78      & .79 & .56 & .66  & .83 & .37 & .51  & .81 & .71 & .76   \\ 
%  & Neutral &   .67 & .91 & .77  & .71 & .91 & .80      & .71 & .82 & .76  & .60 & .94 & .73  & .74 & .86 & .79   \\ 
%  & Positive &  .88 & .65 & .75  & .88 & .63 & .73   & .76 & .81 & .78  & .86 & .62 & .72  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .75 & .75 & .75  & .78 & .78 & .78   & .74 & .74 & .74  & .68 & .68 & .68  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  .80 & .73 & .75  & \textbf{.81} & .76 & .77   & .75 & .73 & .73  & .76 & .64 & .66  & .80 & \textbf{.78} & \textbf{.78}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.15 & -.15 & -.15 & -.14 & -.14 & -.14 & -.02 & -.02 & -.02 & -.17 & -.17 & -.17 & -.14 & -.14 & -.14  \\ 
% % & & Macro-avg &  -.10 & -.17 & -.15 & -.11 & -.16 & -.15 & .01 & -.05 & -.04 & -.16 & -.18 & -.18 & -.08 & -.17 & -.17  \\ 
% \cmidrule{2-17}
    
    
    
%     % Test dataset: Github
%     \multirow{5}{1.4cm}{Test: GitHub Train: Jira  (Cross)} 
%      & Negative &  .91 & .39 & .55  & .90 & .43 & .58      & .85 & .52 & .64  & .88 & .27 & .41  & .81 & .71 & .76   \\ 
%  & Neutral &       .56 & .98 & .72  & .59 & .97 & .73    & .60 & .96 & .74  & .52 & .98 & .68  & .74 & .86 & .79   \\ 
%  & Positive &      .94 & .45 & .60  & .91 & .51 & .65   & .90 & .46 & .61  & .89 & .38 & .53  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .66 & .66 & .66  & .68 & .68 & .68    & .69 & .69 & .69  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  \textbf{.80} & .61 & .62  & \textbf{.80} & .64 & .65    & .78 & .65 & .67  & .76 & .54 & .54  & \textbf{.80} & \textbf{.78} & \textbf{.78}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.24 & -.24 & -.24 & -.23 & -.23 & -.23 & -.08 & -.08 & -.08 & -.22 & -.22 & -.22 & -.23 & -.23 & -.23  \\ 
% % & & Macro-avg &  -.10 & -.29 & -.28 & -.12 & -.28 & -.26 & .02 & -.14 & -.14 & -.13 & -.26 & -.24 & -.08 & -.27 & -.28  \\ 

% \midrule





% %    \multicolumn{18}{c}{\textbf{Test dataset: Stack Overflow}} \\
% %    \midrule
%     \multirow{5}{1.4cm}{Test: SO Train: SO  (Within)} 
%  & Negative &  .84 & .83 & .83  & .86 & .85 & .85    & .80 & .83 & .82  & .80 & .72 & .76  & .76 & .76 & .76   \\ 
%  & Neutral &  .83 & .84 & .84  & .86 & .85 & .85    & .84 & .79 & .81  & .79 & .82 & .81  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .93 & .93  & .93 & .94 & .93    & .90 & .93 & .91  & .88 & .91 & .89  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}    & .85 & .85 & .85  & .82 & .82 & .82  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}    & .85 & .85 & .85  & .82 & .82 & .82  & .80 & .79 & .79   \\ 
 

%     \cmidrule{2-17}
    
%     % Test dataset: Stack Overflow
%     \multirow{5}{1.4cm}{Test: SO Train: GitHub  (Cross)} 
%  & Negative &  .82 & .76 & .79  & .80 & .86 & .83       & .69 & .76 & .72  & .64 & .49 & .55  & .76 & .76 & .76   \\ 
%  & Neutral &   .75 & .85 & .80  & .84 & .80 & .82    & .73 & .76 & .75  & .65 & .85 & .74  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .85 & .89  & .93 & .91 & .92    & .92 & .82 & .87  & .88 & .74 & .80  & .91 & .82 & .86   \\ 
%  & Micro-avg & .83 & .83 & .83  & \textbf{.85} & \textbf{.85} & \textbf{.85}    & .78 & .78 & .78  & .71 & .71 & .71  & .79 & .79 & .79   \\ 
%  & Macro-avg & .83 & .82 & .82  & \textbf{.85} & \textbf{.86} & \textbf{.85}    & .78 & .78 & .78  & .72 & .69 & .70  & .80 & .79 & .79   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.12 & -.12 & -.12 & -.07 & -.07 & -.07 & -.11 & -.11 & -.11  \\ 
% % & & Macro-avg &  -.03 & -.05 & -.04 & -.03 & -.02 & -.03 & -.11 & -.12 & -.12 & -.06 & -.07 & -.07 & -.10 & -.12 & -.12  \\ 

%     \cmidrule{2-17}


%     % Test dataset: Stack Overflow
%     \multirow{5}{1.4cm}{Test: SO Train: Jira  (Cross)}
%  & Negative &  .93 & .31 & .47  & .88 & .55 & .68      & .75 & .30 & .43  & .67 & .22 & .33  & .76 & .76 & .76   \\ 
%  & Neutral &   .54 & .98 & .70  & .63 & .94 & .76    & .54 & .93 & .69  & .50 & .95 & .66  & .73 & .79 & .75   \\ 
%  & Positive &  .98 & .62 & .76  & .97 & .74 & .84    & .96 & .64 & .76  & .96 & .52 & .67  & .91 & .82 & .86   \\ 
%  & Micro-avg & .67 & .67 & .67  & .76 & .76 & .76    & .66 & .66 & .66  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg & .82 & .64 & .64  & \textbf{.83} & .74 & .76   & .75 & .62 & .63  & .71 & .56 & .55  & .80 & \textbf{.79} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.20 & -.20 & -.20 & -.12 & -.12 & -.12 & -.21 & -.21 & -.21 & -.19 & -.19 & -.19 & -.22 & -.22 & -.22  \\ 
% % & & Macro-avg &  -.05 & -.23 & -.23 & -.05 & -.14 & -.12 & -.12 & -.23 & -.24 & -.10 & -.23 & -.22 & -.11 & -.25 & -.27  \\ 

%     \midrule





%     % Test dataset: Jira
% %    \multicolumn{18}{c}{\textbf{Test dataset: Jira}} \\
% %    \midrule
%     \multirow{5}{1.4cm}{Test: Jira Train: Jira  (Within)} 
%  & Negative &  .84 & .68 & .75  & .82 & .76 & .79      & .71 & .55 & .62  & .79 & .66 & .72  & .68 & .73 & .71   \\ 
%  & Neutral &   .89 & .91 & .90  & .90 & .90 & .90     & .84 & .88 & .86  & .89 & .89 & .89  & .92 & .82 & .87   \\ 
%  & Positive &  .79 & .80 & .79  & .78 & .80 & .79    & .73 & .71 & .72  & .75 & .85 & .80  & .68 & .92 & .78   \\ 
%  & Micro-avg &  \textbf{.86} & \textbf{.86} & \textbf{.86}  & \textbf{.86} & \textbf{.86} & \textbf{.86}    & .81 & .81 & .81  & .85 & .85 & .85  & .83 & .83 & .83   \\ 
%  & Macro-avg &  \textbf{.84} & .80 & .81  & .83 & \textbf{.82} & \textbf{.83}   & .76 & .72 & .73  & .81 & .80 & .80  & .76 & \textbf{.82} & .79   \\ 

%     \cmidrule{2-17}
    
    
%     % Test dataset: Jira
%     \multirow{5}{1.4cm}{Test: Jira Train: GitHub (Cross)} 
%  & Negative &  .63 & .75 & .69  & .66 & .74 & .70     & .61 & .64 & .62  & .69 & .60 & .64  & .68 & .73 & .71   \\ 
%  & Neutral &   .93 & .79 & .85  & .93 & .80 & .86    & .89 & .78 & .83  & .90 & .85 & .87  & .92 & .82 & .87   \\ 
%  & Positive &  .66 & .91 & .77  & .65 & .91 & .76    & .62 & .86 & .72  & .69 & .89 & .78  & .68 & .92 & .78   \\ 
%  & Micro-avg & .81 & .81 & .81  & .81 & .81 & .81    & .78 & .78 & .78  & .82 & .82 & .82  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg & .74 & \textbf{.82} & .77  & .75 & \textbf{.82} & .77    & .71 & .76 & .73  & \textbf{.76}& .78 & .76  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.05 & -.05 & -.05 & -.05 & -.05 & -.05 & -.14 & -.14 & -.14 & -.03 & -.03 & -.03 & -.03 & -.03 & -.03  \\ 
% % & & Macro-avg &  -.09 & .02 & -.04 & -.09 & -.00 & -.05 & -.12 & .05 & -.07 & -.05 & .05 & -.01 & -.05 & -.02 & -.04  \\ 

%     \cmidrule{2-17}
    
    
%     % Test dataset: Jira
%     \multirow{5}{1.4cm}{Test: Jira Train: SO (Cross)}
%  & Negative &  .67 & .68 & .67  & .72 & .68 & .70       & .50 & .29 & .37  & .36 & .06 & .10  & .68 & .73 & .71   \\ 
%  & Neutral &   .92 & .81 & .86  & .92 & .82 & .87    & .82 & .81 & .81  & .75 & .94 & .83  & .92 & .82 & .87   \\ 
%  & Positive &  .67 & .93 & .78  & .65 & .93 & .76    & .59 & .80 & .68  & .71 & .49 & .58  & .68 & .92 & .78   \\ 
%  & Micro-avg & .82 & .82 & .82  & .82 & .82 & .82    & .74 & .74 & .74  & .73 & .73 & .73  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg & .75 & .81 & .77  & \textbf{.76} & .81 & .78    & .64 & .63 & .62  & .61 & .49 & .50  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.07 & -.07 & -.07 & -.12 & -.12 & -.12  \\ 
% % & & Macro-avg &  -.08 & .01 & -.04 & -.07 & -.01 & -.05 & -.05 & .06 & .00 & -.12 & -.08 & -.11 & -.20 & -.30 & -.30  \\ 


%     \bottomrule
%     \end{tabular}%
% %}
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance}%
% \end{table*}%
% % \end{sidewaystable}





% % \begin{sidewaystable}
% % \vspace{15cm}
% \begin{table*}%[t]
% \footnotesize
% % \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Performance drop in SE-specific supervised sentiment analysis tools in cross-platform settings (SO = Stack Overflow)}
%   %\vspace{-3mm}
%   % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{cl|rrr|rrr|rrr|rrr}
%     \toprule{}

%     \multirow{2}{*}{\textbf{Train}} & \multirow{2}{*}{\textbf{Performance}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} &  \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} \\
%     \cmidrule{3-14}
%     \textbf{Dataset} & \centering \textbf{Drop} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
    
%     \multicolumn{14}{c}{\textbf{Test dataset: GitHub}} \\
%     \midrule
 
%     \multirow{2}{*}{\textbf{SO}} & $\triangledown$ Micro-avg &  -16\% & -16\% & -16\% & -15\% & -15\% & -15\%  & -18\% & -18\% & -18\% & -17\% & -17\% & -17\%    \\ 
%     &  $\triangledown$ Macro-avg &  -11\% & -19\% & -17\% & -12\% & -18\% & -16\% &  -17\% & -20\% & -19\% & -10\% & -21\% & -20\%  \\ 
%     \cmidrule{2-14}
    
%     \multirow{2}{*}{\textbf{Jira}} &  $\triangledown$ Micro-avg &  -27\% & -27\% & -27\% & -26\% & -26\% & -26\%  & -24\% & -24\% & -24\% & -27\% & -27\% & -27\%   \\ 
%     &  $\triangledown$ Macro-avg &  -11\% & -32\% & -31\% & -13\% & -31\% & -29\% &  -14\% & -29\% & -27\% & -9\% & -34\% & -34\%  \\ 
%     % \cmidrule{2-17}
%     \midrule
    
    
%     \multicolumn{14}{c}{\textbf{Test dataset: Stack Overflow}} \\
%     \midrule
%     \multirow{2}{*}{\textbf{GitHub}} & $\triangledown$  Micro-avg &  -5\% & -5\% & -5\% & -3\% & -3\% & -3\% &  -8\% & -8\% & -8\% & -13\% & -13\% & -13\%   \\ 
%     & $\triangledown$  Macro-avg &  -4\% & -5\% & -5\% & -3\% & -3\% & -3\%  & -7\% & -8\% & -8\% & -12\% & -15\% & -15\%  \\ 
%     \cmidrule{2-14}
%     \multirow{2}{*}{\textbf{Jira}} &  $\triangledown$ Micro-avg &  -23\% & -23\% & -23\% & -13\% & -13\% & -13\%  & -22\% & -22\% & -22\% & -27\% & -27\% & -27\%   \\ 
%     &  $\triangledown$ Macro-avg &  -6\% & -27\% & -26\% & -6\% & -16\% & -14\%  & -11\% & -27\% & -26\% & -14\% & -31\% & -33\%  \\ 
%     % \cmidrule{2-17}
%     \midrule
    
%     \multicolumn{14}{c}{\textbf{Test dataset: Jira}} \\
%     \midrule
%     \multirow{2}{*}{\textbf{GitHub}} &  $\triangledown$ Micro-avg &  -6\% & -6\% & -6\% & -6\% & -6\% & -6\% &  -4\% & -4\% & -4\% & -3\% & -3\% & -3\%    \\ 
%     &  $\triangledown$ Macro-avg &  -11\% & 3\% & -5\% & -10\% & 0\% & -7\% &  -7\% & 7\% & -1\% & -6\% & -2\% & -5\%  \\ 
%     \cmidrule{2-14}
%     \multirow{2}{*}{\textbf{SO}} & $\triangledown$  Micro-avg &  -5\% & -5\% & -5\% & -5\% & -5\% & -5\%  & -9\% & -9\% & -9\% & -14\% & -14\% & -14\%   \\ 
%     &  $\triangledown$ Macro-avg &  -10\% & 1\% & -5\% & -8\% & -1\% & -6\%  & -16\% & -12\% & -15\% & -25\% & -38\% & -37\%  \\ 
%     % \cmidrule{2-17}
%     \midrule



%     \bottomrule
%     \end{tabular}%
% %}
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance_drop}%
% \end{table*}%
% % \end{sidewaystable}





% \begin{figure*}[t]
% \centering
% \captionsetup[subfigure]{labelformat=empty}
% \pgfplotstableread{

% 1	.88  .97 .75 .77     .88  .97  .82 .85      .87  .96  .77 .77
% 2	.87  .96 .62 .65     .85  .93  .64 .76      .85  .93  .77 .78
% }\datatable
%       \subfloat[Test on GitHub]
%       {
%       \resizebox{1.5in}{!}{%
%       \begin{tikzpicture}
%         	\begin{axis}[
%         	%ylabel=label,
%         	xtick=data,
%         	xticklabels={Trained on SO, Trained on Jira},
%         	enlarge y limits=false,
%         	enlarge x limits=0.55,
%         % 	axis y line = none,
%         % 	axis y line=left,
%         %   axis line style={-},
%             axis y line=none,
%             % hide y axis,
%             axis x line*=bottom,
%             axis y line*=left,
%         % 	axis x line=left,
%         % 	axis x line=bottom,
%         % 	axis line style={draw=none},
%         %	nodes near coords,
%         	ymin=0,ymax=1,
%         	ybar,
%         	bar width=0.7cm,
%         	width=3.6in,
%         	height = 2.3in,
%         % 	ytick={0,20,...,80},
%             % yticklabels={0\%,20\%,40\%,60\%,80\%},
%         	%ylabel={Accepted Answer (\%)},
%         	ymajorgrids=false,
%         %	xminorgrids=true,
%          	yticklabel style={font=\LARGE},
%         	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
%         	major x tick style = {opacity=0},
%         	minor x tick num = 1,    
%         	minor tick length=1ex,
%         	legend columns=2, 
%             legend style={
%                 /tikz/column 2/.style={
%                     column sep=5pt,
%                 },
%                 },
%         	legend style={at={(0.5,1.40)},
%         	legend style={font=\LARGE},
%             anchor=north,legend columns=-1
%             },
%             % nodes near coords,
%             nodes near coords style={font=\huge},
%             nodes near coords style={rotate=90,  anchor=west}, %
%         	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
%         	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
%         	]
%         	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=1] \datatable;
%         	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=2] \datatable;
%         	\addplot[draw=black!80, fill=black!70] table[x index=0,y index=3] \datatable;
%         	\addplot[draw=black!80, fill=black!100] table[x index=0,y index=4] \datatable;
        
%             \legend{JS Divergence,
%             		 Cosine Similarity,
%             		 }
%         	\end{axis}
%     	\end{tikzpicture}
%      	}
%     %  	\hspace{-1mm}
%     	\label{presentation-inconsistency}
%     } 
%     \subfloat[Test on Stack Overflow (SO)]
%      {
%       \resizebox{1.5in}{!}{%
%       \begin{tikzpicture}
%         	\begin{axis}[
%         	%ylabel=label,
%         	xtick=data,
%         	xticklabels={Train on GitHub, Train on Jira},
%         	enlarge y limits=false,
%         	enlarge x limits=0.55,
%         % 	axis y line = none,
%         % 	axis y line=left,
%         %   axis line style={-},
%             axis y line=none,
%             % hide y axis,
%             axis x line*=bottom,
%             axis y line*=left,
%         % 	axis x line=left,
%         % 	axis x line=bottom,
%         % 	axis line style={draw=none},
%         %	nodes near coords,
%         	ymin=0,ymax=1,
%         	ybar,
%         	bar width=0.7cm,
%         	width=3.6in,
%         	height = 2.3in,
%         % 	ytick={0,20,...,80},
%             % yticklabels={0\%,20\%,40\%,60\%,80\%},
%         	%ylabel={Accepted Answer (\%)},
%         	ymajorgrids=false,
%         %	xminorgrids=true,
%          	yticklabel style={font=\LARGE},
%          	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
%         	major x tick style = {opacity=0},
%         	minor x tick num = 1,    
%         	minor tick length=1ex,
%         	legend columns=2, 
%             legend style={
%                 /tikz/column 2/.style={
%                     column sep=5pt,
%                 },
%                 },
%         	legend style={at={(0.5,1.40)},
%         	legend style={font=\LARGE},
%             anchor=north,legend columns=-1
%             },
%             nodes near coords style={font=\huge},
%             nodes near coords style={rotate=90,  anchor=west}, %
%         	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
%         	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
%         	]
%         	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=5] \datatable; 
%         	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=6] \datatable; %, postaction={pattern=horizontal lines}
%         	\addplot[draw=black!80, fill=black!60] table[x index=0,y index=7] \datatable;   %, postaction={pattern=vertical lines}
%             \addplot[draw=black!80, fill=black!100] table[x index=0,y index=8] \datatable;  %, postaction={pattern=vertical lines}
%             \legend{,,
%             		 SEntiMoji F1,
%             		 BERT4SentiSE F1
%             		 }
%             % \legend{JS Divergence,
%             % 		 Cosine Similarity,
%             % 		 SEntiMoji F1,
%             % 		 BERT4SentiSE F1
%             % 		 }
%         	\end{axis}
%     	\end{tikzpicture}
%     	}
%     % 	\hspace{-1mm}
%     	\label{signature-inconsistency}
%     }
%     \subfloat[Test on Jira]
%      {
%       \resizebox{1.5in}{!}{%
%       \begin{tikzpicture}
%         	\begin{axis}[
%         	%ylabel=label,
%         	xtick=data,
%         	xticklabels={Train on GitHub, Train on SO
%         	},
%         	enlarge y limits=false,
%         	enlarge x limits=0.55,
%             axis y line=none,
%             % hide y axis,
%             axis x line*=bottom,
%             axis y line*=left,,
%         	ymin=0,ymax=1.08,
%         	ybar,
%         	bar width=0.7cm,
%         	width=3.4in,
%         	height = 2.3in,
%         % 	ytick={0,20,...,80},
%         %     yticklabels={0\%,20\%,40\%,60\%,80\%},
%         	%ylabel={Accepted Answer (\%)},
%         	ymajorgrids=false,
%         %	xminorgrids=true,
%          	yticklabel style={font=\LARGE},
%          	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
%         	major x tick style = {opacity=0},
%         	minor x tick num = 1,    
%         	minor tick length=1ex,
%         	legend style={
%          	at={(0.6,0.98)},
%             anchor=north,legend columns=-1
%             },
%             nodes near coords style={font=\huge},
%             nodes near coords style={rotate=90,  anchor=west}, %
%         	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
%         	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
%         	]
%         	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=9] \datatable;
%         	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=10] \datatable; %, postaction={pattern=horizontal lines}
%         	\addplot[draw=black!80, fill=black!60] table[x index=0,y index=11] \datatable; %, postaction={pattern=vertical lines}
%             \addplot[draw=black!80, fill=black!100] table[x index=0,y index=12] \datatable; %, postaction={pattern=vertical lines}

%         	\end{axis}
%     	\end{tikzpicture}
%     	}
%     % 	%\hspace{-1mm}
%     	\label{fig:status-inconsistency}
%     }
    


    
    
% %\vspace{-3mm}
% \caption{Similarity scores between datasets vs Macro F1-scores per tool (BERT4SentiSE \& SentiMoji) in cross platform settings}


% \vspace{-3mm}
% \label{fig:diversity_performance}
% \end{figure*}







% \begin{sidewaystable}
% \vspace{15cm}
% % \begin{table}
% \renewcommand{\thetable}{\arabic{table}a}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Performance of SE-specific sentiment analysis in cross-platform setting (\bf{Test dataset: GitHub)}}
%     \begin{tabular}{ll|rrr|rrr|rrr|rrr|rrr|ccc}
%     \toprule
%     \multirow{2}{*}{\textbf{Train Dataset}}  & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiSE}}\\
%     \cmidrule{3-20}
%     {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
% \multirow{5}{*}{\parbox{2cm} {\centering GitHub \\ (Within Platform)}} 
% & Negative &  .91 & .39 & .55  & .90 & .43 & .58  & .75 & .39 & .52  & .85 & .52 & .64  & .88 & .27 & .41  & .81 & .71 & .76   \\ 
%  & Neutral &  .56 & .98 & .72  & .59 & .97 & .73  & .54 & .95 & .69  & .60 & .96 & .74  & .52 & .98 & .68  & .74 & .86 & .79   \\ 
%  & Positive &  .94 & .45 & .60  & .91 & .51 & .65  & .80 & .30 & .44  & .90 & .46 & .61  & .89 & .38 & .53  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .66 & .66 & .66  & .68 & .68 & .68  & .60 & .60 & .60  & .69 & .69 & .69  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  \textbf{.80} & .61 & .62  & \textbf{.80} & .64 & .65  & .70 & .55 & .55  & .78 & .65 & .67  & .76 & .54 & .54  & \textbf{.80} & \textbf{.78} & \textbf{.78}   \\
% % \cmidrule{2-20} 
% \midrule

% \multirow{5}{*}{\parbox{2cm} {\centering Stack Overflow \\ (Cross Platform)}} 
%  & Negative &  .85 & .62 & .72  & .83 & .73 & .78  & .69 & .49 & .58  & .79 & .56 & .66  & .83 & .37 & .51  & .81 & .71 & .76   \\ 
%  & Neutral &  .67 & .91 & .77  & .71 & .91 & .80  & .61 & .84 & .71  & .71 & .82 & .76  & .60 & .94 & .73  & .74 & .86 & .79   \\ 
%  & Positive &  .88 & .65 & .75  & .88 & .63 & .73  & .78 & .57 & .66  & .76 & .81 & .78  & .86 & .62 & .72  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .75 & .75 & .75  & .78 & .78 & .78  & .66 & .66 & .66  & .74 & .74 & .74  & .68 & .68 & .68  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  .80 & .73 & .75  & \textbf{.81} & .76 & .77  & .69 & .63 & .65  & .75 & .73 & .73  & .76 & .64 & .66  & .80 & \textbf{.78} & \textbf{.78}   \\ 
%  \cmidrule{2-20}
% \multirow{2}{2cm}{Difference with within-platform} & Micro-avg &  -.15 & -.15 & -.15 & -.14 & -.14 & -.14 & -.02 & -.02 & -.02 & -.17 & -.17 & -.17 & -.14 & -.14 & -.14 & & \multirow{2}{*}{NA}   \\ 
% & Macro-avg &  -.10 & -.17 & -.15 & -.11 & -.16 & -.15 & .01 & -.05 & -.04 & -.16 & -.18 & -.18 & -.08 & -.17 & -.17  \\ 

% \midrule


% \multirow{5}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%      & Negative &  .91 & .39 & .55  & .90 & .43 & .58  & .75 & .39 & .52  & .85 & .52 & .64  & .88 & .27 & .41  & .81 & .71 & .76   \\ 
%  & Neutral &  .56 & .98 & .72  & .59 & .97 & .73  & .54 & .95 & .69  & .60 & .96 & .74  & .52 & .98 & .68  & .74 & .86 & .79   \\ 
%  & Positive &  .94 & .45 & .60  & .91 & .51 & .65  & .80 & .30 & .44  & .90 & .46 & .61  & .89 & .38 & .53  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .66 & .66 & .66  & .68 & .68 & .68  & .60 & .60 & .60  & .69 & .69 & .69  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  \textbf{.80} & .61 & .62  & \textbf{.80} & .64 & .65  & .70 & .55 & .55  & .78 & .65 & .67  & .76 & .54 & .54  & \textbf{.80} & \textbf{.78} & \textbf{.78}   \\ 
% \cmidrule{2-20} 
% \multirow{2}{2cm}{Difference with within-platform} & Micro-avg &  -.24 & -.24 & -.24 & -.23 & -.23 & -.23 & -.08 & -.08 & -.08 & -.22 & -.22 & -.22 & -.23 & -.23 & -.23 & &  \multirow{2}{*}{NA}   \\ 
% & Macro-avg &  -.10 & -.29 & -.28 & -.12 & -.28 & -.26 & .02 & -.14 & -.14 & -.13 & -.26 & -.24 & -.08 & -.27 & -.28  \\ 


%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance_github}%
% % \end{table}%
% \end{sidewaystable}


% % =================================================================================================================== b

% \begin{sidewaystable}
% \vspace{15cm}
% % \begin{table}
% \addtocounter{table}{-1}
% \renewcommand{\thetable}{\arabic{table}b}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Performance of SE-specific sentiment analysis in cross-platform setting (\bf{Test dataset: Stack Overflow)}}
%     \begin{tabular}{ll|rrr|rrr|rrr|rrr|rrr|rrr}
%     \toprule
%     \multirow{2}{*}{\textbf{Train Dataset}}  & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiSE}}\\
%     \cmidrule{3-20}
%     {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
% \multirow{5}{*}{\parbox{2cm} {\centering Stack Overflow \\ (Within Platform)}} 
%  & Negative &  .84 & .83 & .83  & .86 & .85 & .85  & .74 & .73 & .74  & .80 & .83 & .82  & .80 & .72 & .76  & .76 & .76 & .76   \\ 
%  & Neutral &  .83 & .84 & .84  & .86 & .85 & .85  & .75 & .77 & .76  & .84 & .79 & .81  & .79 & .82 & .81  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .93 & .93  & .93 & .94 & .93  & .85 & .85 & .85  & .90 & .93 & .91  & .88 & .91 & .89  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}  & .78 & .78 & .78  & .85 & .85 & .85  & .82 & .82 & .82  & .79 & .79 & .79 \\ 
%  & Macro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}  & .78 & .78 & .78  & .85 & .85 & .85  & .82 & .82 & .82  & .80 & .79 & .79   \\ 

% % \cmidrule{2-20} 
% \midrule

% \multirow{5}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & Negative &  .82 & .76 & .79  & .80 & .86 & .83  & .66 & .60 & .63  & .69 & .76 & .72  & .64 & .49 & .55  & .76 & .76 & .76   \\ 
%  & Neutral &  .75 & .85 & .80  & .84 & .80 & .82  & .61 & .64 & .63  & .73 & .76 & .75  & .65 & .85 & .74  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .85 & .89  & .93 & .91 & .92  & .73 & .74 & .74  & .92 & .82 & .87  & .88 & .74 & .80  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .83 & .83 & .83  & \textbf{.85} & \textbf{.85} & \textbf{.85}  & .67 & .67 & .67  & .78 & .78 & .78  & .71 & .71 & .71  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .83 & .82 & .82  & \textbf{.85} & \textbf{.86} & \textbf{.85}  & .67 & .66 & .66  & .78 & .78 & .78  & .72 & .69 & .70  & .80 & .79 & .79   \\ 
%  \cmidrule{2-20}
% \multirow{2}{2cm}{Difference with within-platform} & Micro-avg &  -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.12 & -.12 & -.12 & -.07 & -.07 & -.07 & -.11 & -.11 & -.11  & & \multirow{2}{*}{NA}   \\ 
%  & Macro-avg &  -.03 & -.05 & -.04 & -.03 & -.02 & -.03 & -.11 & -.12 & -.12 & -.06 & -.07 & -.07 & -.10 & -.12 & -.12  \\ 

% \midrule


% \multirow{5}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%  & Negative &  .93 & .31 & .47  & .88 & .55 & .68  & .66 & .31 & .42  & .75 & .30 & .43  & .67 & .22 & .33  & .76 & .76 & .76   \\ 
%  & Neutral &  .54 & .98 & .70  & .63 & .94 & .76  & .50 & .91 & .65  & .54 & .93 & .69  & .50 & .95 & .66  & .73 & .79 & .75   \\ 
%  & Positive &  .98 & .62 & .76  & .97 & .74 & .84  & .83 & .42 & .56  & .96 & .64 & .76  & .96 & .52 & .67  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .67 & .67 & .67  & .76 & .76 & .76  & .58 & .58 & .58  & .66 & .66 & .66  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  .82 & .64 & .64  & \textbf{.83} & .74 & .76  & .66 & .55 & .54  & .75 & .62 & .63  & .71 & .56 & .55  & .80 & \textbf{.79} & \textbf{.79}   \\ 

% \cmidrule{2-20} 
% \multirow{2}{2cm}{Difference with within-platform} & Micro-avg &  -.20 & -.20 & -.20 & -.12 & -.12 & -.12 & -.21 & -.21 & -.21 & -.19 & -.19 & -.19 & -.22 & -.22 & -.22 & & \multirow{2}{*}{NA}   \\ 
% & Macro-avg &  -.05 & -.23 & -.23 & -.05 & -.14 & -.12 & -.12 & -.23 & -.24 & -.10 & -.23 & -.22 & -.11 & -.25 & -.27  \\  


%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance_so}%
% % \end{table}%
% \end{sidewaystable}


% % =================================================================================================================== c

% \begin{sidewaystable}
% \vspace{15cm}
% % \begin{table}
% \addtocounter{table}{-1}
% \renewcommand{\thetable}{\arabic{table}c}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Performance of SE-specific sentiment analysis in cross-platform setting (\bf{Test dataset: Jira)}}
%     \begin{tabular}{ll|rrr|rrr|rrr|rrr|rrr|rrr}
%     \toprule
%     \multirow{2}{*}{\textbf{Train Dataset}}  & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiSE}}\\
%     \cmidrule{3-20}
%     {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
% \multirow{5}{*}{\parbox{2cm} {\centering Jira \\ (Within Platform)}} 
%  & Negative &  .84 & .68 & .75  & .82 & .76 & .79  & .69 & .46 & .55  & .71 & .55 & .62  & .79 & .66 & .72  & .68 & .73 & .71   \\ 
%  & Neutral &  .89 & .91 & .90  & .90 & .90 & .90  & .83 & .89 & .86  & .84 & .88 & .86  & .89 & .89 & .89  & .92 & .82 & .87   \\ 
%  & Positive &  .79 & .80 & .79  & .78 & .80 & .79  & .73 & .72 & .72  & .73 & .71 & .72  & .75 & .85 & .80  & .68 & .92 & .78   \\ 
%  & Micro-avg &  \textbf{.86} & \textbf{.86} & \textbf{.86}  & \textbf{.86} & \textbf{.86} & \textbf{.86}  & .80 & .80 & .80  & .81 & .81 & .81  & .85 & .85 & .85  & .83 & .83 & .83   \\ 
%  & Macro-avg &  \textbf{.84} & .80 & .81  & .83 & \textbf{.82} & \textbf{.83}  & .75 & .69 & .71  & .76 & .72 & .73  & .81 & .80 & .80  & .76 & \textbf{.82} & .79   \\ 

% % \cmidrule{2-20} 
% \midrule

% \multirow{5}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & Negative &  .63 & .75 & .69  & .66 & .74 & .70  & .51 & .71 & .60  & .61 & .64 & .62  & .69 & .60 & .64  & .68 & .73 & .71   \\ 
%  & Neutral &  .93 & .79 & .85  & .93 & .80 & .86  & .92 & .58 & .71  & .89 & .78 & .83  & .90 & .85 & .87  & .92 & .82 & .87   \\ 
%  & Positive &  .66 & .91 & .77  & .65 & .91 & .76  & .45 & .92 & .61  & .62 & .86 & .72  & .69 & .89 & .78  & .68 & .92 & .78   \\ 
%  & Micro-avg &  .81 & .81 & .81  & .81 & .81 & .81  & .66 & .66 & .66  & .78 & .78 & .78  & .82 & .82 & .82  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg &  .74 & \textbf{.82} & .77  & .75 & \textbf{.82} & .77  & .63 & .74 & .64  & .71 & .76 & .73  & \textbf{.76} & .78 & .76  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\
%  \cmidrule{2-20}
% \multirow{2}{2cm}{Difference with within-platform} & Micro-avg &  -.05 & -.05 & -.05 & -.05 & -.05 & -.05 & -.14 & -.14 & -.14 & -.03 & -.03 & -.03 & -.03 & -.03 & -.03 & & \multirow{2}{*}{NA}   \\ 
% &  Macro-avg &  -.09 & .02 & -.04 & -.09 & -.00 & -.05 & -.12 & .05 & -.07 & -.05 & .05 & -.01 & -.05 & -.02 & -.04  \\ 

% \midrule


% \multirow{5}{*}{\parbox{2cm} {\centering Stack Overflow \\ (Cross Platform)}} 
%  & Negative &  .67 & .68 & .67  & .72 & .68 & .70  & .58 & .61 & .59  & .50 & .29 & .37  & .36 & .06 & .10  & .68 & .73 & .71   \\ 
%  & Neutral &  .92 & .81 & .86  & .92 & .82 & .87  & .88 & .77 & .82  & .82 & .81 & .81  & .75 & .94 & .83  & .92 & .82 & .87   \\ 
%  & Positive &  .67 & .93 & .78  & .65 & .93 & .76  & .62 & .89 & .73  & .59 & .80 & .68  & .71 & .49 & .58  & .68 & .92 & .78   \\ 
%  & Micro-avg &  .82 & .82 & .82  & .82 & .82 & .82  & .77 & .77 & .77  & .74 & .74 & .74  & .73 & .73 & .73  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg &  .75 & .81 & .77  & \textbf{.76} & .81 & .78  & .69 & .75 & .71  & .64 & .63 & .62  & .61 & .49 & .50  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\  

% \cmidrule{2-20} 
% \multirow{2}{2cm}{Difference with within-platform} & Micro-avg &  -.04 & -.04 & -.04 & -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.07 & -.07 & -.07 & -.12 & -.12 & -.12 & & \multirow{2}{*}{NA}   \\ 
% &  Macro-avg &  -.08 & .01 & -.04 & -.07 & -.01 & -.05 & -.05 & .06 & .00 & -.12 & -.08 & -.11 & -.20 & -.30 & -.30  \\


%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance_jira}%
% % \end{table}%
% \end{sidewaystable}













% \begin{sidewaystable}
% \vspace{15cm}

% \end{sidewaystable}





% \begin{sidewaystable}
% \vspace{15cm}
\begin{table*}%[t]
\footnotesize
% \small
  \centering
  %\vspace{-.1in}
  \caption{Performance drop in SE-specific supervised sentiment analysis tools in cross-platform settings (SO = Stack Overflow)}
  %\vspace{-3mm}
  % \resizebox{\textwidth}{!}{%
    \begin{tabular}{cl|rrr|rrr|rrr|rrr|rrr}
    \toprule{}

    \multirow{2}{*}{\textbf{Train}} & \multirow{2}{*}{\textbf{Performance}} & 
    \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} \\
    \cmidrule{3-17}
    \textbf{Dataset} & \centering \textbf{Drop} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
    \midrule
    
    \multicolumn{17}{c}{\textbf{Test dataset: GitHub}} \\
    \midrule
 
    \multirow{2}{*}{\textbf{SO}} & $\triangledown$ Micro-avg &  -16\% & -16\% & -16\% & -15\% & -15\% & -15\% & -3\% & -3\% & -3\% & -18\% & -18\% & -18\% & -17\% & -17\% & -17\%    \\ 
    &  $\triangledown$ Macro-avg &  -11\% & -19\% & -17\% & -12\% & -18\% & -16\% & 2\% & -8\% & -5\% & -17\% & -20\% & -19\% & -10\% & -21\% & -20\%  \\ 
    \cmidrule{2-17}
    
    \multirow{2}{*}{\textbf{Jira}} &  $\triangledown$ Micro-avg &  -27\% & -27\% & -27\% & -26\% & -26\% & -26\% & -12\% & -12\% & -12\% & -24\% & -24\% & -24\% & -27\% & -27\% & -27\%   \\ 
    &  $\triangledown$ Macro-avg &  -11\% & -32\% & -31\% & -13\% & -31\% & -29\% & 2\% & -21\% & -20\% & -14\% & -29\% & -27\% & -9\% & -34\% & -34\%  \\ 
    % \cmidrule{2-17}
    \midrule
    
    
    \multicolumn{17}{c}{\textbf{Test dataset: Stack Overflow}} \\
    \midrule
    \multirow{2}{*}{\textbf{GitHub}} & $\triangledown$  Micro-avg &  -5\% & -5\% & -5\% & -3\% & -3\% & -3\% & -15\% & -15\% & -15\% & -8\% & -8\% & -8\% & -13\% & -13\% & -13\%   \\ 
    & $\triangledown$  Macro-avg &  -4\% & -5\% & -5\% & -3\% & -3\% & -3\% & -15\% & -15\% & -15\% & -7\% & -8\% & -8\% & -12\% & -15\% & -15\%  \\ 
    \cmidrule{2-17}
    \multirow{2}{*}{\textbf{Jira}} &  $\triangledown$ Micro-avg &  -23\% & -23\% & -23\% & -13\% & -13\% & -13\% & -26\% & -26\% & -26\% & -22\% & -22\% & -22\% & -27\% & -27\% & -27\%   \\ 
    &  $\triangledown$ Macro-avg &  -6\% & -27\% & -26\% & -6\% & -16\% & -14\% & -15\% & -30\% & -31\% & -11\% & -27\% & -26\% & -14\% & -31\% & -33\%  \\ 
    % \cmidrule{2-17}
    \midrule
    
    \multicolumn{17}{c}{\textbf{Test dataset: Jira}} \\
    \midrule
    \multirow{2}{*}{\textbf{GitHub}} &  $\triangledown$ Micro-avg &  -6\% & -6\% & -6\% & -6\% & -6\% & -6\% & -17\% & -17\% & -17\% & -4\% & -4\% & -4\% & -3\% & -3\% & -3\%    \\ 
    &  $\triangledown$ Macro-avg &  -11\% & 3\% & -5\% & -10\% & 0\% & -7\% & -16\% & 7\% & -10\% & -7\% & 7\% & -1\% & -6\% & -2\% & -5\%  \\ 
    \cmidrule{2-17}
    \multirow{2}{*}{\textbf{SO}} & $\triangledown$  Micro-avg &  -5\% & -5\% & -5\% & -5\% & -5\% & -5\% & -4\% & -4\% & -4\% & -9\% & -9\% & -9\% & -14\% & -14\% & -14\%   \\ 
    &  $\triangledown$ Macro-avg &  -10\% & 1\% & -5\% & -8\% & -1\% & -6\% & -7\% & 9\% & 1\% & -16\% & -12\% & -15\% & -25\% & -38\% & -37\%  \\ 
    % \cmidrule{2-17}
    \midrule



    \bottomrule
    \end{tabular}%
%}
  % \vspace{-.25in}
  \label{tab:cross_platform_performance_drop}%
\end{table*}%
% \end{sidewaystable}


==> SubmissionTOSEM/RQ2.tex <==

\subsection{RQ$_3$ Can similarity analysis between the studied datasets explain the drop in performance 
of the deep learning SD tools in the datasets in cross-platform settings?}\label{sec:rq-cross-platform-similarity}
\subsubsection{Motivation} Across the supervised SD tools for SE in our three studied datasets, we observe 
a drop in performance in cross-platform settings. While the two deep learning SD tools (BERT4SentiSE and SentiMoji) offer better performance than the 
other supervised SD tools in the majority of cross-platform settings, their performance still varies across the datasets. 
For example, as we noted in RQ$_1$, the tools suffered the most performance drop when the tools were trained in Jira and then tested in the other two datasets. Intuitively, the more similar the textual contents are between the pair of datasets, the less drop we can expect in performance for a tool in those two datasets in cross-platform settings. Therefore, it 
is important to know whether there is a correlation between content similarity of the studied datasets and the performance 
of the studied tools in cross-platform settings. 

% While we observe a drop in performance in
% cross-platform settings, the drop is not uniform across the datasets.
% Intuitively, the more similar the two datasets are in terms of textual contents,
% the less drop in performance we may expect for a tool in cross-platform
% settings. This assumption, however, can be challenged when the two datasets
% differ in size (among other differences). Therefore, it would be interesting to
% know whether and how the similarity between the datasets in our study could be
% correlated with their performance in the tools for cross-platform settings. Such
% insights can be useful to decide when cross-platform adoption of a tool is more
% useful for a suite of SE-specific datasets.


% From our RQ1, we find that DL-based tools perform quite well in within platform and slightly better in cross-platform settings. 
%
% From RQ1, we observer a drop in performance for all machine learning based classifiers. Additionally we notice the drop is more steep when trained on Jira dataset. So, in this research question we aim to explore the correlation of divergence, i.e., difference between each pair of these three benchmark datasets and the drop in performance in cross platform settings. 
% Table \ref{tab:cross_platform_performance} shows that the performance of the DL-based classifiers are not significantly better than shallow ML-based classifiers. But SEntiMoji and BERT4SentiSE are pre-trained DL-based classifier that are already trained on large NLP datasets. These models already have an intuitive understanding about language and use transfer learning to train and learn on new tasks. So, generally we expect that the performance of these pre-trained DL-based tools will be better in cross platform settings (i.e., datasets from different distributions) than shallow ML-based classifiers. 
% However,  So, it motivated us to investigate further into analysing the similarity and diversity of these datasets and their correlation with performance of DL-based classifiers on them in cross platform settings.
% Ideally we want to find the how similar these datasets
% are in terms of software domain specific context. As these three datasets come
% from three different type of software engineering platforms, we expect there are
% certain technical jargons that are common in them and some are more prevalent in
% one dataset than others. 

\subsubsection{Approach} For this analysis, we focus on the two best performing deep learning SD tools for SE from RQ$_1$, i.e., BERT4SentiSE and SentiMoji. 
For each tool and for each cross-platform setting involving two datasets (i.e., one dataset for training and another for testing). we analyze whether there is any correlation between the performance 
of the tool in cross-platform settings and the textual similarity between the two datasets. 
We compute the similarity
between two datasets using two standard metrics, Cosine similarity, and Jensen-Shannon Divergence. We discuss below how we use the two metrics to compute the similarity between two given datasets.

\begin{inparaenum}[(1)]
\item\bf{Cosine similarity~\cite{Manning-IRIntroBook-Cambridge2009}} helps to
find text similarity between two documents irrespective of the size of the
documents.
For each dataset, we take the top 10,000 unigrams after removing stopwords (we
used stopwords from the Python `nltk' library). We then combine those to create a
unified vocabulary list ($V$) for all the datasets. We use $V$ to create a
vectorized representation of each dataset based on the frequency of the words of
each sentence in the dataset. For any two datasets (e.g., A, B), we fed their
resulting vectors into \eq\ref{eq:consine} to compute the similarity between the two
datasets. We cosine\_similarity method from Sklearn library
\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.metrics.pairwise.cosine_similarity.html}}.
%The higher the Cosine distance, the more similar the datasets are.

\begin{equation}\label{eq:consine}
Cosine_{Similarity}(A,B) = \frac{A.B}{|A||B|}   
\end{equation}

\item \bf{Jensen-Shannon Divergence~\cite{fuglede2004jensen} ($D_{JS}$)} is a
symmetric and smoothed version of Kullback-Leibler Divergence $D_{KL}$,
$D_{KL}(A||B) = \sum_{i}^{N} a_i log \frac{a_i}{b_i}$. $D_{KL}$ is a probability
distribution of A and B. While $D_{KL}$ is undefined when any element $a_i \in
A$, has zero probability. Whereas, $D_{JS}$ is a probability distribution of
every word in vocabulary $V$. The metric is originally proposed to calculate the
similarity between two datasets A and B as follows:
\begin{equation}\label{eq:jsd}
D_{JS}(A,B) = \frac{1}{2} [D_{KL}(A||B)+D_{KL}(B||A)]    
\end{equation} With \eq\ref{eq:jsd}, a value of $D_{JS}$ = 0, it signifies the
datasets are most similar a value of 1.0 denotes they are completely different.
Given that Cosine similarity adopts an opposite notion for similarity (i.e., 1
as completely similar), we change \eq\ref{eq:jsd} as follows:
\begin{equation}\label{eq:jsd}
D_{JS}(A,B) = 1- \frac{1}{2} [D_{KL}(A||B)+D_{KL}(B||A)]    
\end{equation} Thus in our case, when $D_{JS}$ = 1.0, it signifies the datasets
are most similar and when $D_{JS}$ = 0.0 it signifies that the datasets are
completely diverse from each other. We compute the metric for each pair of
datasets (A, B) as follows. Similar to cosine similarity approach we create a
vectorized representation of each dataset. For any two datasets (e.g., A, B), we
fed their resulting vectors into \eq\ref{eq:jsd} to compute $D_{JS}$ similarity
between the two datasets.
\end{inparaenum} 

% We also report the internal $D_{JS}$ for each datasets. We randomly shuffle each datasets for 50 times and then we divide each dataset in two equal halves. Then we calculate the $D_{JS}$ for this two halves. Then we report the mean and standard deviation for the 50 $D_{JS}$ distance values for each dataset.

We compute the correlation between the similarity in the two datasets and the performance of a tool in cross-platform settings using 
Mann-Whitney (MW) U Test~\cite{mcknight2010mann}. MW test is non-parametric, which is suitable for our data where data is not normally distributed. We report the significance of correlation using p-value and the effect size using Cliff's $\delta$ value. 
We interpret the $\delta$ following Romano et al.~\cite{Romano-EffectSize-2006}:
\begin{equation}
  \tr{Effect Size} =\left\{
  \begin{array}{@{}ll@{}}
    {negligible~(N)}, & \tr{if}\ |\delta| \leq 0.147 \\
    {small~(S)}, & \tr{if}\ 0.147 < |\delta| \leq 0.33 \\
    {medium~(M)}, & \tr{if}\ 0.33 < |\delta| \leq 0.474 \\
    {large~(L)}, & \tr{if}\ 0.474 < |\delta| \leq 1 
  \end{array}\right.
\end{equation} The effect size categories (negligible, small, medium, 
or large) quantify the differences between the distributions.


%\input{RQ2_tables}



\subsubsection{Results}  \bf{There is a statistically significant correlation
between content similarity of the datasets and their Macro F1 score in
cross-platform settings.} In
\tbl\ref{tab:corrSimAcc}, we report the p-value of the correlation analysis between the dataset similarity and tool performance values using MW U test. We also show the effect size.
\begin{table}[t]
  \centering
  \caption{Correlation between dataset similarity values and Macro-F1 scores in cross-platform settings}
    \begin{tabular}{lrr|rr}\toprule
          & \multicolumn{2}{c}{\bf{BERT4SentiSE}} & \multicolumn{2}{c}{\bf{SentiMoji}} \\
          \cmidrule{2-5}
          & {p-value} & Effect Size     & {p-value} & Effect Size \\
          \midrule
    Jansen Shannon    & 0.04*  & Large (0.6) & 0.003** & Large (1.0) \\
    Cosine & 0.002** & Large (1.0) & 0.003** & Large (1.0) \\
    \bottomrule
    \multicolumn{5}{l}{Signif. codes:  ***$p < 0.001$, **$p < 0.01$, *$p < 0.05$}
    \end{tabular}%
  \label{tab:corrSimAcc}%
\end{table}%
In \fig\ref{fig:diversity_performance}, we show the
similarity scores between the datasets and compare the Macro F1-scores between the datasets for the two best performing
deep learning SD tools from RQ$_1$ (i.e., BERT4SentiSE and SentiMoji). For
example, in the first block (i.e., Test on GitHub), we have two sets of bars:
similarity scores between GitHub and SO datasets and Macro F1-scores of
BERT4SentiSE and SentiMoji for the cross-platform setting (i.e., trained on SO
and tested on GitHub). The Jansen similarity scores between the datasets are at least
0.87 and at least 0.93 for cosine similarity. Therefore, while datasets are produced from different platforms, they
have a considerable number of similar words. Thus the more similar two datasets are, the less performance drop 
we can expect in cross-platform settings. 
\begin{figure*}[h]
\centering
\captionsetup[subfigure]{labelformat=empty}
\pgfplotstableread{

1	.88  .97 .75 .77     .88  .97  .82 .85      .87  .96  .77 .77
2	.87  .96 .62 .65     .85  .93  .64 .76      .85  .93  .77 .78
}\datatable
      \subfloat[Test on GitHub]
      {
      \resizebox{1.5in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Trained on SO, Trained on Jira},
        	enlarge y limits=false,
        	enlarge x limits=0.55,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.7cm,
        	width=3.6in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},
        	major x tick style = {opacity=0},
        	minor x tick num = 1,
        	minor tick length=1ex,
        	legend columns=2,
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend style={draw=none},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\huge},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	]
        	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=1] \datatable;
        	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=2] \datatable;
        	\addplot[draw=black!80, fill=black!70] table[x index=0,y index=3] \datatable;
        	\addplot[draw=black!80, fill=black!100] table[x index=0,y index=4] \datatable;

            \legend{JS Divergence,
            		 Cosine Similarity,
            		 }
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    }
    \subfloat[Test on Stack Overflow (SO)]
     {
      \resizebox{1.5in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub, Train on Jira},
        	enlarge y limits=false,
        	enlarge x limits=0.55,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.7cm,
        	width=3.6in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
         	xticklabel style={font=\LARGE, /pgf/number format/fixed},
        	major x tick style = {opacity=0},
        	minor x tick num = 1,
        	minor tick length=1ex,
        	legend columns=2,
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend style={draw=none},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            nodes near coords style={font=\huge},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	]
        	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=5] \datatable;
        	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=6] \datatable; %, postaction={pattern=horizontal lines}
        	\addplot[draw=black!80, fill=black!60] table[x index=0,y index=7] \datatable;   %, postaction={pattern=vertical lines}
            \addplot[draw=black!80, fill=black!100] table[x index=0,y index=8] \datatable;  %, postaction={pattern=vertical lines}
            \legend{,,
            		 SEntiMoji F1,
            		 BERT4SentiSE F1
            		 }
            % \legend{JS Divergence,
            % 		 Cosine Similarity,
            % 		 SEntiMoji F1,
            % 		 BERT4SentiSE F1
            % 		 }
        	\end{axis}
    	\end{tikzpicture}
    	}
    % 	\hspace{-1mm}
    	\label{signature-inconsistency}
    }
    \subfloat[Test on Jira]
     {
      \resizebox{1.5in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub, Train on SO
        	},
        	enlarge y limits=false,
        	enlarge x limits=0.55,
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,,
        	ymin=0,ymax=1.08,
        	ybar,
        	bar width=0.7cm,
        	width=3.4in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
        %     yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
         	xticklabel style={font=\LARGE, /pgf/number format/fixed},
        	major x tick style = {opacity=0},
        	minor x tick num = 1,
        	minor tick length=1ex,
        	legend style={
         	at={(0.6,0.98)},
            anchor=north,legend columns=-1
            },
            nodes near coords style={font=\huge},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	]
        	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=9] \datatable;
        	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=10] \datatable; %, postaction={pattern=horizontal lines}
        	\addplot[draw=black!80, fill=black!60] table[x index=0,y index=11] \datatable; %, postaction={pattern=vertical lines}
            \addplot[draw=black!80, fill=black!100] table[x index=0,y index=12] \datatable; %, postaction={pattern=vertical lines}

        	\end{axis}
    	\end{tikzpicture}
    	}
    % 	%\hspace{-1mm}
    	\label{fig:status-inconsistency}
    }





%\vspace{-3mm}
\caption{Similarity scores between datasets vs Macro F1-scores per tool (BERT4SentiSE \& SentiMoji) in cross platform settings}
\vspace{-3mm}
\label{fig:diversity_performance}
\end{figure*}


% Table generated by Excel2LaTeX from sheet 'similary_vs_perfdrop'
\begin{table}[h]
\newcolumntype{C}{>{\centering\arraybackslash}p{9em}}
  \centering
  \caption{Distribution of dataset content similarity vs drop in performance (Macro F1-score) in Cross-Platform Settings compared to Within Platform Settings for BERT4SentiSE and SentiMoji}
    \begin{tabular}{lccc|CC}\toprule
    {\textbf{Test}} & {\textbf{Train}} & \multicolumn{2}{c}{\textbf{Similarity Score}} & \multicolumn{2}{c}{\textbf{\% Performance drop in cross-platform  Test Dataset}} \\
    \cmidrule{3-6}
    {\textbf{Dataset}} & \textbf{Dataset} & {\textbf{JS divergence}} & {\textbf{Cosine distance}} & \textbf{SentiMoji} & \textbf{Bert4SentiSE} \\
    \midrule
    \multicolumn{1}{l}{\multirow{2}[0]{*}{GitHub}} & SO    & 0.88  & 0.97  & 17    & 16 \\
          & Jira  & 0.87  & 0.96  & 31    & 29 \\
          \midrule
    \multicolumn{1}{l}{\multirow{2}[0]{*}{SO}} & GitHub & 0.88  & 0.97  & 5     & 3 \\
          & Jira  & 0.85  & 0.93  & 26    & 14 \\
          \midrule
    \multicolumn{1}{l}{\multirow{2}[0]{*}{Jira}} & GitHub & 0.87  & 0.96  & 5     & 7 \\
          & SO    & 0.85  & 0.93  & 5     & 6 \\
          \bottomrule
    \end{tabular}%
  \label{tab:sim_vs_drop}%
\end{table}%

\bf{The significance analysis cannot explain the varying degrees of performance between Jira and non-Jira datasets in cross-platform settings.} Our findings in RQ$_1$ 
show the largest performance drop in the two deep learning SD tools when trained in the Jira dataset and tested in the other two datasets. 
The significance analysis in \tbl\ref{tab:corrSimAcc} suggests that this performance drop could be attributed to the similarity (or lack of thereof) between Jira and the other two datasets. However, \fig\ref{fig:diversity_performance} shows that the Jira dataset has almost similar content similarity scores with the SO and GitHub 
as do SO and GitHub with each other. Moreover, the tools suffer a much bigger drop in performance only when they 
are trained in Jira. For example, BERT4SentiSE shows a Macro F1-score of 0.65 when trained in Jira and tested in GitHub, but it shows 
an F1-score of 0.77 when trained in GitHub and then tested in Jira. In \tbl\ref{tab:sim_vs_drop}, we 
show the percentage drop in Macro F1-score compared to within platform setting for each cross-platform settings. For example, the first two rows in 
\tbl\ref{tab:sim_vs_drop} show that when trained in the SO dataset and then tested in the GitHub dataset, the drop in performance in BERT4SentiSE is 16\% compared to the performance 
of BERT4SentiSE when trained and tested in GitHub. However, when BERT4SentiSE is trained in the Jira dataset and then tested in the GitHub dataset, the drop in performance 
is 29\%. The cosine similarity between GitHub and SO is 0.97 and between GitHub and Jira is 0.96. 
When the tool was trained in GitHub and tested in SO, the drop was 3\%, but the drop was 14\% when the tool was trained in Jira and tested in SO. 
The cosine similarity between SO and GitHub is 0.97, and between SO and Jira is 0.93. Therefore, the drop in performance while using the Jira 
dataset could be due to reasons other than content similarity. 

Instead, the the distribution of the polarity classes in the Jira dataset could offer an alternative explanation (see 
\tbl\ref{tab:benchmark_dataset}). While both GitHub and SO are more balanced towards the three polarity classes (around 27-35\% of sentences per polarity class), the Jira dataset is imbalanced with only 19\% positive and 14\% negative classes. {This means that a tool trained using the Jira dataset 
does not have enough information of the two polarity classes compared to when it is trained 
in the other two datasets.} The imbalance in the Jira dataset may also have
introduced bias in the polarity labeling (e.g., by showing more preference
towards neutral classes), contributing to the high percentage of mild disagreements in 
\tbl\ref{tab:agreement_with_manual_labelling}. This happened despite each tool is designed to 
handle the class imbalance problem in model training.


%Similarly SentiMoji also shows similar performance for the three classes in cross-platform settings. 



\begin{table}[t]
  \centering
  \caption{Distribution of False Neutral and False Non-neutral prediction in cross-platform settings. (False Neutral = Prediction is neutral for non-neutral, False Non-neutral = Prediction is non-neutral for neutral sentences)}
  \resizebox{\columnwidth}{!}{%
    \begin{tabular}{ll|cc|cc|cc}\toprule
    {\textbf{SD}} & \textbf{\% Correct} & \multicolumn{2}{c}{\textbf{Train in GitHub}} & \multicolumn{2}{c}{\textbf{Train in SO}} & \multicolumn{2}{c}{\textbf{Train in Jira}} \\
    \cmidrule{3-8}
    {\textbf{Tool}} & \textbf{Misclassified} & {\textbf{Test SO}} & {\textbf{Test Jira}} & {\textbf{Test GitHub}} & {\textbf{Test Jira}} & {\textbf{Test GitHub}} & {\textbf{Test SO}} \\
    \midrule
\multirow{2}{*}{\textbf{SentiMoji}} &False Neutral &61 &22 &75 &28 &\textbf{94} &\textbf{97} \\
&False Non-neutral &34 &74 &15 &69 &\textbf{2} &\textbf{3} \\
\midrule
\multirow{2}{*}{\textbf{BERT4SentiSE}} &False Neutral &41 &23 &69 &26 &\textbf{91} &\textbf{88} \\
&False Non-neutral &52 &72 &17 &69 &\textbf{3} &\textbf{10} \\

          \bottomrule
    \end{tabular}%
    }
  \label{tab:rq-mild-error-analysis}%
\end{table}%


\textbf{When trained on the imbalanced Jira dataset (67\% neutral), the most dominant error case (around 90\%) is that all the supervised tools predict neutral polarity for non-neutral sentences.}
From Table~\ref{tab:cross_platform_performance}, we can see that when trained in Jira dataset and tested on non-Jira datasets, both SentiMoji and BERT4SentiSE show high precision and low recall for both the non-neutral classes. At the same time, these tools exhibit high recall and low precision for the neutral class. For example, when trained on the Jira dataset and tested on GitHub dataset, BERT4SentiSE shows a precision of 0.90 and recall of 0.43 for the negative class. The tool shows a precision of 0.91 and a recall of 0.51 for the positive class. At the same time, they report a high recall of .97 and low precision of 0.59 for the neutral class. 
This observation is consistent with SentiMoji in cross-platform settings.
Table~\ref{tab:rq-mild-error-analysis} presents details about the drop in performance when the supervised SD tools are trained on cross-platform settings. 
Around 95\% to 99\% misclassifications fall under mild errors (i.e., the sum of `False Neutral' and `False Non-neutral'). Around 88\% to 97\% of the errors are due to `False Neutral' prediction, i.e., the manual label is non-neutral, but the tool predicts as neutral. For example, when BERT4SentiSE is trained on the Jira dataset and tested on GitHub, it has around 29\% performance drop in terms of macro F1-score and 94\% of its total errors are mild error, and 6\% are severe errors. Our analysis shows that in that settings, 91\% of the errors fall under the `False Neutral' category, and only 3\% of errors fall under the `False Non-neutral' category. Novelli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020} also reported a similar performance drop in cross-platform settings for the supervised tools, and the deep-learning-based SD tools outperformed all non-DL based SD tools in within-platform settings even for the imbalanced Jira dataset. As mentioned in \sec\ref{sec:studied-tools}, for this study, we used the best model configuration, hyperparameters, and settings for the studied supervised tools reported by the original authors in respective studies. 






%\bf{Some characteristics of the dataset other than content similarity between them are responsible for the drop in performance in cross platform settings}. To better understand the causes of variation in the drop of performance of the tools across the three datasets, we next check the number of misclassifications in within vs. cross-platform settings. In \fig\ref{fig:diversity_performance_misssclf}, we show three blocks of bars, one block per test dataset. For example, the first block uses GitHub as the test dataset, i.e., it is trained on the other two datasets and then tested on GitHub. The first bar for `Test of GitHub' shows the ratio of misclassified cases in GitHub for within platform setting. Here, the ratio is the total number of misclassified sentences out of all sentences in the GitHub dataset. The second bar shows the ratio of misclassified cases while trained on SO and tested on GitHub, and the third bar shows the ratio of misclassified cases while trained on Jira and tested on GitHub. For both cross-platform cases where Jira is used to train  (i.e., Test on GitHub and Test on SO), we see 19-29\% of misclassified cases. In contrast, we see at most 14\% misclassified cases while Jira is used as the test dataset and GitHub or SO is used as the training dataset. \bf{This denotes that while the three datasets show content similarity, the variation in the drop in performance across the datasets might be due to characteristics specific to the individual datasets that are not necessarily specific to content similarity.}

% Our two similarity metrics shows that the similarity of these datasets are quite high. Figure \ref{fig:diversity_performance} shows that the Jensen-Shannon Divergence and Cosine similarity of the datasets and the micro F1 score of SEntiMoji and BERT4SentiSE. Our experiments show that GitHub has higher similarity with SO than Jira and so when tested on GitHub both SentiMoji and BERT4SentiSE has higher micro F1 score. Similar pattern can also be found when the test on Stack Overflow or Jira dataset.

% From our experiments of internal $D_{JS}$ divergence, we find Jira dataset has the highest diversity and Stack Overflow dataset has the lowest internal divergence. The mean of internal $D_{JS}$ divergence of GitHub, Stack Overflow and Jira datasets are 0.92, 0.93, and 0.87 respectively. In all cases the standard deviation is less than 0.001.

% Mean is 0.915153 and Standard Deviation of Sample set is 0.0007074900782077775
% Mean is 0.930979 and Standard Deviation of Sample set is 0.0005455997749518836
% Mean is 0.870792 and Standard Deviation of Sample set is 0.0009510214319267058


\begin{tcolorbox}[flushleft upper,boxrule=1pt,arc=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=white,after=\ignorespacesafterend\par\noindent]
 \bf{RQ$_3$ Can similarity analysis between the studied datasets explain the drop in performance of the deep learning SD tools in the datasets in cross-platform settings?} There
is a statistically significant positive correlation between similarity of
contents between any two datasets and the performance of a pre-trained DL-based
tools between the two datasets in cross-platform settings (i.e., more similarity
results in more performance). However, the significance analysis is not sufficient to explain the drop in performance in the tools for cross-platform 
settings involving the Jira dataset, which is highly imbalanced and has a much fewer number of non-neutral classes in the data compared to the other two datasets.
%  The drop in performance and ratio of misclassified cases in cross-platform setting is the most for Jira dataset in the cross-platform settings, i.e., tools are more error-prone while they used Jira as the training dataset.
\end{tcolorbox}
















% \begin{table*}[h]
%   \centering
%   %\vspace{-.1in}
%   \caption{Distribution of Error Categories for the deep-learning tools}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{lll}
%     \toprule{}
%     % \textbf{Topics} & \textbf{Authentication} & \textbf{Deployment} & \textbf{Documentation} & \textbf{Feature} & \textbf{Testing/Debugging}\\
%     \textbf{Category} & \textbf{Description} & \textbf{\#Units} \\
%     \midrule

%     Subjectivity in Annotation & Sentences that are labelled inconsistently with-in platform or Cross-platform & 114 (29\%) \\
%     General Error & Tools failing to process linguistic cues & 82 (21\%) \\
%     Implicit Sentiment & Sentences that express emotion without explicit linguistic cues & 57 (14\%) \\
%     Context/Pragmatics & Tools failing to understand the underlying context to detect overall polarity & 55 (14\%) \\
%     Domain Specific & Sentences with polarity in SE-specific context & 49 (12\%) \\
%     Politeness & A neutral sentence is labelled with polar sentiment due to politeness & 27 (7\%) \\
%     Figurative language & Sentences containing humour or irony & 16 (4\%) \\
    

%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:misclassification}%
% \end{table*}%










==> SubmissionTOSEM/RQ3.tex <==

%\input{RQ3_tables}
\subsection{RQ$_4$ What are the error categories of the tools in the cross-platform settings?}\label{subsec:error_analysis}\label{sec:rq-cross-platform-error}

\subsubsection{Motivation} The findings from RQ$_1$ and RQ$_2$ show that all of the supervised SD tools for SE suffer from a drop in performance in cross-platform settings. From RQ$_3$, We find that the more similar two datasets are, the less performance drop we can expect to have from them in cross-platform 
settings. However, it does not entirely explain the performance drop and why an SD predicts incorrectly for a given sentence while another SD tool predicts correctly.
Understanding error types for such sentences can offer further insights into the future improvements of the tools in cross-platform settings.
% In addition, the analysis also does not take into account when both of the tools (i.e., BERT4SentiSE and SentiMoji) can be wrong for a given sentence in 
% cross-platform settings. In the three datasets, across the six cross-platform
% settings, we find a total of 4,188 misclassified sentences where both
% BERT4SentiSE and SentiMoji were wrong. 
    
% The superiority of two deep learning SE-specific SD
% tools (BERT4SentiSE and SentiMoji) over shallow learning SD tools offers hope
% that the two tools are better suited to apply in both within and cross-platform
% settings. The similarity analysis of the datasets shows that the more similar
% two cross-platform datasets can be, the more performance we can expect for the
% two tools in cross-platform settings. However, there is also a drop in the
% performance of the two tools in cross-platform settings. It is important to
% learn the types of misclassifications that the two tools show in cross-platform
% settings. Such insights can then be used to improve the two tools and to improve
% future research in this domain (i.e., improve benchmark datasets).
% From RQ2, we see the diverse the train and test dataset the higher drop in cross-platform performance. In this research question, we aim to complement this qualitative analysis by providing an extensive error analyse to better understand the root cause of the mis-classifications. The goal of this analysis is to explore if the error categorization of the DL-based classifier and shallow ML-based classifier differs\cite{Novielli-SEToolCrossPlatform-MSR2020, Novielli-BenchmarkStudySentiSE-MSR2018}. We also aim to find to what extent SEntiMoji and BERT4SentiSE agree with each other when they make incorrect predictions. 

\subsubsection{Approach} We manually analyze error categories for the misclassified sentences in cross-platform settings. We perform the analysis in three steps. \ul{First}, we randomly select 400 sentences from
the 4,188 misclassified sentences where both
BERT4SentiSE and SentiMoji were wrong. This sample size is statistically significant with a 95\%
confidence level and five intervals. We then manually label each sentence to an
error category from Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020},
who produced the categories for their study on the effectiveness of shallow
SE-specific SD tools in cross-platform settings. In this study, we used the same
7 error categories used by Novielli, but we changed one category name `Polar
facts' to `Domain specific' because what the authors considered as polar facts
are actually software domain-specific jargons that have some inherent desirable
or undesirable polarity (e.g., ``bugs'', ``issues'', ``resolved''). Two authors
participated in the error analysis process. They discussed the guideline of
categorizing the errors into different categories. The authors conducted joint
sessions in multiple iterations to determine the error category for each of the
400 sentences in our sample. % Therefore, our sample is statis
% We study the mis-classification of by randomly selecting a subset of 400 sentences that both of the DL-based classifier SEntiMoji and BERT4SentiSE misclassified. This sample size is statistically significant with 95\% confidence level (5\% confidence interval). Two of the authors participated in the error categorization process. 
\ul{Second}, we analyze our error categories with those from Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}, who 
analyzed the error categories for the two shallow learning SD tools (Senti4SD and SentiCR) in the three datasets for cross-platform 
settings, where both tools were wrong. \ul{Third}, we analyze a random sample of 70 sentences where the rule-based 
tool SentistrengthSE was wrong in the three datasets. The purpose of the analysis in steps 2 and 3 was to determine whether the error categories might differ depending on the types of the tools (i.e., deep learning vs. shallow learning vs. rule-based).

\begin{figure}[h]
	\centering\begin{tikzpicture}[scale=0.3]-
    \pie[
        /tikz/every pin/.style={align=center},
        text=pin, number in legend,
        explode=0.0,
        color={black!0, black!10, black!20, black!30,, black!40, black!50, black!60, black!70},
        ]
        {
            4/\bf{Figurative language}\\ 16 (4\%),
            29/\bf{Subjectivity in Annotation}\\ 114 (29\%),
            21/\bf{General Error}\\  82 (21\%),
            14/\bf{Implicit Sentiment}\\ 57 (14\%),
            14/\bf{Context/Pragmatics}\\ 55 (14\%),
            12/\bf{Domain Specific} \\ 49 (12\%),
            7/\bf{Politeness} \\ 27 (7\%)
        }
    \end{tikzpicture}
	\caption{Distribution of error categories by two deep learning tools (BERT4SentiSE and SentiMoji) in our 400 samples}
	\vspace{-2mm}
	\label{fig:misclassification_chart_dl}
\end{figure}

% BERT4SentiSE correctly predicts within platform settings ``finally getting somewhere( (GitHub, oracle: Positive)'' but mispredicts (neutral) in cross platform settings when trained on Stack Overflow.
% SentiMoji correctly predicts within platform settings ``bug is a duplicate of HIVE-3253. (Jira, oracle: neutral)'' but wrongly predicts (negative) in cross platform settings when trained on GitHub.
% SentiMoji makes correct prediction in within platform settings ``Fixed and I've tested it. (Jira, Oracle: neutral)''. We believe this is an example of subjective annotation. But SentiMoji overfits in within platform settings and makes wrong prediction (positive) when trained on SO dataset. But positive prediction is more suited for this example.

\subsubsection{Results} \bf{Most (29\%) of the errors in our sample where both BERT4SentiSE and SentiMoji are wrong are due to `Subjectivity in Annotation', i.e., 
inconsistency in the manual labeling.} In \fig\ref{fig:misclassification_chart_dl}, we show a pie chart to show the percentage distribution of seven error categories that we observed in the 400 samples of sentences where both BERT4SentiSE and SentiMoji were wrong across the six cross platform settings.  Most of the misclassifications (29\%) were observed due to
`Subjectivity in Annotation'. The second most observed category is `General
Error' (21\%). This distribution is slightly different from the distribution
reported by Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020} for the
shallow ML-based SD tools, where `General Error' was observed the most (68\%).
As we discuss below, a general error occurs due to the inability of the tools to
process sentences (e.g., emoticons). One of the deep learning tools in our
study, SentiMoji, is specifically designed to handle emojis better. This is why
we find much lower coverage of misclassifications related to `General Errors' in
our sample. We now discuss the error categories with examples below. 

% \gias{Instead of \tbl\ref{tab:misclassification}, use a pie chart to show the distribution of the error categories. Use your texts (like my TSE paper) to describe each error category}\gias{can we put \tbl\ref{tab:agreement} in one single column? You can use shortened name each tool reduce the width of the tabel, e.g, SenitMoji can be use Moji, BERT4SentiSE can be just BERT, Senti4SD can be just S4SD, SentiCR can be SCR, RNN4SentiSE can be just RNN. We also don't need the header row `Agreement metrics'.}
%\textbf{The error categories of PTM DL-based vs shallow ML-based vs rule-based SD tools differs.} In \fig\ref{fig:misclassification_chart}, we show the distribution of 
%the six error categories in our random sample of 400 sentences where both BERT4SentiSE and SentiMoji were wrong in cross-platform settings. Most of the misclassifications (29\%) were observed due to `Subjectivity in Annotation'. The second most observed category is `General Error' (21\%). This distribution is slightly different from the distribution reported by Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020} for the shallow ML-based SD tools, where `General Error' was observed the most (68\%). As we discuss below, a general error occurs due to the inability of the tools to process sentences (e.g., emoticons). One of the deep learning tools in our study, SentiMoji, is specifically designed to handle emojis better. This is why we find much lower coverage of misclassifications related to `General Errors' in our sample. We now discuss the error categories with examples below. From our error analysis, we find that the main cause for misclassification for the lexicon based tool SentiStrengthSE is to failure to understand domain specific context (36\%). PTM DL-based SD tools perform quite well in this category (only 12\% errors).
% shows the summary of the six error category type from our analysis. We find that subjectivity in annotation is the biggest cause for the classifier's misclassification. Now, we provide a breif description of each error category.



{\ul{Subjectivity in Annotation (29\%).}} The biggest cause of misclassification is subjectivity in annotation. Human labeling is always subjective to human annotators, even if there is a standard guideline on labeling a dataset~\cite{Novielli-SEToolCrossPlatform-MSR2020}. For example, \emt{+1 looks good.} is labeled as neutral and \emt{+1 great job pat.} is labeled as positive in the same Jira dataset. This is because sometimes a conservative rater might label sentences with mild emotions as neutral~\cite{Novielli-SEToolCrossPlatform-MSR2020}. In particular, subjectivity is quite prevalent for sentences with politeness. For example, this sentence is manually labeled as neutral, but both tools (BERT4SentiSE and SentiMoji) labeled it as positive, \emt{Thanks you for quick response}. 


{\ul{General errors (21\%).}} The inability of the tools to identify the linguistic cues can result in their misclassification of the polarity labeling. As we noted above, this error category is much less observed in our sample than Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}. Two deep learning tools perform relatively better in this category because both are pre-trained, which helps generalize the context of a sentence even when a sentence is not processed properly. In addition, SEngMoji is based on DeepMoji~\cite{deepMoji_2017}, which is good at detecting emoticons like  ``:)'' and ``:smiley:''. However, we still find misclassified cases in the datasets. For example, we find this error in GitHub dataset:\emt{Ok, this can be removed :-)}. The error happened when both tools were trained on Jira and tested on GitHub. Both tools provide correct polarity labels when they are trained using the SO dataset. We find that in the Jira dataset, there are sentences like this \emt{Vadim you're keeping us busy :).} or this \emt{Oh my stupid:)} or this \emt{Stupid user error :)}. The three sentences are manually labeled as non-positive, but the two tools label those as positive. Therefore, while we put such misclassifications under the general error category, another category would have been inconsistency in labeling datasets. 


{\ul{Implicit Sentiment (14\%)}}. The presence of implicit sentiment can confuse any SD tools, especially when the unit of analysis is a sentence with very few words (i.e., without much context). The two deep learning SD tools most misclassify such cases as neutral because the sentences do not contain any lexical cues. For example, the following two sentences are manually labeled as negative, while both SD tools label those as neutral: \begin{inparaenum}
\item \emt{This is not what I build a framework for.}
\item \emt{25 hours gone.}
\end{inparaenum} 


{\ul{Context/Pragmatics (14\%)}.} The lack of proper context or pragmatics in sentences, especially in short sentences, can make it challenging for the tools to determine the correct polarity labels. This can also be problematic when a manual labeling process also took cues from surrounding sentences of a given sentence. As Uddin et al.~\cite{Uddin-OpinionValue-TSE2019} show, lack of context can be problematic for datasets based on SO, if manual annotation of a sentence is done by looking at the entire post of the sentence in SO. For example, the following sentences are labeled as neutral by the tools but are labeled as negative in the benchmarks: \begin{inparaenum}
\item \emt{huh ... i thought i did resolve this.} (in Jira)
\item \emt{How about fixing hashcode too?} (in GitHub).
\end{inparaenum}


{\ul{Domain Specificity (12\%)}} errors occur due to the presence of SE domain-specific jargons in a sentence, which an SD tool has not observed during training. Some SE-specific jargons have inherently desirable or undesirable emotions such as ``bug'' as negative and ``patch accepted'' as positive polarity. This sentence is manually labeled as negative, but the tools predicted it as neutral: \emt{My patch wouldn't compile}. Another example is \emt{`killed that process and restarted, and it worked!}. Here, the polarity in manual labeling is positive because, in the SE context, the issue was fixed after restarting, which is a desirable outcome.
To make matters worse, these SE-specific jargons are inconsistently labeled across datasets, such as bug-related sentences in the Jira dataset are always labeled with positive or negative polarity~\cite{Novielli-SEToolCrossPlatform-MSR2020, Novielli-BenchmarkStudySentiSE-MSR2018, Novielli-SESentimentCP-EMSE2021}. However, in the other two datasets, bug-related discussions are labeled as neutral unless there is a clear expression of emotion. The following is manually labeled as negative but is predicted as neutral by both tools: \emt{The visibility is missing, and the default value seems weird}.


{\ul{Politeness (7\%).}} type errors occur due to two reasons \begin{inparaenum}[(1)]
\item sentences conveying politeness are labeled inconstantly across datasets. For example,  politeness is considered neutral in SO and GitHub datasets (e.g., \emt{Thank you})~\cite{Novielli-SEToolCrossPlatform-MSR2020}. On the other hand, in the Jira dataset, thanking expression is labeled as positive polarity (e.g., \emt{Thanks Ashish For committing the patch.}),
\item sentences with politeness are most vulnerable to subjective annotation, especially in cross-platform datasets (as we noted above under subjective annotation category).
\end{inparaenum} 


{\ul{Figurative language (4\%)}.}  errors occur due to the presence of sarcasm or expletives in sentences. For example, the following sentence is labeled as positive in the GitHub dataset, but both tools predicted it as neutral in cross-platform setting: \emt{There is a backdoor in this commit, i'll give a cookie to the one who finds it first:P}. The following sentences are labeled as neutral in the benchmarks, but the tools predicted those as neutral: \begin{inparaenum}
\item \emt{because hack shit methods must die.} (GitHub),
\item \emt{I used to be the latter, but then I went to law school and got a degree in this shit.} (Jira). 
\end{inparaenum}


\begin{figure}[h]
	\centering\begin{tikzpicture}[scale=0.3]-
    \pie[
        /tikz/every pin/.style={align=center},
        text=pin, number in legend,
        explode=0.0,
        color={black!0, black!10, black!20, black!30,, black!40, black!50, black!60, black!70},
        ]
        {
            68/\bf{General Error}  214 (68\%),
            11/\bf{Subjectivity in Annotation} 35 (11\%),
            8/\bf{Domain Specific (Polar facts)}  25 (8\%),
            6/\bf{Politeness}   19 (6\%),
            5/\bf{Implicit Sentiment} 16 (5\%),   
            2/\bf{Figurative language} 6 (2\%),
            2/\bf{Context/Pragmatics} 6 (2\%)
        }
    \end{tikzpicture}
	\caption{Distribution of error categories by Shallow SD tools (SentiCR and Senti4SD) as reported by Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}}
	\vspace{-2mm}
	\label{fig:misclassification_sentisdsenticr}
\end{figure}

\bf{The distribution of error categories in the two deep learning tools differs \it{slightly} from those observed for shallow SD tools in cross-platform settings.} 
\fig\ref{fig:misclassification_sentisdsenticr} shows the error categories in 320 sentences where both of the two shallow learning-based SD tools (Senti4SD and SentiCR) 
are wrong. We report the results from Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}, i.e., we did not analyze the 320 sentences. 
The most frequent category for the two shallow learning SD tools is `General Error', which was the second most frequent category in \fig\ref{fig:misclassification_chart_dl}, i.e., 
error categories observed for the two deep learning SD tools. The most observed error category for the two deep learning SD tools in \fig\ref{fig:misclassification_chart_dl} 
is `Subjectivity in Annotation', which is the second most observed category for the two shallow learning SD tools in \fig\ref{fig:misclassification_sentisdsenticr}. 
The difference in the distribution of error categories between the shallow learning and deep learning SD tools is due to two reasons: 
\begin{inparaenum}[(1)]
\item General errors mainly occur due to the inability of a tool to analyze non-textual contents that are useful to detect polarity (e.g., emoji). 
The two deep learning SD tools, especially SentiMoji are pre-trained on a large corpus of emojis found in Twitter. Therefore, the two deep learning SD tools 
are more resilient towards such general errors during polarity labeling in cross-platform settings.
\item The two deep learning SD tools, especially BERT4SentiSE is based on BERT. BERT is better designed to infer contexts from a sentence due to the novel use 
of transformer architecture and attention layer. Thus, BERT4SentiSE can recognize the underlying context from training data, which becomes problematic 
for sentences that are similar between the training and testing datasets but that are labeled differently between the two datasets due to the subjectivity 
in manual labeling. Thus, the deep learning SD tools suffer more from such inconsistency.
\end{inparaenum}     

\begin{figure}[h]
	\centering\begin{tikzpicture}[scale=0.3]-
    \pie[
        /tikz/every pin/.style={align=center},
        text=pin, number in legend,
        explode=0.0,
        color={black!0, black!10, black!20, black!30,, black!40, black!50, black!60, black!70},
        ]
        {
            2/\bf{Figurative language} 2 (2\%),
            39/\bf{Domain Specific}  36 (39\%),
            19/\bf{Politeness}   18 (19\%),
            16/\bf{Subjectivity in Annotation} 15 (16\%),
            14/\bf{General Error}  13 (14\%),
            5/\bf{Context/Pragmatics} 5 (5\%),
            4/\bf{Implicit Sentiment} 4 (4\%)
        }
    \end{tikzpicture}
	\caption{Distribution of error categories by the rule-based tool (SentiStrengthSE) in our 93 samples}
	\vspace{-2mm}
	\label{fig:misclassification_sentistrengthse}
\end{figure}
% In some cases, a sentence might be labelled by positive/negative by a annotator by neutral by another annotator. Another critical part is labelling guideline in the Jira dataset is quite different from than other two datasets. For example, non-sentiment facts (e.g., ``This is a bug'') are labelled as neutral in GitHub and Stack Overflow dataset. However, it was labelled with `Negative' polarity in the Jira dataset. Another significant discrepancy is the guideline for politeness. Politeness (e.g., ``Thanks'', ``Sorry'') are labelled with positive/negative polarity in the Jira dataset but neutral in the other two datasets. If a deep learning tool is trained on GitHub dataset and tested on Jira where the Oracle is different for these type of sentences, might confuse the deep learning sentiments tools to underperform. Previous studies~\cite{Novielli-SEToolCrossPlatform-MSR2020} suggest there are around 6\% with politeness labelling and around 8\% sentences are with polarity facts.

\textbf{Lack of understanding of context and underlying domain specificity contributes to the most error in rule-based SD tool SentistrengthSE.} 
In our three datasets, SentiStrengthSE misclassifies 3,470 sentences, out of which we randomly sample 
93 sentences for manual analysis of error categories. This sample is statistically significant with a 95\% confidence level with 10 confidence interval. 
Figure \ref{fig:misclassification_sentistrengthse} shows the highlight
of the error misclassification for SentiStrengthSE. 
From our
error analysis, we find that the main cause for misclassification for the
lexicon-based tool SentiStrengthSE is failure to understand domain-specific
context (39\%). PTM DL-based SD tools perform quite well in this category (only
12\% errors).  Some examples of errors by SentistrengthSE related to `domain specificity' are:  ``Confirm, this breaks compile. :( (GitHub)'', ``ROT13. It's
super efficient too! (Stack Overflow)''). Inconsistent labeling guideline is
the second biggest cause of errors (19\%): politeness such as ``Thanks'',
``Thank you, some\_name'' is always predicted as positive polarity by
SentiStrengthSE but in Jira dataset, politeness is not annotated as positive
unless there is a clear expression of emotions. The third categories of errors
belong to subjective annotation (16\%). The fourth error category is General categories (14\%), i.e., inability to understand linguistic
cues (e.g., ``+1  Patch looks nice.'' ``:+1: for speed!",  ``ya +1 for clearer
code comment :D") this type of language cues are not detected by the
SentiStrengthSE. 

\textbf{When both the two best performing deep learning SD tools (BERT4SentiSE and SentiMoji) have severe disagreement with manual labeling, 
most of the time, it is due to subjectivity in manual labeling.}
From Table \ref{tab:agreement_with_manual_labelling} we see in cross-platform
settings when trained on Stack Overflow and test on GitHub dataset both the
pretrained DL-based SD tools SentiMoji and BERT4SentiSE have the highest severe
disagreement with manual labeling (2\% and 3\% respectively). In order to
better understand the issues, we investigate a little further. We find 74 samples
in GitHub dataset where but BERT4SentiSE and SentiMoji have severe disagreement
with the manual labeling, i.e., if the manual labeling for a particular
sentence is positive, then both the SD tools have predicted negative and vice
versa. After manually categorizing these 74 samples into the seven error
categories, we find that 45 samples (i.e., 61\%) actually have subjective
annotation. That means we do agree with the manual labeling assigned to
those samples, and rather we think the tools' predictions are correct. For
example, ``God I am awful at this :)'' and ``It's quite a bad practice to do so
:)'' are labeled as positive, but both the tools predicted negative for this and
we agree with this. These errors can be fixed by following standard annotation
guidelines.
We also find that in 16 (i.e., 22\%) cases, both tools have made failed to understand
implicit sentiments in sentences. For example,``Thanks for this, but things are
about to explode for me. :( (GitHub, negative)'' and ``yea,right..silly me for
not checking another commits..sorry : (GitHub, positive)''. We find 10 (i.e., 14\%) cases the tools make mistakes because of not properly
understanding software domain concepts. For example, ``Great, again
client freezes ....''. Both the tools have predicted positive for the sample
where the correct prediction should be negative. Our analysis shows the tools
failed to understand SE-domain specific terms such as ``fix'', ``hang'',
``difficult to use a library''. 
%When the tools were trained they did not learn
%this from the dataset. More examples like this might improve SD tools
%performance.

\begin{figure}[h]
\centering
\includegraphics[scale=0.53]{res/barchart_error_complement.png}
% \includegraphics[width=0.35 * linewidth]{res/methology_overview.jpg}
\caption{Misclassifications by both BERT4SentiSE and SentiMoji in \fig\ref{fig:misclassification_chart_dl} that can be corrected by at least one non-deep learning SD tool}
\label{fig:distribution_error_complement}
\end{figure}
\bf{Around 45\% of the misclassified sentences where both deep learning SD tools (BERT4SentiSE, SentiMoji) are wrong, can be corrected by the 
non-deep learning SD tools.}  \fig\ref{fig:distribution_error_complement} shows whether and how each of the 400 sentences in our sample from \fig\ref{fig:misclassification_chart_dl} 
where both of the deep learning SD tools (BERT4SentiSE, SentiMoji), can be corrected by the other three non-deep learning SD tools in our study. 
Most of the general errors by the two deep learning SD tools can be corrected by the non-deep learning SD tools. We found that this is because of the data pre-processing error, e.g., the in-built Tokenizer module in the deep learning SD tools was wrong in some cases to handle emoticons. The shallow learning SD tool SentiCR uses a pre-defined dictionary of emoticons that compensate for many such errors. Overall, the 
deep learning SD tools could benefit from the correct classifications from the non-deep learning SD tools across all seven error categories. 


%\gias{Here we need to compare the above categories to those found by Novielli in their SD tools for cross platform. First, we need to tell the distribution of the error categories they observed and how ours differ from them or similar to them. Then we need to show a bar chart where for each error category we observed above, how many of those could have been correctly classified by one of the SD tools or the rule-based tool. This would then serve also as the motivation for the next RQ}

\begin{tcolorbox}[flushleft upper,boxrule=1pt,arc=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=white,after=\ignorespacesafterend\par\noindent]
\bf{RQ$_4$ What are the error categories of the tools in the cross-platform settings?}
Subjectivity in annotation is responsible for the most amount of errors in our
sample of 400 cases where both BERT4SentiSE and SentiMoji were wrong in
cross-platform settings. We also observed inconsistent cases between datasets
(i.e., similar sentences labeled differently between datasets). General errors are the most prevalent for sentences where 
both shallow learning SD tools (Senti4SD, SentiCR) are wrong. For the rule-based tool SentistrengthSE, lack of understanding of underlying context/domain 
contributed to the most amount of errors.   
% In stead of
% high performance of rule-based tool (SentiStrengthSE), it fails to understand
% software specific context and general linguistic cues.
% Even after following theoretical guideline for labelling, manual labelling are subjective and it is the biggest source of miss-classification we noticed, followed by general errors that happened as the tools were not good enough to capture the correct sentiment. Based on the research goals politeness and SE-domain jargons are inconstantly labelled across datasets.
% \gias{summarize}
% Main reasons of misclassification is the tool's inability to generalize the input sentence. Another issue is annotation guideline for sentences with facts and politeness is different is Jira and (Stack Overflow/GitHub) dataset, this might cause the deep learning models to misclassify when they are tested in cross platform settings. 
\end{tcolorbox}


==> SubmissionTOSEM/RQ4.tex <==

%\input{RQ4_tables}
\subsection{RQ$_5$ To what extent the deep learning and non-deep learning sentiment detection tools can complement each other in cross-platform settings?}\label{sec:cross-platform-agreement}
\subsubsection{Motivation}
Our findings from RQ1 and RQ2 denote that the supervised SD tools suffer from a drop in performance in cross-platform settings. Our manual analysis of misclassifications by the tools in RQ4 shows that 
the errors can be seven types with general errors, subjectivity in annotation, and domain specificity 
being the most prevalent error categories across the tools.  
The SD tools are designed using different techniques and based on different platforms, e.g., SentistrengthSE was designed by primarily analyzing code reviews in Jira while 
SentiMoji uses emojis collected from forums like Twitter. Intuitively, given the diversity of how the tools are designed, the tools can complement each other. Indeed, \fig\ref{fig:distribution_error_complement} in RQ4 shows that 
the non-deep learning SD tools can complement the deep learning SD tools by correcting many of the misclassified cases 
where both of the top two deep learning SD tools (BERT4SentiSE and SentiMoji) are wrong. 
Therefore, it is important to know whether we could reduce the drop in performance in the SD tools 
in cross-platform settings by allowing the tools to complement each other, e.g., by taking 
the final polarity decision of a given sentence based on the polarity labels from multiple SD tools. 

% From the error analysis of RQ3, we find that our benchmark dataset suffer from
% subjectivity in annotation and different annotation guideline across the
% cross-platform datasets. We found that around 29\% error are due to subjectivity
% in annotation and around 7\% error are due to inconsistency is labelling
% guideline towards sentences with politeness. Now, we intend to explore to what
% extent these tools agree and disagree with manual labelling. We want to explore
% to what extent the tools have mild and severe disagreement with oracle
% labelling. This provide more insight for future researchers about the annotation
% inconsistency across datasets. We also want to explore to what extend these
% tools agree and disagree with each other. We also want to find out to what
% extent these tools strongly disagree with each other, i.e., predicting opposite
% polarity. This will help us to better understand the internal working mechanisms
% (i.e., features) of these machine learning classifiers. This similarity between
% tools might be useful to create an ensemble of of SD tools. We want to build a
% simple majority based ensemble tools with the subset of the studied tools and
% explore if their internal working mechanism provides a better result.


\begin{sidewaystable}
\caption{This is a test}
\vspace{15cm}
% \hvFloat[rotAngle=90,nonFloat=true,capWidth=w]
% \begin{table}
\parbox{.32\linewidth}{
\renewcommand{\thetable}{\arabic{table}a}
  \footnotesize
%   \small
  \centering
  \caption{Agreement between tools. Test in GitHub (G). Mji = SentiMoji Brt = BERT4SentiSE K = Cohen $\kappa$}
    \begin{tabular}{clrr|rr}
    \toprule
    \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagree}}\\
    \cmidrule{3-6}
    & & {\bf{$\kappa$}} & {\textbf{P}} & \textbf{S} & \textbf{M} \\
    \midrule
\multirow{15}{*}{G (W)} 
% ==========================  within setting GitHub =========
 & Mji vs Brt & 0.86 & 91\% & 1\% & 8\%  \\
 & Mji vs Rnn & 0.52 & 68\% & 7\% & 25\%  \\
 & Mji vs S4D & 0.83 & 89\% & 1\% & 10\%  \\
 & Mji vs SCr & 0.76 & 85\% & 2\% & 13\%  \\
 & Mji vs SSt & 0.68 & 79\% & 2\% & 18\%  \\
 & Brt vs Rnn & 0.53 & 69\% & 7\% & 24\%  \\
 & Brt vs S4D & 0.85 & 90\% & 2\% & 8\%  \\
 & Brt vs SCr & 0.74 & 83\% & 2\% & 14\%  \\
 & Brt vs SSt & 0.68 & 80\% & 2\% & 18\%  \\
 & Rnn vs S4D & 0.52 & 69\% & 7\% & 25\%  \\
 & Rnn vs SCr & 0.43 & 63\% & 7\% & 31\%  \\
 & Rnn vs SSt & 0.44 & 63\% & 6\% & 31\%  \\
 & S4D vs SCr & 0.74 & 83\% & 2\% & 14\%  \\
 & S4D vs SSt & 0.67 & 79\% & 3\% & 18\%  \\
 & SCr vs SSt & 0.63 & 77\% & 3\% & 21\%  \\
\midrule


\multirow{15}{*}{S(C)} 
% ...........test dataset: GitHub train_dataset: DatasetSenti4SDSO  .........
 & Mji vs Brt & 0.72 & 83\% & 1\% & 15\%  \\
 & Mji vs Rnn & 0.58 & 76\% & 2\% & 22\%  \\
 & Mji vs S4D & 0.51 & 70\% & 3\% & 27\%  \\
 & Mji vs SCr & 0.40 & 68\% & 2\% & 30\%  \\
 & Mji vs SSt & 0.57 & 74\% & 2\% & 25\%  \\
 & Brt vs Rnn & 0.59 & 76\% & 2\% & 22\%  \\
 & Brt vs S4D & 0.52 & 70\% & 4\% & 26\%  \\
 & Brt vs SCr & 0.39 & 66\% & 3\% & 31\%  \\
 & Brt vs SSt & 0.61 & 76\% & 2\% & 22\%  \\
 & Rnn vs S4D & 0.43 & 65\% & 4\% & 31\%  \\
 & Rnn vs SCr & 0.30 & 62\% & 3\% & 35\%  \\
 & Rnn vs SSt & 0.48 & 68\% & 3\% & 29\%  \\
 & S4D vs SCr & 0.45 & 68\% & 2\% & 30\%  \\
 & S4D vs SSt & 0.55 & 72\% & 3\% & 25\%  \\
 & SCr vs SSt & 0.45 & 68\% & 2\% & 31\%  \\
\midrule


\multirow{15}{*}{J(C)} 
% ...........test dataset: GitHub train_dataset: OrtuJIRA  .........
 & Mji vs Brt & 0.78 & 90\% & 0\% & 10\%  \\
 & Mji vs Rnn & 0.54 & 81\% & 1\% & 19\%  \\
 & Mji vs S4D & 0.60 & 82\% & 1\% & 18\%  \\
 & Mji vs SCr & 0.65 & 87\% & 0\% & 13\%  \\
 & Mji vs SSt & 0.46 & 69\% & 0\% & 30\%  \\
 & Brt vs Rnn & 0.56 & 81\% & 1\% & 18\%  \\
 & Brt vs S4D & 0.60 & 81\% & 1\% & 18\%  \\
 & Brt vs SCr & 0.67 & 87\% & 0\% & 13\%  \\
 & Brt vs SSt & 0.51 & 71\% & 1\% & 28\%  \\
 & Rnn vs S4D & 0.44 & 74\% & 2\% & 24\%  \\
 & Rnn vs SCr & 0.45 & 79\% & 1\% & 20\%  \\
 & Rnn vs SSt & 0.36 & 63\% & 2\% & 34\%  \\
 & S4D vs SCr & 0.52 & 79\% & 1\% & 20\%  \\
 & S4D vs SSt & 0.48 & 70\% & 2\% & 29\%  \\
 & SCr vs SSt & 0.39 & 66\% & 0\% & 34\%  \\

    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:agreement_test_github}%
% \end{table}%
% \end{sidewaystable}
}
% \begin{sidewaystable}
% \vspace{15cm}
% \begin{table}
\hfill
\parbox{.32\linewidth}{
\addtocounter{table}{-1}
\renewcommand{\thetable}{\arabic{table}b}
  \footnotesize
%   \small
  \centering
  \caption{Agreement between tools. Test in SO (S). S4D = Senti4SD, Scr = SentiCR, P = Percent Agreement}
    \begin{tabular}{clrr|rr}
    \toprule
    \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagree}}\\
    \cmidrule{3-6}
    & & {\bf{$\kappa$}} & {\textbf{P}} & \textbf{S} & \textbf{M} \\
    \midrule

\multirow{15}{*}{ S (W)} 
% ==========================  within setting DatasetSenti4SDSO =========
 & Mji vs Brt & 0.86 & 91\% & 1\% & 8\%  \\
 & Mji vs Rnn & 0.70 & 80\% & 3\% & 17\%  \\
 & Mji vs S4D & 0.81 & 88\% & 1\% & 12\%  \\
 & Mji vs SCr & 0.78 & 85\% & 2\% & 12\%  \\
 & Mji vs SSt & 0.72 & 81\% & 1\% & 17\%  \\
 & Brt vs Rnn & 0.71 & 81\% & 2\% & 17\%  \\
 & Brt vs S4D & 0.83 & 88\% & 1\% & 11\%  \\
 & Brt vs SCr & 0.78 & 85\% & 3\% & 12\%  \\
 & Brt vs SSt & 0.72 & 81\% & 1\% & 18\%  \\
 & Rnn vs S4D & 0.70 & 80\% & 3\% & 17\%  \\
 & Rnn vs SCr & 0.65 & 77\% & 4\% & 19\%  \\
 & Rnn vs SSt & 0.63 & 75\% & 3\% & 21\%  \\
 & S4D vs SCr & 0.78 & 85\% & 3\% & 12\%  \\
 & S4D vs SSt & 0.73 & 82\% & 1\% & 17\%  \\
 & SCr vs SSt & 0.70 & 81\% & 2\% & 17\%  \\

\midrule

\multirow{15}{*}{ G (C)} 
 % ...........test dataset: DatasetSenti4SDSO train_dataset: GitHub  .........
 & Mji vs Brt & 0.79 & 86\% & 1\% & 13\%  \\
 & Mji vs Rnn & 0.53 & 70\% & 4\% & 27\%  \\
 & Mji vs S4D & 0.70 & 80\% & 3\% & 17\%  \\
 & Mji vs SCr & 0.62 & 75\% & 5\% & 20\%  \\
 & Mji vs SSt & 0.67 & 79\% & 1\% & 20\%  \\
 & Brt vs Rnn & 0.53 & 69\% & 5\% & 26\%  \\
 & Brt vs S4D & 0.73 & 82\% & 2\% & 16\%  \\
 & Brt vs SCr & 0.60 & 74\% & 5\% & 21\%  \\
 & Brt vs SSt & 0.69 & 79\% & 1\% & 20\%  \\
 & Rnn vs S4D & 0.54 & 69\% & 4\% & 26\%  \\
 & Rnn vs SCr & 0.40 & 61\% & 6\% & 33\%  \\
 & Rnn vs SSt & 0.48 & 66\% & 4\% & 30\%  \\
 & S4D vs SCr & 0.58 & 73\% & 4\% & 23\%  \\
 & S4D vs SSt & 0.65 & 77\% & 1\% & 22\%  \\
 & SCr vs SSt & 0.56 & 71\% & 4\% & 25\%  \\
\midrule


\multirow{15}{*}{ J (C)} 
% ...........test dataset: DatasetSenti4SDSO train_dataset: OrtuJIRA  .........
 & Mji vs Brt & 0.66 & 82\% & 0\% & 18\%  \\
 & Mji vs Rnn & 0.47 & 75\% & 1\% & 23\%  \\
 & Mji vs S4D & 0.60 & 81\% & 1\% & 19\%  \\
 & Mji vs SCr & 0.56 & 80\% & 1\% & 19\%  \\
 & Mji vs SSt & 0.49 & 68\% & 0\% & 31\%  \\
 & Brt vs Rnn & 0.43 & 70\% & 2\% & 28\%  \\
 & Brt vs S4D & 0.57 & 77\% & 1\% & 22\%  \\
 & Brt vs SCr & 0.52 & 75\% & 1\% & 25\%  \\
 & Brt vs SSt & 0.60 & 75\% & 0\% & 25\%  \\
 & Rnn vs S4D & 0.42 & 72\% & 2\% & 27\%  \\
 & Rnn vs SCr & 0.33 & 70\% & 1\% & 29\%  \\
 & Rnn vs SSt & 0.36 & 60\% & 3\% & 36\%  \\
 & S4D vs SCr & 0.51 & 77\% & 1\% & 22\%  \\
 & S4D vs SSt & 0.46 & 66\% & 1\% & 33\%  \\
 & SCr vs SSt & 0.40 & 63\% & 1\% & 36\%  \\

% \midrule

    \bottomrule
    \end{tabular}%
  \label{tab:agreement_test_so}%
% \end{table}%
% \end{sidewaystable}
}
\hfill
\parbox{.32\linewidth}{
% \begin{sidewaystable}
% \begin{table}[]
  \addtocounter{table}{-1}
  \renewcommand{\thetable}{\arabic{table}c}
  \footnotesize
%   \small
  \centering
  \caption{Agreement between tools. Test in Jira (J). SSt = SentistrengthSE, C, W = Cross, Within-Platform}
    \begin{tabular}{clrr|rr}
    \toprule
    \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagree}}\\
    \cmidrule{3-6}
    & & {\bf{$\kappa$}} & {\textbf{P}} & \textbf{S} & \textbf{M} \\
    \midrule

\multirow{15}{*}{ J (W)} 
% ==========================  within setting OrtuJIRA =========
 & Mji vs Brt & 0.85 & 93\% & 0\% & 7\%  \\
 & Mji vs Rnn & 0.68 & 86\% & 0\% & 14\%  \\
 & Mji vs S4D & 0.72 & 87\% & 0\% & 13\%  \\
 & Mji vs SCr & 0.81 & 91\% & 0\% & 9\%  \\
 & Mji vs SSt & 0.75 & 87\% & 0\% & 13\%  \\
 & Brt vs Rnn & 0.68 & 85\% & 1\% & 14\%  \\
 & Brt vs S4D & 0.72 & 87\% & 0\% & 13\%  \\
 & Brt vs SCr & 0.79 & 90\% & 0\% & 10\%  \\
 & Brt vs SSt & 0.75 & 87\% & 0\% & 13\%  \\
 & Rnn vs S4D & 0.61 & 83\% & 0\% & 17\%  \\
 & Rnn vs SCr & 0.70 & 86\% & 1\% & 14\%  \\
 & Rnn vs SSt & 0.63 & 81\% & 1\% & 18\%  \\
 & S4D vs SCr & 0.70 & 86\% & 0\% & 13\%  \\
 & S4D vs SSt & 0.67 & 83\% & 1\% & 16\%  \\
 & SCr vs SSt & 0.77 & 88\% & 1\% & 11\%  \\
\midrule

\multirow{15}{*}{ G (C)} 
% ...........test dataset: OrtuJIRA train_dataset: GitHub  .........
 & Mji vs Brt & 0.81 & 89\% & 1\% & 10\%  \\
 & Mji vs Rnn & 0.56 & 72\% & 3\% & 25\%  \\
 & Mji vs S4D & 0.72 & 84\% & 1\% & 14\%  \\
 & Mji vs SCr & 0.75 & 86\% & 1\% & 13\%  \\
 & Mji vs SSt & 0.75 & 86\% & 1\% & 13\%  \\
 & Brt vs Rnn & 0.57 & 73\% & 3\% & 24\%  \\
 & Brt vs S4D & 0.73 & 85\% & 1\% & 14\%  \\
 & Brt vs SCr & 0.75 & 87\% & 1\% & 13\%  \\
 & Brt vs SSt & 0.75 & 86\% & 1\% & 13\%  \\
 & Rnn vs S4D & 0.52 & 70\% & 3\% & 27\%  \\
 & Rnn vs SCr & 0.50 & 69\% & 2\% & 28\%  \\
 & Rnn vs SSt & 0.54 & 71\% & 2\% & 27\%  \\
 & S4D vs SCr & 0.68 & 83\% & 1\% & 16\%  \\
 & S4D vs SSt & 0.70 & 83\% & 1\% & 16\%  \\
 & SCr vs SSt & 0.76 & 87\% & 1\% & 12\%  \\
\midrule


\multirow{15}{*}{ S (C)} 
% ...........test dataset: OrtuJIRA train_dataset: DatasetSenti4SDSO  .........
 & Mji vs Brt & 0.80 & 89\% & 1\% & 10\%  \\
 & Mji vs Rnn & 0.70 & 84\% & 1\% & 15\%  \\
 & Mji vs S4D & 0.61 & 79\% & 1\% & 19\%  \\
 & Mji vs SCr & 0.35 & 70\% & 1\% & 29\%  \\
 & Mji vs SSt & 0.77 & 87\% & 1\% & 12\%  \\
 & Brt vs Rnn & 0.72 & 84\% & 1\% & 14\%  \\
 & Brt vs S4D & 0.60 & 79\% & 2\% & 19\%  \\
 & Brt vs SCr & 0.36 & 71\% & 1\% & 28\%  \\
 & Brt vs SSt & 0.77 & 87\% & 1\% & 12\%  \\
 & Rnn vs S4D & 0.56 & 77\% & 2\% & 22\%  \\
 & Rnn vs SCr & 0.30 & 67\% & 1\% & 32\%  \\
 & Rnn vs SSt & 0.70 & 83\% & 1\% & 16\%  \\
 & S4D vs SCr & 0.41 & 76\% & 1\% & 23\%  \\
 & S4D vs SSt & 0.59 & 78\% & 2\% & 20\%  \\
 & SCr vs SSt & 0.34 & 70\% & 1\% & 29\%  \\
% \midrule
    % \midrule  
    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:agreement_test_jira}%
 }
% \end{table}%
\end{sidewaystable}
\begin{figure*}[t]
\centering
\captionsetup[subfigure]{labelformat=empty}
\pgfplotstableread{
1	.78 .78 .80 .79 .75 .82 .79 .80      .80 .78 .80 .81 .76 .82 .78 .80    .85 .75 .81 .85 .77 .84 .80 .82     .85 .78 .82 .85 .77 .84 .81 .83    .79 .61 .70 .75 .73 .74 .73 .72    .76 .61 .68 .72 .71 .70 .70 .69
2	.78 .80 .81 .68 .69 .81 .80 .81      .80 .80 .81 .80 .79 .82 .81 .81    .79 .81 .83 .78 .68 .82 .80 .83     .80 .80 .82 .84 .75 .82 .80 .82    .79 .69 .72 .76 .61 .75 .73 .74    .76 .67 .69 .74 .62 .72 .70 .71
}\datatable
\pgfplotscreateplotcyclelist{xcolor}{%
red!60, orange, yellow, blue!50, brown, violet, purple, black!60
}

\edef\mylst{"a", "b", "c", "d", "e", "f", "g", "h"}

      \subfloat[Test on GitHub (F1 score)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
      
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Trained on SO\\(Baseline: SentiStrengthSE), Trained on Jira\\(Baseline: SentiStrengthSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.5,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        % 	nodes near coords=\pgfmathsetmacro{\mystring}{{\mylst}[\coordindex]}\mystring,
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=1] \datatable;
        % 	\node [above] at (axis cs:  100,  92.021) {a};
        	\addplot table[x index=0,y index=2] \datatable;
        % 	\node [above] at (axis cs:  100,  92.021) {b};
        	\addplot table[x index=0,y index=3] \datatable;
        	\addplot table[x index=0,y index=4] \datatable;
            \addplot table[x index=0,y index=5] \datatable;
        	\addplot table[x index=0,y index=6] \datatable;
        	\addplot table[x index=0,y index=7] \datatable;
        	\addplot table[x index=0,y index=8] \datatable;

            % \foreach \Point [count=\i] in {
            %     1, 2, 3, 4, 5, 6, 7, 8
            % }{
            % %  \node[dot,label=\i] at \Point {};
            %  \addplot table[x index=0,y index=\Point] \datatable node[above] {a};
            % %  \node[above] at ($(axis cs:table[x index=0,y index=\Point] \datatable$) {200};
            %  \node[label=\i] at (table[x index=0,y index=\Point] \datatable) {};
            % %  \node [above,color=black] at (endofplotsquare) {a};
            % }

            \legend{Baseline,
            		 Majority-All, , ,
                     Majority-Shallow ML,
                     Majority-PMT DL + Rule, , ,
            		 }
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } 
    \subfloat[Test on GitHub (Precision)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Trained on SO\\(Baseline: SentiStrengthSE), Trained on Jira\\(Baseline: SentiStrengthSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.50,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=9] \datatable;
        	\addplot table[x index=0,y index=10] \datatable;
        	\addplot table[x index=0,y index=11] \datatable;
        	\addplot table[x index=0,y index=12] \datatable;
            \addplot table[x index=0,y index=13] \datatable;
        	\addplot table[x index=0,y index=14] \datatable;
        	\addplot table[x index=0,y index=15] \datatable;
        	\addplot table[x index=0,y index=16] \datatable;

            \legend{, , Majority-All (Except RNN4SentiSE),
            		 Majority-PMT DL, , ,
                     Majority-Shallow ML + Rule,
                     Majority-BTPC
            		}
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } \\
    
    \subfloat[Test on Stack Overflow (SO) (F1 score)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub\\(Baseline: BERT4SentiSE), Train on Jira\\(Baseline: BERT4SentiSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.5,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=17] \datatable;
        	\addplot table[x index=0,y index=18] \datatable;
        	\addplot table[x index=0,y index=19] \datatable;
        	\addplot table[x index=0,y index=20] \datatable;
            \addplot table[x index=0,y index=21] \datatable;
        	\addplot table[x index=0,y index=22] \datatable;
        	\addplot table[x index=0,y index=23] \datatable;
        	\addplot table[x index=0,y index=24] \datatable;

            % \legend{Baseline, ,
            % 		 Majority-All,
            % 		 Majority-All (Except RNN4SentiSE),
            % 		 Majority-PMT DL,
            % 		 }
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } 
    \subfloat[Test on Stack Overflow (SO) (Precision)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub\\(Baseline: BERT4SentiSE), Train on Jira\\(Baseline: BERT4SentiSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.50,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=25] \datatable;
        	\addplot table[x index=0,y index=26] \datatable;
        	\addplot table[x index=0,y index=27] \datatable;
        	\addplot table[x index=0,y index=28] \datatable;
            \addplot table[x index=0,y index=29] \datatable;
        	\addplot table[x index=0,y index=30] \datatable;
        	\addplot table[x index=0,y index=31] \datatable;
        	\addplot table[x index=0,y index=32] \datatable;

            % \legend{, , , ,
            %          Majority-Shallow ML,
            %          Majority-PMT DL + Rule,
            %          Majority-Shallow ML + Rule,
            %          Majority-BTP
            % 		}
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } \\
    
    \subfloat[Test on Jira (F1 score)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub\\(Baseline: SentiStrengthSE), Train on SO\\(Baseline: SentiStrengthSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.5,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=33] \datatable;
        	\addplot table[x index=0,y index=34] \datatable;
        	\addplot table[x index=0,y index=35] \datatable;
        	\addplot table[x index=0,y index=36] \datatable;
            \addplot table[x index=0,y index=37] \datatable;
        	\addplot table[x index=0,y index=38] \datatable;
        	\addplot table[x index=0,y index=39] \datatable;
        	\addplot table[x index=0,y index=40] \datatable;

            % \legend{Baseline, ,
            % 		 Majority-All,
            % 		 Majority-All (Except RNN4SentiSE),
            % 		 Majority-PMT DL,
            % 		 }
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } 
    \subfloat[Test on Jira (Precision)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub\\(Baseline: SentiStrengthSE), Train on SO\\(Baseline: SentiStrengthSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.50,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=41] \datatable;
        	\addplot table[x index=0,y index=42] \datatable;
        	\addplot table[x index=0,y index=43] \datatable;
        	\addplot table[x index=0,y index=44] \datatable;
            \addplot table[x index=0,y index=45] \datatable;
        	\addplot table[x index=0,y index=46] \datatable;
        	\addplot table[x index=0,y index=47] \datatable;
        	\addplot table[x index=0,y index=48] \datatable;

            % \legend{, , , ,
            %          Majority-Shallow ML,
            %          Majority-PMT DL + Rule,
            %          Majority-Shallow ML + Rule,
            %          Majority-BTP
            % 		}
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } \\
    
%\vspace{-5mm}
\caption{Performance comparison of majority voting based ensemble tools with the SD tools (All- All of the SD tools except baseline DL-RNN4SEntiSE, BTPC-Best SD tool from PMT DL-based (BERT4SentiSE), Shallow ML-based (Senti4SD), Rule-based (SentiStrengthSE)}


%\vspace{-5mm}
\label{fig:ensemble_result}
\end{figure*}

\subsubsection{Approach} We investigate different combinations of the tools within a majority-based 
voting technique to understand whether and how the tools can complement each other. The purpose is to learn whether such combinations can reduce the drop in performance of the tools in cross-platform settings. 
This means that if we have three tools (e.g., all three deep learning SD tools) as a 
combination, we first take the polarity labels of the three tools for a given sentence and then assign the sentence the 
polarity label that is found in the most number of the tools (i.e., at least 2 tools). 
To understand the different combinations of the tools, we compute the agreement and disagreement 
between the tools in our study for both within and cross-platform settings across the three studied datasets. 
We compute the agreements between two tools for a given setting and a dataset using Cohen $\kappa$ and Percent Agreement. We compute the disagreements using two metrics: Severe and Mild. The metrics are explained in RQ2 (\tbl\ref{tab:agreement_with_manual_labelling}).
Based on the analysis, we investigate seven different combinations of the tools in our majority voting technique:
\begin{itemize}
  \item Majority-All: Majority voting based on SentiMoji, BERT4SentiSE, RNN4SentiSE, Senti4SD, SentiCR, and SentiStrengthSE.
  \item Majority-All except RNN4SentiSE.
  \item Majority-PMT DL: The two best performing deep learning SD tools ( SentiMoji and BERT4SentiSE). 
  \item Majority-Shallow ML: The two best performing shallow learning SD tools (Senti4SD and SentiCR).
  \item Majority-PMT DL + Rule: The two best performing deep learning SD tools plus the rule-based SD tool: (SentiMoji, BERT4SentiSE, and SentiStrengthSE).
  \item Majority-Shallow ML + Rule: The two shallow learning SD tools plus the rule-based SD tool (Senti4SD, SentiCR, and SentiStrengthSE).
  \item Majority-BTPC: The best performing deep learning, shallow learning, and rule-based SD tools: (BERT4SentiSE, Senti4SD, and SentiStrengthSE).
\end{itemize}   
We compute and report the precision, recall and F1-score of each combination across the six cross-platform settings. 
% In order to find the agreement between a pair of the DL-based classifiers, and
% agreement between the classifier and the manual labelling, we use widely used
% Cohen Kappa~\cite{cohen1968weighted} ($K$). Following related
% works~\cite{viera2005understanding, novielli2020can, jongeling2017negative}, we
% interpret the values of $K$ as: agreement is slight if $0.01 \leqslant K
% \geqslant 0.20$, fair if $0.21 \leqslant K \geqslant 0.40$, moderate if $0.41
% \leqslant K \geqslant 0.60$, substantial if $0.61 \leqslant K \geqslant 0.80$,
% almost perfect if $0.81 \leqslant K \geqslant 1.00$.
% 
% We also report the percentage of cases where the tools are in perfect agreement. When the classifiers disagree with each other, we report further analysis on severe and mild disagreement. Severe disagreement occurs when the prediction of the classifiers belongs to opposite polarity classes. Mild disagreement happens when one classifier predicts positive and negative polarity and the tool's prediction is neutral and vice versa.
% 
% 
% We report the performance of a majority voting based ensemble tool. Here the a numeric value is assigned for the prediction of each tool in the ensemble. For example, for positive prediction 1 point, negative prediction -1 and for neutral prediction 0 point is assigned. The prediction point for the tools is aggregated and if it is greater than 0 then the final prediction is positive, if it is less than 0 then final prediction is negative else the final prediction is neutral. In Majority-All, the output of all the tools are considered except RNN4SentiSE because it was only studied as a baseline tool to compare the performance with PTM DL-based tools. Majority-BTPC, Best Tool Per settings, best performing tool from each type DL-based, Shallow ML-based, Ruled based tool is selected. So, in our case BERT4SentiSE, Senti4SD and SentiStrengthSE is used.

\subsubsection{Results}%\gias{here remove RNN4SentiSE from all the results table and texts, given that we don't include RNN4SentiSE after current RQ1 that I just introduced}
% Alamin: agreement with manual labelling should probably be moved to RQ3 because it provides good error analysis
\textbf{The two best performing deep learning SD tools (BERT4SentiSE, SentiMoji) have the highest level of agreement and lowest level disagreement between them among all the six SE-specific SD tools in our study.} In Table~\ref{tab:agreement_test_github},~\ref{tab:agreement_test_so}, and~\ref{tab:agreement_test_jira}, we report the paired comparisons of agreement of
each pair of classifiers. It shows that the SEntiMoji and BERT4SentiSE have the
highest agreement between themselves. They also have the highest percentage of
perfect agreement and the lowest percentage of severe disagreement. Both
SentiMoji and BERT4SentiSE are pre-trained models. They already have an
understanding of languages. These tools are retrained for specific tasks. Both
of them have high performance in terms of correctly predicting polarity.
Conversely, RNN4SentiSE and SentiCR have the lowest agreement between them.

\textbf{A majority voting based ensemble based on the two best performing deep learning SD tools (BERT4SentiSE + SentiMoji) or the two best performing deep learning SD tools (BERT4SentiSE + SentiMoji) 
+ Rule-based tool (SentistrengthSE) provides slightly better performance than the stand-alone SD tools in cross-platform settings.}
\fig\ref{fig:ensemble_result} shows the performance of the seven majority voting-based
combinations in our six cross-platform settings. For each setting, we report the performance of each of the seven combinations (hereafter called as ensemblers) and 
the best performing stand-along SD (denoted as the baseline in \fig\ref{fig:ensemble_result}). For each setting, we report two performance metrics: Precision and Macro F1-score. For example, the topmost row in \fig\ref{fig:ensemble_result} 
shows the Macro F1 score and precision for the baselines and the seven ensemblers when they are tested on GitHub after they are trained on either SO or Jira. The leftmost eight bars show the Macro F1 scores of baseline + seven ensemblers when the tools 
are trained on SO and tested on GitHub. We also note the name of baseline under the eight bars, which in this case is SentistrengthSE. 
In this case, we see that an ensemble of the two best performing deep learning SD tools (BERT4SentiSE, SentiMoji) and SentistrengthSE 
offers the best Macro F1-score of 0.82 out of the baseline and the ensemblers. Overall, in terms of Macro F1-scores, 
an ensemble-based tool is the best performer in three cross-platform settings, which a stand-alone SD tool (i.e., a baseline) 
is the best performer in the other three cross-platform settings. When a baseline 
is the best performer, its SentistrengthSE in two settings (tested on Jira after trained on SO or GitHub) and 
BERT4SentiSE in one setting (trained on GitHub, tested on SO). One of the reasons for the superiority of SentistrengthSE for the 
Jira dataset is that the rules for SentiStrengthSE were developed by studying Jira
platform \cite{Ortu-EmotionalSideJira-MSR2016}. Therefore, the tool might have some advantage
over other tools it is tested on in our Jira dataset. Among the three settings where the majority voting 
based ensemblers offered the best F1-scores, it is always the combination of the two best performing deep learning 
SD tools (BERT4SentiSE, SentiMoji) and SentistrengthSE. 

\bf{The difference in performance between the best performing ensembler and the baseline (i.e., best performing stand-alone tool) in each cross-platform setting 
is almost negligible.} According to \fig\ref{fig:ensemble_result}, the majority based ensemblers are 
the best performers in three cross-platform settings: when tested on GitHub after it is trained on SO (Macro F1-score of the best ensembler 0.82) or 
Jira (F1 = 0.81) and when trained on Jira and then tested on SO (F1 = 0.82). The best performing baselines in those three settings are SentistrengthSE for the first two cases (F1 = 0.78) and BERT4SentiSE in the last setting (F1 = 0.79). Therefore, the maximum gain in performance we can get by using an ensembler over a baseline in those three settings is 0.03. Therefore, majority-based voting of the six tools in cross-platform settings is not 
practical, when we get only a gain of 0.03 in Macro F1-score.

\begin{tcolorbox}[flushleft upper,boxrule=1pt,arc=0pt,left=0pt,right=0pt,top=0pt,bottom=0pt,colback=white,after=\ignorespacesafterend\par\noindent]
 \bf{RQ$_5$ To what extent the deep learning and non-deep learning sentiment detection tools can complement each other in cross-platform settings?}
% \gias{summarize}
%Both BERT4SentiSE and SentiMoji has the highest severe and mild disagreement with manual labelling when they are trained on Stack Overflow dataset. Among the studied tools both the pretrained tools SentiMoji and BERT4SentiSE have the highest similarity in terms on their predictions. They have the highest Cohen $K$ score (e.g., substantial to perfect agreement) and lowest percentage of severe disagreement between them.
The two best performing deep learning SD tools (BERT4SentiSE, SentiMoji) have
the highest level of agreement and lowest level disagreement between them among
all the six SE-specific SD tools in our study. A majority voting based ensemble
based on the two best performing deep learning SD tools (BERT4SentiSE +
SentiMoji) or the two best performing deep learning SD tools (BERT4SentiSE +
SentiMoji) + Rule-based tool (SentistrengthSE) provides slightly better
performance than the stand-alone SD tools in cross-platform settings. The
difference in performance between the best performing ensembler and the baseline
(i.e., best performing stand-alone tool) in each cross-platform setting is
almost negligible.
\end{tcolorbox}


==> SubmissionTOSEM/RQ4_tables.tex <==

% \begin{table}[]
%   \footnotesize
% %   \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Agreement metrics between  tools with manual labelling}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{clrrrr}
%     \toprule{}
%     %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
%     %\cmidrule{3-6}
%     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Classifier }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
%     \cmidrule{5-6}
%     {Dataset} &  & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule
% \multicolumn{6}{c}{\textbf{Test dataset: GitHub}} \\
% \midrule
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Within-platform)}} 
%  & SEntiMoji & 0.84 & 90\% & 1\% & 9\%  \\
%  & BERT4SentiSE & 0.87 & 92\% & 1\% & 7\%  \\
%  & RNN4SentiSE & 0.52 & 68\% & 7\% & 25\%  \\
%  & Senti4SD & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiCR & 0.73 & 83\% & 2\% & 15\%  \\
% % \midrule
% \cmidrule{2-6}
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow \\ (Cross-platform)}}  
%  & SEntiMoji & 0.61 & 75\% & 2\% & 23\%  \\
%  & BERT4SentiSE & 0.65 & 78\% & 3\% & 19\%  \\
%  & RNN4SentiSE & 0.47 & 66\% & 4\% & 30\%  \\
%  & Senti4SD & 0.60 & 74\% & 4\% & 22\%  \\
%  & SentiCR & 0.49 & 68\% & 2\% & 29\%  \\
% % \midrule
% \cmidrule{2-6}
% 
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Cross-platform)}} 
%  & SEntiMoji & 0.44 & 66\% & 1\% & 33\%  \\
%  & BERT4SentiSE & 0.48 & 68\% & 2\% & 30\%  \\
%  & RNN4SentiSE & 0.35 & 60\% & 4\% & 36\%  \\
%  & Senti4SD & 0.50 & 69\% & 2\% & 28\%  \\
%  & SentiCR & 0.34 & 60\% & 1\% & 39\%  \\
% \midrule
% 
% 
% 
% \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% \midrule
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow (Within-platform)}}
%  & SEntiMoji & 0.80 & 87\% & 1\% & 12\%  \\
%  & BERT4SentiSE& 0.82 & 88\% & 1\% & 11\%  \\
%  & RNN4SentiSE & 0.67 & 78\% & 3\% & 19\%  \\
%  & Senti4SD & 0.77 & 85\% & 1\% & 14\%  \\
%  & SentiCR & 0.73 & 82\% & 3\% & 15\%  \\
% % \midrule
% \cmidrule{2-6}
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Cross-platform)}} 
%  & SEntiMoji & 0.73 & 83\% & 1\% & 16\%  \\
%  & BERT4SentiSE & 0.78 & 85\% & 1\% & 14\%  \\
%  & RNN4SentiSE & 0.49 & 67\% & 4\% & 29\%  \\
%  & Senti4SD & 0.67 & 78\% & 2\% & 20\%  \\
%  & SentiCR & 0.56 & 71\% & 5\% & 23\%  \\
% % \midrule
% \cmidrule{2-6}
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Cross-platform)}} 
%  & SEntiMoji & 0.48 & 67\% & 0\% & 33\%  \\
%  & BERT4SentiSE & 0.63 & 76\% & 1\% & 23\%  \\
%  & RNN4SentiSE & 0.34 & 58\% & 4\% & 38\%  \\
%  & Senti4SD & 0.47 & 66\% & 1\% & 33\%  \\
%  & SentiCR & 0.37 & 60\% & 2\% & 38\%  \\
% \midrule
% 
% 
% 
% 
% 
% 
% 
% \multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
% \midrule
% \multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Within-platform)}}
%  & SEntiMoji & 0.71 & 86\% & 0\% & 14\%  \\
%  & BERT4SentiSE& 0.72 & 86\% & 0\% & 13\%  \\
%  & RNN4SentiSE & 0.57 & 80\% & 1\% & 20\%  \\
%  & Senti4SD & 0.59 & 81\% & 0\% & 19\%  \\
%  & SentiCR & 0.69 & 85\% & 0\% & 15\%  \\
% % \midrule
% \cmidrule{2-6}
% 
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Cross-platform)}} 
%  & SEntiMoji & 0.65 & 81\% & 1\% & 18\%  \\
%  & BERT4SentiSE & 0.65 & 81\% & 1\% & 18\%  \\
%  & RNN4SentiSE & 0.45 & 66\% & 2\% & 32\%  \\
%  & Senti4SD & 0.58 & 78\% & 1\% & 21\%  \\
%  & SentiCR & 0.65 & 82\% & 1\% & 17\%  \\
% % \midrule
% \cmidrule{2-6}
% 
% \multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow \\ (Cross-platform)}} 
%  & SEntiMoji & 0.65 & 82\% & 1\% & 18\%  \\
%  & BERT4SentiSE & 0.66 & 82\% & 1\% & 17\%  \\
%  & RNN4SentiSE & 0.57 & 77\% & 1\% & 22\%  \\
%  & Senti4SD & 0.46 & 74\% & 1\% & 25\%  \\
%  & SentiCR & 0.34 & 73\% & 1\% & 26\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_with_manual_labelling}%
% \end{table}%


















% ===================================================================================================>
% \resizebox{\textwidth}{!}{%
\begin{sidewaystable}
\vspace{15cm}
% \hvFloat[rotAngle=90,nonFloat=true,capWidth=w]
% \begin{table}
\parbox{.3\linewidth}{
\renewcommand{\thetable}{\arabic{table}a}
  \footnotesize
%   \small
  \centering
  \caption{Agreement between SD tools (Test dataset: GitHub)}
    \begin{tabular}{clrr|rr}
    \toprule
    \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagree}}\\
    \cmidrule{3-6}
    & & {\bf{$\kappa$}} & {\textbf{P}} & \textbf{S} & \textbf{M} \\
    \midrule
\multirow{15}{*}{G (W)} 
% ==========================  within setting GitHub =========
 & Mji vs Brt & 0.86 & 91\% & 1\% & 8\%  \\
 & Mji vs Rnn & 0.52 & 68\% & 7\% & 25\%  \\
 & Mji vs S4D & 0.83 & 89\% & 1\% & 10\%  \\
 & Mji vs SCr & 0.76 & 85\% & 2\% & 13\%  \\
 & Mji vs SSt & 0.68 & 79\% & 2\% & 18\%  \\
 & Brt vs Rnn & 0.53 & 69\% & 7\% & 24\%  \\
 & Brt vs S4D & 0.85 & 90\% & 2\% & 8\%  \\
 & Brt vs SCr & 0.74 & 83\% & 2\% & 14\%  \\
 & Brt vs SSt & 0.68 & 80\% & 2\% & 18\%  \\
 & Rnn vs S4D & 0.52 & 69\% & 7\% & 25\%  \\
 & Rnn vs SCr & 0.43 & 63\% & 7\% & 31\%  \\
 & Rnn vs SSt & 0.44 & 63\% & 6\% & 31\%  \\
 & S4D vs SCr & 0.74 & 83\% & 2\% & 14\%  \\
 & S4D vs SSt & 0.67 & 79\% & 3\% & 18\%  \\
 & SCr vs SSt & 0.63 & 77\% & 3\% & 21\%  \\
\midrule


\multirow{15}{*}{S(C)} 
% ...........test dataset: GitHub train_dataset: DatasetSenti4SDSO  .........
 & Mji vs Brt & 0.72 & 83\% & 1\% & 15\%  \\
 & Mji vs Rnn & 0.58 & 76\% & 2\% & 22\%  \\
 & Mji vs S4D & 0.51 & 70\% & 3\% & 27\%  \\
 & Mji vs SCr & 0.40 & 68\% & 2\% & 30\%  \\
 & Mji vs SSt & 0.57 & 74\% & 2\% & 25\%  \\
 & Brt vs Rnn & 0.59 & 76\% & 2\% & 22\%  \\
 & Brt vs S4D & 0.52 & 70\% & 4\% & 26\%  \\
 & Brt vs SCr & 0.39 & 66\% & 3\% & 31\%  \\
 & Brt vs SSt & 0.61 & 76\% & 2\% & 22\%  \\
 & Rnn vs S4D & 0.43 & 65\% & 4\% & 31\%  \\
 & Rnn vs SCr & 0.30 & 62\% & 3\% & 35\%  \\
 & Rnn vs SSt & 0.48 & 68\% & 3\% & 29\%  \\
 & S4D vs SCr & 0.45 & 68\% & 2\% & 30\%  \\
 & S4D vs SSt & 0.55 & 72\% & 3\% & 25\%  \\
 & SCr vs SSt & 0.45 & 68\% & 2\% & 31\%  \\
\midrule


\multirow{15}{*}{J(C)} 
% ...........test dataset: GitHub train_dataset: OrtuJIRA  .........
 & Mji vs Brt & 0.78 & 90\% & 0\% & 10\%  \\
 & Mji vs Rnn & 0.54 & 81\% & 1\% & 19\%  \\
 & Mji vs S4D & 0.60 & 82\% & 1\% & 18\%  \\
 & Mji vs SCr & 0.65 & 87\% & 0\% & 13\%  \\
 & Mji vs SSt & 0.46 & 69\% & 0\% & 30\%  \\
 & Brt vs Rnn & 0.56 & 81\% & 1\% & 18\%  \\
 & Brt vs S4D & 0.60 & 81\% & 1\% & 18\%  \\
 & Brt vs SCr & 0.67 & 87\% & 0\% & 13\%  \\
 & Brt vs SSt & 0.51 & 71\% & 1\% & 28\%  \\
 & Rnn vs S4D & 0.44 & 74\% & 2\% & 24\%  \\
 & Rnn vs SCr & 0.45 & 79\% & 1\% & 20\%  \\
 & Rnn vs SSt & 0.36 & 63\% & 2\% & 34\%  \\
 & S4D vs SCr & 0.52 & 79\% & 1\% & 20\%  \\
 & S4D vs SSt & 0.48 & 70\% & 2\% & 29\%  \\
 & SCr vs SSt & 0.39 & 66\% & 0\% & 34\%  \\

    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:agreement_test_github}%
% \end{table}%
% \end{sidewaystable}
}
% \begin{sidewaystable}
% \vspace{15cm}
% \begin{table}
\hfill
\parbox{.3\linewidth}{
\addtocounter{table}{-1}
\renewcommand{\thetable}{\arabic{table}b}
  \footnotesize
%   \small
  \centering
  \caption{Agreement between SD tools (Test dataset: SO)}
    \begin{tabular}{clrr|rr}
    \toprule
    \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagree}}\\
    \cmidrule{3-6}
    & & {\bf{$\kappa$}} & {\textbf{P}} & \textbf{S} & \textbf{M} \\
    \midrule

\multirow{15}{*}{ S (W)} 
% ==========================  within setting DatasetSenti4SDSO =========
 & Mji vs Brt & 0.86 & 91\% & 1\% & 8\%  \\
 & Mji vs Rnn & 0.70 & 80\% & 3\% & 17\%  \\
 & Mji vs S4D & 0.81 & 88\% & 1\% & 12\%  \\
 & Mji vs SCr & 0.78 & 85\% & 2\% & 12\%  \\
 & Mji vs SSt & 0.72 & 81\% & 1\% & 17\%  \\
 & Brt vs Rnn & 0.71 & 81\% & 2\% & 17\%  \\
 & Brt vs S4D & 0.83 & 88\% & 1\% & 11\%  \\
 & Brt vs SCr & 0.78 & 85\% & 3\% & 12\%  \\
 & Brt vs SSt & 0.72 & 81\% & 1\% & 18\%  \\
 & Rnn vs S4D & 0.70 & 80\% & 3\% & 17\%  \\
 & Rnn vs SCr & 0.65 & 77\% & 4\% & 19\%  \\
 & Rnn vs SSt & 0.63 & 75\% & 3\% & 21\%  \\
 & S4D vs SCr & 0.78 & 85\% & 3\% & 12\%  \\
 & S4D vs SSt & 0.73 & 82\% & 1\% & 17\%  \\
 & SCr vs SSt & 0.70 & 81\% & 2\% & 17\%  \\

\midrule

\multirow{15}{*}{ G (C)} 
 % ...........test dataset: DatasetSenti4SDSO train_dataset: GitHub  .........
 & Mji vs Brt & 0.79 & 86\% & 1\% & 13\%  \\
 & Mji vs Rnn & 0.53 & 70\% & 4\% & 27\%  \\
 & Mji vs S4D & 0.70 & 80\% & 3\% & 17\%  \\
 & Mji vs SCr & 0.62 & 75\% & 5\% & 20\%  \\
 & Mji vs SSt & 0.67 & 79\% & 1\% & 20\%  \\
 & Brt vs Rnn & 0.53 & 69\% & 5\% & 26\%  \\
 & Brt vs S4D & 0.73 & 82\% & 2\% & 16\%  \\
 & Brt vs SCr & 0.60 & 74\% & 5\% & 21\%  \\
 & Brt vs SSt & 0.69 & 79\% & 1\% & 20\%  \\
 & Rnn vs S4D & 0.54 & 69\% & 4\% & 26\%  \\
 & Rnn vs SCr & 0.40 & 61\% & 6\% & 33\%  \\
 & Rnn vs SSt & 0.48 & 66\% & 4\% & 30\%  \\
 & S4D vs SCr & 0.58 & 73\% & 4\% & 23\%  \\
 & S4D vs SSt & 0.65 & 77\% & 1\% & 22\%  \\
 & SCr vs SSt & 0.56 & 71\% & 4\% & 25\%  \\
\midrule


\multirow{15}{*}{ J (C)} 
% ...........test dataset: DatasetSenti4SDSO train_dataset: OrtuJIRA  .........
 & Mji vs Brt & 0.66 & 82\% & 0\% & 18\%  \\
 & Mji vs Rnn & 0.47 & 75\% & 1\% & 23\%  \\
 & Mji vs S4D & 0.60 & 81\% & 1\% & 19\%  \\
 & Mji vs SCr & 0.56 & 80\% & 1\% & 19\%  \\
 & Mji vs SSt & 0.49 & 68\% & 0\% & 31\%  \\
 & Brt vs Rnn & 0.43 & 70\% & 2\% & 28\%  \\
 & Brt vs S4D & 0.57 & 77\% & 1\% & 22\%  \\
 & Brt vs SCr & 0.52 & 75\% & 1\% & 25\%  \\
 & Brt vs SSt & 0.60 & 75\% & 0\% & 25\%  \\
 & Rnn vs S4D & 0.42 & 72\% & 2\% & 27\%  \\
 & Rnn vs SCr & 0.33 & 70\% & 1\% & 29\%  \\
 & Rnn vs SSt & 0.36 & 60\% & 3\% & 36\%  \\
 & S4D vs SCr & 0.51 & 77\% & 1\% & 22\%  \\
 & S4D vs SSt & 0.46 & 66\% & 1\% & 33\%  \\
 & SCr vs SSt & 0.40 & 63\% & 1\% & 36\%  \\

% \midrule

    \bottomrule
    \end{tabular}%
  \label{tab:agreement_test_so}%
% \end{table}%
% \end{sidewaystable}
}
\hfill
\parbox{.3\linewidth}{
% \begin{sidewaystable}
% \begin{table}[]
  \addtocounter{table}{-1}
  \renewcommand{\thetable}{\arabic{table}c}
  \footnotesize
%   \small
  \centering
  \caption{Agreement between SD tools (Test dataset: Jira)}
    \begin{tabular}{clrr|rr}
    \toprule
    \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagree}}\\
    \cmidrule{3-6}
    & & {\bf{$\kappa$}} & {\textbf{P}} & \textbf{S} & \textbf{M} \\
    \midrule

\multirow{15}{*}{ J (W)} 
% ==========================  within setting OrtuJIRA =========
 & Mji vs Brt & 0.85 & 93\% & 0\% & 7\%  \\
 & Mji vs Rnn & 0.68 & 86\% & 0\% & 14\%  \\
 & Mji vs S4D & 0.72 & 87\% & 0\% & 13\%  \\
 & Mji vs SCr & 0.81 & 91\% & 0\% & 9\%  \\
 & Mji vs SSt & 0.75 & 87\% & 0\% & 13\%  \\
 & Brt vs Rnn & 0.68 & 85\% & 1\% & 14\%  \\
 & Brt vs S4D & 0.72 & 87\% & 0\% & 13\%  \\
 & Brt vs SCr & 0.79 & 90\% & 0\% & 10\%  \\
 & Brt vs SSt & 0.75 & 87\% & 0\% & 13\%  \\
 & Rnn vs S4D & 0.61 & 83\% & 0\% & 17\%  \\
 & Rnn vs SCr & 0.70 & 86\% & 1\% & 14\%  \\
 & Rnn vs SSt & 0.63 & 81\% & 1\% & 18\%  \\
 & S4D vs SCr & 0.70 & 86\% & 0\% & 13\%  \\
 & S4D vs SSt & 0.67 & 83\% & 1\% & 16\%  \\
 & SCr vs SSt & 0.77 & 88\% & 1\% & 11\%  \\
\midrule

\multirow{15}{*}{ G (C)} 
% ...........test dataset: OrtuJIRA train_dataset: GitHub  .........
 & Mji vs Brt & 0.81 & 89\% & 1\% & 10\%  \\
 & Mji vs Rnn & 0.56 & 72\% & 3\% & 25\%  \\
 & Mji vs S4D & 0.72 & 84\% & 1\% & 14\%  \\
 & Mji vs SCr & 0.75 & 86\% & 1\% & 13\%  \\
 & Mji vs SSt & 0.75 & 86\% & 1\% & 13\%  \\
 & Brt vs Rnn & 0.57 & 73\% & 3\% & 24\%  \\
 & Brt vs S4D & 0.73 & 85\% & 1\% & 14\%  \\
 & Brt vs SCr & 0.75 & 87\% & 1\% & 13\%  \\
 & Brt vs SSt & 0.75 & 86\% & 1\% & 13\%  \\
 & Rnn vs S4D & 0.52 & 70\% & 3\% & 27\%  \\
 & Rnn vs SCr & 0.50 & 69\% & 2\% & 28\%  \\
 & Rnn vs SSt & 0.54 & 71\% & 2\% & 27\%  \\
 & S4D vs SCr & 0.68 & 83\% & 1\% & 16\%  \\
 & S4D vs SSt & 0.70 & 83\% & 1\% & 16\%  \\
 & SCr vs SSt & 0.76 & 87\% & 1\% & 12\%  \\
\midrule


\multirow{15}{*}{ S (C)} 
% ...........test dataset: OrtuJIRA train_dataset: DatasetSenti4SDSO  .........
 & Mji vs Brt & 0.80 & 89\% & 1\% & 10\%  \\
 & Mji vs Rnn & 0.70 & 84\% & 1\% & 15\%  \\
 & Mji vs S4D & 0.61 & 79\% & 1\% & 19\%  \\
 & Mji vs SCr & 0.35 & 70\% & 1\% & 29\%  \\
 & Mji vs SSt & 0.77 & 87\% & 1\% & 12\%  \\
 & Brt vs Rnn & 0.72 & 84\% & 1\% & 14\%  \\
 & Brt vs S4D & 0.60 & 79\% & 2\% & 19\%  \\
 & Brt vs SCr & 0.36 & 71\% & 1\% & 28\%  \\
 & Brt vs SSt & 0.77 & 87\% & 1\% & 12\%  \\
 & Rnn vs S4D & 0.56 & 77\% & 2\% & 22\%  \\
 & Rnn vs SCr & 0.30 & 67\% & 1\% & 32\%  \\
 & Rnn vs SSt & 0.70 & 83\% & 1\% & 16\%  \\
 & S4D vs SCr & 0.41 & 76\% & 1\% & 23\%  \\
 & S4D vs SSt & 0.59 & 78\% & 2\% & 20\%  \\
 & SCr vs SSt & 0.34 & 70\% & 1\% & 29\%  \\
% \midrule
    % \midrule  
    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:agreement_test_jira}%
 }
% \end{table}%
\end{sidewaystable}





% \begin{table}
% \renewcommand{\thetable}{\arabic{table}a}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Agreement between  tools (Test dataset: GitHub)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule
% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Within Platform)}} 
%  & SentiMoji vs BERT4SE & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiMoji vs RNN4SE & 0.52 & 68\% & 7\% & 25\%  \\
%  & SentiMoji vs Senti4SD & 0.83 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs SentiCR & 0.76 & 85\% & 2\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.53 & 69\% & 7\% & 24\%  \\
%  & BERT4SE vs Senti4SD & 0.85 & 90\% & 2\% & 8\%  \\
%  & BERT4SE vs SentiCR & 0.74 & 83\% & 2\% & 14\%  \\
%  & RNN4SE vs Senti4SD & 0.52 & 69\% & 7\% & 25\%  \\
%  & RNN4SE vs SentiCR & 0.43 & 63\% & 7\% & 31\%  \\
%  & Senti4SD vs SentiCR & 0.74 & 83\% & 2\% & 14\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.72 & 83\% & 1\% & 15\%  \\
%  & SentiMoji vs RNN4SE & 0.58 & 76\% & 2\% & 22\%  \\
%  & SentiMoji vs Senti4SD & 0.51 & 70\% & 3\% & 27\%  \\
%  & SentiMoji vs SentiCR & 0.40 & 68\% & 2\% & 30\%  \\
%  & BERT4SE vs RNN4SE & 0.59 & 76\% & 2\% & 22\%  \\
%  & BERT4SE vs Senti4SD & 0.52 & 70\% & 4\% & 26\%  \\
%  & BERT4SE vs SentiCR & 0.39 & 66\% & 3\% & 31\%  \\
%  & RNN4SE vs Senti4SD & 0.43 & 65\% & 4\% & 31\%  \\
%  & RNN4SE vs SentiCR & 0.30 & 62\% & 3\% & 35\%  \\
%  & Senti4SD vs SentiCR & 0.45 & 68\% & 2\% & 30\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.78 & 90\% & 0\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.54 & 81\% & 1\% & 19\%  \\
%  & SentiMoji vs Senti4SD & 0.60 & 82\% & 1\% & 18\%  \\
%  & SentiMoji vs SentiCR & 0.65 & 87\% & 0\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.56 & 81\% & 1\% & 18\%  \\
%  & BERT4SE vs Senti4SD & 0.60 & 81\% & 1\% & 18\%  \\
%  & BERT4SE vs SentiCR & 0.67 & 87\% & 0\% & 13\%  \\
%  & RNN4SE vs Senti4SD & 0.44 & 74\% & 2\% & 24\%  \\
%  & RNN4SE vs SentiCR & 0.45 & 79\% & 1\% & 20\%  \\
%  & Senti4SD vs SentiCR & 0.52 & 79\% & 1\% & 20\%  \\

%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_github}%
% \end{table}%


% ==================================================================================================>

% \begin{table}
% \addtocounter{table}{-1}
% \renewcommand{\thetable}{\arabic{table}b}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Agreement between  tools (Test dataset: SO)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Within Platform)}} 
%  & SentiMoji vs BERT4SE & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiMoji vs RNN4SE & 0.70 & 80\% & 3\% & 17\%  \\
%  & SentiMoji vs Senti4SD & 0.81 & 88\% & 1\% & 12\%  \\
%  & SentiMoji vs SentiCR & 0.78 & 85\% & 2\% & 12\%  \\
%  & BERT4SE vs RNN4SE & 0.71 & 81\% & 2\% & 17\%  \\
%  & BERT4SE vs Senti4SD & 0.83 & 88\% & 1\% & 11\%  \\
%  & BERT4SE vs SentiCR & 0.78 & 85\% & 3\% & 12\%  \\
%  & RNN4SE vs Senti4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & RNN4SE vs SentiCR & 0.65 & 77\% & 4\% & 19\%  \\
%  & Senti4SD vs SentiCR & 0.78 & 85\% & 3\% & 12\%  \\
% \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.79 & 86\% & 1\% & 13\%  \\
%  & SentiMoji vs RNN4SE & 0.53 & 70\% & 4\% & 27\%  \\
%  & SentiMoji vs Senti4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & SentiMoji vs SentiCR & 0.62 & 75\% & 5\% & 20\%  \\
%  & BERT4SE vs RNN4SE & 0.53 & 69\% & 5\% & 26\%  \\
%  & BERT4SE vs Senti4SD & 0.73 & 82\% & 2\% & 16\%  \\
%  & BERT4SE vs SentiCR & 0.60 & 74\% & 5\% & 21\%  \\
%  & RNN4SE vs Senti4SD & 0.54 & 69\% & 4\% & 26\%  \\
%  & RNN4SE vs SentiCR & 0.40 & 61\% & 6\% & 33\%  \\
%  & Senti4SD vs SentiCR & 0.58 & 73\% & 4\% & 23\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.66 & 82\% & 0\% & 18\%  \\
%  & SentiMoji vs RNN4SE & 0.47 & 75\% & 1\% & 23\%  \\
%  & SentiMoji vs Senti4SD & 0.60 & 81\% & 1\% & 19\%  \\
%  & SentiMoji vs SentiCR & 0.56 & 80\% & 1\% & 19\%  \\
%  & BERT4SE vs RNN4SE & 0.43 & 70\% & 2\% & 28\%  \\
%  & BERT4SE vs Senti4SD & 0.57 & 77\% & 1\% & 22\%  \\
%  & BERT4SE vs SentiCR & 0.52 & 75\% & 1\% & 25\%  \\
%  & RNN4SE vs Senti4SD & 0.42 & 72\% & 2\% & 27\%  \\
%  & RNN4SE vs SentiCR & 0.33 & 70\% & 1\% & 29\%  \\
%  & Senti4SD vs SentiCR & 0.51 & 77\% & 1\% & 22\%  \\
% % \midrule

%     \bottomrule
%     \end{tabular}%
%   \label{tab:agreement_test_so}%
% \end{table}%

% % ===================================================================================================>

% \begin{table}[]
%   \addtocounter{table}{-1}
%   \renewcommand{\thetable}{\arabic{table}c}

% %   \footnotesize
%   \small
%   \centering
%   \caption{Agreement between  tools (Test dataset: Jira)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Within Platform}} 
%  & SentiMoji vs BERT4SE & 0.85 & 93\% & 0\% & 7\%  \\
%  & SentiMoji vs RNN4SE & 0.68 & 86\% & 0\% & 14\%  \\
%  & SentiMoji vs Senti4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & SentiMoji vs SentiCR & 0.81 & 91\% & 0\% & 9\%  \\
%  & BERT4SE vs RNN4SE & 0.68 & 85\% & 1\% & 14\%  \\
%  & BERT4SE vs Senti4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & BERT4SE vs SentiCR & 0.79 & 90\% & 0\% & 10\%  \\
%  & RNN4SE vs Senti4SD & 0.61 & 83\% & 0\% & 17\%  \\
%  & RNN4SE vs SentiCR & 0.70 & 86\% & 1\% & 14\%  \\
%  & Senti4SD vs SentiCR & 0.70 & 86\% & 0\% & 13\%  \\
% \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.81 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.56 & 72\% & 3\% & 25\%  \\
%  & SentiMoji vs Senti4SD & 0.72 & 84\% & 1\% & 14\%  \\
%  & SentiMoji vs SentiCR & 0.75 & 86\% & 1\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.57 & 73\% & 3\% & 24\%  \\
%  & BERT4SE vs Senti4SD & 0.73 & 85\% & 1\% & 14\%  \\
%  & BERT4SE vs SentiCR & 0.75 & 87\% & 1\% & 13\%  \\
%  & RNN4SE vs Senti4SD & 0.52 & 70\% & 3\% & 27\%  \\
%  & RNN4SE vs SentiCR & 0.50 & 69\% & 2\% & 28\%  \\
%  & Senti4SD vs SentiCR & 0.68 & 83\% & 1\% & 16\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.80 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.70 & 84\% & 1\% & 15\%  \\
%  & SentiMoji vs Senti4SD & 0.61 & 79\% & 1\% & 19\%  \\
%  & SentiMoji vs SentiCR & 0.35 & 70\% & 1\% & 29\%  \\
%  & BERT4SE vs RNN4SE & 0.72 & 84\% & 1\% & 14\%  \\
%  & BERT4SE vs Senti4SD & 0.60 & 79\% & 2\% & 19\%  \\
%  & BERT4SE vs SentiCR & 0.36 & 71\% & 1\% & 28\%  \\
%  & RNN4SE vs Senti4SD & 0.56 & 77\% & 2\% & 22\%  \\
%  & RNN4SE vs SentiCR & 0.30 & 67\% & 1\% & 32\%  \\
%  & Senti4SD vs SentiCR & 0.41 & 76\% & 1\% & 23\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_jira}%
% \end{table}%








\begin{table}
  \footnotesize
%   \small

  \centering
  \caption{Performance comparison of majority voting based ensemble tools with the SD tools (All- All of the SD tools except baseline DL-RNN4SEntiSE, BTPC-Best SD tool from PMT DL-based (BERT4SentiSE), Shallow ML-based (Senti4SD), Rule-based (SentiStrengthSE) }
    \begin{tabular}{ccllll}
    \toprule
    \multirow{2}{*}{\bf{Test Dataset}} & \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\textbf{Ensemble}} & \multicolumn{3}{c}{\textbf{Macro Performance}}\\
    \cmidrule{4-6}
    & & & {\bf{$P$}} & {\bf{$R$}} & {\bf{$F1$}} \\
    \midrule
    
\multirow{16}{*}{GitHub}  &  \multirow{8}{*}{Stack Overflow} & Baseline: Best (SentiStrengthSE) & .80 & .78 & .78\\
% \cmidrule{4-6}
& & Majority-All &  .78 & .80 & .78  \\
& & Majority-All (Except RNN4SentiSE) &  .80 & .81 & .80  \\
& & Majority-PMT DL &  .81 & .78 & .79  \\
& & Majority-Shallow ML &  .76 & .75 & .75  \\
& & Majority-PMT DL + Rule &  .82 & .83 & .82  \\
& & Majority-Shallow ML + Rule &  .78 & .80 & .79  \\
& & Majority-BTPC &  .80 & .81 & .80  \\
\cmidrule{3-6}

& \multirow{8}{*}{Jira} & Baseline: Best (SentiStrengthSE) & .80 & .78 & .78\\
% \cmidrule{4-6}
& & Majority-All &  .80 & .80 & .80  \\
& & Majority-All (Except RNN4SentiSE) &  .81 & .81 & .81  \\
& & Majority-PMT DL &  .80 & .66 & .68  \\
& & Majority-Shallow ML &  .79 & .67 & .69  \\
& & Majority-PMT DL + Rule &  .82 & .80 & .81  \\
& & Majority-Shallow ML + Rule &  .81 & .80 & .80  \\
& & Majority-BTPC &  .81 & .81 & .81  \\

\midrule
\multirow{16}{*}{Stack Overflow}  &  \multirow{8}{*}{GitHub} & Baseline: Best (BERT4SentiSE) & .85 & .86 & .85\\
% \cmidrule{4-6}
& & Majority-All &  .78 & .78 & .75  \\
& & Majority-All (Except RNN4SentiSE) &  .82 & .83 & .81  \\
& & Majority-PMT DL &  .85 & .86 & .85  \\
& & Majority-Shallow ML &  .77 & .77 & .77  \\
& & Majority-PMT DL + Rule &  .84 & .85 & .84  \\
& & Majority-Shallow ML + Rule &  .81 & .81 & .80  \\
& & Majority-BTPC &  .83 & .83 & .82  \\
\cmidrule{3-6}

& \multirow{8}{*}{Jira} & Baseline: Best (BERT4SentiSE) & .80 & .79 & .79\\
% \cmidrule{4-6}
& & Majority-All &  .80 & .81 & .81  \\
& & Majority-All (Except RNN4SentiSE) &  .82 & .83 & .83  \\
& & Majority-PMT DL &  .84 & .77 & .78  \\
& & Majority-Shallow ML &  .75 & .67 & .68  \\
& & Majority-PMT DL + Rule &  .82 & .83 & .82  \\
& & Majority-Shallow ML + Rule &  .80 & .81 & .80  \\
& & Majority-BTPC &  .82 & .83 & .83  \\

\midrule
\multirow{16}{*}{Jira}  &  \multirow{8}{*}{GitHub} & Baseline: Best (SentiStrengthSE) & .76 & .82 & .79\\
% \cmidrule{4-6}
& & Majority-All &  .61 & .76 & .61  \\
& & Majority-All (Except RNN4SentiSE) &  .68 & .81 & .70  \\
& & Majority-PMT DL &  .72 & .82 & .75  \\
& & Majority-Shallow ML &  .71 & .80 & .73  \\
& & Majority-PMT DL + Rule &  .70 & .83 & .74  \\
& & Majority-Shallow ML + Rule &  .70 & .81 & .73  \\
& & Majority-BTPC &  .69 & .82 & .72  \\
\cmidrule{3-6}

& \multirow{8}{*}{Stack Overflow} & Baseline: Best (SentiStrengthSE) & .76 & .82 & .79\\
% \cmidrule{4-6}
& & Majority-All &  .67 & .80 & .69  \\
& & Majority-All (Except RNN4SentiSE) &  .69 & .81 & .72  \\
& & Majority-PMT DL &  .74 & .82 & .76  \\
& & Majority-Shallow ML &  .62 & .63 & .61  \\
& & Majority-PMT DL + Rule &  .72 & .83 & .75  \\
& & Majority-Shallow ML + Rule &  .70 & .80 & .73  \\
& & Majority-BTPC &  .71 & .82 & .74  \\
% \multirow{10}{*}{S(C)} 

% \midrule


% \multirow{10}{*}{J(C)}
    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:ensemble_result}%
\end{table}%

\begin{figure*}[t]
\centering
\captionsetup[subfigure]{labelformat=empty}
\pgfplotstableread{
1	.78 .78 .80 .79 .75 .82 .79 .80      .80 .78 .80 .81 .76 .82 .78 .80    .85 .75 .81 .85 .77 .84 .80 .82     .85 .78 .82 .85 .77 .84 .81 .83    .79 .61 .70 .75 .73 .74 .73 .72    .76 .61 .68 .72 .71 .70 .70 .69
2	.78 .80 .81 .68 .69 .81 .80 .81      .80 .80 .81 .80 .79 .82 .81 .81    .79 .81 .83 .78 .68 .82 .80 .83     .80 .80 .82 .84 .75 .82 .80 .82    .79 .69 .72 .76 .61 .75 .73 .74    .76 .67 .69 .74 .62 .72 .70 .71
}\datatable
\pgfplotscreateplotcyclelist{xcolor}{%
red!60, orange, yellow, blue!50, brown, violet, purple, black!60
}

\edef\mylst{"a", "b", "c", "d", "e", "f", "g", "h"}

      \subfloat[Test on GitHub (F1 score)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
      
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Trained on SO\\(Baseline: SentiStrengthSE), Trained on Jira\\(Baseline: SentiStrengthSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.5,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend style={draw=none},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        % 	nodes near coords=\pgfmathsetmacro{\mystring}{{\mylst}[\coordindex]}\mystring,
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=1] \datatable;
        % 	\node [above] at (axis cs:  100,  92.021) {a};
        	\addplot table[x index=0,y index=2] \datatable;
        % 	\node [above] at (axis cs:  100,  92.021) {b};
        	\addplot table[x index=0,y index=3] \datatable;
        	\addplot table[x index=0,y index=4] \datatable;
            \addplot table[x index=0,y index=5] \datatable;
        	\addplot table[x index=0,y index=6] \datatable;
        	\addplot table[x index=0,y index=7] \datatable;
        	\addplot table[x index=0,y index=8] \datatable;

            % \foreach \Point [count=\i] in {
            %     1, 2, 3, 4, 5, 6, 7, 8
            % }{
            % %  \node[dot,label=\i] at \Point {};
            %  \addplot table[x index=0,y index=\Point] \datatable node[above] {a};
            % %  \node[above] at ($(axis cs:table[x index=0,y index=\Point] \datatable$) {200};
            %  \node[label=\i] at (table[x index=0,y index=\Point] \datatable) {};
            % %  \node [above,color=black] at (endofplotsquare) {a};
            % }

            \legend{Baseline,
            		 Majority-All, , ,
                     Majority-Shallow ML,
                     Majority-PMT DL + Rule, , ,
            		 }
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } 
    \subfloat[Test on GitHub (Precision)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Trained on SO\\(Baseline: SentiStrengthSE), Trained on Jira\\(Baseline: SentiStrengthSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.50,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=9] \datatable;
        	\addplot table[x index=0,y index=10] \datatable;
        	\addplot table[x index=0,y index=11] \datatable;
        	\addplot table[x index=0,y index=12] \datatable;
            \addplot table[x index=0,y index=13] \datatable;
        	\addplot table[x index=0,y index=14] \datatable;
        	\addplot table[x index=0,y index=15] \datatable;
        	\addplot table[x index=0,y index=16] \datatable;

            \legend{, , Majority-All (Except RNN4SentiSE),
            		 Majority-PMT DL, , ,
                     Majority-Shallow ML + Rule,
                     Majority-BTP
            		}
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } \\
    
    \subfloat[Test on Stack Overflow (SO) (F1 score)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub\\(Baseline: BERT4SentiSE), Train on Jira\\(Baseline: BERT4SentiSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.5,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=17] \datatable;
        	\addplot table[x index=0,y index=18] \datatable;
        	\addplot table[x index=0,y index=19] \datatable;
        	\addplot table[x index=0,y index=20] \datatable;
            \addplot table[x index=0,y index=21] \datatable;
        	\addplot table[x index=0,y index=22] \datatable;
        	\addplot table[x index=0,y index=23] \datatable;
        	\addplot table[x index=0,y index=24] \datatable;

            % \legend{Baseline, ,
            % 		 Majority-All,
            % 		 Majority-All (Except RNN4SentiSE),
            % 		 Majority-PMT DL,
            % 		 }
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } 
    \subfloat[Test on Stack Overflow (SO) (Precision)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub\\(Baseline: BERT4SentiSE), Train on Jira\\(Baseline: BERT4SentiSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.50,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=25] \datatable;
        	\addplot table[x index=0,y index=26] \datatable;
        	\addplot table[x index=0,y index=27] \datatable;
        	\addplot table[x index=0,y index=28] \datatable;
            \addplot table[x index=0,y index=29] \datatable;
        	\addplot table[x index=0,y index=30] \datatable;
        	\addplot table[x index=0,y index=31] \datatable;
        	\addplot table[x index=0,y index=32] \datatable;

            % \legend{, , , ,
            %          Majority-Shallow ML,
            %          Majority-PMT DL + Rule,
            %          Majority-Shallow ML + Rule,
            %          Majority-BTP
            % 		}
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } \\
    
    \subfloat[Test on Jira (F1 score)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub\\(Baseline: SentiStrengthSE), Train on SO\\(Baseline: SentiStrengthSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.5,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=33] \datatable;
        	\addplot table[x index=0,y index=34] \datatable;
        	\addplot table[x index=0,y index=35] \datatable;
        	\addplot table[x index=0,y index=36] \datatable;
            \addplot table[x index=0,y index=37] \datatable;
        	\addplot table[x index=0,y index=38] \datatable;
        	\addplot table[x index=0,y index=39] \datatable;
        	\addplot table[x index=0,y index=40] \datatable;

            % \legend{Baseline, ,
            % 		 Majority-All,
            % 		 Majority-All (Except RNN4SentiSE),
            % 		 Majority-PMT DL,
            % 		 }
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } 
    \subfloat[Test on Jira (Precision)]
      {
       \resizebox{2.9in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub\\(Baseline: SentiStrengthSE), Train on SO\\(Baseline: SentiStrengthSE)},
        	xticklabel style={align=center},
        	enlarge y limits=false,
        	enlarge x limits=0.50,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.6cm,
        	width=5.0in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
            legend style={draw=none},
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\LARGE, text=black},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta},
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	cycle list name = xcolor,
            every axis plot/.append style={fill,draw=black!80}%
        	]
        	\addplot table[x index=0,y index=41] \datatable;
        	\addplot table[x index=0,y index=42] \datatable;
        	\addplot table[x index=0,y index=43] \datatable;
        	\addplot table[x index=0,y index=44] \datatable;
            \addplot table[x index=0,y index=45] \datatable;
        	\addplot table[x index=0,y index=46] \datatable;
        	\addplot table[x index=0,y index=47] \datatable;
        	\addplot table[x index=0,y index=48] \datatable;

            % \legend{, , , ,
            %          Majority-Shallow ML,
            %          Majority-PMT DL + Rule,
            %          Majority-Shallow ML + Rule,
            %          Majority-BTP
            % 		}
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    } \\
    
\vspace{-5mm}
\caption{Performance comparison of majority voting based ensemble tools with the SD tools (All- All of the SD tools except baseline DL-RNN4SEntiSE, BTPC-Best SD tool from PMT DL-based (BERT4SentiSE), Shallow ML-based (Senti4SD), Rule-based (SentiStrengthSE)}


\vspace{-5mm}
\label{fig:ensemble_result}
\end{figure*}




==> SubmissionTOSEM/conclusions.tex <==
\section{Conclusions}\label{sec:conclusion}
The diversity in SE platforms can make it challenging to deploy a supervised
SE-specific SD tool across all the platforms without training it in each
platform. Given that it is expensive and sometimes not possible to train an SD tool in each SE platform, it
can be useful to find an SD tool that can perform reasonably well in both within
and cross-platform settings. We studied three recently introduced deep learning
SD tools for SE in three SE benchmark datasets from three SE platforms. We find that BERT4SentiSE is the best
performer in within platform settings, while it is also the best among the
supervised SD tools for SE in cross-platform settings. BERT4SentiSE is slightly
outperformed by lexicon-based tool SentistrengthSE in cross-platform settings,
but BERT4SentiSE outperforms SentistrengthSE for within platform settings by a
large margin. The pre-trained deep learning-based tools show promise in understanding the software engineering context from a small training dataset. However, inconsistent annotation and lack of standard annotation guidelines for the benchmark dataset are hindering future improvement in this domain. Our future research will focus
on improving deep learning-based SD tools like BERT4SentiSE and SentiMoji based on the limitations outlined in this study regarding the sentiment polarity benchmark datasets and supervised SD tools so that they can perform well in diverse software engineering datasets even without retraining. In the absence of the best performing standalone SD tools in cross-platform settings, we will also focus on creating sophisticated ensemble tools that perform well in various standalone tools in diverse SE datasets.







% In this study, we provide a comparison study of five SE-specific machine learning based sentiment analysis tools in cross-platform settings.
% We find that deep learning-based tools perform slightly better than shallow ML-based tools. Furthermore, the pre-trained DL-based classifiers that use transfer learning to train in SE-dataset performed better in cross-platform settings. BERT4SentiSE provides a slightly better result than other tools. Furthermore, pre-trained DL-based classifier have substantial agreement with each other. We also recommend retraining on the target dataset if possible. Both DL-based and shallow ML-based classifier provides better when they are retrained on the target dataset and the dataset is reasonably balanced and manual annotation follows standard guideline.  
% In the future, we can add more diverse dataset from different SE domains and assess the performance. Furthermore, our analysis shows that there were at least some of the tools that made correct predictions for every incorrectly predicted sentence. In the future, we can add these five tools to an ensemble tool and observe its performance.

% In absence of platform specific gold standard for retraining, we recommend using a pre-trained DL-based sentiment detection tools. We highly recommend check the manually annotation of different sentiment datasets because our error analysis and related studies\cite{novielli2020can, novielli2021assessment} studies suggest that human raters annotation is subjective and different datasets from different research goals have different annotation guideline.
% Supervised models do not perform well, i.e., fail to generalize on SE artefacts for the scarcity of labelled data. On the other hand, rule-based tools are not adaptive. It is hard to find the best SA4SE tool because their performance varies in different datasets.


==> SubmissionTOSEM/discussions.tex <==
\section{Discussions}\label{sec:discussion}
In this section, we discuss major themes that emerged during our study.
\subsection{Learning Curves of the Tools}\label{subsec:learning_curve}
% \gias{report learning curves following Section 6.3 of \url{http://collab.di.uniba.it/nicole/wp-content/uploads/sites/6/2020/03/MSR_2020_cross_within_benchmark_preprint.pdf}}
\begin{figure}
% \begin{subfigure}
%   \centering
%   \includegraphics[scale=0.5]{figs/github_learning_curve.pdf}
%   \caption{Github}
%   \label{fig:sfig1}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[scale=0.5]{figs/so_learning_curve.pdf}
%   \caption{Stack Overflow}
%   \label{fig:sfig2}
% \end{subfigure}
\subfloat[Github]{\includegraphics[scale=0.5]{figs/github_learning_curve.pdf}} \\
\subfloat[Stack Overflow]{\includegraphics[scale=0.5]{figs/so_learning_curve.pdf}} \\
\subfloat[Jira]{\includegraphics[scale=0.5]{figs/jira_learning_curve.pdf}} \\
\caption{Learning Curves of SentiMoji \& BERT4SentiSE for within platform settings on (a) Github, (b) Stack Overflow, and (C) Jira}
\label{fig:learningCurve}
\end{figure} Our performance analysis of the tools finds that the deep learning SD tool BERT4SentiSE is the best performer across all three datasets in within platform settings. It is also the best among the supervised SD tools for cross-platform settings. Another deep learning SD tool, SentiMoji, shows the second-best performance in within platform settings across the datasets. SentiMoji also outperforms the shallow learning SD tools in the majority of cross-platform settings. These two deep learning SD tools are suitable for deployment in wide-range datasets, especially when the tools can be retrained in each dataset. It is thus important to know how much training data they need to provide reasonably well performance. In general, deep learning tools need more data than shallow learning tools for better performance. However, given that both tools use pre-trained embedding, the tools may not need a large amount of training data. In \fig\ref{fig:learningCurve}, we show three charts, one each for the three datasets. For each chart, we show how the tools perform as we increase the size of our training data. In order to generate the learning curves, we test each tool with the same held-out test set of 30\% samples after training it by incrementally using more training samples. At first, we sample 5\% of the training set using stratified sampling, which preserves the class distributions, and then we increment the training set by 5\% and test the models using the already held out test set. A similar method was used by Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020} to plot the learning curves of Senti4SD and SentiCR in the same three datasets.

Across the three datasets, SentiMoji shows better performance (Macro F1-score) while using 5-10\% of the training data. However, after that, BERT4SentiSE starts to outperform SentiMoji in two datasets (GitHub and SO). For the other dataset (Jira), BERT4SentiSE starts to outperform after using around 20-25\% of the training data. Both tools show more than 0.80-0.85 Macro F1-score by using 20-25\% of the training data. The increase in the performance in the tools is less rapid after that. The tools show the best F1-scores of above 0.9 for GitHub and 0.85-0.88 for SO and Jira after they are trained on 30-40\% of the data, after which the increase in performance is negligible. This means that the two tools are sensible options in real-world scenarios where creating a large-scale benchmark data may not be possible, but a smaller size (e.g., 500 - 1500 labeled sentences) might not be challenging.


% To investigate this assumption, we ran the two tools in each of our datasets by varying the number of training cases. For a given dataset, we started with 5\% sentences to train and test a tool. We repeate this process 20 times, each time we increased the training data by adding another 5\% training data from the overall dataset. 


% We analyze the learning curves of the two best performing deep learning based tools SentiMoji\cite{sentimoji_2019} and BERT4SentiSE\cite{biswas2020achieving} in within platform settings to find out how much training samples we need to retrain these classifiers. 


%  So, from the learning curve we can see the SentiMoji takes very little dataset to retrain to provide good performance. On the other hand BERT4SentiSE uses ??? configuration. So, it initially needs little more dataset to perform well in SE-specific tasks. From the Figure\ref{} we see BERT4SentiSE quickly catches up SentiMoji and eventually outperforms it after 3 or 4 iteration of increase in training size.





\subsection{Distribution of Error Categories}\label{sec:error-cat-dist}
In \tbl\ref{tab:misclassification}, we show the distribution of the six error categories that we reported in RQ$_3$ across the three datasets (GitHub, SO, and Jira). Recall that the sample size was 400 sentences for which both of the two best performing deep learning SD tools (BERT4SentiSE and SentiMoji) were wrong. This is a random sample. We see almost a similar proportion of the misclassified cases across the datasets based on the actual representation in the datasets. Overall, most misclassified cases are found in the Jira dataset, where the two tools performed the worst. 
\begin{table}[t]
  \centering
  %\vspace{-.1in}
  \caption{Distribution of error categories in the 400 manually analyzed sample across the three datasets for tools BERT4SentiSE and SentiMoji in cross-platform settings}
  % \vspace{-3mm}
    % \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccc}
    \toprule{}
    % \textbf{Topics} & \textbf{Authentication} & \textbf{Deployment} & \textbf{Documentation} & \textbf{Feature} & \textbf{Testing/Debugging}\\
    \textbf{Category} & \textbf{GitHub} & \textbf{SO} & \textbf{Jira}\\
    \midrule

    Subjectivity in Annotation & 59 & 76 & 44  \\
    General Error & 11 & 34 & 67 \\
    Implicit Sentiment & 4 & 13 & 49 \\
    Context/Pragmatics & 23 & 16 & 29 \\
    Domain Specific & 14 & 16 & 38 \\
    Politeness & 18 & 23 & 8 \\
    Figurative language &  9 & 6 & 11 \\
    \midrule
    Sum &  138 & 184 & 246 \\

    \bottomrule
    \end{tabular}%
%   }
  % \vspace{-.25in}
  \label{tab:misclassification}%
\end{table}%
Among the seven error categories, one category was observed the most when the tools were trained on the GitHub dataset: Subjectivity in Annotation. This error was found the most in the Jira dataset in cross-platform settings, i.e., the Jira dataset has inconsistencies in manual labeling (RQ$_3$). One category was observed the most when the tools were trained on the SO dataset: Politeness. This is because we observe fewer sentences relate to politeness in the SO dataset. As such, the tools fail to learn much about the politeness-related polarities, although both GitHub and Jira contain much more non-neutral sentences with politeness.

The other seven categories are observed the most when the tools were trained on the Jira dataset: \begin{inparaenum}
\item General Error, 
\item Implicit Sentiment, 
\item Context/Pragmatics, 
\item Domain Specificity, and 
\item Figurative Language.
\end{inparaenum} There are several reasons for the higher concentration of error categories. First, the Jira dataset does not have many sentences with emojis compared to the other two datasets, which means the tools could not learn notations in words related to emojis properly. Second, the Jira dataset also has inconsistencies in labeling emojis, as we noted in RQ$_3$, which could confuse the tools during learning and then during their prediction in cross-platform settings. Third, most of the sentences in Jira are shorter than the sentences in the other two datasets, thereby offering fewer contexts during the learning of the tools. In \fig\ref{fig:word_counts}, we show the percentage of sentences in each dataset with a number of words. For example, we have around 6\% sentences with less than five words in the Jira dataset, while in the SO dataset, we have around 2\% sentences with less than five words. This is why we see more errors in the tools related to context/pragmatics while those were trained using the Jira dataset. Therefore, the Jira dataset could benefit from more consistent labeling and richer data points (e.g., longer sentences).
\begin{figure}[h]
\centering
% \includegraphics[scale=0.5]{figs/word_distribution.png}
\includegraphics[scale=0.6]{figs/word_distribution.pdf}
% \includegraphics[width=0.35 * linewidth]{res/methology_overview.jpg}
\caption{Distribution of word counts per sentence}
\label{fig:word_counts}
\end{figure}

%  Some of the sentences in the dataset are very small, e.g., Stack Overflow, GitHub, and Jira dataset have respectively  220, 625, 866 sentences that have less than four words.


\subsection{The \it{Issues} with Polarity for Politeness}
% \gias{discuss how you see different polarity for politeness between two datasets and how that was not helpful. now show a stat like if all polarity labels were equally done how much would F1-score have improved in cross-platform setting. for this only consider polarity cases like thanks, thank you, etc. (that means those that you use regular expression to find and relabel automatically}
As we noted in RQ$_3$, the sentences containing politeness are not consistently labeled in the datasets. For example, in the Jira dataset, we showed that similar sentences are labeled as neutral or positive in different places. The presence of politeness seems to have confused the human coders of the three datasets, making the supervised tools error-prone while predicting the labels of the sentences with politeness. To investigate the extent of this problem, we conducted a simple experiment by first picking a sample of sentences with politeness and determining how many of those got misclassified across the datasets in cross-platform settings. First, we find a sample of sentences with politeness with lexical cues like searching for three keywords in the sentences: ``thanks'', ``thank you'', and ``sorry''. In \tbl\ref{tab:politeness_misclassification}, we show the distribution of such sentences in each dataset. Across the three datasets, there are around 2,700 sentences containing politeness (i.e., 15.5\% of all sentences in the three datasets). Out of the three datasets, Jira has the highest number of politeness, around 1,386 (24\%), followed by GitHub with 928 sentences (13\%) and SO with 430 sentences (10\%). 
The last three columns in \tbl\ref{tab:politeness_misclassification} show the percentage of sentences with politeness in each dataset that got misclassified in cross-platform settings while we used the best performing deep learning SD tool in our study, i.e., BERT4SentiSE. For example, when the tool was trained and tested on Jira (i.e., within platform setting), 37.5\% of the sentences with politeness were misclassified. However, while the tool was trained on Jira but tested on GitHub, the only 4.1\% of sentences with politeness in Github were misclassified and only 0.8\% were misclassified for SO dataset. In fact, the difference between the ratios of misclassified cases in the Jira dataset from the other datasets is quite large. When BERT4SentiSE is trained on GitHub and tested on Jira, 36.2\% of the sentences with politeness in Jira remain misclassified. When the tool is trained in SO and tested on Jira, 36.3\% of the sentences remain misclassified. The analysis results confirm our previous observation that to improve the cross-platform performance of the tools in our three studied datasets; we could benefit from reducing inconsistencies in the labeling of politeness in the Jira dataset.

% According to our analysis most of these politeness related misclassification occurs, when DL-based tools are trained on Jira Dataset. During the labeling of the Jira dataset, politeness was considered as mostly with a polarity label. Even within the Jira dataset we found around 20\% times politeness is subjective to human rater. This type of inconsistency confuses the DL-based classifiers.

\begin{table}[t]
\newcolumntype{C}{>{\centering\arraybackslash}p{4em}}
  \centering
  %\vspace{-.1in}
   \caption{Distribution of sentences with politeness and their misclassifications by BERT4SEntiSE and SEntiMoji in cross-platform settings across the datasets}
  % \vspace{-3mm}
    %\resizebox{\columnwidth}{!}{%
    \begin{tabular}{lcc|CCC}
    %  \begin{tabular}{lpp{0.2\textwidth}p{0.2\textwidth}p{0.3\textwidth}}
    \toprule
    \multirow{2}{1.2cm}{\bf{Trained on}} & \multicolumn{2}{c}{\textbf{Politeness}} & \multicolumn{3}{c}{\bf{\% of Misclassified while tested on}}  \\ \cmidrule{2-6}
     & \# & \% & Jira & GitHub & SO \\ 
    \midrule
    Jira       & 1,386 & 24\% & 37.5\% & 4.1\% &  0.8\% \\
    GitHub       & 928 & 13\% & 36.2\% &  9.3\% &  1.5\%\\
    SO  &         430 & 10\% &  36.3\% &  6.0\% &  0.8\% \\

    % Jira       & 1,386 (24\%) & 225/599 & 83/2038 &  7/851    \\
    % GitHub       & 928 (13\%) & 292/807 &  34/363 &  6/409   \\
    % SO  &         430 (10\%) &  276/760 &  68/1141 &  9/362 \\
    
    \bottomrule
    \end{tabular}%
   %}
   % \vspace{-.25in}
  \label{tab:politeness_misclassification}%
\end{table}%

% #misclassified SO, #misclassified JIra, #misclassified GitHub


% Dataset  #units with less than 4 words 
% Dataset  #units with less than 4 words 

% Dataset StackOverflow #units with less than 3 words 93
% Dataset GitHub #units with less than 3 words 331
% Dataset Jira #units with less than 3 words 506

% Dataset StackOverflow #units with less than 4 words 220
% Dataset GitHub #units with less than 4 words 625
% Dataset Jira #units with less than 4 words 866



% By the way, this is the cross platform results using Twitter dataset as training dataset-
% On Dataset: DatasetSenti4SDSO
% Accuracy: 0.649, Precision (Macro): 0.729, Recall (Macro): 0.679, F1 score (Micro): 0.649, F1 score (Macro): 0.652
% On Dataset: OrtuJIRA
% Accuracy: 0.554, Precision (Macro): 0.607, Recall (Macro): 0.676, F1 score (Micro): 0.554, F1 score (Macro): 0.567
% On Dataset: GitHub
% Accuracy: 0.509, Precision (Macro): 0.641, Recall (Macro): 0.547, F1 score (Micro): 0.509, F1 score (Macro): 0.514



\subsection{Cross-Platform Similarity vs Accuracy}\label{sec:sim-vs-acc-twitter}
% \gias{move the twitter data analysis here. explain why this tells you that similarity does play a role in low variations in terms of accuracy between datasets}
\begin{figure*}[h]
\centering
\captionsetup[subfigure]{labelformat=empty}
\pgfplotstableread{

1	.88  .97  .77     .88  .97   .85      .87  .96   .77
2	.87  .96  .65     .85  .93   .76      .85  .93   .78
3	.74  .74 .51      .74  .76   .65      .72  .72   .57
}\datatable
      \subfloat[Test on GitHub]
      {
       \resizebox{1.6 in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub,  Jira,  Twitter},
        	enlarge y limits=false,
        	enlarge x limits=0.23,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.7cm,
        	width=3.6in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
        	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend style={draw=none},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            % nodes near coords,
            nodes near coords style={font=\huge},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	]
        	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=1] \datatable;
        	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=2] \datatable;
        	\addplot[draw=black!80, fill=black!70] table[x index=0,y index=3] \datatable;
        % 	\addplot[draw=black!80, fill=black!100] table[x index=0,y index=4] \datatable;
        
            \legend{JS Divergence
            		 }
        	\end{axis}
    	\end{tikzpicture}
     	}
    %  	\hspace{-1mm}
    	\label{presentation-inconsistency}
    }
    \subfloat[Test on Stack Overflow (SO)]
     {
      \resizebox{1.6 in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub,  Jira,  Twitter},
        	enlarge y limits=false,
        	enlarge x limits=0.23,
        % 	axis y line = none,
        % 	axis y line=left,
        %   axis line style={-},
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,
        % 	axis x line=left,
        % 	axis x line=bottom,
        % 	axis line style={draw=none},
        %	nodes near coords,
        	ymin=0,ymax=1,
        	ybar,
        	bar width=0.7cm,
        	width=3.6in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
            % yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
         	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend style={draw=none},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            nodes near coords style={font=\huge},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	]
        	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=4] \datatable; 
        	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=5] \datatable; %, postaction={pattern=horizontal lines}
        	\addplot[draw=black!80, fill=black!70] table[x index=0,y index=6] \datatable;   %, postaction={pattern=vertical lines}
            % \addplot[draw=black!80, fill=black!100] table[x index=0,y index=8] \datatable;  %, postaction={pattern=vertical lines}
            \legend{,
            % 		 SEntiMoji F1,
                     Cosine Similarity
            		 }
            % \legend{JS Divergence,
            % 		 Cosine Similarity,
            % 		 SEntiMoji F1,
            % 		 BERT4SentiSE F1
            % 		 }
        	\end{axis}
    	\end{tikzpicture}
    	}
    	\hspace{-1mm}
    	\label{signature-inconsistency}
    }
    \subfloat[Test on Jira]
     {
      \resizebox{1.6 in}{!}{%
      \begin{tikzpicture}
        	\begin{axis}[
        	%ylabel=label,
        	xtick=data,
        	xticklabels={Train on GitHub,  Jira,  Twitter},
        	enlarge y limits=false,
        	enlarge x limits=0.23,
            axis y line=none,
            % hide y axis,
            axis x line*=bottom,
            axis y line*=left,,
        	ymin=0,ymax=1.08,
        	ybar,
        	bar width=0.7cm,
        	width=3.6in,
        	height = 2.3in,
        % 	ytick={0,20,...,80},
        %     yticklabels={0\%,20\%,40\%,60\%,80\%},
        	%ylabel={Accepted Answer (\%)},
        	ymajorgrids=false,
        %	xminorgrids=true,
         	yticklabel style={font=\LARGE},
         	xticklabel style={font=\LARGE, /pgf/number format/fixed},	
        	major x tick style = {opacity=0},
        	minor x tick num = 1,    
        	minor tick length=1ex,
        	legend columns=2, 
            legend style={
                /tikz/column 2/.style={
                    column sep=5pt,
                },
                },
        	legend style={at={(0.5,1.40)},
        	legend style={font=\LARGE},
        	legend style={draw=none},
        	legend image post style={scale=2.0},
            anchor=north,legend columns=-1
            },
            nodes near coords style={font=\huge},
            nodes near coords style={rotate=90,  anchor=west}, %
        	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
        	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
        	]
        	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=7] \datatable;
        	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=8] \datatable; %, postaction={pattern=horizontal lines}
        	\addplot[draw=black!80, fill=black!70] table[x index=0,y index=9] \datatable; %, postaction={pattern=vertical lines}
            % \addplot[draw=black!80, fill=black!100] table[x index=0,y index=12] \datatable; %, postaction={pattern=vertical lines}
            \legend{, ,
            		 BERT4SentiSE F1
            		 }
            
        	\end{axis}
    	\end{tikzpicture}
    	}
    % 	%\hspace{-1mm}
    	\label{fig:status-inconsistency}
    }
    


    
    
%\vspace{-3mm}
\caption{Similarity scores between Twitter and other datasets vs Macro F1-scores of BERT4SentiSE in cross platform settings}


\vspace{-3mm}
\label{fig:diversity_performance_twitter}
\end{figure*}

In RQ3, we observed that the three SE datasets we used in this study have
considerable similarity in terms of textual contents (at least 85\%) and that
there is a statistically significant positive correlation between the similarity
between two datasets and the cross-platform performance of the best performing
deep learning SD tool BERT4SentiSE for the two datasets. To better understand
whether this observation is justified, we also checked the similarity of the
three SE tools against a non-SE dataset. The dataset is called
`tweeter-airline-sentiment'. It is available in
Kaggle\footnote{https://www.kaggle.com/crowdflower/twitter-airline-sentiment}.
This dataset has 14,640 tweets from consumers (and their sentiment polarity
labels) about six major airlines from the USA. We trained BER4SentiSE using this
Twitter dataset and then tested the model on our three SE datasets. We also
computed the similarity between the Twitter dataset and our three SE datasets
using the two metrics we introduced in RQ$_2$, i.e., Jensen Shannon Divergence
and Cosine Similarity. In \fig\ref{fig:diversity_performance_twitter}, we show
three blocks of bars. The first block shows the similarity of the GitHub dataset
with the other three datasets (Twitter, GitHub, Jira) using six bars (two each
for the two similarity metrics). The first block also shows the Macro F1-score
of BERT4SentiSE while the tool is tested on the GitHub dataset after training on
the other three datasets. The second block shows similar data for the `Test on SO
dataset', and the third block shows data for the `Test on Jira' dataset. Across all
three test datasets, the Twitter dataset shows the lowest similarity scores
among all datasets (at most 0.74). The cross-platform F1 scores in the three SE
datasets while trained on Twitter are also significantly low (0.51 - 0.65 while
training on Twitter compared to at least 0.77 while training on an SE dataset).
These results confirm that the SE datasets are indeed more similar to each other
compared to their similarity with a non-SE dataset like Twitter. The increased
similarity does indeed impact the performance of the tool BERT4SentiSE in
cross-platform settings for SE datasets.

% In order to better understand the similarity metrics we also compared the similarity of these three cross platform dataset with an different benchmark dataset from Kagegle which is called ``tweeter-airline-sentiment'' which has around 14,640 tweets from six airline from USA. Our experiments show that the $D_{JS}$ of GitHub, SO, Jira and the Tweeter dataset is 0.74, 0.74, and 0.72 respectively and Cosine similarity is 0.74, 0.76, 0.72 respectively.





% \subsection{Agreement of Manual Labels}
% Table \ref{tab:agreement_with_manual_labelling} shows that BERT4SentiSE has the highest agreement $K$ with the manual labeling and SentiMoji has the highest mild disagreement (33\%) and lowest severe disagreement(0\%) when trained on Jira and tested on Stack Overflow dataset. SentiCR has the highest severe disagreement (5\%) with manual labelling when trained on GitHub and tested on Stack Overflow.
% \begin{table}[h]
% %   \footnotesize
%   \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Agreement between  tools and manual labelling}
%     \begin{tabular}{p{0.9cm}lrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Classifier }} & \multicolumn{2}{c}{\bf{Agreement}}
%      &  \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     {Dataset} &  & \bf{$\kappa$} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
    
    
%     \midrule

% %\multicolumn{6}{c}{\textbf{Test dataset: Github}} \\
% %\midrule

% \multirow{5}{1.2cm}{\textbf{GitHub} (Train on GitHub, Test on GitHub)} 
%  & SEntiMoji & 0.84 & 90\% & 1\% & 9\%  \\
%  & BERT4SentiSE & 0.87 & 92\% & 1\% & 7\%  \\
%  & RNN4SentiSE & 0.52 & 68\% & 7\% & 25\%  \\
%  & Senti4SD & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiCR & 0.73 & 83\% & 2\% & 15\%  \\
% \cmidrule{2-6}


% \multirow{5}{1.2cm}{\textbf{SO} (Train on SO, Test on GitHub)} 
%  & SEntiMoji & 0.61 & 75\% & 2\% & 23\%  \\
%  & BERT4SentiSE & 0.65 & 78\% & 3\% & 19\%  \\
%  & RNN4SentiSE & 0.47 & 66\% & 4\% & 30\%  \\
%  & Senti4SD & 0.60 & 74\% & 4\% & 22\%  \\
%  & SentiCR & 0.49 & 68\% & 2\% & 29\%  \\
% \cmidrule{2-6}


% \multirow{5}{1.2cm}{\textbf{Jira} (Train on Jira, Test on GitHub)} 
%  & SEntiMoji & 0.44 & 66\% & 1\% & 33\%  \\
%  & BERT4SentiSE & 0.48 & 68\% & 2\% & 30\%  \\
%  & RNN4SentiSE & 0.35 & 60\% & 4\% & 36\%  \\
%  & Senti4SD & 0.50 & 69\% & 2\% & 28\%  \\
%  & SentiCR & 0.34 & 60\% & 1\% & 39\%  \\
% \midrule



% % \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% % \midrule

% \multirow{5}{1.2cm}{\textbf{SO} (Train on SO, Test on SO)}
%  & SEntiMoji & 0.80 & 87\% & 1\% & 12\%  \\
%  & BERT4SentiSE & 0.82 & 88\% & 1\% & 11\%  \\
%  & RNN4SentiSE & 0.67 & 78\% & 3\% & 19\%  \\
%  & Senti4SD & 0.77 & 85\% & 1\% & 14\%  \\
%  & SentiCR & 0.73 & 82\% & 3\% & 15\%  \\
% \cmidrule{2-6}

% \multirow{5}{1.2cm}{\textbf{GitHub} (Train on GitHub, Test on SO)} 
%  & SEntiMoji & 0.73 & 83\% & 1\% & 16\%  \\
%  & BERT4SentiSE & 0.78 & 85\% & 1\% & 14\%  \\
%  & RNN4SentiSE & 0.49 & 67\% & 4\% & 29\%  \\
%  & Senti4SD & 0.67 & 78\% & 2\% & 20\%  \\
%  & SentiCR & 0.56 & 71\% & 5\% & 23\%  \\
% \cmidrule{2-6}
% \multirow{5}{1.2cm}{\textbf{Jira} (Train on Jira, Test on SO)} 
%  & SEntiMoji & 0.48 & 67\% & 0\% & 33\%  \\
%  & BERT4SentiSE & 0.63 & 76\% & 1\% & 23\%  \\
%  & RNN4SentiSE & 0.34 & 58\% & 4\% & 38\%  \\
%  & Senti4SD & 0.47 & 66\% & 1\% & 33\%  \\
%  & SentiCR & 0.37 & 60\% & 2\% & 38\%  \\
% \midrule

% % \multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
% % \midrule
% \multirow{5}{1.2cm}{\textbf{Jira} (Train on Jira, Test on Jira)}
%  & SEntiMoji & 0.71 & 86\% & 0\% & 14\%  \\
%  & BERT4SentiSE & 0.72 & 86\% & 0\% & 13\%  \\
%  & RNN4SentiSE & 0.57 & 80\% & 1\% & 20\%  \\
%  & Senti4SD & 0.59 & 81\% & 0\% & 19\%  \\
%  & SentiCR & 0.69 & 85\% & 0\% & 15\%  \\
% \cmidrule{2-6}
% \multirow{5}{1.2cm}{\textbf{GitHub} (Train on GitHub, Test on Jira)} 
%  & SEntiMoji & 0.65 & 81\% & 1\% & 18\%  \\
%  & BERT4SentiSE & 0.65 & 81\% & 1\% & 18\%  \\
%  & RNN4SentiSE & 0.45 & 66\% & 2\% & 32\%  \\
%  & Senti4SD & 0.58 & 78\% & 1\% & 21\%  \\
%  & SentiCR & 0.65 & 82\% & 1\% & 17\%  \\
% \cmidrule{2-6}

% \multirow{5}{1.2cm}{\textbf{SO} (Train on SO, Test on Jira)} 
%  & SEntiMoji & 0.65 & 82\% & 1\% & 18\%  \\
%  & BERT4SentiSE & 0.66 & 82\% & 1\% & 17\%  \\
%  & RNN4SentiSE & 0.57 & 77\% & 1\% & 22\%  \\
%  & Senti4SD & 0.46 & 74\% & 1\% & 25\%  \\
%  & SentiCR & 0.34 & 73\% & 1\% & 26\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_with_manual_labelling}%
% \end{table}%



==> SubmissionTOSEM/empirical-study.tex <==

\section{Empirical Study}\label{sec:result}
The major focus of our empirical study is to determine how well deep learning SE-specific SD tools perform in cross-platform settings compared to within platform settings. A within platform setting denotes the training and testing of an SD tool in the same dataset by splitting the dataset into training and testing sets. A cross-platform setting denotes the training of the tool in one dataset (e.g., GitHub) and the testing of it in another dataset (e.g., Jira/Stack Overflow). In particular, we answer five research questions (RQ):
\begin{enumerate}[label=\bf{RQ\arabic{*}.}]
  \item Can deep learning SD tools for SE perform equally well in both within and cross-platform settings? (\sec\ref{sec:rq0})
  \item Can the deep learning SD tools perform better than non-DL tools in cross-platform settings? (\sec\ref{sec:rq-cross-platform-performance})
    \item Can similarity analysis between the studied datasets explain the drop in performance of the deep learning SD tools in the datasets in cross-platform settings? (\sec\ref{sec:rq-cross-platform-similarity})
%  \item To what extent do the SE-specific sentiment detection tools agree in cross-platform settings? %(\sec\ref{sec:cross-platform-agreement})
  \item What are the error categories of the tools in the cross-platform settings? (\sec\ref{sec:rq-cross-platform-error})
  \item To what extent can the deep learning and non-deep learning sentiment detection tools complement each other in cross-platform settings? (\sec\ref{sec:cross-platform-agreement})
\end{enumerate}
RQ1 compares the performance of three SE-specific deep learning SD tools (BERT4SentiSE, SentiMoji, RNN4SentiSE) between within-platform and cross-platform settings. RQ2 investigates whether the change in performance in the DL tools in cross-platform settings is similar to the change in performance we observe in non-DL tools. RQ3 investigates whether the similarity between two datasets can be correlated to the performance of the two best performing DL tools in cross-platform settings across the two datasets. RQ4 investigates the misclassification reasons of the two best performing DL tools across the datasets. RQ5 explores the possibility of improving the performance of the tools in cross-platform settings by analyzing their agreements and disagreements among themselves.

\input{RQ0}
\input{RQ1}
\input{RQ2}
\input{RQ3}
\input{RQ4}

==> SubmissionTOSEM/implications.tex <==
\section{Implications of Findings}\label{sec:implications}
The findings from this study can guide the following stakeholders in software engineering (SE):
\begin{inparaenum}[(1)]
\item \bf{SE Data Scientists} in the software engineering team to determine the feasibility of an SD tool for SE artifacts across diverse SE data repositories,
\item \bf{SE Managers} to determine the best possible SD tool for SE artifacts to learn about organizational sentiments from SE data repositories,
\item \bf{SE Architects} to design an SE pipeline that can include SE-specific SD tools to analyze SE data repositories,
\item \bf{SE Researchers} to improve the performance of the SE-specific SD tools from diverse SE data sources (i.e., cross-platform settings). 
\end{inparaenum} We discuss the implications below by referring to our results from \sec\ref{sec:result} and \sec\ref{sec:discussion}.

\nd\bf{\ul{$\bullet$ SE Data Scientists.}} Technology companies like Microsoft are now including data scientists in almost each SE team~\cite{amershi_se_case_study_2019}. 
The data scientists can work on developing SD tools to analyze the diverse SE data repositories in an organization. Indeed, software analytics using 
sentiment detection has become an important field to support diverse development tasks like software library selection, bug fixing, and so on~\cite{Uddin-OpinionValue-TSE2019,Uddin-OpinerEval-ASE2017}. 
The data scientists in an SE can use the findings from our study to decide whether and how deep learning SD tools can be used in cross-platform settings. In particular, the data scientists can benefit from the following insights from our study:

\begin{inparaenum}[(1)]
\item \ib{Dataset similarity vs. class imbalance problem.} Our analysis in RQ3 finds that there is a statistically significant positive correlation between the similarity of any two datasets in our study and the performance of the two best performing deep learning SD tools (BERT4SentiSE and SentiMoji) in the two datasets in cross-platform settings. We further validate this assumption in \sec\ref{sec:sim-vs-acc-twitter}, where 
we show that for a non-SE dataset like Twitter, the similarity value as well performance of the tools drop 
when we use the dataset to train a tool and then test it on our SE datasets. However, as we noted in RQ$_3$, this observation fails to explain the drop in performance in the tools when they are trained on the Jira 
dataset and then tested on the other two datasets. As we noted in RQ3, the Jira dataset is considerably imbalanced for the two 
polarity classes (positive, negative) compared to the other two datasets. Therefore, data scientists in an SE team can 
use the above two insights as follows. \begin{inparaenum}[(a)]
\item Make the SD datasets more balanced across the three polarity classes, and 
\item The more similar two SE datasets are, the less drop in performance we can expect in the two tools (BERT4SentiSE, SentiMoji) in cross-platform settings.
\end{inparaenum}

\item \ib{Domain-specificity vs cross-platform performance drop.} The rule-based tool SentistrengthSE outperforms 
the best performing supervised SD tool BERT4SentiSE in five out of the six cross-platform settings. Four of the settings involve 
the Jira dataset, e.g., using Jira to train a tool and then test it on other two datasets or use other two datasets to train a tool and then 
test it on the Jira dataset. As we noted above, the Jira dataset has a class imbalance problem, which means that the supervised tool 
may not get enough information of the imbalanced classes when it is trained on the Jira dataset. Our analysis of the dataset shows that there in the Jira dataset, there is
around less than 5\% examples with less than five words. These short sentences
sometimes do not contain enough contextual information. These two shortcomings (i.e., class imbalance and short sentences) in the Jira dataset 
contributed to the inferior performance of the two supervised SD tools when trained on Jira and tested on other datasets. Therefore as discussed in Section (\ref{sec:rq-cross-platform-similarity}) despite configuring the SD tools with the best performing configuration (model settings, hyperparameters, pre-processing guideline) as mentioned by the authors for within-platform settings, the tools made around 94\% to 99\% of its errors by predicting neutral for non-neutral sentences when they were trained on Jira and tested on non-Jira datasets. Moreover, the Jira dataset has the also the most number of errors related to `General Error' among all the datasets (see \sec\ref{sec:error-cat-dist}) for the two deep learning tools BERT4SentiSE and 
SentiMoji. This means that the two tools failed to properly process the Jira dataset during the testing of the dataset. The rule-based 
tool SentistrengthSE is developed by creating rules based on the Jira dataset created by Ortu et
    al.~\cite{Ortu-EmotionalSideJira-MSR2016}. Therefore, SentistrengthSE can also suffer from a lack of understanding of underlying contexts in cross-platform settings. 
    Indeed, 
    our error analysis in RQ4 finds that the most number of errors in SentistrengthSE in the three datasets is due to the inability of the tool 
    to determine the underlying contexts in the data (i.e., domain specificity). Therefore, data scientists in SE need to investigate further 
    SE-specific SD tools 
    before we claim the superiority of 
    a rule-based tool like SentistrengthSE in cross-platform settings.   


    \item \ib{Pre-trained transformer vs. Recurrent neural network architecture in deep learning SD tools.} 
    While the deep learning SD tool BERT4SentiSE is the best performer among the supervised SD tools in our three datasets, both within and cross-platform settings, another deep learning SD tool, RNN4SentiSE, is the worst performer among all tools. Our 
    analysis of the data and the RNN4SentiSE show that this is not due to any specific obvious shortcomings in the tool itself. 
    Instead, this is due to how the tool is designed and used. For example, BERT4SentiSE uses the pre-trained transformer architecture of BERT. 
    SentiMoji uses the Bi-LSTM architecture and is also pre-trained on a large corpus of Twitter and other emoji data. RNN4SentiSE 
    uses simple RNN architecture, and it is not pre-trained either. The success of pre-trained models over other domains is reported 
    across multiple textual classification tasks. As we noted in RQ2, the best performing supervised SD tool in our study, BERT4SentiSE, also 
    shows an almost negligible difference in performance (0.01 - 0.03) from the best performing rule-based tool SentistrengthSE, while BERT4SentiSE 
    outperforming SentistrengthSE considerably for within platform settings. Therefore, SE data scientists can 
    focus on improving SD tools like BERT4SentiSE, like increasing the number of hidden layers, assessing different loss/optimization parameters, etc.   
    
%     Baseline deep learning based tools (RNN4SentiSE) trained from scratch
%     do not perform well in within platform or cross platform settings compare to
%     pretrained DL-based or shallow ML-based tools. The small size of the
%     training dataset might not be enough to these DL-tools to train. Another
%     possible approach to improve performance can be to use better LSTM-based RNN
%     architecture with domain specific word embeddings.
%     
%     \item Pre-trained DL-based tools (BERT4SentiSE or SentiMoji) shows promising
%     result over shallow ML-based tools (SentiCR, Senti4SD). Transfer learning
%     has shown promising result for deep learning based tools in various domains
%     with small dataset. From Section \ref{subsec:learning_curve}, we see it
%     takes relatively very small amount of dataset (less than 30\% of total
%     training dataset) to train a PTM DL-based tool for SE-specific sentiment
%     analysis tasks. so they have a lot of potential to improve performance. The
%     fact that these DL-based tools are outperforming shallow ML-based tools in
%     terms on accuracy on the benchmark dataset is promising. Success of deep
%     learning in other domains shows how eventually deep learning based tools
%     have outperformed other rule based or shallow ML-based tools. So, future
%     efforts in this domain can explore more on how transfer learning and
%     pre-trained language models can help to develop better SD tools.
    
    
\end{inparaenum}    


\nd\bf{\ul{$\bullet$ SE Architects.}} Given the architects in an SE are responsible for designing a software system, they 
can use the findings from our study to decide on the appropriate tool or combination of tools into a Machine Learning (ML) software pipeline 
that supports the analysis of sentiment polarity in diverse SE datasets. In particular, the following findings can assist them in the decision-making process.  

\begin{inparaenum}[(1)]
\item \ib{The trade-off between the best and a good enough SE-specific SD tool across within and cross-platform settings.} The embedding of an ML pipeline 
into a software development life-cycle can be challenging and complicated due to the constant need of 
updating the model and the data used to train and test the model~\cite{Alamin-MLSASDLCQA-TCAS2021}. 
For an SE architect tasked with embedding a SE-specific SD tool into a software system can be 
challenging given the diversity of data in software repositories and the drop in performance 
of the SE-specific SD tools in cross-platform settings as observed by our study (RQ1-RQ2). 
This means that an SE architect will have to consider different combinations of the tools depending on the 
type of data. Such a setup can become more difficult when each tool needs to be updated with new data to ensure 
the tool does not drift and decay over time. In such cases, a good enough tool across all platforms might be desirable, especially 
if the tool does not show a drastic drop in performance in cross-platform settings. The best performing deep learning 
SD tool BERT4SentiSE outperforms other tools across the 
within platform settings. The tool also is the second-best performer by a narrow margin, behind only the rule-based tool SentistrengthSE, 
across the cross-platform settings. Therefore, BERT4SentiSE could be the best choice for an SE architect 
to use it in a software development life-cycle where the sentiment polarity of diverse SE datasets needs to be analyzed in a production 
environment.    

\item \ib{Learning curve vs. data necessity.} The success of supervised SD tools depends largely on the 
volume and quality of data. Intuitively, the more data and representative data we have, the better we can 
expect the supervised SD tool can be to detect sentiment polarity labels. The use of transfer learning principles into 
the pre-trained deep learning SD tools can reduce the reliance on large volume of data, as long as the diverse 
platforms also have vocabularies/patterns learned from domain-neutral data. Indeed, as we find in \sec\ref{subsec:learning_curve}, 
the two best performing pre-trained deep learning SD tools in our study (BERT4SentiSE, SentiMoji) can achieve the best performance for within platform 
settings just by training on 30\% of all training data. Given data collection and maintenance can complicate a software development 
life-cycle greatly, SE architects can benefit from using tools like BERT4SentiSE and SentiMoji in SE-specific software products.
% 
\end{inparaenum}

\nd\bf{\ul{$\bullet$ SE Researchers.}} We have come a long way towards having no SE-specific SD tools in 2016 to having several high-performing 
SE-specific SD tools that can outperform cross-domain SD tools in diverse SE datasets. However, the drop in performance of the SE-specific SD tools 
in cross-platform settings warrants the need for further research in this area to improve the SE-specific SD tools in cross-platform settings. 
In particular, our study findings can assist SE researchers working on this area as follows.   

\begin{inparaenum}[(1)]
    \item \ib{Needs for standard guidelines on the creation of sentiment
    polarity benchmarks.} Our manual analysis and comparison of error categories in the misclassified cases 
    by the two best performing deep learning SD tools in cross-platform setting shows that  
    subjective annotation in manual labeling was the major reason for misclassification by the two tools. This 
    happened because similar sentences were labeled differently by human coders in a given dataset. This means that 
    the human coders were not instructed on specific annotation guidelines. Subjectivity in annotation also happened 
    when similar sentences between two datasets are labeled differently by human coders in the two datasets. This means 
    that two datasets were created by following two different sentiment polarity annotation guidelines. Therefore, a tool trained in 
    one dataset can be wrong in another dataset when it tried to label a similar sentence based on the training instances. 
    Therefore, future SD research in SE should focus on the standardization of the guideline for annotation. Based on our findings, 
    we also call for fixing current datasets so that they all can follow similar annotation guidelines. 


\begin{figure}[h]
\centering
\includegraphics[scale=0.55]{res/error_category_comparison.png}
% \includegraphics[width=0.35 * linewidth]{res/methology_overview.jpg}
\caption{Comparison of misprediction categories of DL-based vs shallow ML-based vs Rule-based SD tools.}
\label{fig:distribution_error_complement}
\vspace{-5mm}
\end{figure}
\item \ib{Finding proper ensemble tool to utilize the strengths of the different SD tools.} Our error analysis in RQ4 shows that 
the distribution of error categories differs depending on the type of the SD tools (i.e., deep learning vs shallow learning vs rule-based). 
In \fig\ref{fig:distribution_error_complement}, we summarize the distribution of error categories (in percentages) from RQ4 across the three types of 
tools we SD tools we studied in our six cross-platform settings. The summary is created by taking the data from the three pie charts in 
\figs\ref{fig:misclassification_chart_dl}, \ref{fig:misclassification_sentisdsenticr}, and \ref{fig:misclassification_sentistrengthse}. The deep learning SD 
tools (BERT4SentiSE, SentiMoji) show most errors due to subjectivity in manual annotation, the shallow learning SD tools (Senti4SD, SentiCR) show most errors due to general errors, while 
the rule-based SD tool (SentistrengthSE) shows the most amount error due to lack of understanding of domain-specific contexts. Intuitively, the three types of 
tools thus can complement each other for a given dataset. This was the motivation behind our RQ5, where we tried seven different ensembles of the tools 
based on the principles of majority voting. However, the majority-based ensemble tool outperformed the best performing stand-alone SD tools in only three out of 
six cross-platform settings, and that too in a narrow margin. Therefore, future research in this area can investigate ensemble techniques better than 
simply taking the majority of the voting.
    
    \item \ib{The need for `more' transfer learning.} From our experiments, we see
    the pre-trained deep learning SD tool BERT4SentiSE performs better than shallow
    ML-based tools SentiCR and Senti4SD. Rule-based tool SentiStrengthSE
    outperforms it by a little margin. BERT4SentiSE uses the BERT architecture, which is based on 
    the principles of transfer learning. This means the BERT4SentiSE benefits from the learning of domain-neutral 
    word embedding in BERT from large corpus data (e.g., Wikipedia, English novels, etc.). Indeed, transfer learning 
    has shown promise to generalize supervised classification models across multiple domains and to make those models 
    more efficient for a given domain with a little amount of training data from the given domain. Indeed, in \sec\ref{subsec:learning_curve}, 
    we find that BERT4SentiSE can reach the optimal performance level for a given dataset by simply using around 30\% of all training data from that 
    dataset. Transfer learning is a constantly evolving paradigm in natural language processing with new techniques being developed 
    rapidly (e.g., RoBERTa\cite{liu2019roberta}, XLNet\cite{Yang-Xlnet-Arxiv2020}, Multi-lingual LASER models, etc.). Therefore, SE research in SD tools can benefit from creating more 
    SD tools for SE based on transfer learning techniques. 
    
\end{inparaenum}

\nd\bf{\ul{$\bullet$ SE Managers.}} Managers in SE teams and organizations need to assess the productivity and mental health of the fellow employees. 
Automated analysis of sentiments expressed by the employees in the SE repositories can be helpful to the manager to get a real-time and comprehensive as well as organization-wide understanding of the employees. Our findings from this study can guide the SE managers while using the SE-specific SD tools for such analysis as follows.  

\begin{inparaenum}[(1)]
    \item \ib{Assessment of developer productivity using sentiment analysis in cross-platform settings.} 
The productivity in a team may depend on developers' sentiments in/of their
diverse development
activities~\cite{Ortu-AreBulliesMoreProductive-MSR205,Guzman-EmotionalAwareness-FSE2013,Pletea-SecurityEmotionSE-MSR2014,Mika-MiningValenceBurnout-MSR2016}. 
Therefore, SE managers in an organization can utilize the sentiment polarity analysis in the diverse SE repositories of the organization to 
learn about the mental health, productivity, and team cohesion in the organization. However, as we have seen in this study, SE datasets can 
be diverse, and an SD tool trained in one dataset suffers a drop in performance when it is tested on another dataset. 
Therefore, SE managers should train and test their SD tool for SE in a given platform instead of applying the SD tool in cross-platform settings. 
Otherwise, the findings obtained may not give an accurate picture of the sentiments across the organization. 
  
    
    \item \ib{The trade-off between majority voting vs. stand-along tool.} Our error analysis in RQ4 and in \fig\ref{fig:distribution_error_complement} show that 
    the SD tools show different errors in cross-platform settings depending on their types (e.g., deep learning vs shallow learning vs rule-based). However, 
    a majority-based ensemble could not outperform the stand-alone best performing SD tools in 50\% of the cross-platform settings. Therefore, SE managers may refrain from using a majority-based ensemble tool to mine sentiment polarity from SE repositories. 
\end{inparaenum}

==> SubmissionTOSEM/implicationsBKP.tex <==

% \begin{table}[h]
%   \centering
%   % \vspace{-.1in}
%   \caption{Summary of the implications of the findings}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{cp{4cm}p{7cm}}
%     \toprule{}
%     \centering \textbf{Theme} & \centering \textbf{Key finding} & \textbf{Implication for SE Stakeholders} \\
%     \midrule
%     \multirow{10}{*}{\parbox{2cm} {\centering Tool's performance }}  & The accuracy of DL-based tools are better or close to shallow ML-based tools or rule-based tools & Future research effort should explore more on latest DL-based SD tools for SE-specific artifacts because the success of DL in other domains (e.g., Computer Vision~\cite{voulodimos2018deep}, Language translation~\cite{wu2020deep}) suggests they have better chance adopt to diverse datasets and outperform other tools \\
%     \cmidrule{2-3}
%     & Pre-trained deep learning based tools can train with smaller dataset & This demonstrates the effectiveness and adaptability for transfer learning~\cite{ruder2019transfer}. Researchers should explore more on the applicability of the latest pre-trained language models\cite{edunov2019pre, floridi2020gpt} \\
%     \bottomrule
    
%     \multirow{10}{*}{\parbox{2cm} {\centering Benchmark Dataset }}  & Lack of standard SE-specific guideline for annotating dataset & A machine learning model is a good as the dataset it learn from. Future research in this domain needs a standard annotation guideline with large benchmark dataset. \\
%     \cmidrule{2-3}
%     & Lack of benchmark dataset from different SE-artifacts & Rule-based tool can still outperform DL-based tool in cross-platform setting this is a probable indication for researcher to investigate further on the lack of diverseness across these datasets. \\
%     \bottomrule
    
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:implication_summary}%
% \end{table}%


% \section{Implications of Findings}\label{sec:implications}
% % \gias{discuss the implications of findings here. For this, do as follows. First summarize the key findings of this paper in a table. The table should have the following columns: Theme, Key Finding, Implications of Key Finding to SE stakeholder. For example a Theme could be `Accuracy', a key finding would be `DL tools show more accuracy than shallow tools in cross-platform setting, implication. discuss. another key finding under `Accuracy' theme is rule-based tool can still outperform DL tool in cross-platform setting. discuss it's implication .... Once the table is created, use it to discuss the implications of findings. support the table with additional summarized graph/figure from the paper.}
% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.55]{res/error_category_comparison.png}
% % \includegraphics[width=0.35 * linewidth]{res/methology_overview.jpg}
% \caption{Comparison of misprediction categories of DL-based vs shallow ML-based vs Rule-based SD tools.}
% \label{fig:distribution_error_complement}
% \end{figure}

% Lets summarize all the implications here.
% \begin{itemize}
%     \item Baseline deep learning based tools (RNN4SentiSE) trained from scratch do not perform well in within platform or cross platform settings compare to pretrained DL-based or shallow ML-based tools. The small size of the training dataset might not be enough to these DL-tools to train. Another possible approach to improve performance can be to use better LSTM-based RNN architecture with domain specific word embeddings.
    
%     \item Pre-trained DL-based tools (BERT4SentiSE or SentiMoji) shows promising result over shallow ML-based tools (SentiCR, Senti4SD). Transfer learning has shown promising result for deep learning based tools in various domains with small dataset. From Section \ref{subsec:learning_curve}, we see it takes relatively very small amount of dataset (less than 30\% of total training dataset) to train a PTM DL-based tool for SE-specific sentiment analysis tasks. so they have a lot of potential to improve performance. The fact that these DL-based tools are outperforming shallow ML-based tools in terms on accuracy on the benchmark dataset is promising. Success of deep learning in other domains shows how eventually deep learning based tools have outperformed other rule based or shallow ML-based tools. So, future efforts in this domain can explore more on how transfer learning and pre-trained language models can help to develop better SD tools.
    
%     \item The performance drop for the studied tools in cross platform settings are almost similar to that of shallow ML-based tools. As BERT4SentiSE and SentiMoji are pre-trained on large language dataset, we expected a significant less drop in performance in cross-platform settings. From our analysis and related studies we find DL-based perform well against underlying general context. But different annotation guideline for different datasets along with subjectivity in annotation (i.e., incorrect sentiment labelling by human) could explain this not so great performance. So, future research should focus on standardizing the guideline for annotation.
    
%     \item Rule based tool (SentiStrengthSE) outperform both shallow ML-based or DL-based tools. Given that the rules of this tool was developed by Islam and Zibran in 2017 for Jira dataset by Ortu et al.~\cite{Ortu-EmotionalSideJira-MSR2016}. The most likely implication of this is that the datasets used in this study from Stack Overflow, GitHub, Jira are not of different distribution. Our statistical analysis (RQ2) also finds that there is a high degree of similarity among these datasets.
    
%     \item We find that there is a statistically significant positive correlation between similarity of contents between any two datasets and the performance of a pre-trained DL-based tools between the two datasets in cross-platform settings. We also find from the cosine similarity and Jensen-Shannon Divergence between these two datasets is not that much, i.e., datasets are not of very much diverse distribution in terms of words used in them. This could be a possible explanation for the high performance of rule based tool because as the dataset is not very different the rules written for the SentiStrengthSE still holds for all these three datasets and thus it performs better than all machine learning based tools.
    
%     \item Our error analysis of the pre-trained DL tools suggest that the main reason of misclassification is subjective annotation and inconsistent annotation guideline. In the similar study Novielli et al.\cite{novielli2020can} reports that 70\% of errors for shallow ML-based tools belong to General error category which is only 21\% for DL-based tools. Rule-based tool SentiStrengthSE suffers from not understanding SE context (36\%), 18\% not being able to generalize linguistic cues (i.e., general errors). DL-based tools perform well in this two categories.
    
%     \item Pre-trained DL-based tools (BERT4SentiSE) outperform rule-based tools in within platform setting for all of the three datasets. This show the superiority of the DL-based tools in learning, i.e., generalizing training dataset.  Unfortunately of different annotation guideline and subjective annotation of different dataset has led to relatively poor performance of the DL-based tools vs rule-based tools. This might also implicate the the pre-trained SD tools can over fit the training dataset and thus suffer from performance when tested on dataset of different distribution.
    
%     \item Our error analysis of the rule-based tool SentiStrengthSE shows that it fails to understand software domain specific context. It suffers from generalizing and learning linguistic cues. It implies that machine learning tools have a promising application for SD tasks. With better and diverse datasets pre-trained DL-based tools will learn from the examples and outperform rule-based tools. 
    
%     \item Our analysis of the dataset shows that there in Jira dataset there is around less than 5\% examples with less than five words. This short sentences sometimes does not contain enough contextual information and subjected to subjective annotation.
    
%     \item Our details error analysis on disagreement with manual labelling suggests that in cross platform settings both the pre-trained models made mistakes because they did not properly understand SE-domain specific context (e.g., ``fix'', ``hang'', ``difficult to use a library'') and implicit sentiments in sentences. Success in large pre-trained models suggests both of these two can be fixed with properly annotated relatively bigger task specific dataset. Only increasing the dataset size is not going to improve the performance of the DL-based tools because if the dataset has inconsistent annotation this will confuse the SD tools to learn some meaningless feature to improve performance. The DL-based can be trained to learn the SE-specific context as well as implicit sentiments only after removing noises from (inconsistent annotation) which is the reason of around 30\% of the tool's misclassification.
    
%     \item Our simple majority voting based ensemble shows better performance and any standalone tool in cross platform settings except for Jira dataset when SentiStrengthSE outperform the ensemble tool. One reason could be SentiStrengthSE's rules were developed by studying Jira platform. One implication for the very small performance improvement for the ensemble tool can be the we might need a more complex ensemble tool. From our error analysis we find the error categories for the DL-based, ML-based and rule-based tools are not same. So, in some way they complement each other. So, future research can explain more on creating a ensemble tool that will perform best in cross platform settings.
    
%     % \item 
    
    
    
    
% \end{itemize}


% In this section, we discuss the implication of the findings of this study that might be useful for various stakeholders. Table \ref{tab:implication_summary} summarizes the implication of this study and it has two dimensions. First one is based on the result of the performance that we observed from our experiment. And the second one is about some of the limitations that we observed during our error analysis. We also discuss on some of the open limitations that future research can explore more.

% \subsection{Tool's performance}

% \nd \bf{ High performance of DL-based tools.} From our experiments we see DL-based tools' SentiMoji and BERT4SentiSE perform better than shallow ML-based tools SentiCR and Senti4SD. Rule-based tool SentiStrengthSE outperform them by a little margin. However this is promising for future researchers because for rule-based tools suffer from learning new patter for new dataset. Machine learning based tools learn from data and so it provides better generalizability. DL-based tools already outperform shallow ML-based tools. So, future research can focus more on DL-based SD tool.

% \nd \bf{ Pre-trained tools for smaller dataset.} From our experiments, we see the worst performing SD tools is actually RNN4SentiSE which is a RNN based DL-based tools. On the other hand the one the best performing tools in cross-platform settings are also DL-based but they are pretrained models. Our experiments also shows these pre-trained DL-based tools also require very small about of new training dataset to train for new task. So, future efforts in this domain can explore more on how transfer learning and pre-trained language models can help to develop better SD tools.



% \subsection{Benchmark Dataset}

% \nd \bf{Lack of standard annotation guideline.} We error analysis on shows subjective annotation and lack of standard annotation guideline is the biggest cause of misclassification in cross platform settings. If we want to develop a generalized well performing SD tools for SE artifacts then investing resources for a DL-based tools is the best way to go. So, future research should focus on standardizing the guideline for annotation.

% \nd \bf{ Lack of diverse dataset.} From our statistical and manual analysis we see the datasets used in this study is not quite as diverse. From our analysis this is one of the reasons, for the rule-based tool SentiStrengthSE to outperform DL-based tools in cross platform settings. Again the benchmark dataset available for SE-specific sentiment analysis is not large enough for DL-based tool to learn from scratch. That's why our baseline DL-tool RNN4SentiSE's performance were so poor. So, future research on this domain can benefit from a large standard SE-specific sentiment dataset from diverse artifact. Future research can focus mitigating this obvious obstacle.



==> SubmissionTOSEM/introduction.tex <==
\section{Introduction}\label{sec:introduction}
Similar to Natural Language Processing (NLP), textual contents in software
engineering (SE) can broadly be divided into two types: facts and
opinions~\cite{liu-sentimentanalysis-handbookchapter-2010,
Uddin-OpinionValue-TSE2019, Uddin-SurveyOpinion-TSE2019}. Facts are objective
expressions (e.g., ``I use this tool'') while opinions are subjective
expressions (e.g., ``I like this tool''). While opinions can have many forms,
the primary focus in SE research has been on sentiment detection, i.e.,
classifying a sentence/post to one of three polarity labels, positive, negative,
and neutral (i.e., absence of positive/negative polarity).

Research in SE finds that opinions are key determinants to many of the
activities in SE like analyzing developers burn
outs~\cite{Mika-MiningValenceBurnout-MSR2016}, assisting in developer API
selection~\cite{Uddin-OpinerEval-ASE2017, Uddin-OpinerReviewToolDemo-ASE2017},
determining the quality of shared knowledge in online
forums~\cite{Uddin-OpinerAPIUsageScenario-TOSEM2021,Uddin-UsageScenarioMining-IST2020,Uddin-MineAPIAspectReviews-PolyTech2017,Uddin-SurveyOpinion-TSE2019}.
As such, accurate detection of sentiment polarity in SE artifacts is essential,
so that the right information is collected to support analysis.

Sentiment detection for SE domain can be insufficiently accurate for not correctly understanding software domain specific jargons while using
off-the-shelf
tools~\cite{Jongeling-SentimentNegative-EMSE2017,Lin-SentimentDetectionNegativeResults-ICSE2018}.
As such, several SE-specific sentiment detection (denoted as `SD' for brevity
from hereon) tools are developed based on wide-ranging techniques like
\textit{rule-based} (e.g., SentistrengthSE~\cite{Islam-SentistrengthSE-MSR2017},
Opiner~\cite{Uddin-OpinerEval-ASE2017},
POME~\cite{Lin-PatternBasedOpinionMining-ICSE2019}), \textit{supervised shallow learning based}
(e.g., Senti4SD~\cite{Calefato-Senti4SD-EMSE2017},
SentiCR~\cite{Ahmed-SentiCRNIER-ASE2017}), and \textit{supervised deep learning based} (e.g.,
RNN4SentiSE~\cite{Biswas-SentiSEWordEmbedding-MSR2019},
BERT4SentiSE~\cite{Biswas-ReliableSentiSEBERT-ICSME2020},
SentiMoji~\cite{Chen-SentiEmoji-FSE2019}).

The SE-specific SD tools are found to outperform off-the-shelf SD tools in
several SE sentiment datasets~\cite{Chen-SentiEmoji-FSE2019, sentiCR_2017}. Each dataset is developed for a specific platform (e.g., Jira code reviews, Stack Overflow discussions, etc.).
The diversity of SE platforms can still make it challenging to apply a
SE-specific SD tool trained in one SE platform (e.g., Jira code review dataset) to apply to
another platform (e.g., Stack Overflow developer discussions). Recently, Novielli et
al.~\cite{Novielli-SEToolCrossPlatform-MSR2020,Novielli-SESentimentCP-EMSE2021} investigated several
supervised shallow learning SE-specific SD tools in cross-platform settings,
i.e., train in one SE sentiment dataset and then test on a different SE
sentiment dataset. They find that the supervised SD tools suffer a decrease in
performance in cross-platform settings. However, it is not known whether we
could observe similar results while using the SE-specific deep learning  SD tools
like BERT4SentiSE~\cite{Biswas-ReliableSentiSEBERT-ICSME2020}, SentiMoji~\cite{Chen-SentiEmoji-FSE2019}, and RNN4SentiSE~\cite{Biswas-SentiSEWordEmbedding-MSR2019}.
An insight into the performance of SE-specific deep learning SD
tools in cross-platform settings and whether and how the deep learning tools outperform other tools is necessary for the following reasons: 
\begin{enumerate} \item The
SE-specific deep learning SD tools are found to have outperformed the shallow
and rule-based tools in the individual benchmark
datasets~\cite{Biswas-ReliableSentiSEBERT-ICSME2020, Chen-SentiEmoji-FSE2019}, i.e., within platform setting. As such,
a reasonable expectation is that the deep learning tools would also outperform the shallow learning SD tools in the cross-platform setting. 
Any deviation from this expectation may indicate issues with the underlying models or datasets.
\item The deep learning tools like BERT4SentiSE are built on top of the advanced
language-based pre-trained transformer model
BERT~\cite{Delvin-BERTArch-Arxiv2018}. A benefit of such pre-trained models is
that they are already trained on a large amount of non-SE but cross-domain
datasets to learn language-specific embedding. Such insights can help the tools to offer
more precise classification in a relatively new domain with little training data. This can
also denote that such models may be more useful in cross-platform settings.
\end{enumerate}

In this paper, we report the results of an empirical study that we conducted to
determine the effectiveness of three SE-specific deep learning SD tools
(BERT4SentiSE~\cite{Biswas-ReliableSentiSEBERT-ICSME2020},
SentiMoji~\cite{Chen-SentiEmoji-FSE2019},
RNN4SentiSE~\cite{Biswas-SentiSEWordEmbedding-MSR2019}) in three datasets:
GitHub~\cite{Novielli-SEToolCrossPlatform-MSR2020}, Jira~\cite{Ortu-AreBulliesMoreProductive-MSR205}, and Stack Overflow~\cite{Calefato-Senti4SD-EMSE2017}. 
These three datasets were also used by Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020,Novielli-SESentimentCP-EMSE2021} to study the performance of SE shallow learning SD tools in cross-platform settings. We answer five research questions in our empirical study:

\nd\bf{RQ$_1$ Can deep learning SD tools for SE perform equally well in both within and cross-platform settings?} The three Deep Learning (DL) tools, 
especially BERT4SentiSE~\cite{Biswas-ReliableSentiSEBERT-ICSME2020} and SentiMoji~\cite{Chen-SentiEmoji-FSE2019} are found to be the best performers in several SE-specific sentiment datasets. However, the experimentation was done for within-platform settings, i.e., the tools were trained and tested on the same dataset. 
It is thus necessary to know whether the tools show similar performance in cross-platform settings. 
For each of the DL-based SD tools, we checked six cross-platform settings, two for each of our three benchmark datasets 
(i.e., train on one of the datasets and test on the other two datasets). BERT4SentiSE is the best performer in cross-platform settings, followed by SentiMoji. For each setting, we observed a drop in
performance in the tools in cross-platform settings compared to the within platform settings.
For example, BERT4SentiSE shows a Macro F1-score of 0.92 for GitHub dataset in within platform setting (i.e., trained on GitHub dataset too), but in cross-platform settings, its performance for GitHub dataset drops to 0.88 when the tool is trained on Stack Overflow (SO) dataset and to 0.65 when the tool is trained on the Jira dataset. The percentage differences in the drop in performance between within and cross-platform settings are the most for RNN4SentiSE (31\%  drop when trained in SO and then tested in Jira). The findings are consistent with Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}, who also observed a drop in performance in the shallow learning SD tools for SE in cross-platform settings. This observation motivated us to compare the performance of DL tools against non-DL tools based on the following research question.

\nd\bf{RQ$_2$ Can the deep learning SD tools perform better than non-deep learning SD tools in cross-platform settings?} 
Given that the deep learning SD tools outperform shallow learning SD tools in
within platform settings, it is important to know whether the DL tools can still
outperform the shallow learning SD tools in cross-platform settings. Novielli et
al.~\cite{Novielli-SEToolCrossPlatform-MSR2020} reported that the rule-based SD tool
(SentistrengthSE) outperformed the shallow learning SD tools in cross-platform
settings. Therefore, we also need to know whether SentistrengthSE can outperform
the deep learning SD tools in cross-platform settings.
We ran two best performing shallow learning SD tools from (Senti4SD and SentiCR) and rule-based
tools SentistrengthSE  Novielli et
al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}. We find that among the shallow vs.
deep learning SD tools in cross-platform settings, BERT4SentiSE is the best
performer in five out of six settings. However, when we compare BERT4SentiSE
against rule-based SentistrengthSE in cross-platform settings, we find that
BERT4SentiSE outperforms SentistrengthSE in only two out of the six settings.
Similar to Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}, we also find that the best
performing shallow learning SD tool (Senti4SD) was outperformed by
SentistrengthSE in all six settings. However, the two best performing deep
learning SD tools (BERT4SentiSE and SentiMoji), especially BERT4SentiSE,
outperform all other tools in within platform settings and are outperformed by
SentiStrengthSE by a narrow margin in cross-platform settings. This finding offers
BERT4SentiSE can be further improved in cross-platform
settings. In particular, the drop in performance of the two tools varies
depending on the datasets. The varying level of drop of performance could be due
to the fact that three datasets are constructed from three different domains. We
thus formulate the following research question to analyze the relationship
between tool performance and dataset similarity.

% Therefore, it is important to know whether the drop in performance we observed in the deep learning SD tools. Because this would mean that the supervised SD tools in SE are not suitable in cross-platform settings based on 
% the current SD datasets. We find that
% the drop in performance is lower in two deep learning (DL) tools like
% BERT4SentiSE and SentiMoji, than the other tools deep and shallow learning tools
% we studied (Senti4SD, SentiCR, RNN4SentiSE). In terms of Macro and Micro
% F1-scores, BERT4SentiSE consistently outperformed other supervised tools in used
% our study in all cases except one (where Senti4SD has an F1-score of 0.69 and
% BERT4SentiSE has 0.68). However,  SentistrengthSE outperformed BERT4SentiSE in
% four out of the six cases, while BERT4SentiSE outperformed SentistrengthSE in
% one case (the other is a tie). The superiority of SentistrengthSE in the
% cross-platform setting is also observed by Novielli et
% al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}.

\nd\bf{RQ$_3$ Can similarity analysis between the studied datasets explain the
drop in performance of the deep learning SD tools in the datasets in
cross-platform settings?} For each pair
of the three datasets, we compute the similarity between the datasets using two
metrics: Cosine similarity and Jensen Shannon Divergence. We find that there is
a statistically significant positive correlation between the similarity of the
cross-platform dataset and SD tool's performance. Therefore, the more similar
the training and test datasets are, the higher the performance of a tool in a
cross-platform setting. However, when we compare the ratio of misclassifications
across the three datasets, we find more misclassifications for tools when those
were trained in Jira and tested in other datasets. However, when the tools were
trained on non-Jira datasets and tested on Jira, the ratio of misclassifications
drops. This means that the drop in performance in the cross-platform settings
could be attributed to other factors besides content diversity. This observation
motivated us to answer the following research question.

% \nd\bf{RQ$_3$ To what extent do the SE-specific sentiment detection tools agree in cross-platform settings?} 
% Given that the drop in performance varies depending on the type of tools, it is important to know whether and how the tools 
% agree with each in cross-platform settings. We find that the DL tools like BERT4SentiSe and SentiMoji agree more with each other in cross-platform settings than they agree with the shallow learning models. Indeed, the Cohen $\kappa$ score is the highest (0.86 - 0.78) between BERT4SentiSe and SentiMoji, while it is between 0.40-0.83 between BERT4SentiSE and the shallow learning tools. This insight can offer cues to further improve the tool in such settings (e.g., by combining those). 

\nd\bf{RQ$_4$ What are the error categories of the tools in the cross-platform
settings?} The superiority of BERT4SentiSE and SentiMoji over the shallow
learning tools offers hope that deep learning tools could be better suited than
the shallow learning tools in cross-platform settings. The similarity analysis
between datasets shows a positive correlation between the
performance of these two tools and the similarity of the content of the datasets,
but the correlation cannot explain why these two tools show varying ratios of
misclassifications across the datasets. We, therefore, needed to analyze misclassifications by the tools across the three datasets manually. We picked 400
misclassified cases from our three datasets, where both BERT4SentiSE and
SentiMoji were wrong. We find a total of seven misclassification categories. The most
observed reason is `subjectivity in annotation', i.e., inconsistency in manual
labeling in the datasets. This means that there were inconsistencies between
human coders on the polarity label of two sentences that are similar (e.g.,
`Thank you' was labeled as `positive' by some coder and `neutral' by others in
multiple datasets). Such inconsistencies confuse the deep learning tools. For
example, they could learn to label `Thank you' as positive by training on SO,
but then will be considered wrong in the Jira dataset (where it is mostly labeled as
`neutral'). We also observe that around 45\% of the misclassified cases in our 400
samples were correctly classified by non-deep learning SD tools. This means that the deep learning and
non-deep learning tools together could offer better performance than individual tools in
cross-platform settings. We thus formulate the following research question.

\nd\bf{RQ$_5$ To what extent the deep learning and non-deep learning sentiment detection tools can complement each other in cross-platform settings?}  We first want to determine to what extent tools agree with each other, especially whether they agree on correct or incorrect classifications. The purpose of this exercise is to determine the feasibility of combining the multiple SD tools in our study to get better performance than and standalone SD tools. We find that the two best-performing deep learning SD tools (BERT4SentiSE and SentiMoji) agree with each other more than other tools' agreement among themselves. Indeed, when we combine these two DL tools in a majority voting classifier (i.e., we label a sentence by combining polarity labels from BERT4SentiSE and SentiMoji), in only two out of six cases they outperform the standalone best performing tool in that setting. Therefore, in cross-platform settings, it will require further improvement of the tools other than simply taking the majority voting of the tools, e.g., improving the datasets by fixing the inconsistency in data labeling.

Based on the findings of our study, we offer the following implications:
\begin{inparaenum}[(1)]
    \item The deep learning SD tools for SE, BERT4SentiSE outperform other supervised tools in cross-platform settings in most cases, but then the tool is outperformed by the rule-based tool SentistrengthSE in most cases. This finding indicates that the supervised SD tools (both shallow and deep learning) are still not robust enough to offer equal performance in both within and cross-platform settings.
    \item BERT4SentiSE outperforms SentistrengthSE by large margin in within platform settings across the three datasets and is only narrowly outperformed by SentiStrengthSE in four out of the six cross-platform settings. This finding offers hope for the feasibility to further improve a pre-trained transformer model like BERT4SentiSE in cross-platform settings.
    \item The three datasets have almost similar contents, although they are created from three different domains. However, the two best-performing deep learning tools (BERT4SentiSE and SentiMoji) show varying level performance drop across the three datasets. We find that this inconsistency is mainly due to the ``subjectivity in annotation by the human coders''. Therefore, further improvement in performance for the supervised tools in cross-platform settings may require the fixing of such subjectivity in the datasets.\end{inparaenum}

\nd\bf{Replication Package}: \url{https://github.com/disa-lab/DeepSentimentSECrossPlatform}

\nd\bf{Paper Organizations.} Section \ref{sec:tools_datasets} provides an overview of the six SD tools and three benchmark datasets for SE used in this study. 
Section \ref{sec:result} presents the result of the study. In Section \ref{sec:discussion} we discuss some major themes emerged during the study. We discuss the implication of the study in Section \ref{sec:implications} and threats to validity of our study findings in Section \ref{sec:threats_to_validity}. Section \ref{sec:related_work} overviews related work. Section \ref{sec:conclusion} concludes the paper.




% Sentiment analysis is a Natural Language Processing (NLP) technique to detect people's opinions and emotions. Sentiment analysis for software engineering (SA4SE) is getting quite the attention of researchers. Most researchers consider sentiment analysis as sentiment polarity classification, i.e., the positive, negative, and neutral polarity of opinion/sentiment expressed in a text. Researchers are exploring the potentials of sentiment analysis for various Software Engineering(SE) tasks such as analyzing sentiments in developer Q\&A forums~\cite{rahman2015recommending}, detecting negative comments API reviews~\cite{zhang2013extracting}, library recommendation, etc. The productivity of a software team may depend on the sentiments of the team members sentiments/emotions on diverse development activities that can be found from these platforms\cite{Ortu-AreBulliesMoreProductive-MSR205, pletea2014security}.

% Researchers have conducted several studies on the performance of various off-the-shelf general-purpose sentiment analysis tools\cite{thelwall2010sentiment, socher2013recursive, loper2002nltk} in the SE artifacts, such as collaborative knowledge-sharing platform (Stack Overflow (SO)) discussions, issue tracking tools (Jira) issues, coding platform (GitHub) comments\cite{guzman2014sentiment}. As the software engineering domain contains much domain-specific jargon, these tools' performances are not satisfactory\cite{jongeling2017negative}. The shortcomings of cross-domain sentiment detection tools motivated the development of several sentiment detection tools for the SE domain\cite{lin2018sentiment}. So, many researchers study to improve the performance of these tools by adding SE related rules/heuristics for rule-based sentiment detection tools such as SentiStrengthSE\cite{SentistrengthSE_2017}, POME\cite{pome_2019} or retraining machine learning-based supervised sentiment detection tools such as Senti4SD\cite{Calefato-Senti4SD-EMSE2017}, SentiCR\cite{sentiCR_2017}, DEVA\cite{islam2018deva} on SE specific dataset. However, Lin et al.~\cite{lin2018sentiment} reported that these tools' performance widely varies in different datasets, and there are many improvement opportunities. Recently, there is a development of DL-based sentiment detection tools (SEntiMoji\cite{Chen-SentiEmoji-FSE2019}, BERT4SentiSE\cite{biswas2020achieving}) that are re-trained on SE specific datasets and they provide significant improvement in performance.

% Novielli et al.\cite{novielli2018benchmark} conducted a benchmark study where they compared the performance of three SE-specific tools such as Senti4SD, SentiCR, SentiStrengthSE focusing on how SE-specific customization improves performance compared to baseline sentiment tool SentiStrength\cite{mike2010sentiment}. In their later studies, Novielli et al.\cite{Novielli-SEToolCrossPlatform-MSR2020} provided a comparative performance study of two shallow ML-based tools Senti4SD, SentiCR and two rule-based tools SentiStrenghtSE, DEVA SE-specific tools against cross-platform settings, i.e., when the gold standard of the target dataset is not available for re-training. In their study, they trained these tools in one platform's dataset and tested in a different platform's dataset. They also reported to what extent these tools agree with each other and misclassification analysis. In this study, we aim to extend the study by adding performance comparison DL-based sentiment classifier with shallow ML-based classifier in cross-platform settings. In line with previous studies\cite{jongeling2017negative, novielli2018benchmark, Novielli-SEToolCrossPlatform-MSR2020, novielli2021assessment}, we define the following four research questions.
% \begin{enumerate}
%   \item How effective are SE-specific deep learning sentiment detection tools in cross platform settings?
%   \item Does similarity in textual contents between cross platform datasets correlate with the performance of the tools?  
%   \item What are the error categories of the tools in the cross-platform settings?
%   \item To what extent do the SE-specific deep and shallow learning sentiment detection tools agree in cross-platform settings?

% \end{enumerate}




% This paper is organized as follows. Section \ref{sec:tools_datasets} provides an overview of the five machine learning-based sentiment classifier and three benchmark datasets used in this study. 
% % It also provides an overview of our study setup and evolution metrics that are used to report the result.
% Section \ref{sec:results} presents the result of the study. 
% % In Section \ref{sec:discussion} we discuss the implication and some insights of our findings.
% We discuss the threats to validity about this study in Section \ref{sec:threats_to_validity}
% Section \ref{sec:related_work} provides a background overview of sentiment analysis in software engineering and related works.
% And finally Section \ref{sec:conclusion} concludes the study.



% % \gias{make the replication package anonymous similar to MSR low code paper}






==> SubmissionTOSEM/relatedwork.tex <==
\section{Related Work}\label{sec:related_work}
% Sentiment analysis have many applications in software development scenarios, such as IT tickets support\cite{blaz2016sentiment}, messages in commit logs\cite{sinha2016analyzing}, reviews on API usage\cite{opiner_2019, uddin2017opiner}, code review\cite{el2019empirical}. Studies suggest\cite{murgia2014developers, gachechiladze2017anger}, developers emotions conveyed during collaborative development has impact on the time taken to fix the issue. The poor performance\cite{jongeling2015choosing, jongeling2017negative} of the off-the-shelf sentiment detection tools\cite{loper2002nltk} motivated researchers to develop SE-specific sentiment detection tools. Subsequently, a number of SE-specific benchmark dataset and tools were developed for detecting sentiments or emotions in SE-platforms\cite{senti4sd_2017, panichella2015can, pome_2019, sentiCR_2017, SentistrengthSE_2017, novielli2018benchmark, opiner_2019, ortu2015bullies, jongeling2017negative, Novielli-SEToolCrossPlatform-MSR2020, novielli2021assessment, sentimoji_2019, islam2018comparison}. 

% The sentiment detection studies in SE domain can be classified in three categories. Initially, there were rule-based sentiment detection tools such as SentiStrengthSE\cite{SentistrengthSE_2017}, POME\cite{pome_2019}, Opiner\cite{opiner_2019}. Then during 2017, there were were shallow ML-based classifier such as SentiCR\cite{sentiCR_2017} and Senti4SD\cite{senti4sd_2017}. Later Novielli et al.\cite{novielli2018benchmark} provided a benchmark studies on the performance of the Senti4SD, SentiCR and SentiStrengthSE and reported the supervised tools performs well when they are retrained on the target dataset and dataset annotation follows standard guideline. Recently there are some DL-based sentiment detection tools for SE artifacts. In 2020, Chen et al.\cite{sentimoji_2019} proposed SentiMoji, based on DeepMoji\cite{deepMoji_2017}, which is an emoji-powered SE-specific sentiment detection tools. In 2020, several studies reported PTM based tools\cite{biswas2019exploringword, zhang_transformer_model_2020}. Biswas et al.\cite{biswas2019exploringword} reported that BERT based sentiment detection classifier provides better performance than general RNN based tools (RNN4SentiSE) from their previous studies\cite{biswas2019exploringword}. At the same time, Zhang et al.\cite{zhang_transformer_model_2020} studied the performance of four PMTs: BERT, AlBERT, RoBERTa, XLNet. They reported that PTMs outperform state-of-the-art rule-based and shallow ML-based tool in benchmark datasets.

% In 2020, Novielli et al.\cite{Novielli-SEToolCrossPlatform-MSR2020} presented a comparison studies on how the shallow ML-based and rules based tools performs in cross-platform settings, i.e., when the gold standard dataset is not available for retraining. In this study, we aim to extend this study by adding the results of the performance of the DL-tools. We provide insights about the misclassification of the DL-tools and benchmark datasets. Our goal is to address the current limitation of SE-specific sentiment classifier and further improve the state of the art.


Sentiment analysis in SE research has focused on \bf{Studies} of sentiments in diverse SE repositories and by developing SE-specific SD \bf{Tools} for different SE datasets.

\bf{\ul{Studies.}} A significant number of studies are conducted to analyze the prevalence and impact of sentiments in SE repositories and development scenarios, such as IT tickets~\cite{Castaldi-SentimentAnalysisITSupport-MSR2016}, collaborative distributed team communications~\cite{Guzman-SentimentAnalysisGithub-MSR2014}, Twitter feeds~\cite{Guzman-NeedleInHaystackTwitterSoftware-RE2016},  commit logs~\cite{Sinha-DeveloperSentimentCommitLog-MSR2016}, security-related discussions in GitHub~\cite{Pletea-SecurityEmotionSE-MSR2014}, API reviews~\cite{Uddin-OpinionValue-TSE2019,Uddin-OpinerEval-ASE2017,Uddin-OpinerReviewToolDemo-ASE2017}, and code reviews~\cite{Ikram-SentimentCodeReview-IST2019}. Studies also combined sentiment analysis with other techniques to improve domain-specific classification, such as to classify app reviews~\cite{Maalej-AutomaticClassificationAppReviews-RE2016,Panichella-ClassifyAppUserReview-ICSME2015}. While sentiment analysis focuses on polarity, emotion analysis focuses on finer-grained expressions such as anger, love, etc. Emotion analysis is used to determine team cohesion, such as the impact of bullies in an SE team~\cite{Ortu-AreBulliesMoreProductive-MSR205}, the relation of VAD (Valence, Arousal, Dominance) scores~\cite{Warriner-VadLexicons-BRM2013} with productivity and burn-out in SE teams~\cite{Mika-MiningValenceBurnout-MSR2016}, and the usage of expressed emotions to prioritize improvements or raise team awareness~\cite{Guzman-EmotionalAwareness-FSE2013,Gachechiladze-AngerDirectionCollaborativeSE-ICSENIER2017}. Overall, analysis of sentiments and emotions is an increasingly popular field in SE~\cite{Novielli-IntroToSpIssueAffectSE-JSS2019,Novielli-SentimentEmotionSE-IEEESoftware2019} 

\bf{\ul{Tools.}} SE-specific sentiment tools are needed, because off-the-shelf sentiment detection tools from other domains are not very accurate~\cite{Jongeling-SentimentAnalysisToolsSe-ICSME2015,Jongeling-SentimentNegative-EMSE2017}. Subsequently, a number of sentiment and emotion detectors and benchmarks were developed for SE~\cite{Islam-Deva-ACMSAC2018,Islam-SentistrengthSE-MSR2017, Lin-PatternBasedOpinionMining-ICSE2019,Uddin-OpinionValue-TSE2019,Calefato-Senti4SD-EMSE2017,Ahmed-SentiCRNIER-ASE2017,Murgia-DoDevelopersFeelEmotion-MSR2014,Ortu-EmotionalSideJira-MSR2016,Chen-SentiEmoji-FSE2019,Islam-Deva-ACMSAC2018,Calefato-EmoTxt-ACII2017,Maipradit-SentimentClassificationNGram-IEEESW2019}. Largely, sentiment detection efforts for SE can be divided into three categories: rule-based, shallow learning-based, and deep learning-based. In this paper, we studied the most recently introduced three deep learning SD tools in cross-platform settings and compared their performance against the best performing shallow learning and rule-based SD tools for SE.
  
Our empirical study in this paper takes motivation from the recent studies by
Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020} on the effectiveness of shallow learning
SD tools in cross-platform settings. We extend this body of SE knowledge by
analyzing the effectiveness of the three most recent deep learning SD tools for
SE in cross-platform settings. Unlike Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}, we
examine the role of similarity between datasets and show that more similarity
between cross-platform SE datasets could offer higher performance in
cross-platform settings. Unlike Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}, we also examine the benefits of creating ensembles of the different SD tools for SE in cross-platform settings.


==> SubmissionTOSEM/studiedToolsDatasets.tex <==
\section{Studied Tools and Datasets}\label{sec:tools_datasets}
In this section, we describe the six SE-specific SD tools (\sec\ref{sec:studied-tools}) and the three SE sentiment datasets (\sec\ref{sec:studied-datasets}) that we studied in this paper.
\subsection{Studied Tools} \label{sec:studied-tools}
% \gias{we also need to talk about whether and how the tools are hybertuned. also discuss the network architecture of the DL tools at a high-level}
Our study focuses on three recently introduced SE-specific deep learning SD tools: \begin{inparaenum}
\item RNN4SentiSE~\cite{Biswas-SentiSEWordEmbedding-MSR2019}, 
\item SentiMoji~\cite{Chen-SentiEmoji-FSE2019}, and
\item BERT4SentiSE~\cite{Biswas-ReliableSentiSEBERT-ICSME2020}.
\end{inparaenum}
Recently, Zhang et al.~\cite{zhang_transformer_model_2020} showed that advanced pre-trained transformer models (PTM) like BERT can outperform shallow learning SE-specific SD tools. The tool BERT4SentiSE~\cite{Biswas-ReliableSentiSEBERT-ICSME2020} is introduced at the same time of Zhang et al.~\cite{zhang_transformer_model_2020}. We thus do not use any PTMs from Zhang et al.~\cite{zhang_transformer_model_2020}. Among the three tools, BERT4SentiSE~\cite{Biswas-ReliableSentiSEBERT-ICSME2020} is the latest SD tool in SE, and it is found to have outperformed all other SE-specific SD tools. 

We compare the performance of the three tools with two best performing shallow learning SE-specific SD tools in the cross-platform studies of Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}:  Senti4SD~\cite{Calefato-Senti4SD-EMSE2017} and SentiCR~\cite{Ahmed-SentiCRNIER-ASE2017}. In addition, given that the rule-based tool SentistrengthSE~\cite{Islam-SentistrengthSE-MSR2017} was found to be superior by Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}, we also compare its performance with the DL SD tools. So, our studied tools can be classified into three types
\begin{inparaenum}
\item \bf{Deep-learning based:} \textit{SentiMoji, BERT4SentiSE, RNN4SentiSE},
\item \bf{Shallow machine learning based:} \textit{Senti4SD, SentiCR},
\item \bf{Rule based:} \textit{SentiStrengthSE}.
\end{inparaenum} We now briefly describe each tool below.

\begin{inparaenum}
% \nd \bf{Deep-learning based:}

\item\bf{SentiMoji~\cite{Chen-SentiEmoji-FSE2019}}  is customized on DeepMoji~\cite{deepMoji_2017}, which uses word embedding learned from 56.5B tweets in two bi-LSTM layers and one attention layer~\cite{Chen-SentiEmoji-FSE2019}. SentiMoji learns vector representation of texts by leveraging how emojis are used and other texts in Twitter and GitHub. SentiMoji outperforms shallow and rule-based SD tools in the datasets of Lin et al.~\cite{Lin-SentimentDetectionNegativeResults-ICSE2018}. The hyper-parameters of SentiMoji are fine-tuned with one hundred million of GitHub-emoji~\cite{lu2018first} posts~\cite{Chen-SentiEmoji-FSE2019} using chain-thaw approach~\cite{deepMoji_2017}. At the final stage, the layers of DeepMoji are kept unchanged, and the final 64-dimensions of the softmax layer are updated with the training dataset. In this research, we use the best-performing architecture of SentiMoji to retrain on the datasets. The pre-trained version of SentiMoji uses SO posts as word embedding. It also utilizes tweets from Twitter to learn generalized and GitHub posts to learn SE-specific sentiment jargons. 



\item\bf{BERT4SentiSE~\cite{Biswas-ReliableSentiSEBERT-ICSME2020}} is based on the BERT model that is developed by Devlin et al. at Google in 2018~\cite{Delvin-BERTArch-Arxiv2018}. It learns a contextual representation of words in a text by looking at the following and the preceding words. It is pre-trained on task-neutral languages. It uses transfer learning~\cite{ruder2019transfer} and attention-based architecture. Biswas et al.~\cite{Biswas-ReliableSentiSEBERT-ICSME2020} proposed a BERT-based pre-trained model, which so far achieved the best performance for SE datasets. In this study, we used the best model parameters reported by the original authors. We used the pre-trained BERT \footnote{\url{http://goo.gl/language/bert}} model consisting of 12 layers, encoder layer of 768, and it contained 110 Million parameters altogether.

\item\bf{RNN4SEntiSE~\cite{Biswas-SentiSEWordEmbedding-MSR2019}}  is an RNN-based model that uses generic word embedding from Google news data. The authors also reported that software domain-specific word embedding from stack overflow posts did not improve performance much. In this study, We use the Google news word embedding with the same LSTM based RNN configuration that the authors used in the original study. Similar to the original study, we used LSTM unit 30, drop out 0.2, batch size 30, and epochs 100 which provided the best results.
% for hypertuning, i.e., LSTM unit 30, batch size 30, drop out 0.2, and epochs [100, 200].

\item\bf{Senti4SD~\cite{Calefato-Senti4SD-EMSE2017}} is initially trained on 4K SO posts. It uses features as a bag of words (BoW), sentiment lexicons, and word embedding. The word embedding is created using Stack Overflow data dump to offer domain-specific information. For this study, we use the Python version~\cite{calefato2019emtk} of the tool. We also used the best hyperparameters that were used in the original study and provided the best results in our experiments. We used a full feature set like the original study, i.e., lexicon features, semantic features, and keyword features.

\item\bf{SentiCR~\cite{sentiCR_2017}} uses Gradient Boosting Tree (GBT) algorithm. It uses a bag of words as features. It leverages SMOTE~\cite{chawla2002smote} to handle a class imbalance by oversampling. Following Uddin et al.~\cite{Uddin-OpinionValue-TSE2019}, we train SentiCR to detect three polarity classes. In this study, we used the best configuration and hyper-parameters reported by the original authors. We used the GBT algorithm for the classification.

\item\bf{SentiStrengthSE~\cite{Islam-SentistrengthSE-MSR2017}} is developed on top of
SentiStrength~\cite{Thelwall-Sentistrength-ASICT2010} by introducing rules and
sentiment words specific to SE. Each negative word has a score
ranging from -2 to -5; a positive word has a score ranging from +2 to +5. The
polarity scores are \it{a priori}, i.e., they do not depend on the contextual
nature of the sentiment expressed in a unit.
It outputs both positive and negative
scores for an input text. The overall polarity score of
an input text is calculated using the algebraic sum of the positive and
negative scores. The text is labeled as `positive' if the sum of scores is
greater than 0, negative if the sum is less than 0, and neutral otherwise. The rules for this tool was developed and tested on the Jira dataset by Ortu et al.~\cite{Ortu-EmotionalSideJira-MSR2016}
\end{inparaenum}



% The performance of the machine learning classifiers largely depends on the quality of the dataset\cite{tantithamthavorn2015impact}. Previous studies\cite{novielli2018benchmark} show, if the manual annotation is not standard then the SE-specific customization can not deliver reasonable performance. The sentiment labelling is subjective, and prior studies\cite{Lin-SentimentDetectionNegativeResults-ICSE2018} suggest human rater have around 18\% disagreement. Without any standard guideline for annotation the labelling can be subjective and result in noisy standard and thus this can result in unreliable performance\cite{novielli2018benchmark, Novielli-SEToolCrossPlatform-MSR2020}. 

\subsection{Studied Datasets}\label{sec:studied-datasets}
We study three datasets: Stack Overflow (SO)~\cite{Calefato-Senti4SD-EMSE2017}, Jira~\cite{Ortu-AreBulliesMoreProductive-MSR205}, and 
GitHub~\cite{Novielli-SEToolCrossPlatform-MSR2020}. These three datasets were also previously used by Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020} in their cross-platform study. 
Table \ref{tab:benchmark_dataset} provides summary statistics of the datasets.
\begin{table}[h]
  \centering
  %\vspace{-.1in}
   \caption{Descriptive statistics of the studied benchmark datasets}
  % \vspace{-3mm}
    % \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lrrrr}
    \toprule{}
    \textbf{Dataset} & \textbf{\#Units} & \textbf{+VE} & \textbf{VN} & \textbf{-VE}\\
    \midrule
    GitHub~\cite{Novielli-SEToolCrossPlatform-MSR2020} & 7,122 & 2,013 (28\%) & 3,022 (43\%) & 2,087 (29\%) \\
    Jira~\cite{Ortu-AreBulliesMoreProductive-MSR205} & 5,869 & 1,128 (19\%) & 3,955 (67\%) & 786 (14\%) \\
    Stack Overflow~\cite{Calefato-Senti4SD-EMSE2017} & 4,423 & 1,527 (35\%) & 1,694 (38\%) & 1,202 (27\%)\\
    \bottomrule
    \end{tabular}%
%   }
   % \vspace{-.25in}
  \label{tab:benchmark_dataset}%
\end{table}%

% We use the following benchmark dataset for SE sentiment analysis research proposed by different researchers. Each unit is labeled with a sentiment polarity such as positive, negative, or neutral. A unit can be a single sentence or a collection of a few sentences. T
\begin{inparaenum}
\item\bf{Stack Overflow (SO) dataset~\cite{Calefato-Senti4SD-EMSE2017}} contains 4,423 SO posts, including questions, comments, and answers manually annotated by twelve trained coders. Each post was annotated by three raters and received the final polarity based on majority voting based on the guideline of Shaver framework~\cite{shaver1987emotion}. The dataset is quite well balanced 35\% positive emotions, 27\% negative emotions, 38\% neutral emotions, i.e., absence of emotions. The Cohen's~\cite{cohen1968weighted} Kappa, $k$, is 0.74 which signifies substantial inter-rater agreement~\cite{viera2005understanding}. 


\item\bf{Jira dataset~\cite{Ortu-AreBulliesMoreProductive-MSR205}} contains 5,869 sentences and issue comments from different open-source software projects (e.g., Spring, Apache). Software developers originally annotated the dataset with six emotions (i.e., love, joy, anger, fear, sadness, surprise). To be consistent with other datasets, we followed similar studies by Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020} and translate \qu{love} and \qu{joy} as a positive sentiment, \qu{anger} and \qu{sadness} as a negative sentiment. \qu{surprise} sentences are discarded because, based on the context, they can be either positive or negative. Finally, the absence of emotions is labeled as neutral. The dataset is not well balanced 19\% positive emotions, 14\% negative emotions, and 67\% neutral emotions. 

\item\bf{GitHub dataset~\cite{Novielli-SEToolCrossPlatform-MSR2020}} contains 7,122 pull requests and commit messages. Three authors annotated the dataset. The raters were trained to label based on the Shaver model. The dataset is built in three iterative steps. It has around 28\% positive, 29\% negative, 43\% neutral polarity labels.
\end{inparaenum}







% \subsection{Experimental settings}
% To answer RQ1 and RQ2, we evaluate our selected three deep learning and two shallow supervised learning tools' performance against our three gold standard datasets. To evaluate performance, we trained the tools under the configuration mentioned in their respective guideline. All of these have made their source code and dataset publicly available. For this study, we needed to change the data processing and output pipeline of these tools.

% To compare the within-platform benchmark, we divided each of our three gold standard datasets into a 10-fold cross-validation set. As mention in Table \ref{tab:benchmark_dataset}, the datasets have a class imbalance, especially the Jira dataset; we used the stratified sampling with scikit-learn\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.model_selection.StratifiedKFold.html}}. Our final 10-folded cross-validated dataset and code is publicly available in our replication package. Our research result within the platform setting is in line with other related studies that also used some of these tools (Senti4SD, SentiCR) against some of these benchmark datasets.



% \subsection{Evaluation Metrics}
% % Following the related works\cite{evalita_2016, novielli2018benchmark}, we can use precision, recall, and f-score for analyzing the performance for the three polarity classes. Additionally, for a quick comparison of each classifier, we can report micro and macro averages for precision, recall, and f-score. The micro averaged metrics calculate the average of all classes of all classes, mainly influenced by the majority class's performance. On the other hand, the macro average signifies each sentiment class's measurement equally by averaging each class's precision, recall, and F1-score. Micro-average is influenced by the performance of the majority classes\cite{sebastiani2002machine}. On the other hand, macro-average shows the ability to classify instances correctly for each class. As the Jira dataset is very unbalanced, the macro-average provides a better metric for performance for this dataset.

% Furthermore we use weighted Kohen Kappa\cite{cohen1968weighted} $K$ to asses the agreement among tools posed in RQ2. Agreement is slight if $0.01 \leqslant K \geqslant 0.20$, fair if $0.21 \leqslant K \geqslant 0.40$, moderate if $0.41 \leqslant K \geqslant 0.60$, substantial if $0.61 \leqslant K \geqslant 0.80$, almost perfect if $0.81 \leqslant K \geqslant 1.00$.

==> SubmissionTOSEM/tables.tex <==

% \begin{sidewaystable}
% \begin{table*}%[t]
% \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Performance of SE-specific sentiment analysis in within-platform and cross-platform settings (SentiSE = SentistrengthSE, DS = Dataset, WPS = Within Platform Settting, CPS = Cross-Platform Setting \gias{divide into table into 3 tables as you are doing in RQ4. Make the tables sideways. see my other sentiment paper I shared with to understand how to make sideways table. ask me if you are confused.})}
%   %\vspace{-3mm}
%   % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{ll|rrr|rrr|rrr|rrr|rrr|rrr}
%     \toprule{}

%     \multirow{2}{*}{\textbf{Setting}}  & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiSE}}\\
%     \cmidrule{3-20}
%     {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
    
%     %\multicolumn{18}{c}{\textbf{Test dataset: GitHub}} \\
%     %\midrule
 
%      \multirow{5}{1.4cm}{\bf{WPS: Test DS GitHub} (Train DS GitHub)}
%      & Negative &  .89 & .85 & .87  & .89 & .91 & .90  & .68 & .69 & .68  & .90 & .89 & .90  & .87 & .69 & .77  & .81 & .71 & .76   \\ 
%      & Neutral &  .87 & .92 & .89  & .92 & .90 & .91  & .73 & .66 & .69  & .89 & .92 & .91  & .77 & .91 & .84  & .74 & .86 & .79   \\ 
%      & Positive &  .94 & .92 & .93  & .93 & .94 & .94  & .64 & .72 & .68  & .94 & .91 & .93  & .89 & .84 & .86  & .85 & .76 & .80   \\ 
%      & Micro-avg &  .90 & .90 & .90  & \textbf{.92} & \textbf{.92} & \textbf{.92}  & .68 & .68 & .68  & .91 & .91 & .91  & .83 & .83 & .83  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .90 & .89 & .90  & \textbf{.91} & \textbf{.92} & \textbf{.92}  & .68 & .69 & .68  & \textbf{.91} & .91 & .91  & .84 & .81 & .82  & .80 & .78 & .78   \\ 

%     \cmidrule{2-20}     

%      % Test dataset: Github
% \multirow{5}{1.4cm}{\bf{CPS: Test DS GitHub} (Train DS SO)}
%  & Negative &  .85 & .62 & .72  & .83 & .73 & .78  & .69 & .49 & .58  & .79 & .56 & .66  & .83 & .37 & .51  & .81 & .71 & .76   \\ 
%  & Neutral &  .67 & .91 & .77  & .71 & .91 & .80  & .61 & .84 & .71  & .71 & .82 & .76  & .60 & .94 & .73  & .74 & .86 & .79   \\ 
%  & Positive &  .88 & .65 & .75  & .88 & .63 & .73  & .78 & .57 & .66  & .76 & .81 & .78  & .86 & .62 & .72  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .75 & .75 & .75  & .78 & .78 & .78  & .66 & .66 & .66  & .74 & .74 & .74  & .68 & .68 & .68  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  .80 & .73 & .75  & \textbf{.81} & .76 & .77  & .69 & .63 & .65  & .75 & .73 & .73  & .76 & .64 & .66  & .80 & \textbf{.78} & \textbf{.78}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.15 & -.15 & -.15 & -.14 & -.14 & -.14 & -.02 & -.02 & -.02 & -.17 & -.17 & -.17 & -.14 & -.14 & -.14  \\ 
% % & & Macro-avg &  -.10 & -.17 & -.15 & -.11 & -.16 & -.15 & .01 & -.05 & -.04 & -.16 & -.18 & -.18 & -.08 & -.17 & -.17  \\ 
% \cmidrule{2-20}
    
    
    
%     % Test dataset: Github
%     \multirow{5}{1.4cm}{\textbf{CPS: Test DS GitHub} (Train DS Jira)} 
%      & Negative &  .91 & .39 & .55  & .90 & .43 & .58  & .75 & .39 & .52  & .85 & .52 & .64  & .88 & .27 & .41  & .81 & .71 & .76   \\ 
%  & Neutral &  .56 & .98 & .72  & .59 & .97 & .73  & .54 & .95 & .69  & .60 & .96 & .74  & .52 & .98 & .68  & .74 & .86 & .79   \\ 
%  & Positive &  .94 & .45 & .60  & .91 & .51 & .65  & .80 & .30 & .44  & .90 & .46 & .61  & .89 & .38 & .53  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .66 & .66 & .66  & .68 & .68 & .68  & .60 & .60 & .60  & .69 & .69 & .69  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  \textbf{.80} & .61 & .62  & \textbf{.80} & .64 & .65  & .70 & .55 & .55  & .78 & .65 & .67  & .76 & .54 & .54  & \textbf{.80} & \textbf{.78} & \textbf{.78}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.24 & -.24 & -.24 & -.23 & -.23 & -.23 & -.08 & -.08 & -.08 & -.22 & -.22 & -.22 & -.23 & -.23 & -.23  \\ 
% % & & Macro-avg &  -.10 & -.29 & -.28 & -.12 & -.28 & -.26 & .02 & -.14 & -.14 & -.13 & -.26 & -.24 & -.08 & -.27 & -.28  \\ 

% \midrule





% %    \multicolumn{18}{c}{\textbf{Test dataset: Stack Overflow}} \\
% %    \midrule
%     \multirow{5}{1.4cm}{\textbf{WPS: Test DS SO} (Train DS SO)} 
%  & Negative &  .84 & .83 & .83  & .86 & .85 & .85  & .74 & .73 & .74  & .80 & .83 & .82  & .80 & .72 & .76  & .76 & .76 & .76   \\ 
%  & Neutral &  .83 & .84 & .84  & .86 & .85 & .85  & .75 & .77 & .76  & .84 & .79 & .81  & .79 & .82 & .81  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .93 & .93  & .93 & .94 & .93  & .85 & .85 & .85  & .90 & .93 & .91  & .88 & .91 & .89  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}  & .78 & .78 & .78  & .85 & .85 & .85  & .82 & .82 & .82  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}  & .78 & .78 & .78  & .85 & .85 & .85  & .82 & .82 & .82  & .80 & .79 & .79   \\ 
 

%     \cmidrule{2-20}
    
%     % Test dataset: Stack Overflow
%     \multirow{5}{1.4cm}{\textbf{CPS: Test DS SO} (Train DS GitHub)} 
%  & Negative &  .82 & .76 & .79  & .80 & .86 & .83  & .66 & .60 & .63  & .69 & .76 & .72  & .64 & .49 & .55  & .76 & .76 & .76   \\ 
%  & Neutral &  .75 & .85 & .80  & .84 & .80 & .82  & .61 & .64 & .63  & .73 & .76 & .75  & .65 & .85 & .74  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .85 & .89  & .93 & .91 & .92  & .73 & .74 & .74  & .92 & .82 & .87  & .88 & .74 & .80  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .83 & .83 & .83  & \textbf{.85} & \textbf{.85} & \textbf{.85}  & .67 & .67 & .67  & .78 & .78 & .78  & .71 & .71 & .71  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .83 & .82 & .82  & \textbf{.85} & \textbf{.86} & \textbf{.85}  & .67 & .66 & .66  & .78 & .78 & .78  & .72 & .69 & .70  & .80 & .79 & .79   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.12 & -.12 & -.12 & -.07 & -.07 & -.07 & -.11 & -.11 & -.11  \\ 
% % & & Macro-avg &  -.03 & -.05 & -.04 & -.03 & -.02 & -.03 & -.11 & -.12 & -.12 & -.06 & -.07 & -.07 & -.10 & -.12 & -.12  \\ 

%     \cmidrule{2-20}


%     % Test dataset: Stack Overflow
%     \multirow{5}{1.4cm}{\textbf{CPS: Test DS SO} (Train DS Jira)}
%  & Negative &  .93 & .31 & .47  & .88 & .55 & .68  & .66 & .31 & .42  & .75 & .30 & .43  & .67 & .22 & .33  & .76 & .76 & .76   \\ 
%  & Neutral &  .54 & .98 & .70  & .63 & .94 & .76  & .50 & .91 & .65  & .54 & .93 & .69  & .50 & .95 & .66  & .73 & .79 & .75   \\ 
%  & Positive &  .98 & .62 & .76  & .97 & .74 & .84  & .83 & .42 & .56  & .96 & .64 & .76  & .96 & .52 & .67  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .67 & .67 & .67  & .76 & .76 & .76  & .58 & .58 & .58  & .66 & .66 & .66  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  .82 & .64 & .64  & \textbf{.83} & .74 & .76  & .66 & .55 & .54  & .75 & .62 & .63  & .71 & .56 & .55  & .80 & \textbf{.79} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.20 & -.20 & -.20 & -.12 & -.12 & -.12 & -.21 & -.21 & -.21 & -.19 & -.19 & -.19 & -.22 & -.22 & -.22  \\ 
% % & & Macro-avg &  -.05 & -.23 & -.23 & -.05 & -.14 & -.12 & -.12 & -.23 & -.24 & -.10 & -.23 & -.22 & -.11 & -.25 & -.27  \\ 

%     \midrule





%     % Test dataset: Jira
% %    \multicolumn{18}{c}{\textbf{Test dataset: Jira}} \\
% %    \midrule
%     \multirow{5}{1.4cm}{\textbf{WPS: Test DS Jira} (Train DS Jira)} 
%  & Negative &  .84 & .68 & .75  & .82 & .76 & .79  & .69 & .46 & .55  & .71 & .55 & .62  & .79 & .66 & .72  & .68 & .73 & .71   \\ 
%  & Neutral &  .89 & .91 & .90  & .90 & .90 & .90  & .83 & .89 & .86  & .84 & .88 & .86  & .89 & .89 & .89  & .92 & .82 & .87   \\ 
%  & Positive &  .79 & .80 & .79  & .78 & .80 & .79  & .73 & .72 & .72  & .73 & .71 & .72  & .75 & .85 & .80  & .68 & .92 & .78   \\ 
%  & Micro-avg &  \textbf{.86} & \textbf{.86} & \textbf{.86}  & \textbf{.86} & \textbf{.86} & \textbf{.86}  & .80 & .80 & .80  & .81 & .81 & .81  & .85 & .85 & .85  & .83 & .83 & .83   \\ 
%  & Macro-avg &  \textbf{.84} & .80 & .81  & .83 & \textbf{.82} & \textbf{.83}  & .75 & .69 & .71  & .76 & .72 & .73  & .81 & .80 & .80  & .76 & \textbf{.82} & .79   \\ 

%     \cmidrule{2-20}
    
    
%     % Test dataset: Jira
%     \multirow{5}{1.4cm}{\textbf{CPS: Test DS Jira} (Train DS GitHub)} 
%  & Negative &  .63 & .75 & .69  & .66 & .74 & .70  & .51 & .71 & .60  & .61 & .64 & .62  & .69 & .60 & .64  & .68 & .73 & .71   \\ 
%  & Neutral &  .93 & .79 & .85  & .93 & .80 & .86  & .92 & .58 & .71  & .89 & .78 & .83  & .90 & .85 & .87  & .92 & .82 & .87   \\ 
%  & Positive &  .66 & .91 & .77  & .65 & .91 & .76  & .45 & .92 & .61  & .62 & .86 & .72  & .69 & .89 & .78  & .68 & .92 & .78   \\ 
%  & Micro-avg &  .81 & .81 & .81  & .81 & .81 & .81  & .66 & .66 & .66  & .78 & .78 & .78  & .82 & .82 & .82  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg &  .74 & \textbf{.82} & .77  & .75 & \textbf{.82} & .77  & .63 & .74 & .64  & .71 & .76 & .73  & \textbf{.76} & .78 & .76  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.05 & -.05 & -.05 & -.05 & -.05 & -.05 & -.14 & -.14 & -.14 & -.03 & -.03 & -.03 & -.03 & -.03 & -.03  \\ 
% % & & Macro-avg &  -.09 & .02 & -.04 & -.09 & -.00 & -.05 & -.12 & .05 & -.07 & -.05 & .05 & -.01 & -.05 & -.02 & -.04  \\ 

%     \cmidrule{2-20}
    
    
%     % Test dataset: Jira
%     \multirow{5}{1.4cm}{\textbf{CPS: Test DS Jira} (Train DS SO)}
%  & Negative &  .67 & .68 & .67  & .72 & .68 & .70  & .58 & .61 & .59  & .50 & .29 & .37  & .36 & .06 & .10  & .68 & .73 & .71   \\ 
%  & Neutral &  .92 & .81 & .86  & .92 & .82 & .87  & .88 & .77 & .82  & .82 & .81 & .81  & .75 & .94 & .83  & .92 & .82 & .87   \\ 
%  & Positive &  .67 & .93 & .78  & .65 & .93 & .76  & .62 & .89 & .73  & .59 & .80 & .68  & .71 & .49 & .58  & .68 & .92 & .78   \\ 
%  & Micro-avg &  .82 & .82 & .82  & .82 & .82 & .82  & .77 & .77 & .77  & .74 & .74 & .74  & .73 & .73 & .73  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg &  .75 & .81 & .77  & \textbf{.76} & .81 & .78  & .69 & .75 & .71  & .64 & .63 & .62  & .61 & .49 & .50  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.07 & -.07 & -.07 & -.12 & -.12 & -.12  \\ 
% % & & Macro-avg &  -.08 & .01 & -.04 & -.07 & -.01 & -.05 & -.05 & .06 & .00 & -.12 & -.08 & -.11 & -.20 & -.30 & -.30  \\ 


%     \bottomrule
%     \end{tabular}%
% %}
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance}%
% \end{table*}%




















% \begin{table*}%[t]
% %\footnotesize
%   \centering
%   %\vspace{-.1in}
%   \caption{Performance of SE-specific sentiment analysis in cross-platform settings}
%   \vspace{-3mm}
%   % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{lll|ccc|ccc|ccc|ccc|ccc}
%     \toprule{}

%     \multirow{2}{*}{\textbf{Setting}} & \multirow{2}{5px}{\textbf{Train Data}} & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}}\\
%     \cmidrule{4-18}
%     {} & {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
    
%     \multicolumn{18}{c}{\textbf{Test dataset: Github}} \\
%     \midrule
 
%     \multirow{5}{5px}{Within platform} & \multirow{5}{*}{GitHub}
%     & Negative &  .89 & .85 & .87  & .89 & .91 & .90  & .68 & .69 & .68  & .90 & .89 & .90  & .87 & .69 & .77   \\ 
%     & & Neutral &  .87 & .92 & .89  & .92 & .90 & .91  & .73 & .66 & .69  & .89 & .92 & .91  & .77 & .91 & .84   \\ 
%     & & Positive &  .94 & .92 & .93  & .93 & .94 & .94  & .64 & .72 & .68  & .94 & .91 & .93  & .89 & .84 & .86   \\ 
%     & & Micro-avg &  .90 & .90 & \textbf{.90}  & .92 & .92 & \textbf{.92}  & .68 & .68 & \textbf{.68}  & .91 & .91 & \textbf{.91}  & .83 & .83 & \textbf{.83}   \\ 
%     & & Macro-avg &  .90 & .89 & \textbf{.90}  & .91 & .92 & \textbf{.92}  & .68 & .69 & \textbf{.68}  & .91 & .91 & \textbf{.91}  & .84 & .81 & \textbf{.82}   \\ 
%     \midrule     
    
    
    
    
%      % Test dataset: Github
% \multirow{5}{5px}{Cross-platform} & \multirow{5}{5px}{Stack Overflow}
%  & Negative &  .85 & .62 & .72  & .83 & .73 & .78  & .69 & .49 & .58  & .79 & .56 & .66  & .83 & .37 & .51   \\ 
% & & Neutral &  .67 & .91 & .77  & .71 & .91 & .80  & .61 & .84 & .71  & .71 & .82 & .76  & .60 & .94 & .73   \\ 
% & & Positive &  .88 & .65 & .75  & .88 & .63 & .73  & .78 & .57 & .66  & .76 & .81 & .78  & .86 & .62 & .72   \\ 
% & & Micro-avg &  .75 & .75 & \textbf{.75}  & .78 & .78 & \textbf{.78}  & .66 & .66 & \textbf{.66}  & .74 & .74 & \textbf{.74}  & .68 & .68 & \textbf{.68}   \\ 
% & & Macro-avg &  .80 & .73 & \textbf{.75}  & .81 & .76 & \textbf{.77}  & .69 & .63 & \textbf{.65}  & .75 & .73 & \textbf{.73}  & .76 & .64 & \textbf{.66}   \\

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.15 & -.15 & -.15 & -.14 & -.14 & -.14 & -.02 & -.02 & -.02 & -.17 & -.17 & -.17 & -.14 & -.14 & -.14  \\ 
% % & & Macro-avg &  -.10 & -.17 & -.15 & -.11 & -.16 & -.15 & .01 & -.05 & -.04 & -.16 & -.18 & -.18 & -.08 & -.17 & -.17  \\ 
% \midrule
    
    
    
%     % Test dataset: Github
%     \multirow{5}{5px}{Cross-platform} & \multirow{5}{*}{Jira}
%      & Negative &  .91 & .39 & .55  & .90 & .43 & .58  & .75 & .39 & .52  & .85 & .52 & .64  & .88 & .27 & .41   \\ 
% & & Neutral &  .56 & .98 & .72  & .59 & .97 & .73  & .54 & .95 & .69  & .60 & .96 & .74  & .52 & .98 & .68   \\ 
% & & Positive &  .94 & .45 & .60  & .91 & .51 & .65  & .80 & .30 & .44  & .90 & .46 & .61  & .89 & .38 & .53   \\ 
% & & Micro-avg &  .66 & .66 & \textbf{.66}  & .68 & .68 & \textbf{.68}  & .60 & .60 & \textbf{.60}  & .69 & .69 & \textbf{.69}  & .60 & .60 & \textbf{.60}   \\ 
% & & Macro-avg &  .80 & .61 & \textbf{.62}  & .80 & .64 & \textbf{.65}  & .70 & .55 & \textbf{.55}  & .78 & .65 & \textbf{.67}  & .76 & .54 & \textbf{.54}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.24 & -.24 & -.24 & -.23 & -.23 & -.23 & -.08 & -.08 & -.08 & -.22 & -.22 & -.22 & -.23 & -.23 & -.23  \\ 
% % & & Macro-avg &  -.10 & -.29 & -.28 & -.12 & -.28 & -.26 & .02 & -.14 & -.14 & -.13 & -.26 & -.24 & -.08 & -.27 & -.28  \\ 

% \midrule





%     \multicolumn{18}{c}{\textbf{Test dataset: Stack Overflow}} \\
%     \midrule
%     \multirow{5}{5px}{Within-platform} & \multirow{5}{5px}{Stack Overflow} 
%      & Negative &  .84 & .83 & .83  & .86 & .85 & .85  & .74 & .73 & .74  & .80 & .83 & .82  & .80 & .72 & .76   \\ 
%     & & Neutral &  .83 & .84 & .84  & .86 & .85 & .85  & .75 & .77 & .76  & .84 & .79 & .81  & .79 & .82 & .81   \\ 
%     & & Positive &  .93 & .93 & .93  & .93 & .94 & .93  & .85 & .85 & .85  & .90 & .93 & .91  & .88 & .91 & .89   \\ 
%     & & Micro-avg &  .87 & .87 & \textbf{.87}  & .88 & .88 & \textbf{.88}  & .78 & .78 & \textbf{.78}  & .85 & .85 & \textbf{.85}  & .82 & .82 & \textbf{.82}   \\ 
%     & & Macro-avg &  .87 & .87 & \textbf{.87}  & .88 & .88 & \textbf{.88}  & .78 & .78 & \textbf{.78}  & .85 & .85 & \textbf{.85}  & .82 & .82 & \textbf{.82}   \\ 

%     \midrule
    
%     % Test dataset: Stack Overflow
%     \multirow{5}{5px}{Cross-platform} & \multirow{5}{*}{GitHub} 
%  & Negative &  .82 & .76 & .79  & .80 & .86 & .83  & .66 & .60 & .63  & .69 & .76 & .72  & .64 & .49 & .55   \\ 
% & & Neutral &  .75 & .85 & .80  & .84 & .80 & .82  & .61 & .64 & .63  & .73 & .76 & .75  & .65 & .85 & .74   \\ 
% & & Positive &  .93 & .85 & .89  & .93 & .91 & .92  & .73 & .74 & .74  & .92 & .82 & .87  & .88 & .74 & .80   \\ 
% & & Micro-avg &  .83 & .83 & \textbf{.83}  & .85 & .85 & \textbf{.85}  & .67 & .67 & \textbf{.67}  & .78 & .78 & \textbf{.78}  & .71 & .71 & \textbf{.71}   \\ 
% & & Macro-avg &  .83 & .82 & \textbf{.82}  & .85 & .86 & \textbf{.85}  & .67 & .66 & \textbf{.66}  & .78 & .78 & \textbf{.78}  & .72 & .69 & \textbf{.70}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.12 & -.12 & -.12 & -.07 & -.07 & -.07 & -.11 & -.11 & -.11  \\ 
% % & & Macro-avg &  -.03 & -.05 & -.04 & -.03 & -.02 & -.03 & -.11 & -.12 & -.12 & -.06 & -.07 & -.07 & -.10 & -.12 & -.12  \\ 

%     \midrule


%     % Test dataset: Stack Overflow
%     \multirow{5}{5px}{Cross-platform} & \multirow{5}{*}{Jira} 
%  & Negative &  .93 & .31 & .47  & .88 & .55 & .68  & .66 & .31 & .42  & .75 & .30 & .43  & .67 & .22 & .33   \\ 
% & & Neutral &  .54 & .98 & .70  & .63 & .94 & .76  & .50 & .91 & .65  & .54 & .93 & .69  & .50 & .95 & .66   \\ 
% & & Positive &  .98 & .62 & .76  & .97 & .74 & .84  & .83 & .42 & .56  & .96 & .64 & .76  & .96 & .52 & .67   \\ 
% & & Micro-avg &  .67 & .67 & \textbf{.67}  & .76 & .76 & \textbf{.76}  & .58 & .58 & \textbf{.58}  & .66 & .66 & \textbf{.66}  & .60 & .60 & \textbf{.60}   \\ 
% & & Macro-avg &  .82 & .64 & \textbf{.64}  & .83 & .74 & \textbf{.76}  & .66 & .55 & \textbf{.54}  & .75 & .62 & \textbf{.63}  & .71 & .56 & \textbf{.55}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.20 & -.20 & -.20 & -.12 & -.12 & -.12 & -.21 & -.21 & -.21 & -.19 & -.19 & -.19 & -.22 & -.22 & -.22  \\ 
% % & & Macro-avg &  -.05 & -.23 & -.23 & -.05 & -.14 & -.12 & -.12 & -.23 & -.24 & -.10 & -.23 & -.22 & -.11 & -.25 & -.27  \\ 

%     \midrule





%     % Test dataset: Jira
%     \multicolumn{18}{c}{\textbf{Test dataset: Jira}} \\
%     \midrule
%     \multirow{5}{5px}{Within-platform} & \multirow{5}{*}{Jira} 
%      & Negative &  .84 & .68 & .75  & .82 & .76 & .79  & .69 & .46 & .55  & .71 & .55 & .62  & .79 & .66 & .72   \\ 
%     & & Neutral &  .89 & .91 & .90  & .90 & .90 & .90  & .83 & .89 & .86  & .84 & .88 & .86  & .89 & .89 & .89   \\ 
%     & & Positive &  .79 & .80 & .79  & .78 & .80 & .79  & .73 & .72 & .72  & .73 & .71 & .72  & .75 & .85 & .80   \\ 
%     & & Micro-avg &  .86 & .86 & \textbf{.86}  & .86 & .86 & \textbf{.86}  & .80 & .80 & \textbf{.80}  & .81 & .81 & \textbf{.81}  & .85 & .85 & \textbf{.85}   \\ 
%     & & Macro-avg &  .84 & .80 & \textbf{.81}  & .83 & .82 & \textbf{.83}  & .75 & .69 & \textbf{.71}  & .76 & .72 & \textbf{.73}  & .81 & .80 & \textbf{.80}   \\ 

%     \midrule
    
    
%     % Test dataset: Jira
%     \multirow{5}{5px}{Cross-platform} & \multirow{5}{*}{GitHub} 
%  & Negative &  .63 & .75 & .69  & .66 & .74 & .70  & .51 & .71 & .60  & .61 & .64 & .62  & .69 & .60 & .64   \\ 
% & & Neutral &  .93 & .79 & .85  & .93 & .80 & .86  & .92 & .58 & .71  & .89 & .78 & .83  & .90 & .85 & .87   \\ 
% & & Positive &  .66 & .91 & .77  & .65 & .91 & .76  & .45 & .92 & .61  & .62 & .86 & .72  & .69 & .89 & .78   \\ 
% & & Micro-avg &  .81 & .81 & \textbf{.81}  & .81 & .81 & \textbf{.81}  & .66 & .66 & \textbf{.66}  & .78 & .78 & \textbf{.78}  & .82 & .82 & \textbf{.82}   \\ 
% & & Macro-avg &  .74 & .82 & \textbf{.77}  & .75 & .82 & \textbf{.77}  & .63 & .74 & \textbf{.64}  & .71 & .76 & \textbf{.73}  & .76 & .78 & \textbf{.76}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.05 & -.05 & -.05 & -.05 & -.05 & -.05 & -.14 & -.14 & -.14 & -.03 & -.03 & -.03 & -.03 & -.03 & -.03  \\ 
% % & & Macro-avg &  -.09 & .02 & -.04 & -.09 & -.00 & -.05 & -.12 & .05 & -.07 & -.05 & .05 & -.01 & -.05 & -.02 & -.04  \\ 

%     \midrule
    
    
%     % Test dataset: Jira
%     \multirow{5}{5px}{Cross-platform} & \multirow{5}{5px}{Stack Overflow} 
%  & Negative &  .67 & .68 & .67  & .72 & .68 & .70  & .58 & .61 & .59  & .50 & .29 & .37  & .36 & .06 & .10   \\ 
% & & Neutral &  .92 & .81 & .86  & .92 & .82 & .87  & .88 & .77 & .82  & .82 & .81 & .81  & .75 & .94 & .83   \\ 
% & & Positive &  .67 & .93 & .78  & .65 & .93 & .76  & .62 & .89 & .73  & .59 & .80 & .68  & .71 & .49 & .58   \\ 
% & & Micro-avg &  .82 & .82 & \textbf{.82}  & .82 & .82 & \textbf{.82}  & .77 & .77 & \textbf{.77}  & .74 & .74 & \textbf{.74}  & .73 & .73 & \textbf{.73}   \\ 
% & & Macro-avg &  .75 & .81 & \textbf{.77}  & .76 & .81 & \textbf{.78}  & .69 & .75 & \textbf{.71}  & .64 & .63 & \textbf{.62}  & .61 & .49 & \textbf{.50}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.07 & -.07 & -.07 & -.12 & -.12 & -.12  \\ 
% % & & Macro-avg &  -.08 & .01 & -.04 & -.07 & -.01 & -.05 & -.05 & .06 & .00 & -.12 & -.08 & -.11 & -.20 & -.30 & -.30  \\ 


%     \bottomrule
%     \end{tabular}%
% %}
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance}%
% \end{table*}%




% % \begin{table}[]
% %   \footnotesize
% %   \centering
% %   %\vspace{-.1in}
% %   \caption{Agreement metrics between  tools with manual labelling. For brevity, \small{Moji = SentiMoji, BERT = BERT4Senti4SE, RNN = RNN4SentiSE, S4SD = Senti4SD,  SCR = SentiCR}}
% %   % \vspace{-3mm}
% %     % \resizebox{\columnwidth}{!}{%
% %     \begin{tabular}{p{0.6cm}lrrrr}
% %     \toprule{}

% %     %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
% %     %\cmidrule{3-6}
% %     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Classifier }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
% %     \cmidrule{5-6}
% %     {Dataset} &  & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
    
    
% %     \midrule

% % \multicolumn{6}{c}{\textbf{Test dataset: Github}} \\
% % \midrule

% % \multirow{5}{*}{GitHub} 
% %  & Moji & 0.84 & 90\% & 1\% & 9\%  \\
% %  & BERT & 0.87 & 92\% & 1\% & 7\%  \\
% %  & RNN & 0.52 & 68\% & 7\% & 25\%  \\
% %  & S4SD & 0.86 & 91\% & 1\% & 8\%  \\
% %  & SCR & 0.73 & 83\% & 2\% & 15\%  \\
% % \midrule


% % \multirow{5}{*}{SO} 
% %  & SEntiMoji & 0.61 & 75\% & 2\% & 23\%  \\
% %  & BERT4SentiSE & 0.65 & 78\% & 3\% & 19\%  \\
% %  & RNN4SentiSE & 0.47 & 66\% & 4\% & 30\%  \\
% %  & Senti4SD & 0.60 & 74\% & 4\% & 22\%  \\
% %  & SentiCR & 0.49 & 68\% & 2\% & 29\%  \\
% % \midrule


% % \multirow{5}{*}{Jira} 
% %  & SEntiMoji & 0.44 & 66\% & 1\% & 33\%  \\
% %  & BERT4SentiSE & 0.48 & 68\% & 2\% & 30\%  \\
% %  & RNN4SentiSE & 0.35 & 60\% & 4\% & 36\%  \\
% %  & Senti4SD & 0.50 & 69\% & 2\% & 28\%  \\
% %  & SentiCR & 0.34 & 60\% & 1\% & 39\%  \\
% % \midrule



% % \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% % \midrule

% % \multirow{5}{*}{SO}
% %  & Moji & 0.80 & 87\% & 1\% & 12\%  \\
% %  & BERT & 0.82 & 88\% & 1\% & 11\%  \\
% %  & RNN & 0.67 & 78\% & 3\% & 19\%  \\
% %  & S4SD & 0.77 & 85\% & 1\% & 14\%  \\
% %  & SCR & 0.73 & 82\% & 3\% & 15\%  \\
% % \midrule

% % \multirow{5}{*}{GitHub} 
% %  & SEntiMoji & 0.73 & 83\% & 1\% & 16\%  \\
% %  & BERT4SentiSE & 0.78 & 85\% & 1\% & 14\%  \\
% %  & RNN4SentiSE & 0.49 & 67\% & 4\% & 29\%  \\
% %  & Senti4SD & 0.67 & 78\% & 2\% & 20\%  \\
% %  & SentiCR & 0.56 & 71\% & 5\% & 23\%  \\
% % \midrule


% % \multirow{5}{*}{Jira} 
% %  & SEntiMoji & 0.48 & 67\% & 0\% & 33\%  \\
% %  & BERT4SentiSE & 0.63 & 76\% & 1\% & 23\%  \\
% %  & RNN4SentiSE & 0.34 & 58\% & 4\% & 38\%  \\
% %  & Senti4SD & 0.47 & 66\% & 1\% & 33\%  \\
% %  & SentiCR & 0.37 & 60\% & 2\% & 38\%  \\
% % \midrule







% % \multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
% % \midrule
% % \multirow{5}{*}{Jira}
% %  & Moji & 0.71 & 86\% & 0\% & 14\%  \\
% %  & BERT & 0.72 & 86\% & 0\% & 13\%  \\
% %  & RNN & 0.57 & 80\% & 1\% & 20\%  \\
% %  & S4SD & 0.59 & 81\% & 0\% & 19\%  \\
% %  & SCR & 0.69 & 85\% & 0\% & 15\%  \\
% % \midrule

% % \multirow{5}{*}{GitHub} 
% %  & SEntiMoji & 0.65 & 81\% & 1\% & 18\%  \\
% %  & BERT4SentiSE & 0.65 & 81\% & 1\% & 18\%  \\
% %  & RNN4SentiSE & 0.45 & 66\% & 2\% & 32\%  \\
% %  & Senti4SD & 0.58 & 78\% & 1\% & 21\%  \\
% %  & SentiCR & 0.65 & 82\% & 1\% & 17\%  \\
% % \midrule


% % \multirow{5}{*}{SO} 
% %  & SEntiMoji & 0.65 & 82\% & 1\% & 18\%  \\
% %  & BERT4SentiSE & 0.66 & 82\% & 1\% & 17\%  \\
% %  & RNN4SentiSE & 0.57 & 77\% & 1\% & 22\%  \\
% %  & Senti4SD & 0.46 & 74\% & 1\% & 25\%  \\
% %  & SentiCR & 0.34 & 73\% & 1\% & 26\%  \\
% % % \midrule
% %     % \midrule  
% %     \bottomrule
% %     \end{tabular}%
% % %   }
% %   % \vspace{-.25in}
% %   \label{tab:agreement_with_manual_labelling}%
% % \end{table}%




















% \begin{table}[]
%   \footnotesize
%   \centering
%   %\vspace{-.1in}
%   \caption{Agreement metrics between  tools in both within platform and cross-platform settings. For brevity, \small{Moji = SentiMoji, BERT = BERT4Senti4SE, RNN = RNN4SentiSE, S4SD = Senti4SD,  SCR = SentiCR}}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{p{0.6cm}lrrrr}
%     \toprule{}

%     %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
%     %\cmidrule{3-6}
%     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Tool1 vs }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
%     \cmidrule{5-6}
%     {Dataset} & \bf{Tool2} & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
    
    
%     \midrule

% \multicolumn{6}{c}{\textbf{Test dataset: Github}} \\
% \midrule

% \multirow{10}{*}{GitHub} 
%  & Moji vs BERT & 0.86 & 91\% & 1\% & 8\%  \\
%  & Moji vs RNN & 0.52 & 68\% & 7\% & 25\%  \\
%  & Moji vs S4SD & 0.83 & 89\% & 1\% & 10\%  \\
%  & Moji vs SCR & 0.76 & 85\% & 2\% & 13\%  \\
%  & BERT vs RNN & 0.53 & 69\% & 7\% & 24\%  \\
%  & BERT vs S4SD & 0.85 & 90\% & 2\% & 8\%  \\
%  & BERT vs SCR & 0.74 & 83\% & 2\% & 14\%  \\
%  & RNN vs S4SD & 0.52 & 69\% & 7\% & 25\%  \\
%  & RNN vs SCR & 0.43 & 63\% & 7\% & 31\%  \\
%  & S4SD vs SCR & 0.74 & 83\% & 2\% & 14\%  \\
% \midrule


% \multirow{10}{*}{SO} 
%  & Moji vs BERT & 0.72 & 83\% & 1\% & 15\%  \\
%  & Moji vs RNN & 0.58 & 76\% & 2\% & 22\%  \\
%  & Moji vs S4SD & 0.51 & 70\% & 3\% & 27\%  \\
%  & Moji vs SCR & 0.40 & 68\% & 2\% & 30\%  \\
%  & BERT vs RNN & 0.59 & 76\% & 2\% & 22\%  \\
%  & BERT vs S4SD & 0.52 & 70\% & 4\% & 26\%  \\
%  & BERT vs SCR & 0.39 & 66\% & 3\% & 31\%  \\
%  & RNN vs S4SD & 0.43 & 65\% & 4\% & 31\%  \\
%  & RNN vs SCR & 0.30 & 62\% & 3\% & 35\%  \\
%  & S4SD vs SCR & 0.45 & 68\% & 2\% & 30\%  \\
% \midrule


% \multirow{10}{*}{Jira} 
%  & Moji vs BERT & 0.78 & 90\% & 0\% & 10\%  \\
%  & Moji vs RNN & 0.54 & 81\% & 1\% & 19\%  \\
%  & Moji vs S4SD & 0.60 & 82\% & 1\% & 18\%  \\
%  & Moji vs SCR & 0.65 & 87\% & 0\% & 13\%  \\
%  & BERT vs RNN & 0.56 & 81\% & 1\% & 18\%  \\
%  & BERT vs S4SD & 0.60 & 81\% & 1\% & 18\%  \\
%  & BERT vs SCR & 0.67 & 87\% & 0\% & 13\%  \\
%  & RNN vs S4SD & 0.44 & 74\% & 2\% & 24\%  \\
%  & RNN vs SCR & 0.45 & 79\% & 1\% & 20\%  \\
%  & S4SD vs SCR & 0.52 & 79\% & 1\% & 20\%  \\
% \midrule



% % \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% % \midrule

% % \multirow{10}{*}{GitHub} 
% %  & Moji vs BERT & 0.79 & 86\% & 1\% & 13\%  \\
% %  & Moji vs RNN & 0.53 & 70\% & 4\% & 27\%  \\
% %  & Moji vs S4SD & 0.70 & 80\% & 3\% & 17\%  \\
% %  & Moji vs SCR & 0.62 & 75\% & 5\% & 20\%  \\
% %  & BERT vs RNN & 0.53 & 69\% & 5\% & 26\%  \\
% %  & BERT vs S4SD & 0.73 & 82\% & 2\% & 16\%  \\
% %  & BERT vs SCR & 0.60 & 74\% & 5\% & 21\%  \\
% %  & RNN vs S4SD & 0.54 & 69\% & 4\% & 26\%  \\
% %  & RNN vs SCR & 0.40 & 61\% & 6\% & 33\%  \\
% %  & S4SD vs SCR & 0.58 & 73\% & 4\% & 23\%  \\
% % \midrule


% % \multirow{10}{*}{Jira} 
% %  & Moji vs BERT & 0.66 & 82\% & 0\% & 18\%  \\
% %  & Moji vs RNN & 0.47 & 75\% & 1\% & 23\%  \\
% %  & Moji vs S4SD & 0.60 & 81\% & 1\% & 19\%  \\
% %  & Moji vs SCR & 0.56 & 80\% & 1\% & 19\%  \\
% %  & BERT vs RNN & 0.43 & 70\% & 2\% & 28\%  \\
% %  & BERT vs S4SD & 0.57 & 77\% & 1\% & 22\%  \\
% %  & BERT vs SCR & 0.52 & 75\% & 1\% & 25\%  \\
% %  & RNN vs S4SD & 0.42 & 72\% & 2\% & 27\%  \\
% %  & RNN vs SCR & 0.33 & 70\% & 1\% & 29\%  \\
% %  & S4SD vs SCR & 0.51 & 77\% & 1\% & 22\%  \\
% % \midrule







% % \multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
% % \midrule

% % \multirow{10}{*}{GitHub} 
% %  & Moji vs BERT & 0.81 & 89\% & 1\% & 10\%  \\
% %  & Moji vs RNN & 0.56 & 72\% & 3\% & 25\%  \\
% %  & Moji vs S4SD & 0.72 & 84\% & 1\% & 14\%  \\
% %  & Moji vs SCR & 0.75 & 86\% & 1\% & 13\%  \\
% %  & BERT vs RNN & 0.57 & 73\% & 3\% & 24\%  \\
% %  & BERT vs S4SD & 0.73 & 85\% & 1\% & 14\%  \\
% %  & BERT vs SCR & 0.75 & 87\% & 1\% & 13\%  \\
% %  & RNN vs S4SD & 0.52 & 70\% & 3\% & 27\%  \\
% %  & RNN vs SCR & 0.50 & 69\% & 2\% & 28\%  \\
% %  & S4SD vs SCR & 0.68 & 83\% & 1\% & 16\%  \\
% % \midrule


% % \multirow{10}{*}{SO} 
% %  & Moji vs BERT & 0.80 & 89\% & 1\% & 10\%  \\
% %  & Moji vs RNN & 0.70 & 84\% & 1\% & 15\%  \\
% %  & Moji vs S4SD & 0.61 & 79\% & 1\% & 19\%  \\
% %  & Moji vs SCR & 0.35 & 70\% & 1\% & 29\%  \\
% %  & BERT vs RNN & 0.72 & 84\% & 1\% & 14\%  \\
% %  & BERT vs S4SD & 0.60 & 79\% & 2\% & 19\%  \\
% %  & BERT vs SCR & 0.36 & 71\% & 1\% & 28\%  \\
% %  & RNN vs S4SD & 0.56 & 77\% & 2\% & 22\%  \\
% %  & RNN vs SCR & 0.30 & 67\% & 1\% & 32\%  \\
% %  & S4SD vs SCR & 0.41 & 76\% & 1\% & 23\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_github}%
% \end{table}%


% \begin{table}[]
%   \footnotesize
%   \centering
%   %\vspace{-.1in}
%   \caption{Agreement metrics between  tools in both within platform and cross-platform settings. For brevity, \small{Moji = SentiMoji, BERT = BERT4Senti4SE, RNN = RNN4SentiSE, S4SD = Senti4SD,  SCR = SentiCR}}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{p{0.6cm}lrrrr}
%     \toprule{}

%     %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
%     %\cmidrule{3-6}
%     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Tool1 vs }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
%     \cmidrule{5-6}
%     {Dataset} & \bf{Tool2} & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
    
    
%     \midrule

% % \multicolumn{6}{c}{\textbf{Test dataset: Github}} \\
% % \midrule

% % \multirow{10}{*}{GitHub} 
% %  & Moji vs BERT & 0.86 & 91\% & 1\% & 8\%  \\
% %  & Moji vs RNN & 0.52 & 68\% & 7\% & 25\%  \\
% %  & Moji vs S4SD & 0.83 & 89\% & 1\% & 10\%  \\
% %  & Moji vs SCR & 0.76 & 85\% & 2\% & 13\%  \\
% %  & BERT vs RNN & 0.53 & 69\% & 7\% & 24\%  \\
% %  & BERT vs S4SD & 0.85 & 90\% & 2\% & 8\%  \\
% %  & BERT vs SCR & 0.74 & 83\% & 2\% & 14\%  \\
% %  & RNN vs S4SD & 0.52 & 69\% & 7\% & 25\%  \\
% %  & RNN vs SCR & 0.43 & 63\% & 7\% & 31\%  \\
% %  & S4SD vs SCR & 0.74 & 83\% & 2\% & 14\%  \\
% % \midrule


% % \multirow{10}{*}{SO} 
% %  & Moji vs BERT & 0.72 & 83\% & 1\% & 15\%  \\
% %  & Moji vs RNN & 0.58 & 76\% & 2\% & 22\%  \\
% %  & Moji vs S4SD & 0.51 & 70\% & 3\% & 27\%  \\
% %  & Moji vs SCR & 0.40 & 68\% & 2\% & 30\%  \\
% %  & BERT vs RNN & 0.59 & 76\% & 2\% & 22\%  \\
% %  & BERT vs S4SD & 0.52 & 70\% & 4\% & 26\%  \\
% %  & BERT vs SCR & 0.39 & 66\% & 3\% & 31\%  \\
% %  & RNN vs S4SD & 0.43 & 65\% & 4\% & 31\%  \\
% %  & RNN vs SCR & 0.30 & 62\% & 3\% & 35\%  \\
% %  & S4SD vs SCR & 0.45 & 68\% & 2\% & 30\%  \\
% % \midrule


% % \multirow{10}{*}{Jira} 
% %  & Moji vs BERT & 0.78 & 90\% & 0\% & 10\%  \\
% %  & Moji vs RNN & 0.54 & 81\% & 1\% & 19\%  \\
% %  & Moji vs S4SD & 0.60 & 82\% & 1\% & 18\%  \\
% %  & Moji vs SCR & 0.65 & 87\% & 0\% & 13\%  \\
% %  & BERT vs RNN & 0.56 & 81\% & 1\% & 18\%  \\
% %  & BERT vs S4SD & 0.60 & 81\% & 1\% & 18\%  \\
% %  & BERT vs SCR & 0.67 & 87\% & 0\% & 13\%  \\
% %  & RNN vs S4SD & 0.44 & 74\% & 2\% & 24\%  \\
% %  & RNN vs SCR & 0.45 & 79\% & 1\% & 20\%  \\
% %  & S4SD vs SCR & 0.52 & 79\% & 1\% & 20\%  \\
% % \midrule



% \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% \midrule

% \multirow{10}{*}{SO} 
%  & Moji vs BERT & 0.86 & 91\% & 1\% & 8\%  \\
%  & Moji vs RNN & 0.70 & 80\% & 3\% & 17\%  \\
%  & Moji vs S4SD & 0.81 & 88\% & 1\% & 12\%  \\
%  & Moji vs SCR & 0.78 & 85\% & 2\% & 12\%  \\
%  & BERT vs RNN & 0.71 & 81\% & 2\% & 17\%  \\
%  & BERT vs S4SD & 0.83 & 88\% & 1\% & 11\%  \\
%  & BERT vs SCR & 0.78 & 85\% & 3\% & 12\%  \\
%  & RNN vs S4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & RNN vs SCR & 0.65 & 77\% & 4\% & 19\%  \\
%  & S4SD vs SCR & 0.78 & 85\% & 3\% & 12\%  \\
% \midrule

% \multirow{10}{*}{GitHub} 
%  & Moji vs BERT & 0.79 & 86\% & 1\% & 13\%  \\
%  & Moji vs RNN & 0.53 & 70\% & 4\% & 27\%  \\
%  & Moji vs S4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & Moji vs SCR & 0.62 & 75\% & 5\% & 20\%  \\
%  & BERT vs RNN & 0.53 & 69\% & 5\% & 26\%  \\
%  & BERT vs S4SD & 0.73 & 82\% & 2\% & 16\%  \\
%  & BERT vs SCR & 0.60 & 74\% & 5\% & 21\%  \\
%  & RNN vs S4SD & 0.54 & 69\% & 4\% & 26\%  \\
%  & RNN vs SCR & 0.40 & 61\% & 6\% & 33\%  \\
%  & S4SD vs SCR & 0.58 & 73\% & 4\% & 23\%  \\
% \midrule


% \multirow{10}{*}{Jira} 
%  & Moji vs BERT & 0.66 & 82\% & 0\% & 18\%  \\
%  & Moji vs RNN & 0.47 & 75\% & 1\% & 23\%  \\
%  & Moji vs S4SD & 0.60 & 81\% & 1\% & 19\%  \\
%  & Moji vs SCR & 0.56 & 80\% & 1\% & 19\%  \\
%  & BERT vs RNN & 0.43 & 70\% & 2\% & 28\%  \\
%  & BERT vs S4SD & 0.57 & 77\% & 1\% & 22\%  \\
%  & BERT vs SCR & 0.52 & 75\% & 1\% & 25\%  \\
%  & RNN vs S4SD & 0.42 & 72\% & 2\% & 27\%  \\
%  & RNN vs SCR & 0.33 & 70\% & 1\% & 29\%  \\
%  & S4SD vs SCR & 0.51 & 77\% & 1\% & 22\%  \\
% % \midrule

%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_so}%
% \end{table}%



% \begin{table}[]
%   \footnotesize
%   \centering
%   %\vspace{-.1in}
%   \caption{Agreement metrics between  tools in both within platform and cross-platform settings. For brevity, \small{Moji = SentiMoji, BERT = BERT4Senti4SE, RNN = RNN4SentiSE, S4SD = Senti4SD,  SCR = SentiCR}}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{p{0.6cm}lrrrr}
%     \toprule{}

%     %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
%     %\cmidrule{3-6}
%     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Tool1 vs }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
%     \cmidrule{5-6}
%     {Dataset} & \bf{Tool2} & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
    
    
%     \midrule

% % \multicolumn{6}{c}{\textbf{Test dataset: Github}} \\
% % \midrule

% % \multirow{10}{*}{GitHub} 
% %  & Moji vs BERT & 0.86 & 91\% & 1\% & 8\%  \\
% %  & Moji vs RNN & 0.52 & 68\% & 7\% & 25\%  \\
% %  & Moji vs S4SD & 0.83 & 89\% & 1\% & 10\%  \\
% %  & Moji vs SCR & 0.76 & 85\% & 2\% & 13\%  \\
% %  & BERT vs RNN & 0.53 & 69\% & 7\% & 24\%  \\
% %  & BERT vs S4SD & 0.85 & 90\% & 2\% & 8\%  \\
% %  & BERT vs SCR & 0.74 & 83\% & 2\% & 14\%  \\
% %  & RNN vs S4SD & 0.52 & 69\% & 7\% & 25\%  \\
% %  & RNN vs SCR & 0.43 & 63\% & 7\% & 31\%  \\
% %  & S4SD vs SCR & 0.74 & 83\% & 2\% & 14\%  \\
% % \midrule


% % \multirow{10}{*}{SO} 
% %  & Moji vs BERT & 0.72 & 83\% & 1\% & 15\%  \\
% %  & Moji vs RNN & 0.58 & 76\% & 2\% & 22\%  \\
% %  & Moji vs S4SD & 0.51 & 70\% & 3\% & 27\%  \\
% %  & Moji vs SCR & 0.40 & 68\% & 2\% & 30\%  \\
% %  & BERT vs RNN & 0.59 & 76\% & 2\% & 22\%  \\
% %  & BERT vs S4SD & 0.52 & 70\% & 4\% & 26\%  \\
% %  & BERT vs SCR & 0.39 & 66\% & 3\% & 31\%  \\
% %  & RNN vs S4SD & 0.43 & 65\% & 4\% & 31\%  \\
% %  & RNN vs SCR & 0.30 & 62\% & 3\% & 35\%  \\
% %  & S4SD vs SCR & 0.45 & 68\% & 2\% & 30\%  \\
% % \midrule


% % \multirow{10}{*}{Jira} 
% %  & Moji vs BERT & 0.78 & 90\% & 0\% & 10\%  \\
% %  & Moji vs RNN & 0.54 & 81\% & 1\% & 19\%  \\
% %  & Moji vs S4SD & 0.60 & 82\% & 1\% & 18\%  \\
% %  & Moji vs SCR & 0.65 & 87\% & 0\% & 13\%  \\
% %  & BERT vs RNN & 0.56 & 81\% & 1\% & 18\%  \\
% %  & BERT vs S4SD & 0.60 & 81\% & 1\% & 18\%  \\
% %  & BERT vs SCR & 0.67 & 87\% & 0\% & 13\%  \\
% %  & RNN vs S4SD & 0.44 & 74\% & 2\% & 24\%  \\
% %  & RNN vs SCR & 0.45 & 79\% & 1\% & 20\%  \\
% %  & S4SD vs SCR & 0.52 & 79\% & 1\% & 20\%  \\
% % \midrule



% % \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% % \midrule

% % \multirow{10}{*}{SO} 
% %  & Moji vs BERT & 0.86 & 91\% & 1\% & 8\%  \\
% %  & Moji vs RNN & 0.70 & 80\% & 3\% & 17\%  \\
% %  & Moji vs S4SD & 0.81 & 88\% & 1\% & 12\%  \\
% %  & Moji vs SCR & 0.78 & 85\% & 2\% & 12\%  \\
% %  & BERT vs RNN & 0.71 & 81\% & 2\% & 17\%  \\
% %  & BERT vs S4SD & 0.83 & 88\% & 1\% & 11\%  \\
% %  & BERT vs SCR & 0.78 & 85\% & 3\% & 12\%  \\
% %  & RNN vs S4SD & 0.70 & 80\% & 3\% & 17\%  \\
% %  & RNN vs SCR & 0.65 & 77\% & 4\% & 19\%  \\
% %  & S4SD vs SCR & 0.78 & 85\% & 3\% & 12\%  \\
% % \midrule

% % \multirow{10}{*}{GitHub} 
% %  & Moji vs BERT & 0.79 & 86\% & 1\% & 13\%  \\
% %  & Moji vs RNN & 0.53 & 70\% & 4\% & 27\%  \\
% %  & Moji vs S4SD & 0.70 & 80\% & 3\% & 17\%  \\
% %  & Moji vs SCR & 0.62 & 75\% & 5\% & 20\%  \\
% %  & BERT vs RNN & 0.53 & 69\% & 5\% & 26\%  \\
% %  & BERT vs S4SD & 0.73 & 82\% & 2\% & 16\%  \\
% %  & BERT vs SCR & 0.60 & 74\% & 5\% & 21\%  \\
% %  & RNN vs S4SD & 0.54 & 69\% & 4\% & 26\%  \\
% %  & RNN vs SCR & 0.40 & 61\% & 6\% & 33\%  \\
% %  & S4SD vs SCR & 0.58 & 73\% & 4\% & 23\%  \\
% % \midrule


% % \multirow{10}{*}{Jira} 
% %  & Moji vs BERT & 0.66 & 82\% & 0\% & 18\%  \\
% %  & Moji vs RNN & 0.47 & 75\% & 1\% & 23\%  \\
% %  & Moji vs S4SD & 0.60 & 81\% & 1\% & 19\%  \\
% %  & Moji vs SCR & 0.56 & 80\% & 1\% & 19\%  \\
% %  & BERT vs RNN & 0.43 & 70\% & 2\% & 28\%  \\
% %  & BERT vs S4SD & 0.57 & 77\% & 1\% & 22\%  \\
% %  & BERT vs SCR & 0.52 & 75\% & 1\% & 25\%  \\
% %  & RNN vs S4SD & 0.42 & 72\% & 2\% & 27\%  \\
% %  & RNN vs SCR & 0.33 & 70\% & 1\% & 29\%  \\
% %  & S4SD vs SCR & 0.51 & 77\% & 1\% & 22\%  \\
% % \midrule







% \multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
% \midrule


% \multirow{10}{*}{Jira} 
%  & Moji vs BERT & 0.85 & 93\% & 0\% & 7\%  \\
%  & Moji vs RNN & 0.68 & 86\% & 0\% & 14\%  \\
%  & Moji vs S4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & Moji vs SCR & 0.81 & 91\% & 0\% & 9\%  \\
%  & BERT vs RNN & 0.68 & 85\% & 1\% & 14\%  \\
%  & BERT vs S4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & BERT vs SCR & 0.79 & 90\% & 0\% & 10\%  \\
%  & RNN vs S4SD & 0.61 & 83\% & 0\% & 17\%  \\
%  & RNN vs SCR & 0.70 & 86\% & 1\% & 14\%  \\
%  & S4SD vs SCR & 0.70 & 86\% & 0\% & 13\%  \\
% \midrule

% \multirow{10}{*}{GitHub} 
%  & Moji vs BERT & 0.81 & 89\% & 1\% & 10\%  \\
%  & Moji vs RNN & 0.56 & 72\% & 3\% & 25\%  \\
%  & Moji vs S4SD & 0.72 & 84\% & 1\% & 14\%  \\
%  & Moji vs SCR & 0.75 & 86\% & 1\% & 13\%  \\
%  & BERT vs RNN & 0.57 & 73\% & 3\% & 24\%  \\
%  & BERT vs S4SD & 0.73 & 85\% & 1\% & 14\%  \\
%  & BERT vs SCR & 0.75 & 87\% & 1\% & 13\%  \\
%  & RNN vs S4SD & 0.52 & 70\% & 3\% & 27\%  \\
%  & RNN vs SCR & 0.50 & 69\% & 2\% & 28\%  \\
%  & S4SD vs SCR & 0.68 & 83\% & 1\% & 16\%  \\
% \midrule


% \multirow{10}{*}{SO} 
%  & Moji vs BERT & 0.80 & 89\% & 1\% & 10\%  \\
%  & Moji vs RNN & 0.70 & 84\% & 1\% & 15\%  \\
%  & Moji vs S4SD & 0.61 & 79\% & 1\% & 19\%  \\
%  & Moji vs SCR & 0.35 & 70\% & 1\% & 29\%  \\
%  & BERT vs RNN & 0.72 & 84\% & 1\% & 14\%  \\
%  & BERT vs S4SD & 0.60 & 79\% & 2\% & 19\%  \\
%  & BERT vs SCR & 0.36 & 71\% & 1\% & 28\%  \\
%  & RNN vs S4SD & 0.56 & 77\% & 2\% & 22\%  \\
%  & RNN vs SCR & 0.30 & 67\% & 1\% & 32\%  \\
%  & S4SD vs SCR & 0.41 & 76\% & 1\% & 23\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_jira}%
% \end{table}%















% \begin{figure*}[!htb]
% \centering
% \pgfplotstableread{

% 1	.88  .97 .75 .78     .88  .97  .83 .88      .87  .96  .81 .85
% 2	.87  .96 .66 .68     .85  .93  .67 .85      .85  .93  .82 .76
% % 3	31.9  13.6  54.5  40.9  27.3  31.8  31.8  27.3  40.9  20.5  20.4  59.1  27.3  11.3  61.4  20.5  20.4  59.1  20.5  20.4  59.1  27.3  27.2  45.5 
% }\datatable

%       \subfloat[Test dataset GitHub]
%       {
%       \resizebox{1.5in}{!}{%
%       \begin{tikzpicture}
%         	\begin{axis}[
%         	%ylabel=label,
%         	xtick=data,
%         	xticklabels={Trained dataset SO, Trained dataset Jira},
%         	enlarge y limits=false,
%         	enlarge x limits=0.40,
%         % 	axis y line = none,
%         % 	axis y line=left,
%         %   axis line style={-},
%             axis y line=none,
%             % hide y axis,
%             axis x line*=bottom,
%             axis y line*=left,
%         % 	axis x line=left,
%         % 	axis x line=bottom,
%         % 	axis line style={draw=none},
%         %	nodes near coords,
%         	ymin=0,ymax=1,
%         	ybar,
%         	bar width=0.7cm,
%         	width=3.6in,
%         	height = 2.3in,
%         % 	ytick={0,20,...,80},
%             % yticklabels={0\%,20\%,40\%,60\%,80\%},
%         	%ylabel={Accepted Answer (\%)},
%         	ymajorgrids=false,
%         %	xminorgrids=true,
%          	yticklabel style={font=\large},
%         	xticklabel style={font=\large, /pgf/number format/fixed},	
%         	major x tick style = {opacity=0},
%         	minor x tick num = 1,    
%         	minor tick length=1ex,
%         	legend style={
%          	at={(0.6,0.98)},
%             anchor=north,legend columns=-1
%             },
%             % nodes near coords,
%             nodes near coords style={font=\LARGE},
%             nodes near coords style={rotate=90,  anchor=west}, %
%         	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
%         	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
%         	]
%         	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=1] \datatable;
%         	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=2] \datatable;
%         	\addplot[draw=black!80, fill=black!70] table[x index=0,y index=3] \datatable;
%         	\addplot[draw=black!80, fill=black!100] table[x index=0,y index=4] \datatable;
        
%             % \legend	{Jensen-Shannon Divergence,
%             % 		 Cosine Similarity,
%             % 		 SEntiMoji F1 score,
%             % 		 BERT4SentiSE F1 score
%             % 		 }
        	

%         	\end{axis}
%     	\end{tikzpicture}
%      	}
%     %  	\hspace{-1mm}
%     	\label{presentation-inconsistency}
%     } 
%     \subfloat[Test dataset SO]
%      {
%       \resizebox{1.5in}{!}{%
%       \begin{tikzpicture}
%         	\begin{axis}[
%         	%ylabel=label,
%         	xtick=data,
%         	xticklabels={Train dataset GitHub, Train dataset Jira
%         	},
%         	enlarge y limits=false,
%         	enlarge x limits=0.40,
%         % 	axis y line = none,
%         % 	axis y line=left,
%         %   axis line style={-},
%             axis y line=none,
%             % hide y axis,
%             axis x line*=bottom,
%             axis y line*=left,
%         % 	axis x line=left,
%         % 	axis x line=bottom,
%         % 	axis line style={draw=none},
%         %	nodes near coords,
%         	ymin=0,ymax=1,
%         	ybar,
%         	bar width=0.7cm,
%         	width=3.6in,
%         	height = 2.3in,
%         % 	ytick={0,20,...,80},
%             % yticklabels={0\%,20\%,40\%,60\%,80\%},
%         	%ylabel={Accepted Answer (\%)},
%         	ymajorgrids=false,
%         %	xminorgrids=true,
%          	yticklabel style={font=\large},
%          	xticklabel style={font=\large, /pgf/number format/fixed},	
%         	major x tick style = {opacity=0},
%         	minor x tick num = 1,    
%         	minor tick length=1ex,
%         	legend style={
%          	at={(0.5,1.35)},
%         % 	font=\small,
%         % 	legend pos = outer north east,
%         %  	legend pos=north west,
%         %   anchor=west,
%         % 	cells={align=left},
%         % 	legend cell align=left
%             anchor=north,legend columns=-1
%             },
%             nodes near coords style={font=\LARGE},
%             nodes near coords style={rotate=90,  anchor=west}, %
%         	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
%         	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
%         	]
%         	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=5] \datatable;
%         	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=6] \datatable; %, postaction={pattern=horizontal lines}
%         	\addplot[draw=black!80, fill=black!60] table[x index=0,y index=7] \datatable; %, postaction={pattern=vertical lines}
%             \addplot[draw=black!80, fill=black!100] table[x index=0,y index=8] \datatable; %, postaction={pattern=vertical lines}
%             \legend{JS Divergence,
%             		 Cosine Similarity,
%             		 Moji F1,
%             		 BERT F1
%             		 }
%         	\end{axis}
%     	\end{tikzpicture}
%     	}
%     % 	\hspace{-1mm}
%     	\label{signature-inconsistency}
%     }
%     \subfloat[Test dataset Jira]
%      {
%       \resizebox{1.5in}{!}{%
%       \begin{tikzpicture}
%         	\begin{axis}[
%         	%ylabel=label,
%         	xtick=data,
%         	xticklabels={Train dataset GitHub, Train dataset SO
%         	},
%         	enlarge y limits=false,
%         	enlarge x limits=0.40,
%         % 	axis y line = none,
%         % 	axis y line=left,
%         %   axis line style={-},
%             axis y line=none,
%             % hide y axis,
%             axis x line*=bottom,
%             axis y line*=left,
%         % 	axis x line=left,
%         % 	axis x line=bottom,
%         % 	axis line style={draw=none},
%         %	nodes near coords,
%         	ymin=0,ymax=1,
%         	ybar,
%         	bar width=0.7cm,
%         	width=3.4in,
%         	height = 2.3in,
%         % 	ytick={0,20,...,80},
%         %     yticklabels={0\%,20\%,40\%,60\%,80\%},
%         	%ylabel={Accepted Answer (\%)},
%         	ymajorgrids=false,
%         %	xminorgrids=true,
%          	yticklabel style={font=\large},
%          	xticklabel style={font=\large, /pgf/number format/fixed},	
%         	major x tick style = {opacity=0},
%         	minor x tick num = 1,    
%         	minor tick length=1ex,
%         	legend style={
%          	at={(0.6,0.98)},
%         % 	font=\small,
%         % 	legend pos = outer north east,
%         %  	legend pos=north west,
%         %   anchor=west,
%         % 	cells={align=left},
%         % 	legend cell align=left
%             anchor=north,legend columns=-1
%             },
%             nodes near coords style={font=\LARGE},
%             nodes near coords style={rotate=90,  anchor=west}, %
%         	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
%         	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
%         	]
%         	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=9] \datatable;
%         	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=10] \datatable; %, postaction={pattern=horizontal lines}
%         	\addplot[draw=black!80, fill=black!60] table[x index=0,y index=11] \datatable; %, postaction={pattern=vertical lines}
%             \addplot[draw=black!80, fill=black!100] table[x index=0,y index=12] \datatable; %, postaction={pattern=vertical lines}

%         	\end{axis}
%     	\end{tikzpicture}
%     	}
%     % 	%\hspace{-1mm}
%     	\label{status-inconsistency}
%     }
    


    
    
% %\vspace{-3mm}
% \caption{Impact of the similarity between datasets and performance of the DL-tools. The four bars represents the Jensen-Shannon Divergence,  Cosine Similarity, SEntiMoji F1 score,  BERT4SentiSE F1 score respectively.
% % \gias{the fonts above bars very small - make those bigger. The separation betwen two sets of bars per test dataset is too big - shrink. Put those for subfloats a, b, c side by side in one row. also put a legend above to indicate which bar denotes what.}
% }


% \vspace{-3mm}
% \label{fig:impacts-inconsistency-types}
% \end{figure*}























% % \begin{table*}[t]
% %   \centering
% %   %\vspace{-.1in}
% %   \caption{Some examples of severe misclassification by the five tools in cross-platform setting.}

% %     \begin{tabular}{cc}
% %     % \toprule{}
% %     \textbf{Misclassified Positive sentences as Negative} & \textbf{Misclassified Negative sentences as Positive}\\
    
% % \noindent \centering \fbox{%
% %     \parbox{.45\textwidth}{%

% %       \textbf{SEntiMoji} \\
% %       ``Oh, I've misread commit title, my bad :dancers:''\\
% %       ``You made it on top of hacker news. Congratz.''\\
% %       ``come on - friendly pets make presents to their owner sometimes!" \\
% %       ``+1 for this question - I have the same issue."\\
% %       ``Oh, you're right. Misread." \\
      
% %       \textbf{Bert4SentiSE} \\
% %         ``Dennis, you rock. Seriously." \\
% %         ``Sorry about that. The new things are just so shiny!" \\
% %         ``I hereby associate myself with this epic commit thread."" \\
% %         ``This is so badass I don't even know where to begin"" \\
% %         % ``It's Exploit Fix Day!" \\
% %         ``Its safe, at least from a unit testing perspective! I also don't see why it wouldn't be safe. An I missing something?" \\

      
      
% %       \textbf{RNN4SentiSE} \\
% %       ``Is this a fix for the 'Attempted to place a tile entity where there was no entity tile' bug?  Because if so, awesome!" \\
% %  ``Hello Andreas  Thank you for the information.  Shall try the same and upload the patch shortly.  Thanks \& Regards Ravikiran Mane." \\
% %  `` Hi Ramin  The patch looks good except I think it would be good to give import/export its own  SQLState starting with XIE instead of reusing the existing store FILE EXISTS message.  Also it would be good to have test cases for writing the lob files. Kathey" \\
% %  ``God I am awful at this :)" \\

      
      
      
% %       \textbf{Seniti4SD} \\
% % ``When explaining things to someone who seems to still be learning Haskell, I'd avoid using (or even showing) the pointless style. Don't want to scare them ;-)" \\
% % ``I still prefer RAII. Make the compiler do the work of making it leak proof. Safer *and* more convenient."" \\
% % ``Not to worry I've SOLVED it!" \\
% % ``No this was on 3.3.3 (sorry I should have mentioned that before).  That's great to know thanks!" \\
% % ``Holy crap that worked!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!" \\
      
      
      
% %       \textbf{SentiCR} \\
% %  ``@mcsnetworks WOW That looks amazing! Will most likely be moving to this some time in the future."" \\
% %  ``Sorry Jacques I have not seen that it was a grouped bugs.  In this case I have used to set in the grouped bugs the sum of the components used by detailed issues.  I didn't like unknow components.  Otherwise we can add a new fictitious component - GROUPED ISSUES - and assign this component to this type of issue.   Thanks  Marco" \\
% %  ``Yes, it's possible, juste remove the second parameter of your method (it's totally useless) ans it will work (I tested the code) !" \\
% %  ``Don't worry gyus, Vladimir always make the best things. )) Very respected to you........................" \\
% %  ``Thanks.. I really need to remember to run mvn clean package before push changes... I own you some beer" \\
% %     }%
% % }


% % &

% % \noindent \centering \fbox{%
% %     \parbox{.45\textwidth}{%
    
% %      \textbf{SEntiMoji} \\
% %  ``Great, again client freezes ...." \\
% %  ``Permanent Feign Death is permament! ;)" \\
% %  ``Makes sense, and it's very similiar to what I am doing. One ant task for stage and one for production, and just using the defaults for local development. But pain arises from mainting 3 different application contexts which have almost identical content.." \\
% %  ``Damn clean, Mr Kuhn, damn clean!" \\

    
    
% %       \textbf{Bert4SentiSE} \\
% %  ``Would've loved to. But there is no hash\_map in the C++ standard library, and PHB's don't allow code outside of that." \\
% %  ``Lotus Notes....aaaaargh!" \\
% %  ``What, no separators between the values? D:" \\ 
% %  ``+1 Fear the unhappy robots!" \\
% %  ``that's what I get for copying and pasting!" \\
% %  ``Wow, could have probably come across a little friendlier there, Phil!" \\


% %       \textbf{RNN4SentiSE} \\
% % % ``I think this is a great idea, but it's going to screw over a LOT of people who followed bad jQuery tutorials online that all seem to love recommending $() as a shortcut to $(document).''  \\
% % ``boo. Want to come up with something that looks nice in both the scss and docs? create a documentation styleguide?''  \\
% % ``the use of === for these doesn't make sense, consistent or not it's not worth a pull-request for pointless stuff like that''  \\
% % ``No tests bro :(''  \\
% % ``(in other words, my mind is melted down and I trust my basic arithmetic skills even less than before)''  \\


% %       \textbf{Senti4SD} \\
% % % ``Well, I guess I'll be taking my leave like @V10lator.  I need NBT and it's clear after more arguments that it will not be supported, probably along with an AI API and packet API.  Edit: @mbax That was the reason why I was planning to include independent ''  \\
% % ``Yes, the naming is all pretty terrible. I believe it's because we've gone through several iterations of what ""render"" actually means :)  One is used for fullscreen rendering, the other is used for video controls.  This is very much a hack, and hopeful''  \\
% % ``Pretty much hackfix, rather specify knockback immunity in spellauraeffects.cpp''  \\
% % ``Oh, right. That'd be the forum template that generated that. And no worries, I didn't take it personnally !''  \\
% % ``-5 votes?? People who have downvoted this answer should have specified the reason for doing so as well.''  \\




% %       \textbf{SentiCR} \\
% % ``Y U REQUIRE RUBYGEMS HERE !?!?!?!?!? :bomb:''  \\
% % ``Rebase FAIL!''  \\
% % ``Closing connections as side-effect of running assertColumnExists is dirty. For example anybody using transactions will have a nice surprise waiting...''  \\
% % ``This is extremely unsafe! Use mysqli or pdo instead of`mysql\_.''  \\
% % ``I'm -1 on this. It's imo easy enough to do Mailer.expects(:welcome) and then keep mocking from there. I don't like having two ways of doing the same thing purely to make it marginally easier to mock.''  \\
% % ``it worked, weird. thanks.''  \\
      
% %     }%
% % }

% %     \end{tabular}%
% %   \label{tab:misclassification2}%
% % \end{table*}%








% \begin{table}[]
%   \footnotesize
% %   \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Agreement metrics between  tools with manual labelling}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{clrrrr}
%     \toprule{}
%     %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
%     %\cmidrule{3-6}
%     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Classifier }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
%     \cmidrule{5-6}
%     {Dataset} &  & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule
% \multicolumn{6}{c}{\textbf{Test dataset: GitHub}} \\
% \midrule

% \multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Within-platform)}} 
%  & SEntiMoji & 0.84 & 90\% & 1\% & 9\%  \\
%  & BERT4SentiSE & 0.87 & 92\% & 1\% & 7\%  \\
%  & RNN4SentiSE & 0.52 & 68\% & 7\% & 25\%  \\
%  & Senti4SD & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiCR & 0.73 & 83\% & 2\% & 15\%  \\
% % \midrule
% \cmidrule{2-6}

% \multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow \\ (Cross-platform)}}  
%  & SEntiMoji & 0.61 & 75\% & 2\% & 23\%  \\
%  & BERT4SentiSE & 0.65 & 78\% & 3\% & 19\%  \\
%  & RNN4SentiSE & 0.47 & 66\% & 4\% & 30\%  \\
%  & Senti4SD & 0.60 & 74\% & 4\% & 22\%  \\
%  & SentiCR & 0.49 & 68\% & 2\% & 29\%  \\
% % \midrule
% \cmidrule{2-6}


% \multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Cross-platform)}} 
%  & SEntiMoji & 0.44 & 66\% & 1\% & 33\%  \\
%  & BERT4SentiSE & 0.48 & 68\% & 2\% & 30\%  \\
%  & RNN4SentiSE & 0.35 & 60\% & 4\% & 36\%  \\
%  & Senti4SD & 0.50 & 69\% & 2\% & 28\%  \\
%  & SentiCR & 0.34 & 60\% & 1\% & 39\%  \\
% \midrule



% \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% \midrule

% \multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow (Within-platform)}}
%  & SEntiMoji & 0.80 & 87\% & 1\% & 12\%  \\
%  & BERT4SentiSE& 0.82 & 88\% & 1\% & 11\%  \\
%  & RNN4SentiSE & 0.67 & 78\% & 3\% & 19\%  \\
%  & Senti4SD & 0.77 & 85\% & 1\% & 14\%  \\
%  & SentiCR & 0.73 & 82\% & 3\% & 15\%  \\
% % \midrule
% \cmidrule{2-6}

% \multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Cross-platform)}} 
%  & SEntiMoji & 0.73 & 83\% & 1\% & 16\%  \\
%  & BERT4SentiSE & 0.78 & 85\% & 1\% & 14\%  \\
%  & RNN4SentiSE & 0.49 & 67\% & 4\% & 29\%  \\
%  & Senti4SD & 0.67 & 78\% & 2\% & 20\%  \\
%  & SentiCR & 0.56 & 71\% & 5\% & 23\%  \\
% % \midrule
% \cmidrule{2-6}

% \multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Cross-platform)}} 
%  & SEntiMoji & 0.48 & 67\% & 0\% & 33\%  \\
%  & BERT4SentiSE & 0.63 & 76\% & 1\% & 23\%  \\
%  & RNN4SentiSE & 0.34 & 58\% & 4\% & 38\%  \\
%  & Senti4SD & 0.47 & 66\% & 1\% & 33\%  \\
%  & SentiCR & 0.37 & 60\% & 2\% & 38\%  \\
% \midrule







% \multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
% \midrule
% \multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Within-platform)}}
%  & SEntiMoji & 0.71 & 86\% & 0\% & 14\%  \\
%  & BERT4SentiSE& 0.72 & 86\% & 0\% & 13\%  \\
%  & RNN4SentiSE & 0.57 & 80\% & 1\% & 20\%  \\
%  & Senti4SD & 0.59 & 81\% & 0\% & 19\%  \\
%  & SentiCR & 0.69 & 85\% & 0\% & 15\%  \\
% % \midrule
% \cmidrule{2-6}


% \multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Cross-platform)}} 
%  & SEntiMoji & 0.65 & 81\% & 1\% & 18\%  \\
%  & BERT4SentiSE & 0.65 & 81\% & 1\% & 18\%  \\
%  & RNN4SentiSE & 0.45 & 66\% & 2\% & 32\%  \\
%  & Senti4SD & 0.58 & 78\% & 1\% & 21\%  \\
%  & SentiCR & 0.65 & 82\% & 1\% & 17\%  \\
% % \midrule
% \cmidrule{2-6}

% \multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow \\ (Cross-platform)}} 
%  & SEntiMoji & 0.65 & 82\% & 1\% & 18\%  \\
%  & BERT4SentiSE & 0.66 & 82\% & 1\% & 17\%  \\
%  & RNN4SentiSE & 0.57 & 77\% & 1\% & 22\%  \\
%  & Senti4SD & 0.46 & 74\% & 1\% & 25\%  \\
%  & SentiCR & 0.34 & 73\% & 1\% & 26\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_with_manual_labelling}%
% \end{table}%


% \begin{table}
% \renewcommand{\thetable}{\arabic{table}aa}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Agreement between  tools (Test dataset: GitHub)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule
% \multirow{10}{*}{G (W)} 
%  & SM $\leftrightarrow$ BS & 0.86 & 91\% & 1\% & 8\%  \\
%  & SM $\leftrightarrow$ RS & 0.52 & 68\% & 7\% & 25\%  \\
%  & SM $\leftrightarrow$ SD & 0.83 & 89\% & 1\% & 10\%  \\
%  & SM $\leftrightarrow$ SC & 0.76 & 85\% & 2\% & 13\%  \\
%  & BS $\leftrightarrow$ RS & 0.53 & 69\% & 7\% & 24\%  \\
%  & BS vs SD & 0.85 & 90\% & 2\% & 8\%  \\
%  & BS vs SC & 0.74 & 83\% & 2\% & 14\%  \\
%  & RS vs SD & 0.52 & 69\% & 7\% & 25\%  \\
%  & RS vs SC & 0.43 & 63\% & 7\% & 31\%  \\
%  & SD vs SC & 0.74 & 83\% & 2\% & 14\%  \\
% \midrule


% \multirow{10}{*}{S(C)} 
%  & SM vs BS & 0.72 & 83\% & 1\% & 15\%  \\
%  & SM vs RS & 0.58 & 76\% & 2\% & 22\%  \\
%  & SM vs SD & 0.51 & 70\% & 3\% & 27\%  \\
%  & SM vs SC & 0.40 & 68\% & 2\% & 30\%  \\
%  & BS vs RS & 0.59 & 76\% & 2\% & 22\%  \\
%  & BS vs SD & 0.52 & 70\% & 4\% & 26\%  \\
%  & BS vs SC & 0.39 & 66\% & 3\% & 31\%  \\
%  & RS vs SD & 0.43 & 65\% & 4\% & 31\%  \\
%  & RS vs SC & 0.30 & 62\% & 3\% & 35\%  \\
%  & SD vs SC & 0.45 & 68\% & 2\% & 30\%  \\
% \midrule


% \multirow{10}{*}{J(C)} 
%  & SM vs BS & 0.78 & 90\% & 0\% & 10\%  \\
%  & SM vs RS & 0.54 & 81\% & 1\% & 19\%  \\
%  & SM vs SD & 0.60 & 82\% & 1\% & 18\%  \\
%  & SM vs SC & 0.65 & 87\% & 0\% & 13\%  \\
%  & BS vs RS & 0.56 & 81\% & 1\% & 18\%  \\
%  & BS vs SD & 0.60 & 81\% & 1\% & 18\%  \\
%  & BS vs SC & 0.67 & 87\% & 0\% & 13\%  \\
%  & RS vs SD & 0.44 & 74\% & 2\% & 24\%  \\
%  & RS vs SC & 0.45 & 79\% & 1\% & 20\%  \\
%  & SD vs SC & 0.52 & 79\% & 1\% & 20\%  \\

%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_github}%
% \end{table}%



% \begin{table}
% \renewcommand{\thetable}{\arabic{table}a}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Agreement between  tools (Test dataset: GitHub)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule
% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Within Platform)}} 
%  & SentiMoji vs BERT4SE & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiMoji vs RNN4SE & 0.52 & 68\% & 7\% & 25\%  \\
%  & SentiMoji vs Senti4SD & 0.83 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs SentiCR & 0.76 & 85\% & 2\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.53 & 69\% & 7\% & 24\%  \\
%  & BERT4SE vs Senti4SD & 0.85 & 90\% & 2\% & 8\%  \\
%  & BERT4SE vs SentiCR & 0.74 & 83\% & 2\% & 14\%  \\
%  & RNN4SE vs Senti4SD & 0.52 & 69\% & 7\% & 25\%  \\
%  & RNN4SE vs SentiCR & 0.43 & 63\% & 7\% & 31\%  \\
%  & Senti4SD vs SentiCR & 0.74 & 83\% & 2\% & 14\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.72 & 83\% & 1\% & 15\%  \\
%  & SentiMoji vs RNN4SE & 0.58 & 76\% & 2\% & 22\%  \\
%  & SentiMoji vs Senti4SD & 0.51 & 70\% & 3\% & 27\%  \\
%  & SentiMoji vs SentiCR & 0.40 & 68\% & 2\% & 30\%  \\
%  & BERT4SE vs RNN4SE & 0.59 & 76\% & 2\% & 22\%  \\
%  & BERT4SE vs Senti4SD & 0.52 & 70\% & 4\% & 26\%  \\
%  & BERT4SE vs SentiCR & 0.39 & 66\% & 3\% & 31\%  \\
%  & RNN4SE vs Senti4SD & 0.43 & 65\% & 4\% & 31\%  \\
%  & RNN4SE vs SentiCR & 0.30 & 62\% & 3\% & 35\%  \\
%  & Senti4SD vs SentiCR & 0.45 & 68\% & 2\% & 30\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.78 & 90\% & 0\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.54 & 81\% & 1\% & 19\%  \\
%  & SentiMoji vs Senti4SD & 0.60 & 82\% & 1\% & 18\%  \\
%  & SentiMoji vs SentiCR & 0.65 & 87\% & 0\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.56 & 81\% & 1\% & 18\%  \\
%  & BERT4SE vs Senti4SD & 0.60 & 81\% & 1\% & 18\%  \\
%  & BERT4SE vs SentiCR & 0.67 & 87\% & 0\% & 13\%  \\
%  & RNN4SE vs Senti4SD & 0.44 & 74\% & 2\% & 24\%  \\
%  & RNN4SE vs SentiCR & 0.45 & 79\% & 1\% & 20\%  \\
%  & Senti4SD vs SentiCR & 0.52 & 79\% & 1\% & 20\%  \\

%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_github}%
% \end{table}%


% \begin{table}
% \addtocounter{table}{-1}
% \renewcommand{\thetable}{\arabic{table}b}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Agreement between  tools (Test dataset: SO)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Within Platform)}} 
%  & SentiMoji vs BERT4SE & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiMoji vs RNN4SE & 0.70 & 80\% & 3\% & 17\%  \\
%  & SentiMoji vs Senti4SD & 0.81 & 88\% & 1\% & 12\%  \\
%  & SentiMoji vs SentiCR & 0.78 & 85\% & 2\% & 12\%  \\
%  & BERT4SE vs RNN4SE & 0.71 & 81\% & 2\% & 17\%  \\
%  & BERT4SE vs Senti4SD & 0.83 & 88\% & 1\% & 11\%  \\
%  & BERT4SE vs SentiCR & 0.78 & 85\% & 3\% & 12\%  \\
%  & RNN4SE vs Senti4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & RNN4SE vs SentiCR & 0.65 & 77\% & 4\% & 19\%  \\
%  & Senti4SD vs SentiCR & 0.78 & 85\% & 3\% & 12\%  \\
% \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.79 & 86\% & 1\% & 13\%  \\
%  & SentiMoji vs RNN4SE & 0.53 & 70\% & 4\% & 27\%  \\
%  & SentiMoji vs Senti4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & SentiMoji vs SentiCR & 0.62 & 75\% & 5\% & 20\%  \\
%  & BERT4SE vs RNN4SE & 0.53 & 69\% & 5\% & 26\%  \\
%  & BERT4SE vs Senti4SD & 0.73 & 82\% & 2\% & 16\%  \\
%  & BERT4SE vs SentiCR & 0.60 & 74\% & 5\% & 21\%  \\
%  & RNN4SE vs Senti4SD & 0.54 & 69\% & 4\% & 26\%  \\
%  & RNN4SE vs SentiCR & 0.40 & 61\% & 6\% & 33\%  \\
%  & Senti4SD vs SentiCR & 0.58 & 73\% & 4\% & 23\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.66 & 82\% & 0\% & 18\%  \\
%  & SentiMoji vs RNN4SE & 0.47 & 75\% & 1\% & 23\%  \\
%  & SentiMoji vs Senti4SD & 0.60 & 81\% & 1\% & 19\%  \\
%  & SentiMoji vs SentiCR & 0.56 & 80\% & 1\% & 19\%  \\
%  & BERT4SE vs RNN4SE & 0.43 & 70\% & 2\% & 28\%  \\
%  & BERT4SE vs Senti4SD & 0.57 & 77\% & 1\% & 22\%  \\
%  & BERT4SE vs SentiCR & 0.52 & 75\% & 1\% & 25\%  \\
%  & RNN4SE vs Senti4SD & 0.42 & 72\% & 2\% & 27\%  \\
%  & RNN4SE vs SentiCR & 0.33 & 70\% & 1\% & 29\%  \\
%  & Senti4SD vs SentiCR & 0.51 & 77\% & 1\% & 22\%  \\
% % \midrule

%     \bottomrule
%     \end{tabular}%
%   \label{tab:agreement_test_so}%
% \end{table}%



% \begin{table}[]
%   \addtocounter{table}{-1}
%   \renewcommand{\thetable}{\arabic{table}c}

% %   \footnotesize
%   \small
%   \centering
%   \caption{Agreement between  tools (Test dataset: Jira)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Within Platform}} 
%  & SentiMoji vs BERT4SE & 0.85 & 93\% & 0\% & 7\%  \\
%  & SentiMoji vs RNN4SE & 0.68 & 86\% & 0\% & 14\%  \\
%  & SentiMoji vs Senti4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & SentiMoji vs SentiCR & 0.81 & 91\% & 0\% & 9\%  \\
%  & BERT4SE vs RNN4SE & 0.68 & 85\% & 1\% & 14\%  \\
%  & BERT4SE vs Senti4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & BERT4SE vs SentiCR & 0.79 & 90\% & 0\% & 10\%  \\
%  & RNN4SE vs Senti4SD & 0.61 & 83\% & 0\% & 17\%  \\
%  & RNN4SE vs SentiCR & 0.70 & 86\% & 1\% & 14\%  \\
%  & Senti4SD vs SentiCR & 0.70 & 86\% & 0\% & 13\%  \\
% \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.81 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.56 & 72\% & 3\% & 25\%  \\
%  & SentiMoji vs Senti4SD & 0.72 & 84\% & 1\% & 14\%  \\
%  & SentiMoji vs SentiCR & 0.75 & 86\% & 1\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.57 & 73\% & 3\% & 24\%  \\
%  & BERT4SE vs Senti4SD & 0.73 & 85\% & 1\% & 14\%  \\
%  & BERT4SE vs SentiCR & 0.75 & 87\% & 1\% & 13\%  \\
%  & RNN4SE vs Senti4SD & 0.52 & 70\% & 3\% & 27\%  \\
%  & RNN4SE vs SentiCR & 0.50 & 69\% & 2\% & 28\%  \\
%  & Senti4SD vs SentiCR & 0.68 & 83\% & 1\% & 16\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.80 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.70 & 84\% & 1\% & 15\%  \\
%  & SentiMoji vs Senti4SD & 0.61 & 79\% & 1\% & 19\%  \\
%  & SentiMoji vs SentiCR & 0.35 & 70\% & 1\% & 29\%  \\
%  & BERT4SE vs RNN4SE & 0.72 & 84\% & 1\% & 14\%  \\
%  & BERT4SE vs Senti4SD & 0.60 & 79\% & 2\% & 19\%  \\
%  & BERT4SE vs SentiCR & 0.36 & 71\% & 1\% & 28\%  \\
%  & RNN4SE vs Senti4SD & 0.56 & 77\% & 2\% & 22\%  \\
%  & RNN4SE vs SentiCR & 0.30 & 67\% & 1\% & 32\%  \\
%  & Senti4SD vs SentiCR & 0.41 & 76\% & 1\% & 23\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_jira}%
% \end{table}%


==> SubmissionTOSEM/threats.tex <==
\section{Threats to Validity}\label{sec:threats_to_validity}
 In this Section we discuss the threats to validity of our study following the guideline for empirical studies \cite{wohlin2012experimentation}.

\nd\bf{Construct Validity} threats relate to potential errors in the research methodology. In this study, we used the same three benchmark datasets used by Novielli et al. ~\cite{Novielli-SEToolCrossPlatform-MSR2020} and by others for similar studies\cite{Chen-SentiEmoji-FSE2019, Lin-PatternBasedOpinionMining-ICSE2019}. During our error analysis of the deep learning SD tools, we followed the similar guideline of related studies~\cite{Novielli-SEToolCrossPlatform-MSR2020, opiner_2019}. We also observed the same error categories that were previously reported by Novielli et al.~\cite{Novielli-SEToolCrossPlatform-MSR2020}. Another issue can be reporting the performance that may not be standard. In order to mitigate this threat, following standard reporting practices in this domain, we report both Macro and micro scores and Cohen Kappa agreement values.  



\nd\bf{Internal Validity} threats concern about the authors' bias while conducting the study. It refers to errors that can occur due to not using optimal configuration parameters for sentiment detection tools. For each tool in our study, we used the code provided by the authors to run and fine-tune their performance (e.g., hyper-parameter tuning). In within platform settings, we adopted 10-fold cross-validation settings and trained and tested each tool ten times to mitigate variance of the model's prediction. In order to mitigate the coding errors, we used widely used open-source libraries (e.g., SciKit-learn ~\cite{website:python-scikit-learn}) to compute the metrics presented in this study. Another area of bias can be the human bias while categorizing the misclassification of the SD tools. Two authors discussed and participated in the error categorization process to reduce human biases. We also share our manual categorization with our replication package.



\nd\bf{External Validity} threats refer to the generalizability of the findings. For this study, we used three datasets that represent all the available datasets for sentiment detection for the software engineering domain and used in similar studies.  We used datasets of around 17K units from three popular and widely used collaboration platforms: question-answering (Stack Overflow), collaborative development platform (GitHub), issue tracking platform (Jira). Transposing the results to another new SE platform may introduce new insights regarding the cross-platform adoption of the tools. In summary, our study shows promising results for PTM DL-based tools for sentiment detection tasks because compared to other tools, they show promising results to understand and generalize SE-domain context. 

\nd\bf{Reliability} threats concern about to what extent procedures are followed and the possibility of replicating the evaluation of the study. In order to mitigate this, we provide necessary details in our replication package~\cite{website:deep_learning_cross_platform}.


% \gias{We need more contents in this section. See Section 7 of this paper \url{https://giasuddin.files.wordpress.com/2020/11/opinerusagedoctosem2020-2.pdf}}

% We train and test each tool 10 times for each dataset and thus it reduces the variance of the model's training.

==> tables.tex <==

% \begin{sidewaystable}
% \begin{table*}%[t]
% \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Performance of SE-specific sentiment analysis in within-platform and cross-platform settings (SentiSE = SentistrengthSE, DS = Dataset, WPS = Within Platform Settting, CPS = Cross-Platform Setting \gias{divide into table into 3 tables as you are doing in RQ4. Make the tables sideways. see my other sentiment paper I shared with to understand how to make sideways table. ask me if you are confused.})}
%   %\vspace{-3mm}
%   % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{ll|rrr|rrr|rrr|rrr|rrr|rrr}
%     \toprule{}

%     \multirow{2}{*}{\textbf{Setting}}  & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentiSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}} & \multicolumn{3}{c}{\textbf{SentiSE}}\\
%     \cmidrule{3-20}
%     {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
    
%     %\multicolumn{18}{c}{\textbf{Test dataset: GitHub}} \\
%     %\midrule
 
%      \multirow{5}{1.4cm}{\bf{WPS: Test DS GitHub} (Train DS GitHub)}
%      & Negative &  .89 & .85 & .87  & .89 & .91 & .90  & .68 & .69 & .68  & .90 & .89 & .90  & .87 & .69 & .77  & .81 & .71 & .76   \\ 
%      & Neutral &  .87 & .92 & .89  & .92 & .90 & .91  & .73 & .66 & .69  & .89 & .92 & .91  & .77 & .91 & .84  & .74 & .86 & .79   \\ 
%      & Positive &  .94 & .92 & .93  & .93 & .94 & .94  & .64 & .72 & .68  & .94 & .91 & .93  & .89 & .84 & .86  & .85 & .76 & .80   \\ 
%      & Micro-avg &  .90 & .90 & .90  & \textbf{.92} & \textbf{.92} & \textbf{.92}  & .68 & .68 & .68  & .91 & .91 & .91  & .83 & .83 & .83  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .90 & .89 & .90  & \textbf{.91} & \textbf{.92} & \textbf{.92}  & .68 & .69 & .68  & \textbf{.91} & .91 & .91  & .84 & .81 & .82  & .80 & .78 & .78   \\ 

%     \cmidrule{2-20}     

%      % Test dataset: Github
% \multirow{5}{1.4cm}{\bf{CPS: Test DS GitHub} (Train DS SO)}
%  & Negative &  .85 & .62 & .72  & .83 & .73 & .78  & .69 & .49 & .58  & .79 & .56 & .66  & .83 & .37 & .51  & .81 & .71 & .76   \\ 
%  & Neutral &  .67 & .91 & .77  & .71 & .91 & .80  & .61 & .84 & .71  & .71 & .82 & .76  & .60 & .94 & .73  & .74 & .86 & .79   \\ 
%  & Positive &  .88 & .65 & .75  & .88 & .63 & .73  & .78 & .57 & .66  & .76 & .81 & .78  & .86 & .62 & .72  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .75 & .75 & .75  & .78 & .78 & .78  & .66 & .66 & .66  & .74 & .74 & .74  & .68 & .68 & .68  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  .80 & .73 & .75  & \textbf{.81} & .76 & .77  & .69 & .63 & .65  & .75 & .73 & .73  & .76 & .64 & .66  & .80 & \textbf{.78} & \textbf{.78}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.15 & -.15 & -.15 & -.14 & -.14 & -.14 & -.02 & -.02 & -.02 & -.17 & -.17 & -.17 & -.14 & -.14 & -.14  \\ 
% % & & Macro-avg &  -.10 & -.17 & -.15 & -.11 & -.16 & -.15 & .01 & -.05 & -.04 & -.16 & -.18 & -.18 & -.08 & -.17 & -.17  \\ 
% \cmidrule{2-20}
    
    
    
%     % Test dataset: Github
%     \multirow{5}{1.4cm}{\textbf{CPS: Test DS GitHub} (Train DS Jira)} 
%      & Negative &  .91 & .39 & .55  & .90 & .43 & .58  & .75 & .39 & .52  & .85 & .52 & .64  & .88 & .27 & .41  & .81 & .71 & .76   \\ 
%  & Neutral &  .56 & .98 & .72  & .59 & .97 & .73  & .54 & .95 & .69  & .60 & .96 & .74  & .52 & .98 & .68  & .74 & .86 & .79   \\ 
%  & Positive &  .94 & .45 & .60  & .91 & .51 & .65  & .80 & .30 & .44  & .90 & .46 & .61  & .89 & .38 & .53  & .85 & .76 & .80   \\ 
%  & Micro-avg &  .66 & .66 & .66  & .68 & .68 & .68  & .60 & .60 & .60  & .69 & .69 & .69  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  \textbf{.80} & .61 & .62  & \textbf{.80} & .64 & .65  & .70 & .55 & .55  & .78 & .65 & .67  & .76 & .54 & .54  & \textbf{.80} & \textbf{.78} & \textbf{.78}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.24 & -.24 & -.24 & -.23 & -.23 & -.23 & -.08 & -.08 & -.08 & -.22 & -.22 & -.22 & -.23 & -.23 & -.23  \\ 
% % & & Macro-avg &  -.10 & -.29 & -.28 & -.12 & -.28 & -.26 & .02 & -.14 & -.14 & -.13 & -.26 & -.24 & -.08 & -.27 & -.28  \\ 

% \midrule





% %    \multicolumn{18}{c}{\textbf{Test dataset: Stack Overflow}} \\
% %    \midrule
%     \multirow{5}{1.4cm}{\textbf{WPS: Test DS SO} (Train DS SO)} 
%  & Negative &  .84 & .83 & .83  & .86 & .85 & .85  & .74 & .73 & .74  & .80 & .83 & .82  & .80 & .72 & .76  & .76 & .76 & .76   \\ 
%  & Neutral &  .83 & .84 & .84  & .86 & .85 & .85  & .75 & .77 & .76  & .84 & .79 & .81  & .79 & .82 & .81  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .93 & .93  & .93 & .94 & .93  & .85 & .85 & .85  & .90 & .93 & .91  & .88 & .91 & .89  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}  & .78 & .78 & .78  & .85 & .85 & .85  & .82 & .82 & .82  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .87 & .87 & .87  & \textbf{.88} & \textbf{.88} & \textbf{.88}  & .78 & .78 & .78  & .85 & .85 & .85  & .82 & .82 & .82  & .80 & .79 & .79   \\ 
 

%     \cmidrule{2-20}
    
%     % Test dataset: Stack Overflow
%     \multirow{5}{1.4cm}{\textbf{CPS: Test DS SO} (Train DS GitHub)} 
%  & Negative &  .82 & .76 & .79  & .80 & .86 & .83  & .66 & .60 & .63  & .69 & .76 & .72  & .64 & .49 & .55  & .76 & .76 & .76   \\ 
%  & Neutral &  .75 & .85 & .80  & .84 & .80 & .82  & .61 & .64 & .63  & .73 & .76 & .75  & .65 & .85 & .74  & .73 & .79 & .75   \\ 
%  & Positive &  .93 & .85 & .89  & .93 & .91 & .92  & .73 & .74 & .74  & .92 & .82 & .87  & .88 & .74 & .80  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .83 & .83 & .83  & \textbf{.85} & \textbf{.85} & \textbf{.85}  & .67 & .67 & .67  & .78 & .78 & .78  & .71 & .71 & .71  & .79 & .79 & .79   \\ 
%  & Macro-avg &  .83 & .82 & .82  & \textbf{.85} & \textbf{.86} & \textbf{.85}  & .67 & .66 & .66  & .78 & .78 & .78  & .72 & .69 & .70  & .80 & .79 & .79   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.12 & -.12 & -.12 & -.07 & -.07 & -.07 & -.11 & -.11 & -.11  \\ 
% % & & Macro-avg &  -.03 & -.05 & -.04 & -.03 & -.02 & -.03 & -.11 & -.12 & -.12 & -.06 & -.07 & -.07 & -.10 & -.12 & -.12  \\ 

%     \cmidrule{2-20}


%     % Test dataset: Stack Overflow
%     \multirow{5}{1.4cm}{\textbf{CPS: Test DS SO} (Train DS Jira)}
%  & Negative &  .93 & .31 & .47  & .88 & .55 & .68  & .66 & .31 & .42  & .75 & .30 & .43  & .67 & .22 & .33  & .76 & .76 & .76   \\ 
%  & Neutral &  .54 & .98 & .70  & .63 & .94 & .76  & .50 & .91 & .65  & .54 & .93 & .69  & .50 & .95 & .66  & .73 & .79 & .75   \\ 
%  & Positive &  .98 & .62 & .76  & .97 & .74 & .84  & .83 & .42 & .56  & .96 & .64 & .76  & .96 & .52 & .67  & .91 & .82 & .86   \\ 
%  & Micro-avg &  .67 & .67 & .67  & .76 & .76 & .76  & .58 & .58 & .58  & .66 & .66 & .66  & .60 & .60 & .60  & \textbf{.79} & \textbf{.79} & \textbf{.79}   \\ 
%  & Macro-avg &  .82 & .64 & .64  & \textbf{.83} & .74 & .76  & .66 & .55 & .54  & .75 & .62 & .63  & .71 & .56 & .55  & .80 & \textbf{.79} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.20 & -.20 & -.20 & -.12 & -.12 & -.12 & -.21 & -.21 & -.21 & -.19 & -.19 & -.19 & -.22 & -.22 & -.22  \\ 
% % & & Macro-avg &  -.05 & -.23 & -.23 & -.05 & -.14 & -.12 & -.12 & -.23 & -.24 & -.10 & -.23 & -.22 & -.11 & -.25 & -.27  \\ 

%     \midrule





%     % Test dataset: Jira
% %    \multicolumn{18}{c}{\textbf{Test dataset: Jira}} \\
% %    \midrule
%     \multirow{5}{1.4cm}{\textbf{WPS: Test DS Jira} (Train DS Jira)} 
%  & Negative &  .84 & .68 & .75  & .82 & .76 & .79  & .69 & .46 & .55  & .71 & .55 & .62  & .79 & .66 & .72  & .68 & .73 & .71   \\ 
%  & Neutral &  .89 & .91 & .90  & .90 & .90 & .90  & .83 & .89 & .86  & .84 & .88 & .86  & .89 & .89 & .89  & .92 & .82 & .87   \\ 
%  & Positive &  .79 & .80 & .79  & .78 & .80 & .79  & .73 & .72 & .72  & .73 & .71 & .72  & .75 & .85 & .80  & .68 & .92 & .78   \\ 
%  & Micro-avg &  \textbf{.86} & \textbf{.86} & \textbf{.86}  & \textbf{.86} & \textbf{.86} & \textbf{.86}  & .80 & .80 & .80  & .81 & .81 & .81  & .85 & .85 & .85  & .83 & .83 & .83   \\ 
%  & Macro-avg &  \textbf{.84} & .80 & .81  & .83 & \textbf{.82} & \textbf{.83}  & .75 & .69 & .71  & .76 & .72 & .73  & .81 & .80 & .80  & .76 & \textbf{.82} & .79   \\ 

%     \cmidrule{2-20}
    
    
%     % Test dataset: Jira
%     \multirow{5}{1.4cm}{\textbf{CPS: Test DS Jira} (Train DS GitHub)} 
%  & Negative &  .63 & .75 & .69  & .66 & .74 & .70  & .51 & .71 & .60  & .61 & .64 & .62  & .69 & .60 & .64  & .68 & .73 & .71   \\ 
%  & Neutral &  .93 & .79 & .85  & .93 & .80 & .86  & .92 & .58 & .71  & .89 & .78 & .83  & .90 & .85 & .87  & .92 & .82 & .87   \\ 
%  & Positive &  .66 & .91 & .77  & .65 & .91 & .76  & .45 & .92 & .61  & .62 & .86 & .72  & .69 & .89 & .78  & .68 & .92 & .78   \\ 
%  & Micro-avg &  .81 & .81 & .81  & .81 & .81 & .81  & .66 & .66 & .66  & .78 & .78 & .78  & .82 & .82 & .82  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg &  .74 & \textbf{.82} & .77  & .75 & \textbf{.82} & .77  & .63 & .74 & .64  & .71 & .76 & .73  & \textbf{.76} & .78 & .76  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.05 & -.05 & -.05 & -.05 & -.05 & -.05 & -.14 & -.14 & -.14 & -.03 & -.03 & -.03 & -.03 & -.03 & -.03  \\ 
% % & & Macro-avg &  -.09 & .02 & -.04 & -.09 & -.00 & -.05 & -.12 & .05 & -.07 & -.05 & .05 & -.01 & -.05 & -.02 & -.04  \\ 

%     \cmidrule{2-20}
    
    
%     % Test dataset: Jira
%     \multirow{5}{1.4cm}{\textbf{CPS: Test DS Jira} (Train DS SO)}
%  & Negative &  .67 & .68 & .67  & .72 & .68 & .70  & .58 & .61 & .59  & .50 & .29 & .37  & .36 & .06 & .10  & .68 & .73 & .71   \\ 
%  & Neutral &  .92 & .81 & .86  & .92 & .82 & .87  & .88 & .77 & .82  & .82 & .81 & .81  & .75 & .94 & .83  & .92 & .82 & .87   \\ 
%  & Positive &  .67 & .93 & .78  & .65 & .93 & .76  & .62 & .89 & .73  & .59 & .80 & .68  & .71 & .49 & .58  & .68 & .92 & .78   \\ 
%  & Micro-avg &  .82 & .82 & .82  & .82 & .82 & .82  & .77 & .77 & .77  & .74 & .74 & .74  & .73 & .73 & .73  & \textbf{.83} & \textbf{.83} & \textbf{.83}   \\ 
%  & Macro-avg &  .75 & .81 & .77  & \textbf{.76} & .81 & .78  & .69 & .75 & .71  & .64 & .63 & .62  & .61 & .49 & .50  & \textbf{.76} & \textbf{.82} & \textbf{.79}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.07 & -.07 & -.07 & -.12 & -.12 & -.12  \\ 
% % & & Macro-avg &  -.08 & .01 & -.04 & -.07 & -.01 & -.05 & -.05 & .06 & .00 & -.12 & -.08 & -.11 & -.20 & -.30 & -.30  \\ 


%     \bottomrule
%     \end{tabular}%
% %}
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance}%
% \end{table*}%




















% \begin{table*}%[t]
% %\footnotesize
%   \centering
%   %\vspace{-.1in}
%   \caption{Performance of SE-specific sentiment analysis in cross-platform settings}
%   \vspace{-3mm}
%   % \resizebox{\textwidth}{!}{%
%     \begin{tabular}{lll|ccc|ccc|ccc|ccc|ccc}
%     \toprule{}

%     \multirow{2}{*}{\textbf{Setting}} & \multirow{2}{5px}{\textbf{Train Data}} & \multirow{2}{*}{\textbf{Polarity}} & 
%     \multicolumn{3}{c}{\textbf{SEntiMoji}} & \multicolumn{3}{c}{\textbf{BERT4SEntiSE}} & \multicolumn{3}{c}{\textbf{RNN4SentSE}} & \multicolumn{3}{c}{\textbf{Senti4SD}} & \multicolumn{3}{c}{\textbf{SentiCR}}\\
%     \cmidrule{4-18}
%     {} & {} & {} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
    
%     \multicolumn{18}{c}{\textbf{Test dataset: Github}} \\
%     \midrule
 
%     \multirow{5}{5px}{Within platform} & \multirow{5}{*}{GitHub}
%     & Negative &  .89 & .85 & .87  & .89 & .91 & .90  & .68 & .69 & .68  & .90 & .89 & .90  & .87 & .69 & .77   \\ 
%     & & Neutral &  .87 & .92 & .89  & .92 & .90 & .91  & .73 & .66 & .69  & .89 & .92 & .91  & .77 & .91 & .84   \\ 
%     & & Positive &  .94 & .92 & .93  & .93 & .94 & .94  & .64 & .72 & .68  & .94 & .91 & .93  & .89 & .84 & .86   \\ 
%     & & Micro-avg &  .90 & .90 & \textbf{.90}  & .92 & .92 & \textbf{.92}  & .68 & .68 & \textbf{.68}  & .91 & .91 & \textbf{.91}  & .83 & .83 & \textbf{.83}   \\ 
%     & & Macro-avg &  .90 & .89 & \textbf{.90}  & .91 & .92 & \textbf{.92}  & .68 & .69 & \textbf{.68}  & .91 & .91 & \textbf{.91}  & .84 & .81 & \textbf{.82}   \\ 
%     \midrule     
    
    
    
    
%      % Test dataset: Github
% \multirow{5}{5px}{Cross-platform} & \multirow{5}{5px}{Stack Overflow}
%  & Negative &  .85 & .62 & .72  & .83 & .73 & .78  & .69 & .49 & .58  & .79 & .56 & .66  & .83 & .37 & .51   \\ 
% & & Neutral &  .67 & .91 & .77  & .71 & .91 & .80  & .61 & .84 & .71  & .71 & .82 & .76  & .60 & .94 & .73   \\ 
% & & Positive &  .88 & .65 & .75  & .88 & .63 & .73  & .78 & .57 & .66  & .76 & .81 & .78  & .86 & .62 & .72   \\ 
% & & Micro-avg &  .75 & .75 & \textbf{.75}  & .78 & .78 & \textbf{.78}  & .66 & .66 & \textbf{.66}  & .74 & .74 & \textbf{.74}  & .68 & .68 & \textbf{.68}   \\ 
% & & Macro-avg &  .80 & .73 & \textbf{.75}  & .81 & .76 & \textbf{.77}  & .69 & .63 & \textbf{.65}  & .75 & .73 & \textbf{.73}  & .76 & .64 & \textbf{.66}   \\

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.15 & -.15 & -.15 & -.14 & -.14 & -.14 & -.02 & -.02 & -.02 & -.17 & -.17 & -.17 & -.14 & -.14 & -.14  \\ 
% % & & Macro-avg &  -.10 & -.17 & -.15 & -.11 & -.16 & -.15 & .01 & -.05 & -.04 & -.16 & -.18 & -.18 & -.08 & -.17 & -.17  \\ 
% \midrule
    
    
    
%     % Test dataset: Github
%     \multirow{5}{5px}{Cross-platform} & \multirow{5}{*}{Jira}
%      & Negative &  .91 & .39 & .55  & .90 & .43 & .58  & .75 & .39 & .52  & .85 & .52 & .64  & .88 & .27 & .41   \\ 
% & & Neutral &  .56 & .98 & .72  & .59 & .97 & .73  & .54 & .95 & .69  & .60 & .96 & .74  & .52 & .98 & .68   \\ 
% & & Positive &  .94 & .45 & .60  & .91 & .51 & .65  & .80 & .30 & .44  & .90 & .46 & .61  & .89 & .38 & .53   \\ 
% & & Micro-avg &  .66 & .66 & \textbf{.66}  & .68 & .68 & \textbf{.68}  & .60 & .60 & \textbf{.60}  & .69 & .69 & \textbf{.69}  & .60 & .60 & \textbf{.60}   \\ 
% & & Macro-avg &  .80 & .61 & \textbf{.62}  & .80 & .64 & \textbf{.65}  & .70 & .55 & \textbf{.55}  & .78 & .65 & \textbf{.67}  & .76 & .54 & \textbf{.54}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.24 & -.24 & -.24 & -.23 & -.23 & -.23 & -.08 & -.08 & -.08 & -.22 & -.22 & -.22 & -.23 & -.23 & -.23  \\ 
% % & & Macro-avg &  -.10 & -.29 & -.28 & -.12 & -.28 & -.26 & .02 & -.14 & -.14 & -.13 & -.26 & -.24 & -.08 & -.27 & -.28  \\ 

% \midrule





%     \multicolumn{18}{c}{\textbf{Test dataset: Stack Overflow}} \\
%     \midrule
%     \multirow{5}{5px}{Within-platform} & \multirow{5}{5px}{Stack Overflow} 
%      & Negative &  .84 & .83 & .83  & .86 & .85 & .85  & .74 & .73 & .74  & .80 & .83 & .82  & .80 & .72 & .76   \\ 
%     & & Neutral &  .83 & .84 & .84  & .86 & .85 & .85  & .75 & .77 & .76  & .84 & .79 & .81  & .79 & .82 & .81   \\ 
%     & & Positive &  .93 & .93 & .93  & .93 & .94 & .93  & .85 & .85 & .85  & .90 & .93 & .91  & .88 & .91 & .89   \\ 
%     & & Micro-avg &  .87 & .87 & \textbf{.87}  & .88 & .88 & \textbf{.88}  & .78 & .78 & \textbf{.78}  & .85 & .85 & \textbf{.85}  & .82 & .82 & \textbf{.82}   \\ 
%     & & Macro-avg &  .87 & .87 & \textbf{.87}  & .88 & .88 & \textbf{.88}  & .78 & .78 & \textbf{.78}  & .85 & .85 & \textbf{.85}  & .82 & .82 & \textbf{.82}   \\ 

%     \midrule
    
%     % Test dataset: Stack Overflow
%     \multirow{5}{5px}{Cross-platform} & \multirow{5}{*}{GitHub} 
%  & Negative &  .82 & .76 & .79  & .80 & .86 & .83  & .66 & .60 & .63  & .69 & .76 & .72  & .64 & .49 & .55   \\ 
% & & Neutral &  .75 & .85 & .80  & .84 & .80 & .82  & .61 & .64 & .63  & .73 & .76 & .75  & .65 & .85 & .74   \\ 
% & & Positive &  .93 & .85 & .89  & .93 & .91 & .92  & .73 & .74 & .74  & .92 & .82 & .87  & .88 & .74 & .80   \\ 
% & & Micro-avg &  .83 & .83 & \textbf{.83}  & .85 & .85 & \textbf{.85}  & .67 & .67 & \textbf{.67}  & .78 & .78 & \textbf{.78}  & .71 & .71 & \textbf{.71}   \\ 
% & & Macro-avg &  .83 & .82 & \textbf{.82}  & .85 & .86 & \textbf{.85}  & .67 & .66 & \textbf{.66}  & .78 & .78 & \textbf{.78}  & .72 & .69 & \textbf{.70}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.12 & -.12 & -.12 & -.07 & -.07 & -.07 & -.11 & -.11 & -.11  \\ 
% % & & Macro-avg &  -.03 & -.05 & -.04 & -.03 & -.02 & -.03 & -.11 & -.12 & -.12 & -.06 & -.07 & -.07 & -.10 & -.12 & -.12  \\ 

%     \midrule


%     % Test dataset: Stack Overflow
%     \multirow{5}{5px}{Cross-platform} & \multirow{5}{*}{Jira} 
%  & Negative &  .93 & .31 & .47  & .88 & .55 & .68  & .66 & .31 & .42  & .75 & .30 & .43  & .67 & .22 & .33   \\ 
% & & Neutral &  .54 & .98 & .70  & .63 & .94 & .76  & .50 & .91 & .65  & .54 & .93 & .69  & .50 & .95 & .66   \\ 
% & & Positive &  .98 & .62 & .76  & .97 & .74 & .84  & .83 & .42 & .56  & .96 & .64 & .76  & .96 & .52 & .67   \\ 
% & & Micro-avg &  .67 & .67 & \textbf{.67}  & .76 & .76 & \textbf{.76}  & .58 & .58 & \textbf{.58}  & .66 & .66 & \textbf{.66}  & .60 & .60 & \textbf{.60}   \\ 
% & & Macro-avg &  .82 & .64 & \textbf{.64}  & .83 & .74 & \textbf{.76}  & .66 & .55 & \textbf{.54}  & .75 & .62 & \textbf{.63}  & .71 & .56 & \textbf{.55}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.20 & -.20 & -.20 & -.12 & -.12 & -.12 & -.21 & -.21 & -.21 & -.19 & -.19 & -.19 & -.22 & -.22 & -.22  \\ 
% % & & Macro-avg &  -.05 & -.23 & -.23 & -.05 & -.14 & -.12 & -.12 & -.23 & -.24 & -.10 & -.23 & -.22 & -.11 & -.25 & -.27  \\ 

%     \midrule





%     % Test dataset: Jira
%     \multicolumn{18}{c}{\textbf{Test dataset: Jira}} \\
%     \midrule
%     \multirow{5}{5px}{Within-platform} & \multirow{5}{*}{Jira} 
%      & Negative &  .84 & .68 & .75  & .82 & .76 & .79  & .69 & .46 & .55  & .71 & .55 & .62  & .79 & .66 & .72   \\ 
%     & & Neutral &  .89 & .91 & .90  & .90 & .90 & .90  & .83 & .89 & .86  & .84 & .88 & .86  & .89 & .89 & .89   \\ 
%     & & Positive &  .79 & .80 & .79  & .78 & .80 & .79  & .73 & .72 & .72  & .73 & .71 & .72  & .75 & .85 & .80   \\ 
%     & & Micro-avg &  .86 & .86 & \textbf{.86}  & .86 & .86 & \textbf{.86}  & .80 & .80 & \textbf{.80}  & .81 & .81 & \textbf{.81}  & .85 & .85 & \textbf{.85}   \\ 
%     & & Macro-avg &  .84 & .80 & \textbf{.81}  & .83 & .82 & \textbf{.83}  & .75 & .69 & \textbf{.71}  & .76 & .72 & \textbf{.73}  & .81 & .80 & \textbf{.80}   \\ 

%     \midrule
    
    
%     % Test dataset: Jira
%     \multirow{5}{5px}{Cross-platform} & \multirow{5}{*}{GitHub} 
%  & Negative &  .63 & .75 & .69  & .66 & .74 & .70  & .51 & .71 & .60  & .61 & .64 & .62  & .69 & .60 & .64   \\ 
% & & Neutral &  .93 & .79 & .85  & .93 & .80 & .86  & .92 & .58 & .71  & .89 & .78 & .83  & .90 & .85 & .87   \\ 
% & & Positive &  .66 & .91 & .77  & .65 & .91 & .76  & .45 & .92 & .61  & .62 & .86 & .72  & .69 & .89 & .78   \\ 
% & & Micro-avg &  .81 & .81 & \textbf{.81}  & .81 & .81 & \textbf{.81}  & .66 & .66 & \textbf{.66}  & .78 & .78 & \textbf{.78}  & .82 & .82 & \textbf{.82}   \\ 
% & & Macro-avg &  .74 & .82 & \textbf{.77}  & .75 & .82 & \textbf{.77}  & .63 & .74 & \textbf{.64}  & .71 & .76 & \textbf{.73}  & .76 & .78 & \textbf{.76}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.05 & -.05 & -.05 & -.05 & -.05 & -.05 & -.14 & -.14 & -.14 & -.03 & -.03 & -.03 & -.03 & -.03 & -.03  \\ 
% % & & Macro-avg &  -.09 & .02 & -.04 & -.09 & -.00 & -.05 & -.12 & .05 & -.07 & -.05 & .05 & -.01 & -.05 & -.02 & -.04  \\ 

%     \midrule
    
    
%     % Test dataset: Jira
%     \multirow{5}{5px}{Cross-platform} & \multirow{5}{5px}{Stack Overflow} 
%  & Negative &  .67 & .68 & .67  & .72 & .68 & .70  & .58 & .61 & .59  & .50 & .29 & .37  & .36 & .06 & .10   \\ 
% & & Neutral &  .92 & .81 & .86  & .92 & .82 & .87  & .88 & .77 & .82  & .82 & .81 & .81  & .75 & .94 & .83   \\ 
% & & Positive &  .67 & .93 & .78  & .65 & .93 & .76  & .62 & .89 & .73  & .59 & .80 & .68  & .71 & .49 & .58   \\ 
% & & Micro-avg &  .82 & .82 & \textbf{.82}  & .82 & .82 & \textbf{.82}  & .77 & .77 & \textbf{.77}  & .74 & .74 & \textbf{.74}  & .73 & .73 & \textbf{.73}   \\ 
% & & Macro-avg &  .75 & .81 & \textbf{.77}  & .76 & .81 & \textbf{.78}  & .69 & .75 & \textbf{.71}  & .64 & .63 & \textbf{.62}  & .61 & .49 & \textbf{.50}   \\ 

% % \multirow{2}{*}{Diff.} & & Micro-avg &  -.04 & -.04 & -.04 & -.04 & -.04 & -.04 & -.03 & -.03 & -.03 & -.07 & -.07 & -.07 & -.12 & -.12 & -.12  \\ 
% % & & Macro-avg &  -.08 & .01 & -.04 & -.07 & -.01 & -.05 & -.05 & .06 & .00 & -.12 & -.08 & -.11 & -.20 & -.30 & -.30  \\ 


%     \bottomrule
%     \end{tabular}%
% %}
%   % \vspace{-.25in}
%   \label{tab:cross_platform_performance}%
% \end{table*}%




% % \begin{table}[]
% %   \footnotesize
% %   \centering
% %   %\vspace{-.1in}
% %   \caption{Agreement metrics between  tools with manual labelling. For brevity, \small{Moji = SentiMoji, BERT = BERT4Senti4SE, RNN = RNN4SentiSE, S4SD = Senti4SD,  SCR = SentiCR}}
% %   % \vspace{-3mm}
% %     % \resizebox{\columnwidth}{!}{%
% %     \begin{tabular}{p{0.6cm}lrrrr}
% %     \toprule{}

% %     %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
% %     %\cmidrule{3-6}
% %     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Classifier }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
% %     \cmidrule{5-6}
% %     {Dataset} &  & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
    
    
% %     \midrule

% % \multicolumn{6}{c}{\textbf{Test dataset: Github}} \\
% % \midrule

% % \multirow{5}{*}{GitHub} 
% %  & Moji & 0.84 & 90\% & 1\% & 9\%  \\
% %  & BERT & 0.87 & 92\% & 1\% & 7\%  \\
% %  & RNN & 0.52 & 68\% & 7\% & 25\%  \\
% %  & S4SD & 0.86 & 91\% & 1\% & 8\%  \\
% %  & SCR & 0.73 & 83\% & 2\% & 15\%  \\
% % \midrule


% % \multirow{5}{*}{SO} 
% %  & SEntiMoji & 0.61 & 75\% & 2\% & 23\%  \\
% %  & BERT4SentiSE & 0.65 & 78\% & 3\% & 19\%  \\
% %  & RNN4SentiSE & 0.47 & 66\% & 4\% & 30\%  \\
% %  & Senti4SD & 0.60 & 74\% & 4\% & 22\%  \\
% %  & SentiCR & 0.49 & 68\% & 2\% & 29\%  \\
% % \midrule


% % \multirow{5}{*}{Jira} 
% %  & SEntiMoji & 0.44 & 66\% & 1\% & 33\%  \\
% %  & BERT4SentiSE & 0.48 & 68\% & 2\% & 30\%  \\
% %  & RNN4SentiSE & 0.35 & 60\% & 4\% & 36\%  \\
% %  & Senti4SD & 0.50 & 69\% & 2\% & 28\%  \\
% %  & SentiCR & 0.34 & 60\% & 1\% & 39\%  \\
% % \midrule



% % \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% % \midrule

% % \multirow{5}{*}{SO}
% %  & Moji & 0.80 & 87\% & 1\% & 12\%  \\
% %  & BERT & 0.82 & 88\% & 1\% & 11\%  \\
% %  & RNN & 0.67 & 78\% & 3\% & 19\%  \\
% %  & S4SD & 0.77 & 85\% & 1\% & 14\%  \\
% %  & SCR & 0.73 & 82\% & 3\% & 15\%  \\
% % \midrule

% % \multirow{5}{*}{GitHub} 
% %  & SEntiMoji & 0.73 & 83\% & 1\% & 16\%  \\
% %  & BERT4SentiSE & 0.78 & 85\% & 1\% & 14\%  \\
% %  & RNN4SentiSE & 0.49 & 67\% & 4\% & 29\%  \\
% %  & Senti4SD & 0.67 & 78\% & 2\% & 20\%  \\
% %  & SentiCR & 0.56 & 71\% & 5\% & 23\%  \\
% % \midrule


% % \multirow{5}{*}{Jira} 
% %  & SEntiMoji & 0.48 & 67\% & 0\% & 33\%  \\
% %  & BERT4SentiSE & 0.63 & 76\% & 1\% & 23\%  \\
% %  & RNN4SentiSE & 0.34 & 58\% & 4\% & 38\%  \\
% %  & Senti4SD & 0.47 & 66\% & 1\% & 33\%  \\
% %  & SentiCR & 0.37 & 60\% & 2\% & 38\%  \\
% % \midrule







% % \multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
% % \midrule
% % \multirow{5}{*}{Jira}
% %  & Moji & 0.71 & 86\% & 0\% & 14\%  \\
% %  & BERT & 0.72 & 86\% & 0\% & 13\%  \\
% %  & RNN & 0.57 & 80\% & 1\% & 20\%  \\
% %  & S4SD & 0.59 & 81\% & 0\% & 19\%  \\
% %  & SCR & 0.69 & 85\% & 0\% & 15\%  \\
% % \midrule

% % \multirow{5}{*}{GitHub} 
% %  & SEntiMoji & 0.65 & 81\% & 1\% & 18\%  \\
% %  & BERT4SentiSE & 0.65 & 81\% & 1\% & 18\%  \\
% %  & RNN4SentiSE & 0.45 & 66\% & 2\% & 32\%  \\
% %  & Senti4SD & 0.58 & 78\% & 1\% & 21\%  \\
% %  & SentiCR & 0.65 & 82\% & 1\% & 17\%  \\
% % \midrule


% % \multirow{5}{*}{SO} 
% %  & SEntiMoji & 0.65 & 82\% & 1\% & 18\%  \\
% %  & BERT4SentiSE & 0.66 & 82\% & 1\% & 17\%  \\
% %  & RNN4SentiSE & 0.57 & 77\% & 1\% & 22\%  \\
% %  & Senti4SD & 0.46 & 74\% & 1\% & 25\%  \\
% %  & SentiCR & 0.34 & 73\% & 1\% & 26\%  \\
% % % \midrule
% %     % \midrule  
% %     \bottomrule
% %     \end{tabular}%
% % %   }
% %   % \vspace{-.25in}
% %   \label{tab:agreement_with_manual_labelling}%
% % \end{table}%




















% \begin{table}[]
%   \footnotesize
%   \centering
%   %\vspace{-.1in}
%   \caption{Agreement metrics between  tools in both within platform and cross-platform settings. For brevity, \small{Moji = SentiMoji, BERT = BERT4Senti4SE, RNN = RNN4SentiSE, S4SD = Senti4SD,  SCR = SentiCR}}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{p{0.6cm}lrrrr}
%     \toprule{}

%     %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
%     %\cmidrule{3-6}
%     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Tool1 vs }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
%     \cmidrule{5-6}
%     {Dataset} & \bf{Tool2} & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
    
    
%     \midrule

% \multicolumn{6}{c}{\textbf{Test dataset: Github}} \\
% \midrule

% \multirow{10}{*}{GitHub} 
%  & Moji vs BERT & 0.86 & 91\% & 1\% & 8\%  \\
%  & Moji vs RNN & 0.52 & 68\% & 7\% & 25\%  \\
%  & Moji vs S4SD & 0.83 & 89\% & 1\% & 10\%  \\
%  & Moji vs SCR & 0.76 & 85\% & 2\% & 13\%  \\
%  & BERT vs RNN & 0.53 & 69\% & 7\% & 24\%  \\
%  & BERT vs S4SD & 0.85 & 90\% & 2\% & 8\%  \\
%  & BERT vs SCR & 0.74 & 83\% & 2\% & 14\%  \\
%  & RNN vs S4SD & 0.52 & 69\% & 7\% & 25\%  \\
%  & RNN vs SCR & 0.43 & 63\% & 7\% & 31\%  \\
%  & S4SD vs SCR & 0.74 & 83\% & 2\% & 14\%  \\
% \midrule


% \multirow{10}{*}{SO} 
%  & Moji vs BERT & 0.72 & 83\% & 1\% & 15\%  \\
%  & Moji vs RNN & 0.58 & 76\% & 2\% & 22\%  \\
%  & Moji vs S4SD & 0.51 & 70\% & 3\% & 27\%  \\
%  & Moji vs SCR & 0.40 & 68\% & 2\% & 30\%  \\
%  & BERT vs RNN & 0.59 & 76\% & 2\% & 22\%  \\
%  & BERT vs S4SD & 0.52 & 70\% & 4\% & 26\%  \\
%  & BERT vs SCR & 0.39 & 66\% & 3\% & 31\%  \\
%  & RNN vs S4SD & 0.43 & 65\% & 4\% & 31\%  \\
%  & RNN vs SCR & 0.30 & 62\% & 3\% & 35\%  \\
%  & S4SD vs SCR & 0.45 & 68\% & 2\% & 30\%  \\
% \midrule


% \multirow{10}{*}{Jira} 
%  & Moji vs BERT & 0.78 & 90\% & 0\% & 10\%  \\
%  & Moji vs RNN & 0.54 & 81\% & 1\% & 19\%  \\
%  & Moji vs S4SD & 0.60 & 82\% & 1\% & 18\%  \\
%  & Moji vs SCR & 0.65 & 87\% & 0\% & 13\%  \\
%  & BERT vs RNN & 0.56 & 81\% & 1\% & 18\%  \\
%  & BERT vs S4SD & 0.60 & 81\% & 1\% & 18\%  \\
%  & BERT vs SCR & 0.67 & 87\% & 0\% & 13\%  \\
%  & RNN vs S4SD & 0.44 & 74\% & 2\% & 24\%  \\
%  & RNN vs SCR & 0.45 & 79\% & 1\% & 20\%  \\
%  & S4SD vs SCR & 0.52 & 79\% & 1\% & 20\%  \\
% \midrule



% % \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% % \midrule

% % \multirow{10}{*}{GitHub} 
% %  & Moji vs BERT & 0.79 & 86\% & 1\% & 13\%  \\
% %  & Moji vs RNN & 0.53 & 70\% & 4\% & 27\%  \\
% %  & Moji vs S4SD & 0.70 & 80\% & 3\% & 17\%  \\
% %  & Moji vs SCR & 0.62 & 75\% & 5\% & 20\%  \\
% %  & BERT vs RNN & 0.53 & 69\% & 5\% & 26\%  \\
% %  & BERT vs S4SD & 0.73 & 82\% & 2\% & 16\%  \\
% %  & BERT vs SCR & 0.60 & 74\% & 5\% & 21\%  \\
% %  & RNN vs S4SD & 0.54 & 69\% & 4\% & 26\%  \\
% %  & RNN vs SCR & 0.40 & 61\% & 6\% & 33\%  \\
% %  & S4SD vs SCR & 0.58 & 73\% & 4\% & 23\%  \\
% % \midrule


% % \multirow{10}{*}{Jira} 
% %  & Moji vs BERT & 0.66 & 82\% & 0\% & 18\%  \\
% %  & Moji vs RNN & 0.47 & 75\% & 1\% & 23\%  \\
% %  & Moji vs S4SD & 0.60 & 81\% & 1\% & 19\%  \\
% %  & Moji vs SCR & 0.56 & 80\% & 1\% & 19\%  \\
% %  & BERT vs RNN & 0.43 & 70\% & 2\% & 28\%  \\
% %  & BERT vs S4SD & 0.57 & 77\% & 1\% & 22\%  \\
% %  & BERT vs SCR & 0.52 & 75\% & 1\% & 25\%  \\
% %  & RNN vs S4SD & 0.42 & 72\% & 2\% & 27\%  \\
% %  & RNN vs SCR & 0.33 & 70\% & 1\% & 29\%  \\
% %  & S4SD vs SCR & 0.51 & 77\% & 1\% & 22\%  \\
% % \midrule







% % \multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
% % \midrule

% % \multirow{10}{*}{GitHub} 
% %  & Moji vs BERT & 0.81 & 89\% & 1\% & 10\%  \\
% %  & Moji vs RNN & 0.56 & 72\% & 3\% & 25\%  \\
% %  & Moji vs S4SD & 0.72 & 84\% & 1\% & 14\%  \\
% %  & Moji vs SCR & 0.75 & 86\% & 1\% & 13\%  \\
% %  & BERT vs RNN & 0.57 & 73\% & 3\% & 24\%  \\
% %  & BERT vs S4SD & 0.73 & 85\% & 1\% & 14\%  \\
% %  & BERT vs SCR & 0.75 & 87\% & 1\% & 13\%  \\
% %  & RNN vs S4SD & 0.52 & 70\% & 3\% & 27\%  \\
% %  & RNN vs SCR & 0.50 & 69\% & 2\% & 28\%  \\
% %  & S4SD vs SCR & 0.68 & 83\% & 1\% & 16\%  \\
% % \midrule


% % \multirow{10}{*}{SO} 
% %  & Moji vs BERT & 0.80 & 89\% & 1\% & 10\%  \\
% %  & Moji vs RNN & 0.70 & 84\% & 1\% & 15\%  \\
% %  & Moji vs S4SD & 0.61 & 79\% & 1\% & 19\%  \\
% %  & Moji vs SCR & 0.35 & 70\% & 1\% & 29\%  \\
% %  & BERT vs RNN & 0.72 & 84\% & 1\% & 14\%  \\
% %  & BERT vs S4SD & 0.60 & 79\% & 2\% & 19\%  \\
% %  & BERT vs SCR & 0.36 & 71\% & 1\% & 28\%  \\
% %  & RNN vs S4SD & 0.56 & 77\% & 2\% & 22\%  \\
% %  & RNN vs SCR & 0.30 & 67\% & 1\% & 32\%  \\
% %  & S4SD vs SCR & 0.41 & 76\% & 1\% & 23\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_github}%
% \end{table}%


% \begin{table}[]
%   \footnotesize
%   \centering
%   %\vspace{-.1in}
%   \caption{Agreement metrics between  tools in both within platform and cross-platform settings. For brevity, \small{Moji = SentiMoji, BERT = BERT4Senti4SE, RNN = RNN4SentiSE, S4SD = Senti4SD,  SCR = SentiCR}}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{p{0.6cm}lrrrr}
%     \toprule{}

%     %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
%     %\cmidrule{3-6}
%     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Tool1 vs }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
%     \cmidrule{5-6}
%     {Dataset} & \bf{Tool2} & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
    
    
%     \midrule

% % \multicolumn{6}{c}{\textbf{Test dataset: Github}} \\
% % \midrule

% % \multirow{10}{*}{GitHub} 
% %  & Moji vs BERT & 0.86 & 91\% & 1\% & 8\%  \\
% %  & Moji vs RNN & 0.52 & 68\% & 7\% & 25\%  \\
% %  & Moji vs S4SD & 0.83 & 89\% & 1\% & 10\%  \\
% %  & Moji vs SCR & 0.76 & 85\% & 2\% & 13\%  \\
% %  & BERT vs RNN & 0.53 & 69\% & 7\% & 24\%  \\
% %  & BERT vs S4SD & 0.85 & 90\% & 2\% & 8\%  \\
% %  & BERT vs SCR & 0.74 & 83\% & 2\% & 14\%  \\
% %  & RNN vs S4SD & 0.52 & 69\% & 7\% & 25\%  \\
% %  & RNN vs SCR & 0.43 & 63\% & 7\% & 31\%  \\
% %  & S4SD vs SCR & 0.74 & 83\% & 2\% & 14\%  \\
% % \midrule


% % \multirow{10}{*}{SO} 
% %  & Moji vs BERT & 0.72 & 83\% & 1\% & 15\%  \\
% %  & Moji vs RNN & 0.58 & 76\% & 2\% & 22\%  \\
% %  & Moji vs S4SD & 0.51 & 70\% & 3\% & 27\%  \\
% %  & Moji vs SCR & 0.40 & 68\% & 2\% & 30\%  \\
% %  & BERT vs RNN & 0.59 & 76\% & 2\% & 22\%  \\
% %  & BERT vs S4SD & 0.52 & 70\% & 4\% & 26\%  \\
% %  & BERT vs SCR & 0.39 & 66\% & 3\% & 31\%  \\
% %  & RNN vs S4SD & 0.43 & 65\% & 4\% & 31\%  \\
% %  & RNN vs SCR & 0.30 & 62\% & 3\% & 35\%  \\
% %  & S4SD vs SCR & 0.45 & 68\% & 2\% & 30\%  \\
% % \midrule


% % \multirow{10}{*}{Jira} 
% %  & Moji vs BERT & 0.78 & 90\% & 0\% & 10\%  \\
% %  & Moji vs RNN & 0.54 & 81\% & 1\% & 19\%  \\
% %  & Moji vs S4SD & 0.60 & 82\% & 1\% & 18\%  \\
% %  & Moji vs SCR & 0.65 & 87\% & 0\% & 13\%  \\
% %  & BERT vs RNN & 0.56 & 81\% & 1\% & 18\%  \\
% %  & BERT vs S4SD & 0.60 & 81\% & 1\% & 18\%  \\
% %  & BERT vs SCR & 0.67 & 87\% & 0\% & 13\%  \\
% %  & RNN vs S4SD & 0.44 & 74\% & 2\% & 24\%  \\
% %  & RNN vs SCR & 0.45 & 79\% & 1\% & 20\%  \\
% %  & S4SD vs SCR & 0.52 & 79\% & 1\% & 20\%  \\
% % \midrule



% \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% \midrule

% \multirow{10}{*}{SO} 
%  & Moji vs BERT & 0.86 & 91\% & 1\% & 8\%  \\
%  & Moji vs RNN & 0.70 & 80\% & 3\% & 17\%  \\
%  & Moji vs S4SD & 0.81 & 88\% & 1\% & 12\%  \\
%  & Moji vs SCR & 0.78 & 85\% & 2\% & 12\%  \\
%  & BERT vs RNN & 0.71 & 81\% & 2\% & 17\%  \\
%  & BERT vs S4SD & 0.83 & 88\% & 1\% & 11\%  \\
%  & BERT vs SCR & 0.78 & 85\% & 3\% & 12\%  \\
%  & RNN vs S4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & RNN vs SCR & 0.65 & 77\% & 4\% & 19\%  \\
%  & S4SD vs SCR & 0.78 & 85\% & 3\% & 12\%  \\
% \midrule

% \multirow{10}{*}{GitHub} 
%  & Moji vs BERT & 0.79 & 86\% & 1\% & 13\%  \\
%  & Moji vs RNN & 0.53 & 70\% & 4\% & 27\%  \\
%  & Moji vs S4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & Moji vs SCR & 0.62 & 75\% & 5\% & 20\%  \\
%  & BERT vs RNN & 0.53 & 69\% & 5\% & 26\%  \\
%  & BERT vs S4SD & 0.73 & 82\% & 2\% & 16\%  \\
%  & BERT vs SCR & 0.60 & 74\% & 5\% & 21\%  \\
%  & RNN vs S4SD & 0.54 & 69\% & 4\% & 26\%  \\
%  & RNN vs SCR & 0.40 & 61\% & 6\% & 33\%  \\
%  & S4SD vs SCR & 0.58 & 73\% & 4\% & 23\%  \\
% \midrule


% \multirow{10}{*}{Jira} 
%  & Moji vs BERT & 0.66 & 82\% & 0\% & 18\%  \\
%  & Moji vs RNN & 0.47 & 75\% & 1\% & 23\%  \\
%  & Moji vs S4SD & 0.60 & 81\% & 1\% & 19\%  \\
%  & Moji vs SCR & 0.56 & 80\% & 1\% & 19\%  \\
%  & BERT vs RNN & 0.43 & 70\% & 2\% & 28\%  \\
%  & BERT vs S4SD & 0.57 & 77\% & 1\% & 22\%  \\
%  & BERT vs SCR & 0.52 & 75\% & 1\% & 25\%  \\
%  & RNN vs S4SD & 0.42 & 72\% & 2\% & 27\%  \\
%  & RNN vs SCR & 0.33 & 70\% & 1\% & 29\%  \\
%  & S4SD vs SCR & 0.51 & 77\% & 1\% & 22\%  \\
% % \midrule

%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_so}%
% \end{table}%



% \begin{table}[]
%   \footnotesize
%   \centering
%   %\vspace{-.1in}
%   \caption{Agreement metrics between  tools in both within platform and cross-platform settings. For brevity, \small{Moji = SentiMoji, BERT = BERT4Senti4SE, RNN = RNN4SentiSE, S4SD = Senti4SD,  SCR = SentiCR}}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{p{0.6cm}lrrrr}
%     \toprule{}

%     %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
%     %\cmidrule{3-6}
%     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Tool1 vs }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
%     \cmidrule{5-6}
%     {Dataset} & \bf{Tool2} & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
    
    
%     \midrule

% % \multicolumn{6}{c}{\textbf{Test dataset: Github}} \\
% % \midrule

% % \multirow{10}{*}{GitHub} 
% %  & Moji vs BERT & 0.86 & 91\% & 1\% & 8\%  \\
% %  & Moji vs RNN & 0.52 & 68\% & 7\% & 25\%  \\
% %  & Moji vs S4SD & 0.83 & 89\% & 1\% & 10\%  \\
% %  & Moji vs SCR & 0.76 & 85\% & 2\% & 13\%  \\
% %  & BERT vs RNN & 0.53 & 69\% & 7\% & 24\%  \\
% %  & BERT vs S4SD & 0.85 & 90\% & 2\% & 8\%  \\
% %  & BERT vs SCR & 0.74 & 83\% & 2\% & 14\%  \\
% %  & RNN vs S4SD & 0.52 & 69\% & 7\% & 25\%  \\
% %  & RNN vs SCR & 0.43 & 63\% & 7\% & 31\%  \\
% %  & S4SD vs SCR & 0.74 & 83\% & 2\% & 14\%  \\
% % \midrule


% % \multirow{10}{*}{SO} 
% %  & Moji vs BERT & 0.72 & 83\% & 1\% & 15\%  \\
% %  & Moji vs RNN & 0.58 & 76\% & 2\% & 22\%  \\
% %  & Moji vs S4SD & 0.51 & 70\% & 3\% & 27\%  \\
% %  & Moji vs SCR & 0.40 & 68\% & 2\% & 30\%  \\
% %  & BERT vs RNN & 0.59 & 76\% & 2\% & 22\%  \\
% %  & BERT vs S4SD & 0.52 & 70\% & 4\% & 26\%  \\
% %  & BERT vs SCR & 0.39 & 66\% & 3\% & 31\%  \\
% %  & RNN vs S4SD & 0.43 & 65\% & 4\% & 31\%  \\
% %  & RNN vs SCR & 0.30 & 62\% & 3\% & 35\%  \\
% %  & S4SD vs SCR & 0.45 & 68\% & 2\% & 30\%  \\
% % \midrule


% % \multirow{10}{*}{Jira} 
% %  & Moji vs BERT & 0.78 & 90\% & 0\% & 10\%  \\
% %  & Moji vs RNN & 0.54 & 81\% & 1\% & 19\%  \\
% %  & Moji vs S4SD & 0.60 & 82\% & 1\% & 18\%  \\
% %  & Moji vs SCR & 0.65 & 87\% & 0\% & 13\%  \\
% %  & BERT vs RNN & 0.56 & 81\% & 1\% & 18\%  \\
% %  & BERT vs S4SD & 0.60 & 81\% & 1\% & 18\%  \\
% %  & BERT vs SCR & 0.67 & 87\% & 0\% & 13\%  \\
% %  & RNN vs S4SD & 0.44 & 74\% & 2\% & 24\%  \\
% %  & RNN vs SCR & 0.45 & 79\% & 1\% & 20\%  \\
% %  & S4SD vs SCR & 0.52 & 79\% & 1\% & 20\%  \\
% % \midrule



% % \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% % \midrule

% % \multirow{10}{*}{SO} 
% %  & Moji vs BERT & 0.86 & 91\% & 1\% & 8\%  \\
% %  & Moji vs RNN & 0.70 & 80\% & 3\% & 17\%  \\
% %  & Moji vs S4SD & 0.81 & 88\% & 1\% & 12\%  \\
% %  & Moji vs SCR & 0.78 & 85\% & 2\% & 12\%  \\
% %  & BERT vs RNN & 0.71 & 81\% & 2\% & 17\%  \\
% %  & BERT vs S4SD & 0.83 & 88\% & 1\% & 11\%  \\
% %  & BERT vs SCR & 0.78 & 85\% & 3\% & 12\%  \\
% %  & RNN vs S4SD & 0.70 & 80\% & 3\% & 17\%  \\
% %  & RNN vs SCR & 0.65 & 77\% & 4\% & 19\%  \\
% %  & S4SD vs SCR & 0.78 & 85\% & 3\% & 12\%  \\
% % \midrule

% % \multirow{10}{*}{GitHub} 
% %  & Moji vs BERT & 0.79 & 86\% & 1\% & 13\%  \\
% %  & Moji vs RNN & 0.53 & 70\% & 4\% & 27\%  \\
% %  & Moji vs S4SD & 0.70 & 80\% & 3\% & 17\%  \\
% %  & Moji vs SCR & 0.62 & 75\% & 5\% & 20\%  \\
% %  & BERT vs RNN & 0.53 & 69\% & 5\% & 26\%  \\
% %  & BERT vs S4SD & 0.73 & 82\% & 2\% & 16\%  \\
% %  & BERT vs SCR & 0.60 & 74\% & 5\% & 21\%  \\
% %  & RNN vs S4SD & 0.54 & 69\% & 4\% & 26\%  \\
% %  & RNN vs SCR & 0.40 & 61\% & 6\% & 33\%  \\
% %  & S4SD vs SCR & 0.58 & 73\% & 4\% & 23\%  \\
% % \midrule


% % \multirow{10}{*}{Jira} 
% %  & Moji vs BERT & 0.66 & 82\% & 0\% & 18\%  \\
% %  & Moji vs RNN & 0.47 & 75\% & 1\% & 23\%  \\
% %  & Moji vs S4SD & 0.60 & 81\% & 1\% & 19\%  \\
% %  & Moji vs SCR & 0.56 & 80\% & 1\% & 19\%  \\
% %  & BERT vs RNN & 0.43 & 70\% & 2\% & 28\%  \\
% %  & BERT vs S4SD & 0.57 & 77\% & 1\% & 22\%  \\
% %  & BERT vs SCR & 0.52 & 75\% & 1\% & 25\%  \\
% %  & RNN vs S4SD & 0.42 & 72\% & 2\% & 27\%  \\
% %  & RNN vs SCR & 0.33 & 70\% & 1\% & 29\%  \\
% %  & S4SD vs SCR & 0.51 & 77\% & 1\% & 22\%  \\
% % \midrule







% \multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
% \midrule


% \multirow{10}{*}{Jira} 
%  & Moji vs BERT & 0.85 & 93\% & 0\% & 7\%  \\
%  & Moji vs RNN & 0.68 & 86\% & 0\% & 14\%  \\
%  & Moji vs S4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & Moji vs SCR & 0.81 & 91\% & 0\% & 9\%  \\
%  & BERT vs RNN & 0.68 & 85\% & 1\% & 14\%  \\
%  & BERT vs S4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & BERT vs SCR & 0.79 & 90\% & 0\% & 10\%  \\
%  & RNN vs S4SD & 0.61 & 83\% & 0\% & 17\%  \\
%  & RNN vs SCR & 0.70 & 86\% & 1\% & 14\%  \\
%  & S4SD vs SCR & 0.70 & 86\% & 0\% & 13\%  \\
% \midrule

% \multirow{10}{*}{GitHub} 
%  & Moji vs BERT & 0.81 & 89\% & 1\% & 10\%  \\
%  & Moji vs RNN & 0.56 & 72\% & 3\% & 25\%  \\
%  & Moji vs S4SD & 0.72 & 84\% & 1\% & 14\%  \\
%  & Moji vs SCR & 0.75 & 86\% & 1\% & 13\%  \\
%  & BERT vs RNN & 0.57 & 73\% & 3\% & 24\%  \\
%  & BERT vs S4SD & 0.73 & 85\% & 1\% & 14\%  \\
%  & BERT vs SCR & 0.75 & 87\% & 1\% & 13\%  \\
%  & RNN vs S4SD & 0.52 & 70\% & 3\% & 27\%  \\
%  & RNN vs SCR & 0.50 & 69\% & 2\% & 28\%  \\
%  & S4SD vs SCR & 0.68 & 83\% & 1\% & 16\%  \\
% \midrule


% \multirow{10}{*}{SO} 
%  & Moji vs BERT & 0.80 & 89\% & 1\% & 10\%  \\
%  & Moji vs RNN & 0.70 & 84\% & 1\% & 15\%  \\
%  & Moji vs S4SD & 0.61 & 79\% & 1\% & 19\%  \\
%  & Moji vs SCR & 0.35 & 70\% & 1\% & 29\%  \\
%  & BERT vs RNN & 0.72 & 84\% & 1\% & 14\%  \\
%  & BERT vs S4SD & 0.60 & 79\% & 2\% & 19\%  \\
%  & BERT vs SCR & 0.36 & 71\% & 1\% & 28\%  \\
%  & RNN vs S4SD & 0.56 & 77\% & 2\% & 22\%  \\
%  & RNN vs SCR & 0.30 & 67\% & 1\% & 32\%  \\
%  & S4SD vs SCR & 0.41 & 76\% & 1\% & 23\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_jira}%
% \end{table}%















% \begin{figure*}[!htb]
% \centering
% \pgfplotstableread{

% 1	.88  .97 .75 .78     .88  .97  .83 .88      .87  .96  .81 .85
% 2	.87  .96 .66 .68     .85  .93  .67 .85      .85  .93  .82 .76
% % 3	31.9  13.6  54.5  40.9  27.3  31.8  31.8  27.3  40.9  20.5  20.4  59.1  27.3  11.3  61.4  20.5  20.4  59.1  20.5  20.4  59.1  27.3  27.2  45.5 
% }\datatable

%       \subfloat[Test dataset GitHub]
%       {
%       \resizebox{1.5in}{!}{%
%       \begin{tikzpicture}
%         	\begin{axis}[
%         	%ylabel=label,
%         	xtick=data,
%         	xticklabels={Trained dataset SO, Trained dataset Jira},
%         	enlarge y limits=false,
%         	enlarge x limits=0.40,
%         % 	axis y line = none,
%         % 	axis y line=left,
%         %   axis line style={-},
%             axis y line=none,
%             % hide y axis,
%             axis x line*=bottom,
%             axis y line*=left,
%         % 	axis x line=left,
%         % 	axis x line=bottom,
%         % 	axis line style={draw=none},
%         %	nodes near coords,
%         	ymin=0,ymax=1,
%         	ybar,
%         	bar width=0.7cm,
%         	width=3.6in,
%         	height = 2.3in,
%         % 	ytick={0,20,...,80},
%             % yticklabels={0\%,20\%,40\%,60\%,80\%},
%         	%ylabel={Accepted Answer (\%)},
%         	ymajorgrids=false,
%         %	xminorgrids=true,
%          	yticklabel style={font=\large},
%         	xticklabel style={font=\large, /pgf/number format/fixed},	
%         	major x tick style = {opacity=0},
%         	minor x tick num = 1,    
%         	minor tick length=1ex,
%         	legend style={
%          	at={(0.6,0.98)},
%             anchor=north,legend columns=-1
%             },
%             % nodes near coords,
%             nodes near coords style={font=\LARGE},
%             nodes near coords style={rotate=90,  anchor=west}, %
%         	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
%         	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
%         	]
%         	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=1] \datatable;
%         	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=2] \datatable;
%         	\addplot[draw=black!80, fill=black!70] table[x index=0,y index=3] \datatable;
%         	\addplot[draw=black!80, fill=black!100] table[x index=0,y index=4] \datatable;
        
%             % \legend	{Jensen-Shannon Divergence,
%             % 		 Cosine Similarity,
%             % 		 SEntiMoji F1 score,
%             % 		 BERT4SentiSE F1 score
%             % 		 }
        	

%         	\end{axis}
%     	\end{tikzpicture}
%      	}
%     %  	\hspace{-1mm}
%     	\label{presentation-inconsistency}
%     } 
%     \subfloat[Test dataset SO]
%      {
%       \resizebox{1.5in}{!}{%
%       \begin{tikzpicture}
%         	\begin{axis}[
%         	%ylabel=label,
%         	xtick=data,
%         	xticklabels={Train dataset GitHub, Train dataset Jira
%         	},
%         	enlarge y limits=false,
%         	enlarge x limits=0.40,
%         % 	axis y line = none,
%         % 	axis y line=left,
%         %   axis line style={-},
%             axis y line=none,
%             % hide y axis,
%             axis x line*=bottom,
%             axis y line*=left,
%         % 	axis x line=left,
%         % 	axis x line=bottom,
%         % 	axis line style={draw=none},
%         %	nodes near coords,
%         	ymin=0,ymax=1,
%         	ybar,
%         	bar width=0.7cm,
%         	width=3.6in,
%         	height = 2.3in,
%         % 	ytick={0,20,...,80},
%             % yticklabels={0\%,20\%,40\%,60\%,80\%},
%         	%ylabel={Accepted Answer (\%)},
%         	ymajorgrids=false,
%         %	xminorgrids=true,
%          	yticklabel style={font=\large},
%          	xticklabel style={font=\large, /pgf/number format/fixed},	
%         	major x tick style = {opacity=0},
%         	minor x tick num = 1,    
%         	minor tick length=1ex,
%         	legend style={
%          	at={(0.5,1.35)},
%         % 	font=\small,
%         % 	legend pos = outer north east,
%         %  	legend pos=north west,
%         %   anchor=west,
%         % 	cells={align=left},
%         % 	legend cell align=left
%             anchor=north,legend columns=-1
%             },
%             nodes near coords style={font=\LARGE},
%             nodes near coords style={rotate=90,  anchor=west}, %
%         	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
%         	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
%         	]
%         	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=5] \datatable;
%         	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=6] \datatable; %, postaction={pattern=horizontal lines}
%         	\addplot[draw=black!80, fill=black!60] table[x index=0,y index=7] \datatable; %, postaction={pattern=vertical lines}
%             \addplot[draw=black!80, fill=black!100] table[x index=0,y index=8] \datatable; %, postaction={pattern=vertical lines}
%             \legend{JS Divergence,
%             		 Cosine Similarity,
%             		 Moji F1,
%             		 BERT F1
%             		 }
%         	\end{axis}
%     	\end{tikzpicture}
%     	}
%     % 	\hspace{-1mm}
%     	\label{signature-inconsistency}
%     }
%     \subfloat[Test dataset Jira]
%      {
%       \resizebox{1.5in}{!}{%
%       \begin{tikzpicture}
%         	\begin{axis}[
%         	%ylabel=label,
%         	xtick=data,
%         	xticklabels={Train dataset GitHub, Train dataset SO
%         	},
%         	enlarge y limits=false,
%         	enlarge x limits=0.40,
%         % 	axis y line = none,
%         % 	axis y line=left,
%         %   axis line style={-},
%             axis y line=none,
%             % hide y axis,
%             axis x line*=bottom,
%             axis y line*=left,
%         % 	axis x line=left,
%         % 	axis x line=bottom,
%         % 	axis line style={draw=none},
%         %	nodes near coords,
%         	ymin=0,ymax=1,
%         	ybar,
%         	bar width=0.7cm,
%         	width=3.4in,
%         	height = 2.3in,
%         % 	ytick={0,20,...,80},
%         %     yticklabels={0\%,20\%,40\%,60\%,80\%},
%         	%ylabel={Accepted Answer (\%)},
%         	ymajorgrids=false,
%         %	xminorgrids=true,
%          	yticklabel style={font=\large},
%          	xticklabel style={font=\large, /pgf/number format/fixed},	
%         	major x tick style = {opacity=0},
%         	minor x tick num = 1,    
%         	minor tick length=1ex,
%         	legend style={
%          	at={(0.6,0.98)},
%         % 	font=\small,
%         % 	legend pos = outer north east,
%         %  	legend pos=north west,
%         %   anchor=west,
%         % 	cells={align=left},
%         % 	legend cell align=left
%             anchor=north,legend columns=-1
%             },
%             nodes near coords style={font=\LARGE},
%             nodes near coords style={rotate=90,  anchor=west}, %
%         	nodes near coords =\pgfmathprintnumber{\pgfplotspointmeta}
%         	%nodes near coords*={\pgfmathprintnumber[precision=2]\pgfplotspointmeta \%}
%         	]
%         	\addplot[draw=black!80, fill=black!5] table[x index=0,y index=9] \datatable;
%         	\addplot[draw=black!80, fill=black!30] table[x index=0,y index=10] \datatable; %, postaction={pattern=horizontal lines}
%         	\addplot[draw=black!80, fill=black!60] table[x index=0,y index=11] \datatable; %, postaction={pattern=vertical lines}
%             \addplot[draw=black!80, fill=black!100] table[x index=0,y index=12] \datatable; %, postaction={pattern=vertical lines}

%         	\end{axis}
%     	\end{tikzpicture}
%     	}
%     % 	%\hspace{-1mm}
%     	\label{status-inconsistency}
%     }
    


    
    
% %\vspace{-3mm}
% \caption{Impact of the similarity between datasets and performance of the DL-tools. The four bars represents the Jensen-Shannon Divergence,  Cosine Similarity, SEntiMoji F1 score,  BERT4SentiSE F1 score respectively.
% % \gias{the fonts above bars very small - make those bigger. The separation betwen two sets of bars per test dataset is too big - shrink. Put those for subfloats a, b, c side by side in one row. also put a legend above to indicate which bar denotes what.}
% }


% \vspace{-3mm}
% \label{fig:impacts-inconsistency-types}
% \end{figure*}























% % \begin{table*}[t]
% %   \centering
% %   %\vspace{-.1in}
% %   \caption{Some examples of severe misclassification by the five tools in cross-platform setting.}

% %     \begin{tabular}{cc}
% %     % \toprule{}
% %     \textbf{Misclassified Positive sentences as Negative} & \textbf{Misclassified Negative sentences as Positive}\\
    
% % \noindent \centering \fbox{%
% %     \parbox{.45\textwidth}{%

% %       \textbf{SEntiMoji} \\
% %       ``Oh, I've misread commit title, my bad :dancers:''\\
% %       ``You made it on top of hacker news. Congratz.''\\
% %       ``come on - friendly pets make presents to their owner sometimes!" \\
% %       ``+1 for this question - I have the same issue."\\
% %       ``Oh, you're right. Misread." \\
      
% %       \textbf{Bert4SentiSE} \\
% %         ``Dennis, you rock. Seriously." \\
% %         ``Sorry about that. The new things are just so shiny!" \\
% %         ``I hereby associate myself with this epic commit thread."" \\
% %         ``This is so badass I don't even know where to begin"" \\
% %         % ``It's Exploit Fix Day!" \\
% %         ``Its safe, at least from a unit testing perspective! I also don't see why it wouldn't be safe. An I missing something?" \\

      
      
% %       \textbf{RNN4SentiSE} \\
% %       ``Is this a fix for the 'Attempted to place a tile entity where there was no entity tile' bug?  Because if so, awesome!" \\
% %  ``Hello Andreas  Thank you for the information.  Shall try the same and upload the patch shortly.  Thanks \& Regards Ravikiran Mane." \\
% %  `` Hi Ramin  The patch looks good except I think it would be good to give import/export its own  SQLState starting with XIE instead of reusing the existing store FILE EXISTS message.  Also it would be good to have test cases for writing the lob files. Kathey" \\
% %  ``God I am awful at this :)" \\

      
      
      
% %       \textbf{Seniti4SD} \\
% % ``When explaining things to someone who seems to still be learning Haskell, I'd avoid using (or even showing) the pointless style. Don't want to scare them ;-)" \\
% % ``I still prefer RAII. Make the compiler do the work of making it leak proof. Safer *and* more convenient."" \\
% % ``Not to worry I've SOLVED it!" \\
% % ``No this was on 3.3.3 (sorry I should have mentioned that before).  That's great to know thanks!" \\
% % ``Holy crap that worked!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!" \\
      
      
      
% %       \textbf{SentiCR} \\
% %  ``@mcsnetworks WOW That looks amazing! Will most likely be moving to this some time in the future."" \\
% %  ``Sorry Jacques I have not seen that it was a grouped bugs.  In this case I have used to set in the grouped bugs the sum of the components used by detailed issues.  I didn't like unknow components.  Otherwise we can add a new fictitious component - GROUPED ISSUES - and assign this component to this type of issue.   Thanks  Marco" \\
% %  ``Yes, it's possible, juste remove the second parameter of your method (it's totally useless) ans it will work (I tested the code) !" \\
% %  ``Don't worry gyus, Vladimir always make the best things. )) Very respected to you........................" \\
% %  ``Thanks.. I really need to remember to run mvn clean package before push changes... I own you some beer" \\
% %     }%
% % }


% % &

% % \noindent \centering \fbox{%
% %     \parbox{.45\textwidth}{%
    
% %      \textbf{SEntiMoji} \\
% %  ``Great, again client freezes ...." \\
% %  ``Permanent Feign Death is permament! ;)" \\
% %  ``Makes sense, and it's very similiar to what I am doing. One ant task for stage and one for production, and just using the defaults for local development. But pain arises from mainting 3 different application contexts which have almost identical content.." \\
% %  ``Damn clean, Mr Kuhn, damn clean!" \\

    
    
% %       \textbf{Bert4SentiSE} \\
% %  ``Would've loved to. But there is no hash\_map in the C++ standard library, and PHB's don't allow code outside of that." \\
% %  ``Lotus Notes....aaaaargh!" \\
% %  ``What, no separators between the values? D:" \\ 
% %  ``+1 Fear the unhappy robots!" \\
% %  ``that's what I get for copying and pasting!" \\
% %  ``Wow, could have probably come across a little friendlier there, Phil!" \\


% %       \textbf{RNN4SentiSE} \\
% % % ``I think this is a great idea, but it's going to screw over a LOT of people who followed bad jQuery tutorials online that all seem to love recommending $() as a shortcut to $(document).''  \\
% % ``boo. Want to come up with something that looks nice in both the scss and docs? create a documentation styleguide?''  \\
% % ``the use of === for these doesn't make sense, consistent or not it's not worth a pull-request for pointless stuff like that''  \\
% % ``No tests bro :(''  \\
% % ``(in other words, my mind is melted down and I trust my basic arithmetic skills even less than before)''  \\


% %       \textbf{Senti4SD} \\
% % % ``Well, I guess I'll be taking my leave like @V10lator.  I need NBT and it's clear after more arguments that it will not be supported, probably along with an AI API and packet API.  Edit: @mbax That was the reason why I was planning to include independent ''  \\
% % ``Yes, the naming is all pretty terrible. I believe it's because we've gone through several iterations of what ""render"" actually means :)  One is used for fullscreen rendering, the other is used for video controls.  This is very much a hack, and hopeful''  \\
% % ``Pretty much hackfix, rather specify knockback immunity in spellauraeffects.cpp''  \\
% % ``Oh, right. That'd be the forum template that generated that. And no worries, I didn't take it personnally !''  \\
% % ``-5 votes?? People who have downvoted this answer should have specified the reason for doing so as well.''  \\




% %       \textbf{SentiCR} \\
% % ``Y U REQUIRE RUBYGEMS HERE !?!?!?!?!? :bomb:''  \\
% % ``Rebase FAIL!''  \\
% % ``Closing connections as side-effect of running assertColumnExists is dirty. For example anybody using transactions will have a nice surprise waiting...''  \\
% % ``This is extremely unsafe! Use mysqli or pdo instead of`mysql\_.''  \\
% % ``I'm -1 on this. It's imo easy enough to do Mailer.expects(:welcome) and then keep mocking from there. I don't like having two ways of doing the same thing purely to make it marginally easier to mock.''  \\
% % ``it worked, weird. thanks.''  \\
      
% %     }%
% % }

% %     \end{tabular}%
% %   \label{tab:misclassification2}%
% % \end{table*}%








% \begin{table}[]
%   \footnotesize
% %   \small
%   \centering
%   %\vspace{-.1in}
%   \caption{Agreement metrics between  tools with manual labelling}
%   % \vspace{-3mm}
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{clrrrr}
%     \toprule{}
%     %\multirow{3}{*}{\textbf{Train}} & \multirow{3}{*}{\textbf{Tools}} & %\multicolumn{4}{c}{\textbf{Agreement metrics}} \\
%     %\cmidrule{3-6}
%     \multirow{2}{*}{\bf{Train}} & \multirow{2}{*}{\bf{Classifier }} & \multirow{2}{*}{\bf{K}} & \multirow{2}{*}{\textbf{Perfect}} & \multicolumn{2}{c}{Disagreement}\\
%     \cmidrule{5-6}
%     {Dataset} &  & {} & {\textbf{Agreement}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule
% \multicolumn{6}{c}{\textbf{Test dataset: GitHub}} \\
% \midrule

% \multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Within-platform)}} 
%  & SEntiMoji & 0.84 & 90\% & 1\% & 9\%  \\
%  & BERT4SentiSE & 0.87 & 92\% & 1\% & 7\%  \\
%  & RNN4SentiSE & 0.52 & 68\% & 7\% & 25\%  \\
%  & Senti4SD & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiCR & 0.73 & 83\% & 2\% & 15\%  \\
% % \midrule
% \cmidrule{2-6}

% \multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow \\ (Cross-platform)}}  
%  & SEntiMoji & 0.61 & 75\% & 2\% & 23\%  \\
%  & BERT4SentiSE & 0.65 & 78\% & 3\% & 19\%  \\
%  & RNN4SentiSE & 0.47 & 66\% & 4\% & 30\%  \\
%  & Senti4SD & 0.60 & 74\% & 4\% & 22\%  \\
%  & SentiCR & 0.49 & 68\% & 2\% & 29\%  \\
% % \midrule
% \cmidrule{2-6}


% \multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Cross-platform)}} 
%  & SEntiMoji & 0.44 & 66\% & 1\% & 33\%  \\
%  & BERT4SentiSE & 0.48 & 68\% & 2\% & 30\%  \\
%  & RNN4SentiSE & 0.35 & 60\% & 4\% & 36\%  \\
%  & Senti4SD & 0.50 & 69\% & 2\% & 28\%  \\
%  & SentiCR & 0.34 & 60\% & 1\% & 39\%  \\
% \midrule



% \multicolumn{6}{c}{\textbf{Test dataset: Stack Overflow}} \\
% \midrule

% \multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow (Within-platform)}}
%  & SEntiMoji & 0.80 & 87\% & 1\% & 12\%  \\
%  & BERT4SentiSE& 0.82 & 88\% & 1\% & 11\%  \\
%  & RNN4SentiSE & 0.67 & 78\% & 3\% & 19\%  \\
%  & Senti4SD & 0.77 & 85\% & 1\% & 14\%  \\
%  & SentiCR & 0.73 & 82\% & 3\% & 15\%  \\
% % \midrule
% \cmidrule{2-6}

% \multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Cross-platform)}} 
%  & SEntiMoji & 0.73 & 83\% & 1\% & 16\%  \\
%  & BERT4SentiSE & 0.78 & 85\% & 1\% & 14\%  \\
%  & RNN4SentiSE & 0.49 & 67\% & 4\% & 29\%  \\
%  & Senti4SD & 0.67 & 78\% & 2\% & 20\%  \\
%  & SentiCR & 0.56 & 71\% & 5\% & 23\%  \\
% % \midrule
% \cmidrule{2-6}

% \multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Cross-platform)}} 
%  & SEntiMoji & 0.48 & 67\% & 0\% & 33\%  \\
%  & BERT4SentiSE & 0.63 & 76\% & 1\% & 23\%  \\
%  & RNN4SentiSE & 0.34 & 58\% & 4\% & 38\%  \\
%  & Senti4SD & 0.47 & 66\% & 1\% & 33\%  \\
%  & SentiCR & 0.37 & 60\% & 2\% & 38\%  \\
% \midrule







% \multicolumn{6}{c}{\textbf{Test dataset: Jira}} \\
% \midrule
% \multirow{5}{*}{\parbox{2.5cm} {\centering Jira \\ (Within-platform)}}
%  & SEntiMoji & 0.71 & 86\% & 0\% & 14\%  \\
%  & BERT4SentiSE& 0.72 & 86\% & 0\% & 13\%  \\
%  & RNN4SentiSE & 0.57 & 80\% & 1\% & 20\%  \\
%  & Senti4SD & 0.59 & 81\% & 0\% & 19\%  \\
%  & SentiCR & 0.69 & 85\% & 0\% & 15\%  \\
% % \midrule
% \cmidrule{2-6}


% \multirow{5}{*}{\parbox{2.5cm} {\centering GitHub \\ (Cross-platform)}} 
%  & SEntiMoji & 0.65 & 81\% & 1\% & 18\%  \\
%  & BERT4SentiSE & 0.65 & 81\% & 1\% & 18\%  \\
%  & RNN4SentiSE & 0.45 & 66\% & 2\% & 32\%  \\
%  & Senti4SD & 0.58 & 78\% & 1\% & 21\%  \\
%  & SentiCR & 0.65 & 82\% & 1\% & 17\%  \\
% % \midrule
% \cmidrule{2-6}

% \multirow{5}{*}{\parbox{2.5cm} {\centering Stack Overflow \\ (Cross-platform)}} 
%  & SEntiMoji & 0.65 & 82\% & 1\% & 18\%  \\
%  & BERT4SentiSE & 0.66 & 82\% & 1\% & 17\%  \\
%  & RNN4SentiSE & 0.57 & 77\% & 1\% & 22\%  \\
%  & Senti4SD & 0.46 & 74\% & 1\% & 25\%  \\
%  & SentiCR & 0.34 & 73\% & 1\% & 26\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_with_manual_labelling}%
% \end{table}%


% \begin{table}
% \renewcommand{\thetable}{\arabic{table}aa}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Agreement between  tools (Test dataset: GitHub)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Data}} & \multirow{2}{*}{\bf{T1 $\leftrightarrow$ T2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule
% \multirow{10}{*}{G (W)} 
%  & SM $\leftrightarrow$ BS & 0.86 & 91\% & 1\% & 8\%  \\
%  & SM $\leftrightarrow$ RS & 0.52 & 68\% & 7\% & 25\%  \\
%  & SM $\leftrightarrow$ SD & 0.83 & 89\% & 1\% & 10\%  \\
%  & SM $\leftrightarrow$ SC & 0.76 & 85\% & 2\% & 13\%  \\
%  & BS $\leftrightarrow$ RS & 0.53 & 69\% & 7\% & 24\%  \\
%  & BS vs SD & 0.85 & 90\% & 2\% & 8\%  \\
%  & BS vs SC & 0.74 & 83\% & 2\% & 14\%  \\
%  & RS vs SD & 0.52 & 69\% & 7\% & 25\%  \\
%  & RS vs SC & 0.43 & 63\% & 7\% & 31\%  \\
%  & SD vs SC & 0.74 & 83\% & 2\% & 14\%  \\
% \midrule


% \multirow{10}{*}{S(C)} 
%  & SM vs BS & 0.72 & 83\% & 1\% & 15\%  \\
%  & SM vs RS & 0.58 & 76\% & 2\% & 22\%  \\
%  & SM vs SD & 0.51 & 70\% & 3\% & 27\%  \\
%  & SM vs SC & 0.40 & 68\% & 2\% & 30\%  \\
%  & BS vs RS & 0.59 & 76\% & 2\% & 22\%  \\
%  & BS vs SD & 0.52 & 70\% & 4\% & 26\%  \\
%  & BS vs SC & 0.39 & 66\% & 3\% & 31\%  \\
%  & RS vs SD & 0.43 & 65\% & 4\% & 31\%  \\
%  & RS vs SC & 0.30 & 62\% & 3\% & 35\%  \\
%  & SD vs SC & 0.45 & 68\% & 2\% & 30\%  \\
% \midrule


% \multirow{10}{*}{J(C)} 
%  & SM vs BS & 0.78 & 90\% & 0\% & 10\%  \\
%  & SM vs RS & 0.54 & 81\% & 1\% & 19\%  \\
%  & SM vs SD & 0.60 & 82\% & 1\% & 18\%  \\
%  & SM vs SC & 0.65 & 87\% & 0\% & 13\%  \\
%  & BS vs RS & 0.56 & 81\% & 1\% & 18\%  \\
%  & BS vs SD & 0.60 & 81\% & 1\% & 18\%  \\
%  & BS vs SC & 0.67 & 87\% & 0\% & 13\%  \\
%  & RS vs SD & 0.44 & 74\% & 2\% & 24\%  \\
%  & RS vs SC & 0.45 & 79\% & 1\% & 20\%  \\
%  & SD vs SC & 0.52 & 79\% & 1\% & 20\%  \\

%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_github}%
% \end{table}%



% \begin{table}
% \renewcommand{\thetable}{\arabic{table}a}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Agreement between  tools (Test dataset: GitHub)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule
% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Within Platform)}} 
%  & SentiMoji vs BERT4SE & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiMoji vs RNN4SE & 0.52 & 68\% & 7\% & 25\%  \\
%  & SentiMoji vs Senti4SD & 0.83 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs SentiCR & 0.76 & 85\% & 2\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.53 & 69\% & 7\% & 24\%  \\
%  & BERT4SE vs Senti4SD & 0.85 & 90\% & 2\% & 8\%  \\
%  & BERT4SE vs SentiCR & 0.74 & 83\% & 2\% & 14\%  \\
%  & RNN4SE vs Senti4SD & 0.52 & 69\% & 7\% & 25\%  \\
%  & RNN4SE vs SentiCR & 0.43 & 63\% & 7\% & 31\%  \\
%  & Senti4SD vs SentiCR & 0.74 & 83\% & 2\% & 14\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.72 & 83\% & 1\% & 15\%  \\
%  & SentiMoji vs RNN4SE & 0.58 & 76\% & 2\% & 22\%  \\
%  & SentiMoji vs Senti4SD & 0.51 & 70\% & 3\% & 27\%  \\
%  & SentiMoji vs SentiCR & 0.40 & 68\% & 2\% & 30\%  \\
%  & BERT4SE vs RNN4SE & 0.59 & 76\% & 2\% & 22\%  \\
%  & BERT4SE vs Senti4SD & 0.52 & 70\% & 4\% & 26\%  \\
%  & BERT4SE vs SentiCR & 0.39 & 66\% & 3\% & 31\%  \\
%  & RNN4SE vs Senti4SD & 0.43 & 65\% & 4\% & 31\%  \\
%  & RNN4SE vs SentiCR & 0.30 & 62\% & 3\% & 35\%  \\
%  & Senti4SD vs SentiCR & 0.45 & 68\% & 2\% & 30\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.78 & 90\% & 0\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.54 & 81\% & 1\% & 19\%  \\
%  & SentiMoji vs Senti4SD & 0.60 & 82\% & 1\% & 18\%  \\
%  & SentiMoji vs SentiCR & 0.65 & 87\% & 0\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.56 & 81\% & 1\% & 18\%  \\
%  & BERT4SE vs Senti4SD & 0.60 & 81\% & 1\% & 18\%  \\
%  & BERT4SE vs SentiCR & 0.67 & 87\% & 0\% & 13\%  \\
%  & RNN4SE vs Senti4SD & 0.44 & 74\% & 2\% & 24\%  \\
%  & RNN4SE vs SentiCR & 0.45 & 79\% & 1\% & 20\%  \\
%  & Senti4SD vs SentiCR & 0.52 & 79\% & 1\% & 20\%  \\

%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_github}%
% \end{table}%


% \begin{table}
% \addtocounter{table}{-1}
% \renewcommand{\thetable}{\arabic{table}b}

% %   \footnotesize
%   \small

%   \centering
%   \caption{Agreement between  tools (Test dataset: SO)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Within Platform)}} 
%  & SentiMoji vs BERT4SE & 0.86 & 91\% & 1\% & 8\%  \\
%  & SentiMoji vs RNN4SE & 0.70 & 80\% & 3\% & 17\%  \\
%  & SentiMoji vs Senti4SD & 0.81 & 88\% & 1\% & 12\%  \\
%  & SentiMoji vs SentiCR & 0.78 & 85\% & 2\% & 12\%  \\
%  & BERT4SE vs RNN4SE & 0.71 & 81\% & 2\% & 17\%  \\
%  & BERT4SE vs Senti4SD & 0.83 & 88\% & 1\% & 11\%  \\
%  & BERT4SE vs SentiCR & 0.78 & 85\% & 3\% & 12\%  \\
%  & RNN4SE vs Senti4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & RNN4SE vs SentiCR & 0.65 & 77\% & 4\% & 19\%  \\
%  & Senti4SD vs SentiCR & 0.78 & 85\% & 3\% & 12\%  \\
% \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.79 & 86\% & 1\% & 13\%  \\
%  & SentiMoji vs RNN4SE & 0.53 & 70\% & 4\% & 27\%  \\
%  & SentiMoji vs Senti4SD & 0.70 & 80\% & 3\% & 17\%  \\
%  & SentiMoji vs SentiCR & 0.62 & 75\% & 5\% & 20\%  \\
%  & BERT4SE vs RNN4SE & 0.53 & 69\% & 5\% & 26\%  \\
%  & BERT4SE vs Senti4SD & 0.73 & 82\% & 2\% & 16\%  \\
%  & BERT4SE vs SentiCR & 0.60 & 74\% & 5\% & 21\%  \\
%  & RNN4SE vs Senti4SD & 0.54 & 69\% & 4\% & 26\%  \\
%  & RNN4SE vs SentiCR & 0.40 & 61\% & 6\% & 33\%  \\
%  & Senti4SD vs SentiCR & 0.58 & 73\% & 4\% & 23\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.66 & 82\% & 0\% & 18\%  \\
%  & SentiMoji vs RNN4SE & 0.47 & 75\% & 1\% & 23\%  \\
%  & SentiMoji vs Senti4SD & 0.60 & 81\% & 1\% & 19\%  \\
%  & SentiMoji vs SentiCR & 0.56 & 80\% & 1\% & 19\%  \\
%  & BERT4SE vs RNN4SE & 0.43 & 70\% & 2\% & 28\%  \\
%  & BERT4SE vs Senti4SD & 0.57 & 77\% & 1\% & 22\%  \\
%  & BERT4SE vs SentiCR & 0.52 & 75\% & 1\% & 25\%  \\
%  & RNN4SE vs Senti4SD & 0.42 & 72\% & 2\% & 27\%  \\
%  & RNN4SE vs SentiCR & 0.33 & 70\% & 1\% & 29\%  \\
%  & Senti4SD vs SentiCR & 0.51 & 77\% & 1\% & 22\%  \\
% % \midrule

%     \bottomrule
%     \end{tabular}%
%   \label{tab:agreement_test_so}%
% \end{table}%



% \begin{table}[]
%   \addtocounter{table}{-1}
%   \renewcommand{\thetable}{\arabic{table}c}

% %   \footnotesize
%   \small
%   \centering
%   \caption{Agreement between  tools (Test dataset: Jira)}
%     \begin{tabular}{clrr|rr}
%     \toprule
%     \multirow{2}{*}{\bf{Train Dataset}} & \multirow{2}{*}{\bf{Tool1 $\Longleftrightarrow$ Tool2}} &  \multicolumn{2}{c}{\textbf{Agreement}} & \multicolumn{2}{c}{\bf{Disagreement}}\\
%     \cmidrule{3-6}
%     & & {\bf{$\kappa$}} & {\textbf{Perfect}} & \textbf{Severe} & \textbf{Mild} \\
%     \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering Jira \\ (Within Platform}} 
%  & SentiMoji vs BERT4SE & 0.85 & 93\% & 0\% & 7\%  \\
%  & SentiMoji vs RNN4SE & 0.68 & 86\% & 0\% & 14\%  \\
%  & SentiMoji vs Senti4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & SentiMoji vs SentiCR & 0.81 & 91\% & 0\% & 9\%  \\
%  & BERT4SE vs RNN4SE & 0.68 & 85\% & 1\% & 14\%  \\
%  & BERT4SE vs Senti4SD & 0.72 & 87\% & 0\% & 13\%  \\
%  & BERT4SE vs SentiCR & 0.79 & 90\% & 0\% & 10\%  \\
%  & RNN4SE vs Senti4SD & 0.61 & 83\% & 0\% & 17\%  \\
%  & RNN4SE vs SentiCR & 0.70 & 86\% & 1\% & 14\%  \\
%  & Senti4SD vs SentiCR & 0.70 & 86\% & 0\% & 13\%  \\
% \midrule

% \multirow{10}{*}{\parbox{2cm} {\centering GitHub \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.81 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.56 & 72\% & 3\% & 25\%  \\
%  & SentiMoji vs Senti4SD & 0.72 & 84\% & 1\% & 14\%  \\
%  & SentiMoji vs SentiCR & 0.75 & 86\% & 1\% & 13\%  \\
%  & BERT4SE vs RNN4SE & 0.57 & 73\% & 3\% & 24\%  \\
%  & BERT4SE vs Senti4SD & 0.73 & 85\% & 1\% & 14\%  \\
%  & BERT4SE vs SentiCR & 0.75 & 87\% & 1\% & 13\%  \\
%  & RNN4SE vs Senti4SD & 0.52 & 70\% & 3\% & 27\%  \\
%  & RNN4SE vs SentiCR & 0.50 & 69\% & 2\% & 28\%  \\
%  & Senti4SD vs SentiCR & 0.68 & 83\% & 1\% & 16\%  \\
% \midrule


% \multirow{10}{*}{\parbox{2cm} {\centering SO \\ (Cross Platform)}} 
%  & SentiMoji vs BERT4SE & 0.80 & 89\% & 1\% & 10\%  \\
%  & SentiMoji vs RNN4SE & 0.70 & 84\% & 1\% & 15\%  \\
%  & SentiMoji vs Senti4SD & 0.61 & 79\% & 1\% & 19\%  \\
%  & SentiMoji vs SentiCR & 0.35 & 70\% & 1\% & 29\%  \\
%  & BERT4SE vs RNN4SE & 0.72 & 84\% & 1\% & 14\%  \\
%  & BERT4SE vs Senti4SD & 0.60 & 79\% & 2\% & 19\%  \\
%  & BERT4SE vs SentiCR & 0.36 & 71\% & 1\% & 28\%  \\
%  & RNN4SE vs Senti4SD & 0.56 & 77\% & 2\% & 22\%  \\
%  & RNN4SE vs SentiCR & 0.30 & 67\% & 1\% & 32\%  \\
%  & Senti4SD vs SentiCR & 0.41 & 76\% & 1\% & 23\%  \\
% % \midrule
%     % \midrule  
%     \bottomrule
%     \end{tabular}%
% %   }
%   % \vspace{-.25in}
%   \label{tab:agreement_test_jira}%
% \end{table}%

